An LP-Based Approach for Goal Recognition as Planning

Goal recognition aims to recognize the set of candidate goals that are compatible with the observed behavior of an agent. In this paper, we develop a method based on the operator-counting framework that efficiently computes solutions that satisfy the observations and uses the information generated to solve goal recognition tasks. Our method reasons explicitly about both partial and noisy observations: estimating uncertainty for the former, and satisfying observations given the unreliability of the sensor for the latter. We evaluate our approach empirically over a large data set, analyzing its components on how each can impact the quality of the solutions. In general, our approach is superior to previous methods in terms of agreement ratio, accuracy, and spread. Finally, our approach paves the way for new research on combinatorial optimization to solve goal recognition tasks.

==> exemplo.tex <==
\begin{tikzpicture}
\matrix (A) [
    very thin,
    matrix of nodes, 
    nodes in empty cells,
    nodes={draw, minimum size=0.7cm, anchor=center},
    row sep=-\pgflinewidth,
    column sep=-\pgflinewidth
]
{$\goalstate_2$&  &  &  & \\  
               &  &$s_0$&  & \\
 $\goalstate_1$&  &  &  & \\};
 
\draw[black,dashed,shorten <=2mm, shorten >=1mm,->] (A-1-1.center) -- (A-1-2.center) node[font=\tiny\selectfont,above,xshift=-1mm] {$o_{11}$};

\draw[black,shorten <=2mm, shorten >=2mm,->] 
    (A-2-3.center) edge (A-2-2.center) node[font=\tiny\selectfont,above,xshift=-5mm] {$o_1$}
    (A-2-2.center) edge (A-2-1.center) node[font=\tiny\selectfont,above,xshift=-5mm] {$o_2$}
    (A-2-1.center) -- (A-3-1.center) node[font=\tiny\selectfont,left,xshift=1mm,yshift=4.5mm] {$o_3$};

\draw[black,shorten <=2mm, shorten >=2mm,->] 
    (A-2-3.center) edge (A-2-4.center) node[font=\tiny\selectfont,above,xshift=5mm] {$o_4$}
    (A-2-4.center) edge (A-2-5.center) node[font=\tiny\selectfont,above,xshift=5mm] {$o_5$}
    (A-2-5.center) edge (A-3-5.center) node[font=\tiny\selectfont,right,xshift=-2,yshift=-5mm] {$o_6$}
    (A-3-5.center) edge (A-3-4.center) node[font=\tiny\selectfont,above,xshift=-2.mm] {$o_7$}
    (A-3-4.center) edge (A-3-3.center) node[font=\tiny\selectfont,above,xshift=-2.mm] {$o_8$}
    (A-3-3.center) edge (A-3-2.center) node[font=\tiny\selectfont,above,xshift=-2.mm] {$o_9$}
    (A-3-2.center) -- (A-3-1.center) node[font=\tiny\selectfont,above,xshift=6mm] {$o_{10}$};   
    
%\draw [ultra thick] (A-2-3.north west) -- (A-2-3.south west);
%\draw [ultra thick] (A-2-3.north west) -- (A-2-3.north east);
%\draw [ultra thick] (A-2-3.south west) -- (A-2-3.south east);
\end{tikzpicture}

==> tables-avg/constraints.tex <==
\begin{tabular}{cc|ccc|ccc||ccc|ccc}
\toprule
\multicolumn{2}{c}{} & \multicolumn{6}{c}{Optimal} & \multicolumn{6}{c}{Sub-Optimal}\\
\cmidrule(lr){3-8}\cmidrule(lr){9-14}
\# & \% & S & L & P & S, L & L, P & S, P%
& S & L & P & S, L & L, P & S, P\\
\midrule
\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{blocks}}}%
 & 10 & \textbf{0.45} & 0.42 & 0.44 & \textbf{0.45} & 0.41 & 0.44 & \textbf{0.44} & 0.41 & 0.39 & \textbf{0.44} & 0.39 & 0.41\\ & 30 & \textbf{0.43} & 0.33 & \textbf{0.43} & 0.43 & \textbf{0.47} & \textbf{0.47} & \textbf{0.5} & 0.44 & 0.41 & \textbf{0.5} & 0.44 & 0.49\\ & 50 & \textbf{0.55} & 0.46 & 0.44 & 0.55 & 0.58 & \textbf{0.59} & 0.5 & 0.37 & \textbf{0.51} & 0.5 & \textbf{0.57} & 0.55\\ & 70 & \textbf{0.75} & 0.54 & 0.58 & 0.75 & 0.81 & \textbf{0.85} & \textbf{0.64} & 0.45 & 0.55 & 0.64 & 0.69 & \textbf{0.71}\\ & 100 & \textbf{0.82} & 0.58 & 0.62 & 0.82 & 0.88 & \textbf{0.92} & \textbf{0.74} & 0.52 & 0.58 & 0.74 & 0.79 & \textbf{0.84}\\\hline
\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{ipc-grid}}}%
 & 10 & 0.65 & \textbf{0.92} & 0.4 & 0.87 & \textbf{0.92} & 0.68 & 0.6 & \textbf{0.86} & 0.25 & 0.76 & \textbf{0.86} & 0.63\\ & 30 & 0.73 & \textbf{0.97} & 0.25 & 0.93 & \textbf{0.97} & 0.78 & 0.69 & \textbf{0.88} & 0.23 & 0.82 & \textbf{0.88} & 0.71\\ & 50 & 0.83 & \textbf{0.97} & 0.27 & 0.96 & \textbf{0.97} & 0.9 & 0.81 & \textbf{0.89} & 0.29 & 0.84 & \textbf{0.89} & 0.87\\ & 70 & 0.9 & \textbf{0.97} & 0.3 & \textbf{0.97} & \textbf{0.97} & 0.95 & 0.87 & \textbf{0.91} & 0.08 & 0.89 & \textbf{0.91} & 0.89\\ & 100 & \textbf{1.0} & \textbf{1.0} & 0.23 & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{0.94} & \textbf{0.94} & 0.05 & \textbf{0.94} & \textbf{0.94} & \textbf{0.94}\\\hline
%
\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{sokoban}}}%
 & 10 & \textbf{0.38} & \textbf{0.38} & 0.24 & \textbf{0.39} & 0.34 & 0.31 & \textbf{0.38} & 0.3 & 0.24 & \textbf{0.52} & 0.25 & 0.36\\ & 30 & \textbf{0.59} & 0.41 & 0.14 & \textbf{0.75} & 0.38 & 0.59 & \textbf{0.72} & 0.43 & 0.14 & \textbf{0.77} & 0.37 & 0.68\\ & 50 & \textbf{0.82} & 0.53 & 0.21 & \textbf{0.92} & 0.49 & 0.82 & \textbf{0.77} & 0.51 & 0.17 & \textbf{0.79} & 0.41 & \textbf{0.79}\\ & 70 & \textbf{0.93} & 0.73 & 0.21 & \textbf{0.99} & 0.62 & 0.93 & \textbf{0.85} & 0.58 & 0.17 & 0.8 & 0.51 & \textbf{0.85}\\ & 100 & \textbf{0.96} & 0.85 & 0.23 & \textbf{1.0} & 0.81 & 0.96 & \textbf{0.88} & 0.73 & 0.22 & 0.83 & 0.72 & \textbf{0.88}\\\hline%
\multicolumn{2}{c|}{\textsc{Other}} & \textbf{0.82} & 0.81 & 0.61 & \textbf{0.88} & 0.8 & 0.82 & \textbf{0.79} & 0.78 & 0.6 & \textbf{0.86} & 0.78 & 0.8\\\hline%
\multicolumn{2}{c|}{AVG}  & \textbf{0.79} & 0.77 & 0.54 & \textbf{0.86} & 0.78 & 0.8 & \textbf{0.76} & 0.74 & 0.52 & \textbf{0.82} & 0.75 & 0.78\\
\bottomrule
\end{tabular}\\

==> tables-avg/domains.tex <==
\begin{tabular}{cc|c|cc|cc}
\toprule
\multicolumn{3}{c}{} & \multicolumn{2}{c}{Optimal} & \multicolumn{2}{c}{Sub-Optimal}\\
\midrule
\# & \% & $|\goalconditions|$ & $|\observations|$ & $|\grsolution|$ & $|\observations|$ & $|\grsolution|$ \\
\midrule
\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{blocks}}}%
	 & 10
 & \multirow{5}{*}{20.33} & 1.25 & 8.0 & 1.42 & 7.61\\
	 & 30
 &  & 3.08 & 3.97 & 3.83 & 3.58\\
	 & 50
 &  & 4.42 & 2.5 & 5.92 & 3.19\\
	 & 70
 &  & 6.67 & 1.94 & 8.5 & 2.53\\
	 & 100
 &  & 8.83 & 1.83 & 11.83 & 2.25\\\hline
 \multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{ipc-grid}}}%
	 & 10
 & \multirow{5}{*}{7.5} & 1.63 & 2.71 & 2.06 & 1.58\\
	 & 30
 &  & 4.0 & 1.21 & 5.56 & 1.4\\
	 & 50
 &  & 6.19 & 1.13 & 8.88 & 1.35\\
	 & 70
 &  & 8.69 & 1.04 & 12.56 & 1.31\\
	 & 100
 &  & 11.88 & 1.0 & 17.25 & 1.5\\\hline
 \multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{sokoban}}}%
	 & 10
 & \multirow{5}{*}{8.67} & 2.33 & 2.11 & 3.33 & 1.83\\
	 & 30
 &  & 6.5 & 1.25 & 8.67 & 1.28\\
	 & 50
 &  & 10.33 & 1.22 & 13.75 & 1.33\\
	 & 70
 &  & 14.67 & 1.03 & 19.33 & 1.36\\
	 & 100
 &  & 20.17 & 1.0 & 27.0 & 1.33\\\hline
 \multicolumn{2}{c|}{\textsc{Other}} & 6.89 & 7.84 & 1.6 & 10.51 & 1.44\\
\bottomrule
\end{tabular}\\

==> tables-avg/noisy.tex <==
\begin{tabular}{cc|cccc|cccc}
\toprule
 \multicolumn{2}{c}{} & \multicolumn{4}{c}{Optimal} & \multicolumn{4}{c}{Sub-Optimal}\\
\cmidrule(lr){3-6}\cmidrule(lr){7-10}
%
\# & \% & \dhc & \dhcf & \rg & \pom & \dhc & \dhcf & \rg & \pom\\%
%
\midrule
\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{blocks}}}%
 & 10 & \textbf{0.32} & \textbf{0.32} & 0.31 & 0.06 & 0.38 & 0.38 & \textbf{0.42} & 0.05\\ & 30 & 0.37 & 0.37 & \textbf{0.39} & 0.13 & 0.36 & 0.37 & \textbf{0.49} & 0.22\\ & 50 & \textbf{0.64} & \textbf{0.64} & 0.6 & 0.37 & 0.53 & 0.53 & \textbf{0.55} & 0.28\\ & 70 & 0.79 & \textbf{0.81} & 0.77 & 0.47 & \textbf{0.67} & \textbf{0.67} & 0.63 & 0.38\\ & 100 & 0.88 & 0.88 & \textbf{0.89} & 0.57 & 0.78 & \textbf{0.82} & 0.74 & 0.51\\\hline%
 \multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{ipc-grid}}}%
 & 10 & \textbf{0.57} & \textbf{0.57} & 0.16 & 0.38 & \textbf{0.62} & \textbf{0.62} & 0.12 & 0.54\\ & 30 & \textbf{0.85} & \textbf{0.85} & 0.28 & 0.71 & 0.68 & 0.68 & 0.08 & \textbf{0.72}\\ & 50 & \textbf{0.89} & \textbf{0.89} & 0.07 & 0.81 & 0.84 & 0.84 & 0.04 & \textbf{0.85}\\ & 70 & \textbf{0.95} & \textbf{0.95} & 0.15 & 0.93 & 0.89 & 0.89 & 0.02 & \textbf{0.9}\\ & 100 & \textbf{1.0} & \textbf{1.0} & 0.08 & 0.99 & \textbf{0.94} & \textbf{0.94} & 0.04 & 0.92\\\hline%
 \multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{sokoban}}}%
 & 10 & \textbf{0.27} & \textbf{0.27} & 0.1 & 0.24 & 0.31 & \textbf{0.32} & 0.13 & 0.25\\ & 30 & 0.56 & \textbf{0.7} & 0.2 & 0.34 & 0.48 & \textbf{0.56} & 0.12 & 0.29\\ & 50 & 0.61 & \textbf{0.82} & 0.2 & 0.57 & 0.5 & \textbf{0.73} & 0.01 & 0.46\\ & 70 & 0.6 & \textbf{0.97} & 0.08 & 0.84 & 0.54 & \textbf{0.8} & 0.06 & 0.58\\ & 100 & 0.66 & \textbf{1.0} & 0.04 & 0.96 & 0.35 & \textbf{0.85} & 0.04 & 0.77\\\hline%
\multicolumn{2}{c|}{\textsc{Other}} & 0.72 & \textbf{0.73} & 0.37 & 0.63 & 0.72 & \textbf{0.74} & 0.38 & 0.64\\\hline%

\multicolumn{2}{c|}{AVG} & 0.71 & \textbf{0.73} & 0.35 & 0.61 & 0.69 & \textbf{0.72} & 0.34 & 0.61\\\midrule\midrule%
\multicolumn{2}{c|}{ACC} & 0.89 & \textbf{0.9} & 0.5 & 0.73 & 0.87 & \textbf{0.89} & 0.48 & 0.76\\\midrule%
\multicolumn{2}{c|}{SPR} & 1.91 & 1.78 & 1.38 & \textbf{1.3} & 1.93 & 1.72 & 1.34 & \textbf{1.31}%
\\
\bottomrule
\end{tabular}\\

==> tables-avg/uncertainty-sub.tex <==
\begin{tabular}{cc|ccc|ccc|ccc|ccc|ccc|ccc}
\toprule
 \multicolumn{2}{c}{} & \multicolumn{18}{c}{Sub-Optimal}\\
\cmidrule(lr){3-20}
%
 \multicolumn{2}{c}{} & \multicolumn{3}{c}{\dhc} & \multicolumn{3}{c}{\dhcu} & \multicolumn{3}{c}{\rg} & \multicolumn{3}{c}{\pom} & \multicolumn{3}{c}{\pomA} & \multicolumn{3}{c}{\pomC}\\%
%
\cmidrule(lr){3-5}\cmidrule(lr){6-8}\cmidrule(lr){9-11}\cmidrule(lr){12-14}\cmidrule(lr){15-17}\cmidrule(lr){18-20}\\
\# & \% %
& AGR & ACC & SPR & AGR & ACC & SPR & AGR & ACC & SPR & AGR & ACC & SPR & AGR & ACC & SPR & AGR & ACC & SPR\\
\midrule
\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{blocks}}}%
 & 10 & 0.41 & 0.86 & 6.86 & 0.42 & 0.89 & 7.42 & \textbf{0.46} & 0.97 & 10.61 & 0.06 & 0.19 & 1.19 & 0.19 & 0.58 & 4.44 & 0.34 & 1.0 & 17.53\\ & 30 & 0.49 & 0.78 & 3.17 & 0.35 & 0.86 & 6.92 & \textbf{0.54} & 1.0 & 4.86 & 0.28 & 0.56 & 1.17 & 0.32 & 0.89 & 3.36 & 0.26 & 1.0 & 13.47\\ & 50 & 0.55 & 0.86 & 3.08 & 0.42 & 0.94 & 5.61 & \textbf{0.62} & 0.97 & 2.72 & 0.39 & 0.72 & 1.08 & 0.36 & 0.81 & 2.17 & 0.27 & 1.0 & 9.89\\ & 70 & \textbf{0.71} & 0.92 & 2.06 & 0.56 & 0.94 & 3.06 & 0.68 & 1.0 & 2.44 & 0.51 & 0.94 & 1.33 & 0.44 & 1.0 & 2.22 & 0.26 & 1.0 & 8.61\\ & 100 & \textbf{0.84} & 1.0 & 1.67 & \textbf{0.84} & 1.0 & 1.67 & 0.8 & 1.0 & 2.08 & 0.51 & 1.0 & 1.67 & 0.48 & 1.0 & 1.92 & 0.28 & 1.0 & 6.42\\\hline%
 \multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{ipc-grid}}}%
 & 10 & 0.77 & 0.92 & 1.81 & 0.75 & 0.98 & 2.4 & \textbf{0.81} & 1.0 & 2.73 & 0.64 & 0.88 & 2.23 & 0.59 & 0.98 & 3.44 & 0.42 & 1.0 & 5.6\\ & 30 & 0.82 & 0.94 & 1.13 & 0.77 & 0.98 & 1.6 & \textbf{0.9} & 1.0 & 1.27 & 0.81 & 0.96 & 1.35 & 0.8 & 0.96 & 1.52 & 0.67 & 0.96 & 2.23\\ & 50 & 0.84 & 0.94 & 1.13 & 0.84 & 1.0 & 1.56 & \textbf{0.92} & 1.0 & 1.1 & 0.87 & 1.0 & 1.08 & 0.86 & 1.0 & 1.13 & 0.86 & 1.0 & 1.21\\ & 70 & 0.89 & 1.0 & 1.1 & 0.85 & 1.0 & 1.23 & \textbf{0.93} & 1.0 & 1.02 & 0.92 & 1.0 & 1.0 & 0.92 & 1.0 & 1.0 & 0.92 & 1.0 & 1.0\\ & 100 & \textbf{0.94} & 1.0 & 1.0 & \textbf{0.94} & 1.0 & 1.0 & \textbf{0.94} & 1.0 & 1.0 & \textbf{0.94} & 1.0 & 1.0 & \textbf{0.94} & 1.0 & 1.0 & \textbf{0.94} & 1.0 & 1.0\\\hline%
 \multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{sokoban}}}%
 & 10 & \textbf{0.52} & 0.61 & 1.78 & 0.44 & 0.72 & 3.17 & 0.29 & 0.64 & 4.56 & 0.35 & 0.64 & 2.47 & 0.38 & 0.92 & 4.08 & 0.24 & 1.0 & 6.86\\ & 30 & \textbf{0.77} & 0.83 & 1.08 & 0.62 & 0.97 & 2.67 & 0.43 & 0.75 & 2.92 & 0.56 & 0.75 & 1.72 & 0.51 & 0.86 & 2.64 & 0.24 & 0.97 & 5.5\\ & 50 & \textbf{0.79} & 0.92 & 1.17 & 0.66 & 1.0 & 2.58 & 0.53 & 0.72 & 1.83 & 0.58 & 0.75 & 1.39 & 0.53 & 0.86 & 2.31 & 0.25 & 0.97 & 5.14\\ & 70 & 0.8 & 0.97 & 1.03 & \textbf{0.85} & 1.0 & 1.39 & 0.54 & 0.61 & 1.28 & 0.63 & 0.86 & 1.25 & 0.59 & 0.92 & 1.75 & 0.3 & 1.0 & 4.11\\ & 100 & \textbf{0.83} & 1.0 & 1.0 & \textbf{0.83} & 1.0 & 1.0 & 0.58 & 0.58 & 1.33 & \textbf{0.83} & 1.0 & 1.0 & \textbf{0.83} & 1.0 & 1.0 & 0.38 & 1.0 & 2.75\\\hline%
\multicolumn{2}{c|}{\textsc{Other}} & \textbf{0.85} & 0.94 & 1.63 & 0.77 & 0.97 & 2.24 & 0.76 & 0.95 & 2.16 & 0.74 & 0.84 & 1.29 & 0.67 & 0.93 & 2.16 & 0.36 & 1.0 & 4.69\\\midrule%
\multicolumn{2}{c|}{AVG} & \textbf{0.82} & 0.93 & 1.71 & 0.75 & 0.97 & 2.39 & 0.74 & 0.93 & 2.3 & 0.7 & 0.83 & 1.31 & 0.65 & 0.93 & 2.19 & 0.38 & 1.0 & 5.01%
\\
\bottomrule
\end{tabular}\\

==> tables-avg/uncertainty.tex <==
\begin{tabular}{cc|ccc|ccc|ccc|ccc|ccc|ccc}
\toprule
 \multicolumn{2}{c}{} & \multicolumn{18}{c}{Optimal}\\
\cmidrule(lr){3-20}
%
 \multicolumn{2}{c}{} & \multicolumn{3}{c}{\dhc} & \multicolumn{3}{c}{\dhcu} & \multicolumn{3}{c}{\rg} & \multicolumn{3}{c}{\pom} & \multicolumn{3}{c}{\pomA} & \multicolumn{3}{c}{\pomC}\\%
%
\cmidrule(lr){3-5}\cmidrule(lr){6-8}\cmidrule(lr){9-11}\cmidrule(lr){12-14}\cmidrule(lr){15-17}\cmidrule(lr){18-20}\\
\# & \% %
& AGR & ACC & SPR & AGR & ACC & SPR & AGR & ACC & SPR & AGR & ACC & SPR & AGR & ACC & SPR & AGR & ACC & SPR\\
\midrule
\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{blocks}}}%
 & 10 & 0.44 & 0.86 & 7.53 & 0.44 & 0.86 & 7.56 & \textbf{0.47} & 0.92 & 9.83 & 0.06 & 0.17 & 1.44 & 0.13 & 0.47 & 4.06 & 0.38 & 1.0 & 18.14\\ & 30 & \textbf{0.46} & 0.78 & 2.5 & 0.44 & 0.86 & 4.67 & 0.45 & 0.92 & 5.56 & 0.21 & 0.39 & 1.17 & 0.3 & 0.75 & 2.94 & 0.24 & 1.0 & 15.25\\ & 50 & 0.59 & 0.89 & 3.03 & 0.52 & 0.89 & 3.86 & \textbf{0.62} & 0.97 & 3.69 & 0.33 & 0.58 & 1.25 & 0.37 & 0.81 & 3.08 & 0.25 & 0.97 & 12.17\\ & 70 & \textbf{0.85} & 0.97 & 1.83 & 0.76 & 0.97 & 2.42 & 0.81 & 1.0 & 2.22 & 0.51 & 0.72 & 1.14 & 0.45 & 0.94 & 2.19 & 0.25 & 1.0 & 9.22\\ & 100 & \textbf{0.92} & 1.0 & 1.67 & \textbf{0.92} & 1.0 & 1.67 & 0.9 & 1.0 & 2.08 & 0.59 & 1.0 & 1.67 & 0.55 & 1.0 & 1.92 & 0.31 & 1.0 & 6.42\\\hline%
 \multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{ipc-grid}}}%
 & 10 & 0.87 & 0.94 & 2.67 & 0.88 & 0.96 & 2.69 & \textbf{0.91} & 1.0 & 3.23 & 0.47 & 0.75 & 2.35 & 0.55 & 0.98 & 4.38 & 0.49 & 1.0 & 6.25\\ & 30 & 0.93 & 0.96 & 1.15 & 0.94 & 0.98 & 1.17 & \textbf{0.99} & 1.0 & 1.25 & 0.85 & 0.98 & 1.52 & 0.81 & 1.0 & 1.96 & 0.64 & 1.0 & 3.17\\ & 50 & 0.96 & 0.98 & 1.08 & 0.96 & 0.98 & 1.08 & \textbf{1.0} & 1.0 & 1.13 & 0.86 & 1.0 & 1.44 & 0.86 & 1.0 & 1.56 & 0.77 & 1.0 & 2.15\\ & 70 & 0.97 & 0.98 & 1.06 & 0.97 & 0.98 & 1.06 & \textbf{1.0} & 1.0 & 1.04 & 0.97 & 0.98 & 1.02 & 0.97 & 0.98 & 1.02 & 0.93 & 0.98 & 1.15\\ & 100 & \textbf{1.0} & 1.0 & 1.0 & \textbf{1.0} & 1.0 & 1.0 & \textbf{1.0} & 1.0 & 1.0 & \textbf{1.0} & 1.0 & 1.0 & \textbf{1.0} & 1.0 & 1.0 & \textbf{1.0} & 1.0 & 1.0\\\hline%
 \multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{sokoban}}}%
 & 10 & 0.39 & 0.53 & 2.08 & 0.38 & 0.61 & 2.94 & \textbf{0.4} & 0.81 & 4.86 & 0.28 & 0.53 & 2.14 & 0.32 & 0.89 & 4.39 & 0.26 & 0.97 & 7.0\\ & 30 & \textbf{0.75} & 0.81 & 1.25 & 0.64 & 0.92 & 2.06 & 0.56 & 0.86 & 2.53 & 0.57 & 0.69 & 1.22 & 0.48 & 0.75 & 1.89 & 0.23 & 0.94 & 5.17\\ & 50 & \textbf{0.92} & 1.0 & 1.19 & 0.83 & 1.0 & 1.39 & 0.61 & 0.86 & 2.14 & 0.61 & 0.69 & 1.42 & 0.55 & 0.81 & 2.14 & 0.28 & 1.0 & 5.08\\ & 70 & \textbf{0.99} & 1.0 & 1.0 & 0.94 & 1.0 & 1.08 & 0.64 & 0.83 & 1.53 & 0.85 & 0.92 & 1.17 & 0.81 & 0.94 & 1.39 & 0.36 & 1.0 & 3.64\\ & 100 & \textbf{1.0} & 1.0 & 1.0 & \textbf{1.0} & 1.0 & 1.0 & 0.67 & 0.75 & 1.17 & \textbf{1.0} & 1.0 & 1.0 & \textbf{1.0} & 1.0 & 1.0 & 0.42 & 1.0 & 2.75\\\hline%
\multicolumn{2}{c|}{\textsc{Other}} & \textbf{0.88} & 0.95 & 1.71 & 0.86 & 0.96 & 1.87 & 0.79 & 0.95 & 2.23 & 0.73 & 0.79 & 1.28 & 0.69 & 0.92 & 2.18 & 0.37 & 0.99 & 4.75\\\midrule%
\multicolumn{2}{c|}{AVG}  & \textbf{0.86} & 0.94 & 1.79 & 0.84 & 0.95 & 1.99 & 0.77 & 0.95 & 2.39 & 0.7 & 0.79 & 1.31 & 0.67 & 0.91 & 2.22 & 0.39 & 0.99 & 5.2%
\\
\bottomrule
\end{tabular}\\

==> tables-new/constraints.tex <==
\begin{tabular}{cc|ccc|ccc||ccc|ccc}
\toprule
\multicolumn{2}{c}{} & \multicolumn{6}{c}{Optimal} & \multicolumn{6}{c}{Sub-Optimal}\\
\cmidrule(lr){3-8}\cmidrule(lr){9-14}
\# & \% & S & L & P & S, L & L, P & S, P%
& S & L & P & S, L & L, P & S, P\\
\midrule
\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{blocks}}}%
 & 10 & \textbf{0.45} & 0.42 & 0.44 & \textbf{0.45} & 0.41 & 0.44 & \textbf{0.44} & 0.41 & 0.39 & \textbf{0.44} & 0.39 & 0.41\\ & 30 & \textbf{0.43} & 0.33 & \textbf{0.43} & 0.43 & \textbf{0.47} & \textbf{0.47} & \textbf{0.5} & 0.44 & 0.41 & \textbf{0.5} & 0.44 & 0.49\\ & 50 & \textbf{0.55} & 0.46 & 0.44 & 0.55 & 0.58 & \textbf{0.59} & 0.5 & 0.37 & \textbf{0.51} & 0.5 & \textbf{0.57} & 0.55\\ & 70 & \textbf{0.75} & 0.54 & 0.58 & 0.75 & 0.81 & \textbf{0.85} & \textbf{0.64} & 0.45 & 0.55 & 0.64 & 0.69 & \textbf{0.71}\\ & 100 & \textbf{0.82} & 0.58 & 0.62 & 0.82 & 0.88 & \textbf{0.92} & \textbf{0.74} & 0.52 & 0.58 & 0.74 & 0.79 & \textbf{0.84}\\\hline
\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{ipc-grid}}}%
 & 10 & 0.65 & \textbf{0.92} & 0.4 & 0.87 & \textbf{0.92} & 0.68 & 0.6 & \textbf{0.86} & 0.25 & 0.76 & \textbf{0.86} & 0.63\\ & 30 & 0.73 & \textbf{0.97} & 0.25 & 0.93 & \textbf{0.97} & 0.78 & 0.69 & \textbf{0.88} & 0.23 & 0.82 & \textbf{0.88} & 0.71\\ & 50 & 0.83 & \textbf{0.97} & 0.27 & 0.96 & \textbf{0.97} & 0.9 & 0.81 & \textbf{0.89} & 0.29 & 0.84 & \textbf{0.89} & 0.87\\ & 70 & 0.9 & \textbf{0.97} & 0.3 & \textbf{0.97} & \textbf{0.97} & 0.95 & 0.87 & \textbf{0.91} & 0.08 & 0.89 & \textbf{0.91} & 0.89\\ & 100 & \textbf{1.0} & \textbf{1.0} & 0.23 & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{0.94} & \textbf{0.94} & 0.05 & \textbf{0.94} & \textbf{0.94} & \textbf{0.94}\\\hline
%
\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{sokoban}}}%
 & 10 & \textbf{0.38} & \textbf{0.38} & 0.24 & \textbf{0.39} & 0.34 & 0.31 & \textbf{0.38} & 0.3 & 0.24 & \textbf{0.52} & 0.25 & 0.36\\ & 30 & \textbf{0.59} & 0.41 & 0.14 & \textbf{0.75} & 0.38 & 0.59 & \textbf{0.72} & 0.43 & 0.14 & \textbf{0.77} & 0.37 & 0.68\\ & 50 & \textbf{0.82} & 0.53 & 0.21 & \textbf{0.92} & 0.49 & 0.82 & \textbf{0.77} & 0.51 & 0.17 & \textbf{0.79} & 0.41 & \textbf{0.79}\\ & 70 & \textbf{0.93} & 0.73 & 0.21 & \textbf{0.99} & 0.62 & 0.93 & \textbf{0.85} & 0.58 & 0.17 & 0.8 & 0.51 & \textbf{0.85}\\ & 100 & \textbf{0.96} & 0.85 & 0.23 & \textbf{1.0} & 0.81 & 0.96 & \textbf{0.88} & 0.73 & 0.22 & 0.83 & 0.72 & \textbf{0.88}\\\hline%
\multicolumn{2}{c|}{\textsc{De}} & \textbf{0.71} & 0.59 & 0.28 & \textbf{0.78} & 0.53 & 0.68 & \textbf{0.69} & 0.56 & 0.22 & \textbf{0.76} & 0.54 & 0.68\\\hline%
\multicolumn{2}{c|}{\textsc{Dr}} & \textbf{0.67} & 0.6 & 0.48 & \textbf{0.75} & 0.65 & 0.67 & \textbf{0.61} & \textbf{0.61} & 0.52 & \textbf{0.73} & 0.63 & 0.61\\\hline%
\multicolumn{2}{c|}{\textsc{dwr}} & \textbf{0.82} & 0.6 & 0.34 & \textbf{0.86} & 0.61 & 0.82 & \textbf{0.82} & 0.58 & 0.39 & \textbf{0.82} & 0.58 & \textbf{0.82}\\\hline%
\multicolumn{2}{c|}{\textsc{Fe}} & \textbf{0.95} & \textbf{0.95} & 0.48 & \textbf{0.95} & \textbf{0.95} & \textbf{0.95} & \textbf{0.88} & \textbf{0.88} & 0.47 & \textbf{0.88} & \textbf{0.88} & \textbf{0.88}\\\hline%
\multicolumn{2}{c|}{\textsc{Lo}} & 0.92 & \textbf{0.96} & 0.7 & \textbf{0.96} & 0.92 & 0.88 & 0.9 & \textbf{0.93} & 0.72 & \textbf{0.93} & 0.92 & 0.9\\\hline%
\multicolumn{2}{c|}{\textsc{Mi}} & 0.82 & \textbf{0.89} & 0.79 & \textbf{0.96} & 0.89 & 0.82 & 0.79 & \textbf{0.88} & 0.79 & \textbf{0.93} & 0.88 & 0.79\\\hline%
\multicolumn{2}{c|}{\textsc{Ro}} & 0.77 & \textbf{0.92} & 0.88 & \textbf{0.93} & 0.92 & 0.87 & 0.76 & \textbf{0.92} & 0.85 & \textbf{0.92} & \textbf{0.92} & 0.85\\\hline%
\multicolumn{2}{c|}{\textsc{Sa}} & 0.86 & \textbf{0.91} & 0.9 & \textbf{0.91} & \textbf{0.91} & 0.85 & 0.82 & \textbf{0.86} & 0.83 & \textbf{0.9} & 0.86 & 0.81\\\hline%
\multicolumn{2}{c|}{\textsc{ZT}} & \textbf{0.86} & 0.84 & 0.61 & 0.86 & 0.85 & \textbf{0.88} & \textbf{0.85} & 0.82 & 0.61 & 0.84 & 0.84 & \textbf{0.86}\\\hline%
\multicolumn{2}{c|}{AVG}  & \textbf{0.79} & 0.77 & 0.54 & \textbf{0.86} & 0.78 & 0.8 & \textbf{0.76} & 0.74 & 0.52 & \textbf{0.82} & 0.75 & 0.78\\
\bottomrule
\end{tabular}\\

==> tables-new/domains-full.tex <==
\begin{tabular}{cc|c|cc|cc}
\toprule
\multicolumn{3}{c}{} & \multicolumn{2}{c}{Optimal} & \multicolumn{2}{c}{Sub-Optimal}\\
\midrule
\# & \% & $|\goalconditions|$ & $|\observations|$ & $|\grsolution|$ & $|\observations|$ & $|\grsolution|$ \\
\midrule
\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{blocks}}}%

	 & 10
 & \multirow{5}{*}{20.33} & 1.25 & 8.0 & 1.42 & 7.61\\
	 & 30
 &  & 3.08 & 3.97 & 3.83 & 3.58\\
	 & 50
 &  & 4.42 & 2.5 & 5.92 & 3.19\\
	 & 70
 &  & 6.67 & 1.94 & 8.5 & 2.53\\
	 & 100
 &  & 8.83 & 1.83 & 11.83 & 2.25\\\hline\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{depots}}}%

	 & 10
 & \multirow{5}{*}{8.0} & 1.0 & 4.17 & 1.92 & 2.17\\
	 & 30
 &  & 2.92 & 1.94 & 4.5 & 1.83\\
	 & 50
 &  & 4.83 & 1.14 & 6.75 & 1.14\\
	 & 70
 &  & 6.83 & 1.06 & 9.75 & 1.14\\
	 & 100
 &  & 9.5 & 1.0 & 13.33 & 1.0\\\hline\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{driverlog}}}%

	 & 10
 & \multirow{5}{*}{6.67} & 1.75 & 2.36 & 2.17 & 1.92\\
	 & 30
 &  & 4.17 & 1.58 & 5.58 & 1.31\\
	 & 50
 &  & 6.33 & 1.22 & 8.75 & 1.33\\
	 & 70
 &  & 8.92 & 1.14 & 12.33 & 1.31\\
	 & 100
 &  & 12.17 & 1.08 & 17.0 & 1.17\\\hline\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{dwr}}}%

	 & 10
 & \multirow{5}{*}{6.67} & 2.83 & 3.47 & 3.25 & 2.89\\
	 & 30
 &  & 6.92 & 1.89 & 9.08 & 1.83\\
	 & 50
 &  & 11.33 & 1.36 & 14.5 & 1.53\\
	 & 70
 &  & 16.08 & 1.19 & 20.25 & 1.17\\
	 & 100
 &  & 22.0 & 1.08 & 28.33 & 1.08\\\hline\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{ipc-grid}}}%

	 & 10
 & \multirow{5}{*}{7.5} & 1.63 & 2.71 & 2.06 & 1.58\\
	 & 30
 &  & 4.0 & 1.21 & 5.56 & 1.4\\
	 & 50
 &  & 6.19 & 1.13 & 8.88 & 1.35\\
	 & 70
 &  & 8.69 & 1.04 & 12.56 & 1.31\\
	 & 100
 &  & 11.88 & 1.0 & 17.25 & 1.5\\\hline\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{ferry}}}%

	 & 10
 & \multirow{5}{*}{6.67} & 2.25 & 3.58 & 3.33 & 2.69\\
	 & 30
 &  & 6.0 & 1.64 & 8.75 & 1.42\\
	 & 50
 &  & 9.67 & 1.22 & 14.0 & 1.28\\
	 & 70
 &  & 13.5 & 1.19 & 19.67 & 1.28\\
	 & 100
 &  & 18.83 & 1.17 & 27.5 & 1.25\\\hline\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{logistics}}}%

	 & 10
 & \multirow{5}{*}{10.0} & 2.0 & 2.83 & 2.67 & 2.0\\
	 & 30
 &  & 5.75 & 1.19 & 7.5 & 1.14\\
	 & 50
 &  & 9.42 & 1.06 & 11.92 & 1.06\\
	 & 70
 &  & 13.25 & 1.03 & 16.67 & 1.03\\
	 & 100
 &  & 18.17 & 1.0 & 23.17 & 1.0\\\hline\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{miconic}}}%

	 & 10
 & \multirow{5}{*}{6.0} & 2.0 & 2.53 & 3.0 & 1.83\\
	 & 30
 &  & 5.42 & 1.22 & 7.67 & 1.25\\
	 & 50
 &  & 8.42 & 1.06 & 12.25 & 1.03\\
	 & 70
 &  & 11.92 & 1.0 & 17.33 & 1.0\\
	 & 100
 &  & 16.33 & 1.0 & 24.0 & 1.0\\\hline\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{rovers}}}%

	 & 10
 & \multirow{5}{*}{6.0} & 1.67 & 2.28 & 1.83 & 2.39\\
	 & 30
 &  & 3.67 & 1.31 & 4.5 & 1.39\\
	 & 50
 &  & 5.75 & 1.19 & 7.17 & 1.11\\
	 & 70
 &  & 8.17 & 1.0 & 10.0 & 1.06\\
	 & 100
 &  & 10.83 & 1.0 & 13.67 & 1.0\\\hline\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{satellite}}}%

	 & 10
 & \multirow{5}{*}{6.0} & 1.42 & 3.53 & 2.0 & 3.25\\
	 & 30
 &  & 3.42 & 2.39 & 4.33 & 1.78\\
	 & 50
 &  & 5.75 & 1.58 & 6.75 & 1.36\\
	 & 70
 &  & 8.08 & 1.31 & 9.42 & 1.33\\
	 & 100
 &  & 10.75 & 1.25 & 12.75 & 1.25\\\hline\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{sokoban}}}%

	 & 10
 & \multirow{5}{*}{8.67} & 2.33 & 2.11 & 3.33 & 1.83\\
	 & 30
 &  & 6.5 & 1.25 & 8.67 & 1.28\\
	 & 50
 &  & 10.33 & 1.22 & 13.75 & 1.33\\
	 & 70
 &  & 14.67 & 1.03 & 19.33 & 1.36\\
	 & 100
 &  & 20.17 & 1.0 & 27.0 & 1.33\\\hline\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{zeno}}}%

	 & 10
 & \multirow{5}{*}{6.0} & 1.75 & 2.36 & 2.0 & 1.78\\
	 & 30
 &  & 4.0 & 1.33 & 5.42 & 1.14\\
	 & 50
 &  & 6.17 & 1.03 & 8.25 & 1.06\\
	 & 70
 &  & 8.75 & 1.0 & 11.75 & 1.0\\
	 & 100
 &  & 12.0 & 1.0 & 16.17 & 1.0\\
\bottomrule
\end{tabular}\\

==> tables-new/domains-v2.tex <==
\begin{tabular}{c|c|c|cccccc}
\toprule
\multicolumn{3}{c|}{} & \rotatebox[origin=c]{90}{ \textsc{blocks} } & \rotatebox[origin=c]{90}{ \textsc{depots} } & \rotatebox[origin=c]{90}{ \textsc{driverlog} } & \rotatebox[origin=c]{90}{ \textsc{dwr} } & \rotatebox[origin=c]{90}{ \textsc{ipc-grid} } & \rotatebox[origin=c]{90}{ \textsc{ferry} }\\\midrule
\multicolumn{3}{c|}{$|\goalconditions|$} & 20.33 & 8.0 & 6.67 & 6.67 & 7.5 & 6.67\\\midrule
\multirow{10}{*}{ \rotatebox[origin=c]{90}{\textsc{Optimal}} }& \multicolumn{1}{c}{ \multirow{5}{*}{$|\observations|$} }& \multicolumn{1}{|c|}{10\%}& 1.25& 1.0& 1.75& 2.83& 1.63& 2.25\\
& \multicolumn{1}{c}{}& \multicolumn{1}{|c|}{30\%}& 3.08& 2.92& 4.17& 6.92& 4.0& 6.0\\
& \multicolumn{1}{c}{}& \multicolumn{1}{|c|}{50\%}& 4.42& 4.83& 6.33& 11.33& 6.19& 9.67\\
& \multicolumn{1}{c}{}& \multicolumn{1}{|c|}{70\%}& 6.67& 6.83& 8.92& 16.08& 8.69& 13.5\\
& \multicolumn{1}{c}{}& \multicolumn{1}{|c|}{100\%}& 8.83& 9.5& 12.17& 22.0& 11.88& 18.83\\
\cline{2-9}
& \multicolumn{1}{c}{ \multirow{5}{*}{$|\grsolution|$} }& \multicolumn{1}{|c|}{10\%} & 8.0 & 4.17 & 2.36 & 3.47 & 2.71 & 3.58\\
& \multicolumn{1}{c}{}& \multicolumn{1}{|c|}{30\%} & 3.97 & 1.94 & 1.58 & 1.89 & 1.21 & 1.64\\
& \multicolumn{1}{c}{}& \multicolumn{1}{|c|}{50\%} & 2.5 & 1.14 & 1.22 & 1.36 & 1.13 & 1.22\\
& \multicolumn{1}{c}{}& \multicolumn{1}{|c|}{70\%} & 1.94 & 1.06 & 1.14 & 1.19 & 1.04 & 1.19\\
& \multicolumn{1}{c}{}& \multicolumn{1}{|c|}{100\%} & 1.83 & 1.0 & 1.08 & 1.08 & 1.0 & 1.17\\
\midrule
\multirow{10}{*}{ \rotatebox[origin=c]{90}{\textsc{Sub-optimal}} }& \multicolumn{1}{c}{ \multirow{5}{*}{$|\observations|$} }& \multicolumn{1}{|c|}{10\%}& 1.42& 1.92& 2.17& 3.25& 2.06& 3.33\\
& \multicolumn{1}{c}{}& \multicolumn{1}{|c|}{30\%}& 3.83& 4.5& 5.58& 9.08& 5.56& 8.75\\
& \multicolumn{1}{c}{}& \multicolumn{1}{|c|}{50\%}& 5.92& 6.75& 8.75& 14.5& 8.88& 14.0\\
& \multicolumn{1}{c}{}& \multicolumn{1}{|c|}{70\%}& 8.5& 9.75& 12.33& 20.25& 12.56& 19.67\\
& \multicolumn{1}{c}{}& \multicolumn{1}{|c|}{100\%}& 11.83& 13.33& 17.0& 28.33& 17.25& 27.5\\
\cline{2-9}
& \multicolumn{1}{c}{ \multirow{5}{*}{$|\grsolution|$} }& \multicolumn{1}{|c|}{10\%} & 7.61 & 2.17 & 1.92 & 2.89 & 1.58 & 2.69\\
& \multicolumn{1}{c}{}& \multicolumn{1}{|c|}{30\%} & 3.58 & 1.83 & 1.31 & 1.83 & 1.4 & 1.42\\
& \multicolumn{1}{c}{}& \multicolumn{1}{|c|}{50\%} & 3.19 & 1.14 & 1.33 & 1.53 & 1.35 & 1.28\\
& \multicolumn{1}{c}{}& \multicolumn{1}{|c|}{70\%} & 2.53 & 1.14 & 1.31 & 1.17 & 1.31 & 1.28\\
& \multicolumn{1}{c}{}& \multicolumn{1}{|c|}{100\%} & 2.25 & 1.0 & 1.17 & 1.08 & 1.5 & 1.25\\
\bottomrule
\end{tabular}
\vspace{0.25cm}
\begin{tabular}{c|c|c|cccccc}
\toprule
\multicolumn{3}{c|}{} & \rotatebox[origin=c]{90}{ \textsc{logistics} } & \rotatebox[origin=c]{90}{ \textsc{miconic} } & \rotatebox[origin=c]{90}{ \textsc{rovers} } & \rotatebox[origin=c]{90}{ \textsc{satellite} } & \rotatebox[origin=c]{90}{ \textsc{sokoban} } & \rotatebox[origin=c]{90}{ \textsc{zeno} }\\\midrule
\multicolumn{3}{c|}{$|\goalconditions|$} & 10.0 & 6.0 & 6.0 & 6.0 & 8.67 & 6.0\\\midrule
\multirow{10}{*}{ \rotatebox[origin=c]{90}{\textsc{Optimal}} }& \multicolumn{1}{c}{ \multirow{5}{*}{$|\observations|$} }& \multicolumn{1}{|c|}{10\%}& 2.0& 2.0& 1.67& 1.42& 2.33& 1.75\\
& \multicolumn{1}{c}{}& \multicolumn{1}{|c|}{30\%}& 5.75& 5.42& 3.67& 3.42& 6.5& 4.0\\
& \multicolumn{1}{c}{}& \multicolumn{1}{|c|}{50\%}& 9.42& 8.42& 5.75& 5.75& 10.33& 6.17\\
& \multicolumn{1}{c}{}& \multicolumn{1}{|c|}{70\%}& 13.25& 11.92& 8.17& 8.08& 14.67& 8.75\\
& \multicolumn{1}{c}{}& \multicolumn{1}{|c|}{100\%}& 18.17& 16.33& 10.83& 10.75& 20.17& 12.0\\
\cline{2-9}
& \multicolumn{1}{c}{ \multirow{5}{*}{$|\grsolution|$} }& \multicolumn{1}{|c|}{10\%} & 2.83 & 2.53 & 2.28 & 3.53 & 2.11 & 2.36\\
& \multicolumn{1}{c}{}& \multicolumn{1}{|c|}{30\%} & 1.19 & 1.22 & 1.31 & 2.39 & 1.25 & 1.33\\
& \multicolumn{1}{c}{}& \multicolumn{1}{|c|}{50\%} & 1.06 & 1.06 & 1.19 & 1.58 & 1.22 & 1.03\\
& \multicolumn{1}{c}{}& \multicolumn{1}{|c|}{70\%} & 1.03 & 1.0 & 1.0 & 1.31 & 1.03 & 1.0\\
& \multicolumn{1}{c}{}& \multicolumn{1}{|c|}{100\%} & 1.0 & 1.0 & 1.0 & 1.25 & 1.0 & 1.0\\
\midrule
\multirow{10}{*}{ \rotatebox[origin=c]{90}{\textsc{Sub-optimal}} }& \multicolumn{1}{c}{ \multirow{5}{*}{$|\observations|$} }& \multicolumn{1}{|c|}{10\%}& 2.67& 3.0& 1.83& 2.0& 3.33& 2.0\\
& \multicolumn{1}{c}{}& \multicolumn{1}{|c|}{30\%}& 7.5& 7.67& 4.5& 4.33& 8.67& 5.42\\
& \multicolumn{1}{c}{}& \multicolumn{1}{|c|}{50\%}& 11.92& 12.25& 7.17& 6.75& 13.75& 8.25\\
& \multicolumn{1}{c}{}& \multicolumn{1}{|c|}{70\%}& 16.67& 17.33& 10.0& 9.42& 19.33& 11.75\\
& \multicolumn{1}{c}{}& \multicolumn{1}{|c|}{100\%}& 23.17& 24.0& 13.67& 12.75& 27.0& 16.17\\
\cline{2-9}
& \multicolumn{1}{c}{ \multirow{5}{*}{$|\grsolution|$} }& \multicolumn{1}{|c|}{10\%} & 2.0 & 1.83 & 2.39 & 3.25 & 1.83 & 1.78\\
& \multicolumn{1}{c}{}& \multicolumn{1}{|c|}{30\%} & 1.14 & 1.25 & 1.39 & 1.78 & 1.28 & 1.14\\
& \multicolumn{1}{c}{}& \multicolumn{1}{|c|}{50\%} & 1.06 & 1.03 & 1.11 & 1.36 & 1.33 & 1.06\\
& \multicolumn{1}{c}{}& \multicolumn{1}{|c|}{70\%} & 1.03 & 1.0 & 1.06 & 1.33 & 1.36 & 1.0\\
& \multicolumn{1}{c}{}& \multicolumn{1}{|c|}{100\%} & 1.0 & 1.0 & 1.0 & 1.25 & 1.33 & 1.0\\

\bottomrule
\end{tabular}\\

==> tables-new/domains.tex <==
\begin{tabular}{cc|c|cc|cc}
\toprule
\multicolumn{3}{c}{} & \multicolumn{2}{c}{Optimal} & \multicolumn{2}{c}{Sub-Optimal}\\
\midrule
\# & \% & $|\goalconditions|$ & $|\observations|$ & $|\grsolution|$ & $|\observations|$ & $|\grsolution|$ \\
\midrule
\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{blocks}}}%
	 & 10
 & \multirow{5}{*}{20.33} & 1.25 & 8.0 & 1.42 & 7.61\\
	 & 30
 &  & 3.08 & 3.97 & 3.83 & 3.58\\
	 & 50
 &  & 4.42 & 2.5 & 5.92 & 3.19\\
	 & 70
 &  & 6.67 & 1.94 & 8.5 & 2.53\\
	 & 100
 &  & 8.83 & 1.83 & 11.83 & 2.25\\\hline
 \multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{ipc-grid}}}%
	 & 10
 & \multirow{5}{*}{7.5} & 1.63 & 2.71 & 2.06 & 1.58\\
	 & 30
 &  & 4.0 & 1.21 & 5.56 & 1.4\\
	 & 50
 &  & 6.19 & 1.13 & 8.88 & 1.35\\
	 & 70
 &  & 8.69 & 1.04 & 12.56 & 1.31\\
	 & 100
 &  & 11.88 & 1.0 & 17.25 & 1.5\\\hline
 \multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{sokoban}}}%
	 & 10
 & \multirow{5}{*}{8.67} & 2.33 & 2.11 & 3.33 & 1.83\\
	 & 30
 &  & 6.5 & 1.25 & 8.67 & 1.28\\
	 & 50
 &  & 10.33 & 1.22 & 13.75 & 1.33\\
	 & 70
 &  & 14.67 & 1.03 & 19.33 & 1.36\\
	 & 100
 &  & 20.17 & 1.0 & 27.0 & 1.33\\\hline
 \multicolumn{2}{c|}{\textsc{De}} & 8.0 & 5.02 & 1.86 & 7.25 & 1.46\\\hline
 \multicolumn{2}{c|}{\textsc{Dr}} & 6.67 & 6.67 & 1.48 & 9.17 & 1.41\\\hline
 \multicolumn{2}{c|}{\textsc{dwr}} & 6.67 & 11.83 & 1.8 & 15.08 & 1.7\\\hline
 \multicolumn{2}{c|}{\textsc{Fe}} & 6.67 & 10.05 & 1.76 & 14.65 & 1.58\\\hline
 \multicolumn{2}{c|}{\textsc{Lo}} & 10.0 & 9.72 & 1.42 & 12.38 & 1.24\\\hline
 \multicolumn{2}{c|}{\textsc{Mi}} & 6.0 & 8.82 & 1.36 & 12.85 & 1.22\\\hline
 \multicolumn{2}{c|}{\textsc{Ro}} & 6.0 & 6.02 & 1.36 & 7.43 & 1.39\\\hline
 \multicolumn{2}{c|}{\textsc{Sa}} & 6.0 & 5.88 & 2.01 & 7.05 & 1.79\\\hline
 \multicolumn{2}{c|}{\textsc{ZT}} & 6.0 & 6.53 & 1.34 & 8.72 & 1.19\\
\bottomrule
\end{tabular}\\

==> tables-new/noisy.tex <==
\begin{tabular}{cc|cccc|cccc}
\toprule
 \multicolumn{2}{c}{} & \multicolumn{4}{c}{Optimal} & \multicolumn{4}{c}{Sub-Optimal}\\
\cmidrule(lr){3-6}\cmidrule(lr){7-10}
%
\# & \% & \dhc & \dhcf & \rg & \pom & \dhc & \dhcf & \rg & \pom\\%
%
\midrule
\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{blocks}}}%
 & 10 & \textbf{0.32} & \textbf{0.32} & 0.31 & 0.06 & 0.38 & 0.38 & \textbf{0.42} & 0.05\\ & 30 & 0.37 & 0.37 & \textbf{0.39} & 0.13 & 0.36 & 0.37 & \textbf{0.49} & 0.22\\ & 50 & \textbf{0.64} & \textbf{0.64} & 0.6 & 0.37 & 0.53 & 0.53 & \textbf{0.55} & 0.28\\ & 70 & 0.79 & \textbf{0.81} & 0.77 & 0.47 & \textbf{0.67} & \textbf{0.67} & 0.63 & 0.38\\ & 100 & 0.88 & 0.88 & \textbf{0.89} & 0.57 & 0.78 & \textbf{0.82} & 0.74 & 0.51\\\hline%
 \multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{ipc-grid}}}%
 & 10 & \textbf{0.57} & \textbf{0.57} & 0.16 & 0.38 & \textbf{0.62} & \textbf{0.62} & 0.12 & 0.54\\ & 30 & \textbf{0.85} & \textbf{0.85} & 0.28 & 0.71 & 0.68 & 0.68 & 0.08 & \textbf{0.72}\\ & 50 & \textbf{0.89} & \textbf{0.89} & 0.07 & 0.81 & 0.84 & 0.84 & 0.04 & \textbf{0.85}\\ & 70 & \textbf{0.95} & \textbf{0.95} & 0.15 & 0.93 & 0.89 & 0.89 & 0.02 & \textbf{0.9}\\ & 100 & \textbf{1.0} & \textbf{1.0} & 0.08 & 0.99 & \textbf{0.94} & \textbf{0.94} & 0.04 & 0.92\\\hline%
 \multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{sokoban}}}%
 & 10 & \textbf{0.27} & \textbf{0.27} & 0.1 & 0.24 & 0.31 & \textbf{0.32} & 0.13 & 0.25\\ & 30 & 0.56 & \textbf{0.7} & 0.2 & 0.34 & 0.48 & \textbf{0.56} & 0.12 & 0.29\\ & 50 & 0.61 & \textbf{0.82} & 0.2 & 0.57 & 0.5 & \textbf{0.73} & 0.01 & 0.46\\ & 70 & 0.6 & \textbf{0.97} & 0.08 & 0.84 & 0.54 & \textbf{0.8} & 0.06 & 0.58\\ & 100 & 0.66 & \textbf{1.0} & 0.04 & 0.96 & 0.35 & \textbf{0.85} & 0.04 & 0.77\\\hline%
\multicolumn{2}{c|}{\textsc{De}} & \textbf{0.65} & \textbf{0.65} & 0.02 & 0.46 & 0.65 & \textbf{0.68} & 0.02 & 0.45\\\hline%
\multicolumn{2}{c|}{\textsc{Dr}} & 0.68 & \textbf{0.69} & 0.23 & 0.49 & 0.66 & \textbf{0.68} & 0.21 & 0.49\\\hline%
\multicolumn{2}{c|}{\textsc{dwr}} & 0.66 & \textbf{0.67} & 0.15 & 0.57 & 0.64 & \textbf{0.65} & 0.11 & 0.64\\\hline%
\multicolumn{2}{c|}{\textsc{Fe}} & 0.69 & \textbf{0.71} & 0.58 & 0.64 & 0.65 & \textbf{0.67} & 0.57 & 0.6\\\hline%
\multicolumn{2}{c|}{\textsc{Lo}} & \textbf{0.85} & \textbf{0.85} & 0.05 & 0.81 & 0.84 & \textbf{0.85} & 0.09 & 0.82\\\hline%
\multicolumn{2}{c|}{\textsc{Mi}} & 0.76 & \textbf{0.79} & 0.76 & 0.74 & 0.78 & \textbf{0.81} & 0.79 & 0.78\\\hline%
\multicolumn{2}{c|}{\textsc{Ro}} & \textbf{0.77} & 0.76 & 0.36 & 0.72 & \textbf{0.78} & 0.77 & 0.37 & 0.69\\\hline%
\multicolumn{2}{c|}{\textsc{Sa}} & \textbf{0.7} & \textbf{0.7} & 0.52 & 0.59 & 0.72 & \textbf{0.75} & 0.53 & 0.63\\\hline%
\multicolumn{2}{c|}{\textsc{ZT}} & 0.73 & \textbf{0.75} & 0.66 & 0.61 & 0.73 & \textbf{0.76} & 0.7 & 0.68\\\hline%

\multicolumn{2}{c|}{AVG} & 0.71 & \textbf{0.73} & 0.35 & 0.61 & 0.69 & \textbf{0.72} & 0.34 & 0.61\\\midrule\midrule%
\multicolumn{2}{c|}{ACC} & 0.89 & \textbf{0.9} & 0.5 & 0.73 & 0.87 & \textbf{0.89} & 0.48 & 0.76\\\midrule%
\multicolumn{2}{c|}{SPR} & 1.91 & 1.78 & 1.38 & \textbf{1.3} & 1.93 & 1.72 & 1.34 & \textbf{1.31}%
\\
\bottomrule
\end{tabular}\\

==> tables-new/uncertainty-sub.tex <==
\begin{tabular}{cc|ccc|ccc|ccc|ccc|ccc|ccc}
\toprule
 \multicolumn{2}{c}{} & \multicolumn{18}{c}{Sub-Optimal}\\
\cmidrule(lr){3-20}
%
 \multicolumn{2}{c}{} & \multicolumn{3}{c}{\dhc} & \multicolumn{3}{c}{\dhcu} & \multicolumn{3}{c}{\rg} & \multicolumn{3}{c}{\pom} & \multicolumn{3}{c}{\pomA} & \multicolumn{3}{c}{\pomC}\\%
%
\cmidrule(lr){3-5}\cmidrule(lr){6-8}\cmidrule(lr){9-11}\cmidrule(lr){12-14}\cmidrule(lr){15-17}\cmidrule(lr){18-20}\\
\# & \% %
& AGR & ACC & SPR & AGR & ACC & SPR & AGR & ACC & SPR & AGR & ACC & SPR & AGR & ACC & SPR & AGR & ACC & SPR\\
\midrule
\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{blocks}}}%
 & 10 & 0.41 & 0.86 & 6.86 & 0.42 & 0.89 & 7.42 & \textbf{0.46} & 0.97 & 10.61 & 0.06 & 0.19 & 1.19 & 0.19 & 0.58 & 4.44 & 0.34 & 1.0 & 17.53\\ & 30 & 0.49 & 0.78 & 3.17 & 0.35 & 0.86 & 6.92 & \textbf{0.54} & 1.0 & 4.86 & 0.28 & 0.56 & 1.17 & 0.32 & 0.89 & 3.36 & 0.26 & 1.0 & 13.47\\ & 50 & 0.55 & 0.86 & 3.08 & 0.42 & 0.94 & 5.61 & \textbf{0.62} & 0.97 & 2.72 & 0.39 & 0.72 & 1.08 & 0.36 & 0.81 & 2.17 & 0.27 & 1.0 & 9.89\\ & 70 & \textbf{0.71} & 0.92 & 2.06 & 0.56 & 0.94 & 3.06 & 0.68 & 1.0 & 2.44 & 0.51 & 0.94 & 1.33 & 0.44 & 1.0 & 2.22 & 0.26 & 1.0 & 8.61\\ & 100 & \textbf{0.84} & 1.0 & 1.67 & \textbf{0.84} & 1.0 & 1.67 & 0.8 & 1.0 & 2.08 & 0.51 & 1.0 & 1.67 & 0.48 & 1.0 & 1.92 & 0.28 & 1.0 & 6.42\\\hline%
 \multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{ipc-grid}}}%
 & 10 & 0.77 & 0.92 & 1.81 & 0.75 & 0.98 & 2.4 & \textbf{0.81} & 1.0 & 2.73 & 0.64 & 0.88 & 2.23 & 0.59 & 0.98 & 3.44 & 0.42 & 1.0 & 5.6\\ & 30 & 0.82 & 0.94 & 1.13 & 0.77 & 0.98 & 1.6 & \textbf{0.9} & 1.0 & 1.27 & 0.81 & 0.96 & 1.35 & 0.8 & 0.96 & 1.52 & 0.67 & 0.96 & 2.23\\ & 50 & 0.84 & 0.94 & 1.13 & 0.84 & 1.0 & 1.56 & \textbf{0.92} & 1.0 & 1.1 & 0.87 & 1.0 & 1.08 & 0.86 & 1.0 & 1.13 & 0.86 & 1.0 & 1.21\\ & 70 & 0.89 & 1.0 & 1.1 & 0.85 & 1.0 & 1.23 & \textbf{0.93} & 1.0 & 1.02 & 0.92 & 1.0 & 1.0 & 0.92 & 1.0 & 1.0 & 0.92 & 1.0 & 1.0\\ & 100 & \textbf{0.94} & 1.0 & 1.0 & \textbf{0.94} & 1.0 & 1.0 & \textbf{0.94} & 1.0 & 1.0 & \textbf{0.94} & 1.0 & 1.0 & \textbf{0.94} & 1.0 & 1.0 & \textbf{0.94} & 1.0 & 1.0\\\hline%
 \multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{sokoban}}}%
 & 10 & \textbf{0.52} & 0.61 & 1.78 & 0.44 & 0.72 & 3.17 & 0.29 & 0.64 & 4.56 & 0.35 & 0.64 & 2.47 & 0.38 & 0.92 & 4.08 & 0.24 & 1.0 & 6.86\\ & 30 & \textbf{0.77} & 0.83 & 1.08 & 0.62 & 0.97 & 2.67 & 0.43 & 0.75 & 2.92 & 0.56 & 0.75 & 1.72 & 0.51 & 0.86 & 2.64 & 0.24 & 0.97 & 5.5\\ & 50 & \textbf{0.79} & 0.92 & 1.17 & 0.66 & 1.0 & 2.58 & 0.53 & 0.72 & 1.83 & 0.58 & 0.75 & 1.39 & 0.53 & 0.86 & 2.31 & 0.25 & 0.97 & 5.14\\ & 70 & 0.8 & 0.97 & 1.03 & \textbf{0.85} & 1.0 & 1.39 & 0.54 & 0.61 & 1.28 & 0.63 & 0.86 & 1.25 & 0.59 & 0.92 & 1.75 & 0.3 & 1.0 & 4.11\\ & 100 & \textbf{0.83} & 1.0 & 1.0 & \textbf{0.83} & 1.0 & 1.0 & 0.58 & 0.58 & 1.33 & \textbf{0.83} & 1.0 & 1.0 & \textbf{0.83} & 1.0 & 1.0 & 0.38 & 1.0 & 2.75\\\hline%
\multicolumn{2}{c|}{\textsc{De}} & \textbf{0.76} & 0.85 & 1.6 & 0.6 & 0.92 & 2.97 & 0.62 & 0.87 & 2.63 & 0.57 & 0.66 & 1.51 & 0.52 & 0.81 & 2.36 & 0.28 & 0.98 & 5.29\\\hline%
\multicolumn{2}{c|}{\textsc{Dr}} & \textbf{0.73} & 0.92 & 1.67 & 0.6 & 0.96 & 2.62 & 0.51 & 0.92 & 2.87 & 0.57 & 0.8 & 1.41 & 0.52 & 0.84 & 1.83 & 0.31 & 0.98 & 4.3\\\hline%
\multicolumn{2}{c|}{\textsc{dwr}} & \textbf{0.82} & 0.93 & 1.7 & 0.73 & 0.98 & 2.7 & 0.71 & 0.92 & 2.31 & 0.74 & 0.84 & 1.16 & 0.73 & 0.97 & 2.44 & 0.3 & 1.0 & 5.68\\\hline%
\multicolumn{2}{c|}{\textsc{Fe}} & \textbf{0.88} & 1.0 & 1.96 & 0.76 & 1.0 & 2.62 & 0.84 & 0.98 & 1.86 & 0.79 & 0.88 & 1.26 & 0.75 & 0.96 & 1.92 & 0.37 & 1.0 & 4.57\\\hline%
\multicolumn{2}{c|}{\textsc{Lo}} & \textbf{0.93} & 0.99 & 1.42 & 0.87 & 1.0 & 1.71 & 0.9 & 0.98 & 1.56 & 0.87 & 0.91 & 1.27 & 0.81 & 0.98 & 2.07 & 0.45 & 1.0 & 4.62\\\hline%
\multicolumn{2}{c|}{\textsc{Mi}} & \textbf{0.93} & 1.0 & 1.45 & 0.82 & 1.0 & 1.86 & 0.83 & 1.0 & 1.79 & 0.87 & 0.89 & 1.09 & 0.72 & 0.98 & 2.17 & 0.31 & 1.0 & 4.62\\\hline%
\multicolumn{2}{c|}{\textsc{Ro}} & \textbf{0.92} & 0.93 & 1.5 & 0.88 & 0.94 & 1.64 & 0.9 & 1.0 & 1.79 & 0.76 & 0.84 & 1.15 & 0.67 & 0.98 & 2.14 & 0.39 & 1.0 & 4.02\\\hline%
\multicolumn{2}{c|}{\textsc{Sa}} & \textbf{0.9} & 0.97 & 1.92 & 0.89 & 0.97 & 2.01 & 0.75 & 0.97 & 2.76 & 0.73 & 0.89 & 1.51 & 0.59 & 0.96 & 2.88 & 0.43 & 1.0 & 4.71\\\hline%
\multicolumn{2}{c|}{\textsc{ZT}} & \textbf{0.84} & 0.91 & 1.42 & 0.78 & 0.97 & 1.87 & 0.78 & 0.93 & 1.72 & 0.76 & 0.82 & 1.19 & 0.74 & 0.93 & 1.64 & 0.36 & 1.0 & 4.03\\\midrule%
\multicolumn{2}{c|}{AVG} & \textbf{0.82} & 0.93 & 1.71 & 0.75 & 0.97 & 2.39 & 0.74 & 0.93 & 2.3 & 0.7 & 0.83 & 1.31 & 0.65 & 0.93 & 2.19 & 0.38 & 1.0 & 5.01%
\\
\bottomrule
\end{tabular}\\

==> tables-new/uncertainty.tex <==
\begin{tabular}{cc|ccc|ccc|ccc|ccc|ccc|ccc}
\toprule
 \multicolumn{2}{c}{} & \multicolumn{18}{c}{Optimal}\\
\cmidrule(lr){3-20}
%
 \multicolumn{2}{c}{} & \multicolumn{3}{c}{\dhc} & \multicolumn{3}{c}{\dhcu} & \multicolumn{3}{c}{\rg} & \multicolumn{3}{c}{\pom} & \multicolumn{3}{c}{\pomA} & \multicolumn{3}{c}{\pomC}\\%
%
\cmidrule(lr){3-5}\cmidrule(lr){6-8}\cmidrule(lr){9-11}\cmidrule(lr){12-14}\cmidrule(lr){15-17}\cmidrule(lr){18-20}\\
\# & \% %
& AGR & ACC & SPR & AGR & ACC & SPR & AGR & ACC & SPR & AGR & ACC & SPR & AGR & ACC & SPR & AGR & ACC & SPR\\
\midrule
\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{blocks}}}%
 & 10 & 0.44 & 0.86 & 7.53 & 0.44 & 0.86 & 7.56 & \textbf{0.47} & 0.92 & 9.83 & 0.06 & 0.17 & 1.44 & 0.13 & 0.47 & 4.06 & 0.38 & 1.0 & 18.14\\ & 30 & \textbf{0.46} & 0.78 & 2.5 & 0.44 & 0.86 & 4.67 & 0.45 & 0.92 & 5.56 & 0.21 & 0.39 & 1.17 & 0.3 & 0.75 & 2.94 & 0.24 & 1.0 & 15.25\\ & 50 & 0.59 & 0.89 & 3.03 & 0.52 & 0.89 & 3.86 & \textbf{0.62} & 0.97 & 3.69 & 0.33 & 0.58 & 1.25 & 0.37 & 0.81 & 3.08 & 0.25 & 0.97 & 12.17\\ & 70 & \textbf{0.85} & 0.97 & 1.83 & 0.76 & 0.97 & 2.42 & 0.81 & 1.0 & 2.22 & 0.51 & 0.72 & 1.14 & 0.45 & 0.94 & 2.19 & 0.25 & 1.0 & 9.22\\ & 100 & \textbf{0.92} & 1.0 & 1.67 & \textbf{0.92} & 1.0 & 1.67 & 0.9 & 1.0 & 2.08 & 0.59 & 1.0 & 1.67 & 0.55 & 1.0 & 1.92 & 0.31 & 1.0 & 6.42\\\hline%
 \multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{ipc-grid}}}%
 & 10 & 0.87 & 0.94 & 2.67 & 0.88 & 0.96 & 2.69 & \textbf{0.91} & 1.0 & 3.23 & 0.47 & 0.75 & 2.35 & 0.55 & 0.98 & 4.38 & 0.49 & 1.0 & 6.25\\ & 30 & 0.93 & 0.96 & 1.15 & 0.94 & 0.98 & 1.17 & \textbf{0.99} & 1.0 & 1.25 & 0.85 & 0.98 & 1.52 & 0.81 & 1.0 & 1.96 & 0.64 & 1.0 & 3.17\\ & 50 & 0.96 & 0.98 & 1.08 & 0.96 & 0.98 & 1.08 & \textbf{1.0} & 1.0 & 1.13 & 0.86 & 1.0 & 1.44 & 0.86 & 1.0 & 1.56 & 0.77 & 1.0 & 2.15\\ & 70 & 0.97 & 0.98 & 1.06 & 0.97 & 0.98 & 1.06 & \textbf{1.0} & 1.0 & 1.04 & 0.97 & 0.98 & 1.02 & 0.97 & 0.98 & 1.02 & 0.93 & 0.98 & 1.15\\ & 100 & \textbf{1.0} & 1.0 & 1.0 & \textbf{1.0} & 1.0 & 1.0 & \textbf{1.0} & 1.0 & 1.0 & \textbf{1.0} & 1.0 & 1.0 & \textbf{1.0} & 1.0 & 1.0 & \textbf{1.0} & 1.0 & 1.0\\\hline%
 \multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{sokoban}}}%
 & 10 & 0.39 & 0.53 & 2.08 & 0.38 & 0.61 & 2.94 & \textbf{0.4} & 0.81 & 4.86 & 0.28 & 0.53 & 2.14 & 0.32 & 0.89 & 4.39 & 0.26 & 0.97 & 7.0\\ & 30 & \textbf{0.75} & 0.81 & 1.25 & 0.64 & 0.92 & 2.06 & 0.56 & 0.86 & 2.53 & 0.57 & 0.69 & 1.22 & 0.48 & 0.75 & 1.89 & 0.23 & 0.94 & 5.17\\ & 50 & \textbf{0.92} & 1.0 & 1.19 & 0.83 & 1.0 & 1.39 & 0.61 & 0.86 & 2.14 & 0.61 & 0.69 & 1.42 & 0.55 & 0.81 & 2.14 & 0.28 & 1.0 & 5.08\\ & 70 & \textbf{0.99} & 1.0 & 1.0 & 0.94 & 1.0 & 1.08 & 0.64 & 0.83 & 1.53 & 0.85 & 0.92 & 1.17 & 0.81 & 0.94 & 1.39 & 0.36 & 1.0 & 3.64\\ & 100 & \textbf{1.0} & 1.0 & 1.0 & \textbf{1.0} & 1.0 & 1.0 & 0.67 & 0.75 & 1.17 & \textbf{1.0} & 1.0 & 1.0 & \textbf{1.0} & 1.0 & 1.0 & 0.42 & 1.0 & 2.75\\\hline%
\multicolumn{2}{c|}{\textsc{De}} & \textbf{0.77} & 0.83 & 1.94 & 0.73 & 0.86 & 2.25 & 0.69 & 0.89 & 2.82 & 0.57 & 0.58 & 1.39 & 0.53 & 0.74 & 2.28 & 0.33 & 0.97 & 5.23\\\hline%
\multicolumn{2}{c|}{\textsc{Dr}} & \textbf{0.75} & 0.91 & 1.69 & 0.73 & 0.92 & 1.83 & 0.5 & 0.94 & 3.36 & 0.56 & 0.71 & 1.32 & 0.54 & 0.78 & 1.72 & 0.3 & 0.96 & 4.57\\\hline%
\multicolumn{2}{c|}{\textsc{dwr}} & \textbf{0.86} & 0.93 & 1.77 & 0.81 & 0.98 & 2.44 & 0.72 & 0.87 & 2.24 & 0.71 & 0.79 & 1.14 & 0.73 & 0.98 & 2.47 & 0.32 & 1.0 & 5.75\\\hline%
\multicolumn{2}{c|}{\textsc{Fe}} & \textbf{0.95} & 1.0 & 1.98 & 0.92 & 1.0 & 2.09 & 0.92 & 0.98 & 1.83 & 0.81 & 0.84 & 1.3 & 0.8 & 0.97 & 2.01 & 0.38 & 1.0 & 4.74\\\hline%
\multicolumn{2}{c|}{\textsc{Lo}} & \textbf{0.95} & 1.0 & 1.64 & \textbf{0.95} & 1.0 & 1.64 & 0.93 & 1.0 & 1.77 & 0.82 & 0.88 & 1.33 & 0.8 & 0.98 & 2.29 & 0.46 & 1.0 & 4.87\\\hline%
\multicolumn{2}{c|}{\textsc{Mi}} & \textbf{0.96} & 1.0 & 1.5 & \textbf{0.96} & 1.0 & 1.5 & 0.83 & 1.0 & 1.86 & 0.82 & 0.87 & 1.19 & 0.73 & 0.99 & 2.19 & 0.34 & 1.0 & 4.67\\\hline%
\multicolumn{2}{c|}{\textsc{Ro}} & \textbf{0.93} & 0.97 & 1.46 & \textbf{0.93} & 0.97 & 1.46 & 0.9 & 1.0 & 1.72 & 0.79 & 0.84 & 1.13 & 0.72 & 0.96 & 2.01 & 0.39 & 1.0 & 3.86\\\hline%
\multicolumn{2}{c|}{\textsc{Sa}} & \textbf{0.91} & 0.97 & 2.04 & \textbf{0.91} & 0.97 & 2.06 & 0.81 & 0.97 & 2.68 & 0.73 & 0.86 & 1.56 & 0.67 & 0.96 & 2.84 & 0.45 & 1.0 & 4.71\\\hline%
\multicolumn{2}{c|}{\textsc{ZT}} & \textbf{0.85} & 0.91 & 1.39 & 0.83 & 0.93 & 1.54 & 0.77 & 0.92 & 1.8 & 0.72 & 0.78 & 1.2 & 0.67 & 0.89 & 1.81 & 0.35 & 1.0 & 4.37\\\midrule%
\multicolumn{2}{c|}{AVG}  & \textbf{0.86} & 0.94 & 1.79 & 0.84 & 0.95 & 1.99 & 0.77 & 0.95 & 2.39 & 0.7 & 0.79 & 1.31 & 0.67 & 0.91 & 2.22 & 0.39 & 0.99 & 5.2%
\\
\bottomrule
\end{tabular}\\

==> tables/constraints-1.tex <==
\begin{tabular}[t]{cc|ccc|ccc|c||ccc|ccc|c}
\toprule
\multicolumn{2}{c}{} & \multicolumn{7}{c}{Optimal} & \multicolumn{7}{c}{Sub-Optimal}\\
\cmidrule(lr){3-9}\cmidrule(lr){10-16}
\# & \% & S & L & P & S, L & L, P & L, P & S, L, P%
& S & L & P & S, L & L, P & S, P & S, L, P\\
\midrule
\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{blocks}}}%
 & 10 & \textbf{0.45} & 0.42 & 0.44 & \textbf{0.45} & 0.41 & 0.44 & 0.44 & \textbf{0.44} & 0.41 & 0.39 & \textbf{0.44} & 0.39 & 0.41 & 0.41\\ & 30 & \textbf{0.43} & 0.33 & \textbf{0.43} & 0.43 & \textbf{0.47} & \textbf{0.47} & 0.46 & \textbf{0.5} & 0.44 & 0.41 & \textbf{0.5} & 0.44 & 0.49 & 0.49\\ & 50 & \textbf{0.55} & 0.46 & 0.44 & 0.55 & 0.58 & \textbf{0.59} & \textbf{0.59} & 0.5 & 0.37 & \textbf{0.51} & 0.5 & \textbf{0.57} & 0.55 & 0.55\\ & 70 & \textbf{0.75} & 0.54 & 0.58 & 0.75 & 0.81 & \textbf{0.85} & \textbf{0.85} & \textbf{0.64} & 0.45 & 0.55 & 0.64 & 0.69 & \textbf{0.71} & \textbf{0.71}\\ & 100 & \textbf{0.82} & 0.58 & 0.62 & 0.82 & 0.88 & \textbf{0.92} & \textbf{0.92} & \textbf{0.74} & 0.52 & 0.58 & 0.74 & 0.79 & \textbf{0.84} & \textbf{0.84}\\\hline
 \multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{depots}}}%
 & 10 & 0.58 & 0.55 & \textbf{0.59} & \textbf{0.68} & 0.52 & 0.48 & \textbf{0.69} & \textbf{0.35} & 0.33 & 0.32 & \textbf{0.52} & 0.27 & 0.37 & \textbf{0.53}\\ & 30 & \textbf{0.46} & 0.33 & 0.31 & \textbf{0.54} & 0.24 & 0.47 & 0.51 & \textbf{0.53} & 0.37 & 0.27 & \textbf{0.55} & 0.27 & 0.51 & 0.5\\ & 50 & \textbf{0.64} & 0.46 & 0.22 & \textbf{0.69} & 0.36 & 0.61 & 0.68 & \textbf{0.71} & 0.44 & 0.17 & \textbf{0.78} & 0.42 & 0.72 & \textbf{0.8}\\ & 70 & \textbf{0.93} & 0.66 & 0.16 & \textbf{0.98} & 0.52 & 0.91 & 0.95 & \textbf{0.9} & 0.71 & 0.19 & \textbf{0.96} & 0.73 & 0.89 & \textbf{0.96}\\ & 100 & \textbf{0.94} & \textbf{0.94} & 0.15 & \textbf{1.0} & \textbf{1.0} & 0.93 & \textbf{1.0} & \textbf{0.94} & \textbf{0.94} & 0.15 & \textbf{1.0} & \textbf{1.0} & 0.93 & \textbf{1.0}\\\hline
 \multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{driverlog}}}%
 & 10 & 0.53 & \textbf{0.54} & 0.49 & 0.54 & \textbf{0.57} & 0.53 & 0.54 & \textbf{0.47} & \textbf{0.47} & 0.41 & \textbf{0.49} & 0.47 & 0.47 & \textbf{0.49}\\ & 30 & \textbf{0.64} & 0.57 & 0.44 & \textbf{0.66} & 0.6 & 0.64 & \textbf{0.66} & 0.48 & \textbf{0.55} & 0.49 & \textbf{0.67} & 0.56 & 0.48 & \textbf{0.67}\\ & 50 & \textbf{0.61} & 0.53 & 0.4 & \textbf{0.69} & 0.57 & 0.61 & \textbf{0.69} & 0.61 & \textbf{0.64} & 0.54 & \textbf{0.72} & 0.64 & 0.61 & \textbf{0.72}\\ & 70 & \textbf{0.75} & 0.64 & 0.52 & \textbf{0.9} & 0.72 & 0.75 & \textbf{0.9} & 0.71 & \textbf{0.72} & 0.59 & \textbf{0.85} & 0.74 & 0.71 & \textbf{0.85}\\ & 100 & \textbf{0.81} & 0.71 & 0.55 & \textbf{0.96} & 0.76 & 0.81 & \textbf{0.96} & \textbf{0.79} & 0.69 & 0.58 & \textbf{0.93} & 0.75 & 0.79 & \textbf{0.93}\\\hline
 \multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{dwr}}}%
 & 10 & \textbf{0.72} & 0.55 & 0.45 & \textbf{0.79} & 0.55 & 0.72 & \textbf{0.79} & \textbf{0.76} & 0.5 & 0.44 & 0.75 & 0.5 & \textbf{0.76} & 0.75\\ & 30 & \textbf{0.72} & 0.42 & 0.32 & \textbf{0.8} & 0.42 & 0.72 & \textbf{0.8} & \textbf{0.69} & 0.43 & 0.39 & \textbf{0.71} & 0.44 & 0.69 & \textbf{0.71}\\ & 50 & \textbf{0.83} & 0.54 & 0.28 & \textbf{0.91} & 0.56 & 0.83 & \textbf{0.91} & \textbf{0.82} & 0.51 & 0.4 & \textbf{0.84} & 0.51 & 0.82 & \textbf{0.84}\\ & 70 & \textbf{0.9} & 0.68 & 0.27 & \textbf{0.9} & 0.7 & \textbf{0.9} & \textbf{0.9} & \textbf{0.89} & 0.66 & 0.36 & 0.88 & 0.67 & \textbf{0.89} & 0.88\\ & 100 & \textbf{0.92} & 0.81 & 0.38 & \textbf{0.92} & 0.81 & \textbf{0.92} & \textbf{0.92} & \textbf{0.92} & 0.81 & 0.38 & \textbf{0.92} & 0.81 & \textbf{0.92} & \textbf{0.92}\\\hline
 \textsc{f}%
 & AVG & \textbf{0.95} & \textbf{0.95} & 0.48 & \textbf{0.95} & \textbf{0.95} & \textbf{0.95} & \textbf{0.95} & \textbf{0.88} & \textbf{0.88} & 0.47 & \textbf{0.88} & \textbf{0.88} & \textbf{0.88} & \textbf{0.88}\\\hline
 \textsc{l}%
 & AVG & 0.92 & \textbf{0.96} & 0.7 & \textbf{0.96} & 0.92 & 0.88 & 0.95 & 0.9 & \textbf{0.93} & 0.72 & \textbf{0.93} & 0.92 & 0.9 & \textbf{0.93}
 \\\hline
\end{tabular}

==> tables/constraints-2.tex <==
\begin{tabular}{cc|ccc|ccc|c||ccc|ccc|c}
\toprule
\multicolumn{2}{c}{} & \multicolumn{7}{c}{Optimal} & \multicolumn{7}{c}{Sub-Optimal}\\
\cmidrule(lr){3-9}\cmidrule(lr){10-16}
\# & \% & S & L & P & S, L & L, P & L, P & S, L, P%
& S & L & P & S, L & L, P & S, P & S, L, P\\
\midrule
 \multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{ferry}}}%
 & 10 & \textbf{0.88} & \textbf{0.88} & 0.66 & \textbf{0.88} & \textbf{0.88} & \textbf{0.88} & \textbf{0.88} & 0.71 & \textbf{0.72} & 0.5 & 0.71 & \textbf{0.72} & 0.71 & 0.71\\ & 30 & \textbf{0.9} & \textbf{0.9} & 0.39 & \textbf{0.9} & \textbf{0.9} & \textbf{0.9} & \textbf{0.9} & 0.88 & \textbf{0.89} & 0.39 & 0.88 & \textbf{0.89} & 0.88 & 0.88\\ & 50 & \textbf{0.98} & \textbf{0.98} & 0.41 & \textbf{0.98} & \textbf{0.98} & \textbf{0.98} & \textbf{0.98} & \textbf{0.88} & \textbf{0.88} & 0.44 & \textbf{0.88} & \textbf{0.88} & \textbf{0.88} & \textbf{0.88}\\ & 70 & \textbf{0.99} & \textbf{0.99} & 0.46 & \textbf{0.99} & \textbf{0.99} & \textbf{0.99} & \textbf{0.99} & \textbf{0.96} & \textbf{0.96} & 0.5 & \textbf{0.96} & \textbf{0.96} & \textbf{0.96} & \textbf{0.96}\\ & 100 & \textbf{1.0} & \textbf{1.0} & 0.47 & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{0.96} & \textbf{0.96} & 0.51 & \textbf{0.96} & \textbf{0.96} & \textbf{0.96} & \textbf{0.96}\\\hline
\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{logistics}}}%
 & 10 & 0.85 & \textbf{0.89} & 0.71 & \textbf{0.9} & 0.86 & 0.73 & \textbf{0.9} & 0.8 & \textbf{0.81} & 0.78 & 0.83 & \textbf{0.84} & 0.82 & \textbf{0.88}\\ & 30 & 0.86 & \textbf{0.92} & 0.67 & \textbf{0.92} & 0.88 & 0.79 & \textbf{0.92} & 0.85 & \textbf{0.93} & 0.7 & \textbf{0.9} & 0.88 & 0.83 & 0.91\\ & 50 & 0.93 & \textbf{0.96} & 0.72 & \textbf{0.96} & 0.91 & 0.92 & \textbf{0.96} & 0.87 & \textbf{0.94} & 0.7 & \textbf{0.93} & 0.91 & 0.87 & 0.88\\ & 70 & 0.99 & \textbf{1.0} & 0.71 & \textbf{1.0} & 0.96 & 0.99 & 0.99 & 0.96 & \textbf{0.99} & 0.71 & \textbf{0.99} & \textbf{0.99} & 0.96 & 0.97\\ & 100 & \textbf{1.0} & \textbf{1.0} & 0.69 & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & 0.69 & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0}\\\hline\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{miconic}}}%
 & 10 & 0.73 & \textbf{0.8} & 0.62 & \textbf{0.89} & 0.8 & 0.73 & \textbf{0.89} & 0.54 & \textbf{0.68} & 0.51 & \textbf{0.76} & 0.68 & 0.54 & \textbf{0.76}\\ & 30 & 0.63 & \textbf{0.77} & 0.63 & \textbf{0.95} & 0.77 & 0.63 & \textbf{0.95} & 0.6 & \textbf{0.77} & 0.6 & \textbf{0.89} & 0.77 & 0.6 & \textbf{0.89}\\ & 50 & 0.81 & \textbf{0.9} & 0.81 & \textbf{0.97} & 0.9 & 0.81 & \textbf{0.97} & 0.88 & \textbf{0.97} & 0.88 & \textbf{0.98} & 0.97 & 0.88 & \textbf{0.98}\\ & 70 & 0.91 & \textbf{0.97} & 0.91 & \textbf{0.98} & 0.97 & 0.91 & \textbf{0.98} & 0.94 & \textbf{0.99} & 0.94 & \textbf{0.99} & \textbf{0.99} & 0.94 & \textbf{0.99}\\ & 100 & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0}\\\hline
\\
\bottomrule
\end{tabular}

==> tables/constraints-3.tex <==
\begin{tabular}[t]{cc|ccc|ccc|c||ccc|ccc|c}
\toprule
\multicolumn{2}{c}{} & \multicolumn{7}{c}{Optimal} & \multicolumn{7}{c}{Sub-Optimal}\\
\cmidrule(lr){3-9}\cmidrule(lr){10-16}
\# & \% & S & L & P & S, L & L, P & L, P & S, L, P%
& S & L & P & S, L & L, P & S, P & S, L, P\\
\midrule
 \multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{ipc-grid}}}%
 & 10 & 0.65 & \textbf{0.92} & 0.4 & 0.87 & \textbf{0.92} & 0.68 & 0.87 & 0.6 & \textbf{0.86} & 0.25 & 0.76 & \textbf{0.86} & 0.63 & 0.77\\ & 30 & 0.73 & \textbf{0.97} & 0.25 & 0.93 & \textbf{0.97} & 0.78 & 0.93 & 0.69 & \textbf{0.88} & 0.23 & 0.82 & \textbf{0.88} & 0.71 & 0.82\\ & 50 & 0.83 & \textbf{0.97} & 0.27 & 0.96 & \textbf{0.97} & 0.9 & 0.96 & 0.81 & \textbf{0.89} & 0.29 & 0.84 & \textbf{0.89} & 0.87 & 0.84\\ & 70 & 0.9 & \textbf{0.97} & 0.3 & \textbf{0.97} & \textbf{0.97} & 0.95 & \textbf{0.97} & 0.87 & \textbf{0.91} & 0.08 & 0.89 & \textbf{0.91} & 0.89 & 0.89\\ & 100 & \textbf{1.0} & \textbf{1.0} & 0.23 & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{0.94} & \textbf{0.94} & 0.05 & \textbf{0.94} & \textbf{0.94} & \textbf{0.94} & \textbf{0.94}\\\hline
 \multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{satellite}}}%
 & 10 & 0.81 & \textbf{0.88} & 0.84 & 0.85 & \textbf{0.88} & 0.83 & 0.85 & 0.79 & \textbf{0.8} & 0.78 & \textbf{0.9} & 0.8 & 0.77 & \textbf{0.9}\\ & 30 & 0.8 & \textbf{0.81} & 0.78 & \textbf{0.86} & 0.81 & 0.82 & \textbf{0.86} & 0.67 & \textbf{0.74} & 0.7 & \textbf{0.8} & 0.74 & 0.68 & \textbf{0.8}\\ & 50 & 0.86 & \textbf{0.92} & 0.91 & \textbf{0.93} & 0.92 & 0.83 & \textbf{0.93} & \textbf{0.84} & 0.83 & 0.78 & \textbf{0.92} & 0.83 & 0.86 & \textbf{0.92}\\ & 70 & 0.89 & \textbf{0.97} & \textbf{0.97} & 0.94 & \textbf{0.97} & 0.86 & 0.94 & 0.87 & \textbf{0.92} & 0.9 & \textbf{0.94} & 0.92 & 0.85 & \textbf{0.94}\\ & 100 & 0.96 & \textbf{1.0} & \textbf{1.0} & 0.96 & \textbf{1.0} & 0.92 & 0.96 & 0.96 & \textbf{1.0} & \textbf{1.0} & 0.96 & \textbf{1.0} & 0.92 & 0.96\\\hline
 \multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{sokoban}}}%
 & 10 & \textbf{0.38} & \textbf{0.38} & 0.24 & \textbf{0.39} & 0.34 & 0.31 & \textbf{0.39} & \textbf{0.38} & 0.3 & 0.24 & \textbf{0.52} & 0.25 & 0.36 & \textbf{0.52}\\ & 30 & \textbf{0.59} & 0.41 & 0.14 & \textbf{0.75} & 0.38 & 0.59 & \textbf{0.75} & \textbf{0.72} & 0.43 & 0.14 & \textbf{0.77} & 0.37 & 0.68 & \textbf{0.77}\\ & 50 & \textbf{0.82} & 0.53 & 0.21 & \textbf{0.92} & 0.49 & 0.82 & \textbf{0.92} & \textbf{0.77} & 0.51 & 0.17 & \textbf{0.79} & 0.41 & \textbf{0.79} & \textbf{0.79}\\ & 70 & \textbf{0.93} & 0.73 & 0.21 & \textbf{0.99} & 0.62 & 0.93 & \textbf{0.99} & \textbf{0.85} & 0.58 & 0.17 & 0.8 & 0.51 & \textbf{0.85} & 0.8\\ & 100 & \textbf{0.96} & 0.85 & 0.23 & \textbf{1.0} & 0.81 & 0.96 & \textbf{1.0} & \textbf{0.88} & 0.73 & 0.22 & 0.83 & 0.72 & \textbf{0.88} & 0.83\\\hline
 \multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{zeno}}}%
 & 10 & 0.65 & \textbf{0.72} & 0.6 & 0.67 & 0.68 & \textbf{0.71} & 0.67 & \textbf{0.68} & 0.59 & 0.55 & 0.65 & 0.58 & \textbf{0.7} & 0.64\\ & 30 & \textbf{0.84} & 0.72 & 0.55 & 0.78 & 0.77 & \textbf{0.83} & 0.76 & \textbf{0.76} & \textbf{0.76} & 0.55 & 0.72 & 0.77 & \textbf{0.78} & 0.73\\ & 50 & \textbf{0.88} & 0.83 & 0.57 & \textbf{0.9} & 0.83 & 0.89 & \textbf{0.9} & 0.85 & \textbf{0.86} & 0.67 & 0.87 & 0.87 & \textbf{0.88} & 0.87\\ & 70 & \textbf{0.94} & \textbf{0.94} & 0.65 & 0.94 & \textbf{0.98} & 0.97 & 0.94 & \textbf{0.94} & \textbf{0.94} & 0.64 & 0.94 & \textbf{0.99} & 0.96 & 0.94\\ & 100 & \textbf{1.0} & 0.96 & 0.66 & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & 0.96 & 0.66 & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0}\\\hline
 \textsc{m}%
 & AVG & 0.82 & \textbf{0.89} & 0.79 & \textbf{0.96} & 0.89 & 0.82 & \textbf{0.96} & 0.79 & \textbf{0.88} & 0.79 & \textbf{0.93} & 0.88 & 0.79 & \textbf{0.93}\\\hline
 \textsc{r}%
 & AVG & 0.77 & \textbf{0.92} & 0.88 & \textbf{0.93} & 0.92 & 0.87 & \textbf{0.93} & 0.76 & \textbf{0.92} & 0.85 & \textbf{0.92} & \textbf{0.92} & 0.85 & \textbf{0.92}\\\hline
\multicolumn{2}{c}{AVG} & \textbf{0.79} & 0.77 & 0.54 & \textbf{0.86} & 0.78 & 0.8 & \textbf{0.86} & \textbf{0.76} & 0.74 & 0.52 & \textbf{0.82} & 0.75 & 0.78 & \textbf{0.82}\\
\bottomrule
\end{tabular}\\

==> tables/constraints-full.tex <==
\begin{tabular}{c|c|ccc|ccc|c||ccc|ccc|c}
\toprule
\multicolumn{2}{c}{} & \multicolumn{7}{c}{Optimal} & \multicolumn{7}{c}{Sub-Optimal}\\
\cmidrule(lr){3-9}\cmidrule(lr){10-16}
\% & \# & S & L & P & S, L & L, P & S, P & S, L, P%
& S & L & P & S, L & L, P & S, P & S, L, P\\
\midrule%
10 & \multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{blocks}}} & \textbf{0.45} & 0.42 & 0.44 & \textbf{0.45} & 0.41 & 0.44 & 0.44 & \textbf{0.44} & 0.41 & 0.39 & \textbf{0.44} & 0.39 & 0.41 & 0.41\\
30 & & \textbf{0.43} & 0.33 & \textbf{0.43} & 0.43 & \textbf{0.47} & \textbf{0.47} & 0.46 & \textbf{0.5} & 0.44 & 0.41 & \textbf{0.5} & 0.44 & 0.49 & 0.49\\
50 & & \textbf{0.55} & 0.46 & 0.44 & 0.55 & 0.58 & \textbf{0.59} & \textbf{0.59} & 0.5 & 0.37 & \textbf{0.51} & 0.5 & \textbf{0.57} & 0.55 & 0.55\\
70 & & \textbf{0.75} & 0.54 & 0.58 & 0.75 & 0.81 & \textbf{0.85} & \textbf{0.85} & \textbf{0.64} & 0.45 & 0.55 & 0.64 & 0.69 & \textbf{0.71} & \textbf{0.71}\\
100 & & \textbf{0.82} & 0.58 & 0.62 & 0.82 & 0.88 & \textbf{0.92} & \textbf{0.92} & \textbf{0.74} & 0.52 & 0.58 & 0.74 & 0.79 & \textbf{0.84} & \textbf{0.84}\\\hline
10 & \multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{depots}}} & 0.58 & 0.55 & \textbf{0.59} & \textbf{0.68} & 0.52 & 0.48 & \textbf{0.69} & \textbf{0.35} & 0.33 & 0.32 & \textbf{0.52} & 0.27 & 0.37 & \textbf{0.53}\\
30 & & \textbf{0.46} & 0.33 & 0.31 & \textbf{0.54} & 0.24 & 0.47 & 0.51 & \textbf{0.53} & 0.37 & 0.27 & \textbf{0.55} & 0.27 & 0.51 & 0.5\\
50 & & \textbf{0.64} & 0.46 & 0.22 & \textbf{0.69} & 0.36 & 0.61 & 0.68 & \textbf{0.71} & 0.44 & 0.17 & \textbf{0.78} & 0.42 & 0.72 & \textbf{0.8}\\
70 & & \textbf{0.93} & 0.66 & 0.16 & \textbf{0.98} & 0.52 & 0.91 & 0.95 & \textbf{0.9} & 0.71 & 0.19 & \textbf{0.96} & 0.73 & 0.89 & \textbf{0.96}\\
100 & & \textbf{0.94} & \textbf{0.94} & 0.15 & \textbf{1.0} & \textbf{1.0} & 0.93 & \textbf{1.0} & \textbf{0.94} & \textbf{0.94} & 0.15 & \textbf{1.0} & \textbf{1.0} & 0.93 & \textbf{1.0}\\\hline
10 & \multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{driverlog}}} & 0.53 & \textbf{0.54} & 0.49 & 0.54 & \textbf{0.57} & 0.53 & 0.54 & \textbf{0.47} & \textbf{0.47} & 0.41 & \textbf{0.49} & 0.47 & 0.47 & \textbf{0.49}\\
30 & & \textbf{0.64} & 0.57 & 0.44 & \textbf{0.66} & 0.6 & 0.64 & \textbf{0.66} & 0.48 & \textbf{0.55} & 0.49 & \textbf{0.67} & 0.56 & 0.48 & \textbf{0.67}\\
50 & & \textbf{0.61} & 0.53 & 0.4 & \textbf{0.69} & 0.57 & 0.61 & \textbf{0.69} & 0.61 & \textbf{0.64} & 0.54 & \textbf{0.72} & 0.64 & 0.61 & \textbf{0.72}\\
70 & & \textbf{0.75} & 0.64 & 0.52 & \textbf{0.9} & 0.72 & 0.75 & \textbf{0.9} & 0.71 & \textbf{0.72} & 0.59 & \textbf{0.85} & 0.74 & 0.71 & \textbf{0.85}\\
100 & & \textbf{0.81} & 0.71 & 0.55 & \textbf{0.96} & 0.76 & 0.81 & \textbf{0.96} & \textbf{0.79} & 0.69 & 0.58 & \textbf{0.93} & 0.75 & 0.79 & \textbf{0.93}\\\hline
10 & \multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{dwr}}} & \textbf{0.72} & 0.55 & 0.45 & \textbf{0.79} & 0.55 & 0.72 & \textbf{0.79} & \textbf{0.76} & 0.5 & 0.44 & 0.75 & 0.5 & \textbf{0.76} & 0.75\\
30 & & \textbf{0.72} & 0.42 & 0.32 & \textbf{0.8} & 0.42 & 0.72 & \textbf{0.8} & \textbf{0.69} & 0.43 & 0.39 & \textbf{0.71} & 0.44 & 0.69 & \textbf{0.71}\\
50 & & \textbf{0.83} & 0.54 & 0.28 & \textbf{0.91} & 0.56 & 0.83 & \textbf{0.91} & \textbf{0.82} & 0.51 & 0.4 & \textbf{0.84} & 0.51 & 0.82 & \textbf{0.84}\\
70 & & \textbf{0.9} & 0.68 & 0.27 & \textbf{0.9} & 0.7 & \textbf{0.9} & \textbf{0.9} & \textbf{0.89} & 0.66 & 0.36 & 0.88 & 0.67 & \textbf{0.89} & 0.88\\
100 & & \textbf{0.92} & 0.81 & 0.38 & \textbf{0.92} & 0.81 & \textbf{0.92} & \textbf{0.92} & \textbf{0.92} & 0.81 & 0.38 & \textbf{0.92} & 0.81 & \textbf{0.92} & \textbf{0.92}\\\hline
10 & \multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{ferry}}} & \textbf{0.88} & \textbf{0.88} & 0.66 & \textbf{0.88} & \textbf{0.88} & \textbf{0.88} & \textbf{0.88} & 0.71 & \textbf{0.72} & 0.5 & 0.71 & \textbf{0.72} & 0.71 & 0.71\\
30 & & \textbf{0.9} & \textbf{0.9} & 0.39 & \textbf{0.9} & \textbf{0.9} & \textbf{0.9} & \textbf{0.9} & 0.88 & \textbf{0.89} & 0.39 & 0.88 & \textbf{0.89} & 0.88 & 0.88\\
50 & & \textbf{0.98} & \textbf{0.98} & 0.41 & \textbf{0.98} & \textbf{0.98} & \textbf{0.98} & \textbf{0.98} & \textbf{0.88} & \textbf{0.88} & 0.44 & \textbf{0.88} & \textbf{0.88} & \textbf{0.88} & \textbf{0.88}\\
70 & & \textbf{0.99} & \textbf{0.99} & 0.46 & \textbf{0.99} & \textbf{0.99} & \textbf{0.99} & \textbf{0.99} & \textbf{0.96} & \textbf{0.96} & 0.5 & \textbf{0.96} & \textbf{0.96} & \textbf{0.96} & \textbf{0.96}\\
100 & & \textbf{1.0} & \textbf{1.0} & 0.47 & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{0.96} & \textbf{0.96} & 0.51 & \textbf{0.96} & \textbf{0.96} & \textbf{0.96} & \textbf{0.96}\\\hline
10 & \multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{ipc-grid}}} & 0.65 & \textbf{0.92} & 0.4 & 0.87 & \textbf{0.92} & 0.68 & 0.87 & 0.6 & \textbf{0.86} & 0.25 & 0.76 & \textbf{0.86} & 0.63 & 0.77\\
30 & & 0.73 & \textbf{0.97} & 0.25 & 0.93 & \textbf{0.97} & 0.78 & 0.93 & 0.69 & \textbf{0.88} & 0.23 & 0.82 & \textbf{0.88} & 0.71 & 0.82\\
50 & & 0.83 & \textbf{0.97} & 0.27 & 0.96 & \textbf{0.97} & 0.9 & 0.96 & 0.81 & \textbf{0.89} & 0.29 & 0.84 & \textbf{0.89} & 0.87 & 0.84\\
70 & & 0.9 & \textbf{0.97} & 0.3 & \textbf{0.97} & \textbf{0.97} & 0.95 & \textbf{0.97} & 0.87 & \textbf{0.91} & 0.08 & 0.89 & \textbf{0.91} & 0.89 & 0.89\\
100 & & \textbf{1.0} & \textbf{1.0} & 0.23 & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{0.94} & \textbf{0.94} & 0.05 & \textbf{0.94} & \textbf{0.94} & \textbf{0.94} & \textbf{0.94}\\\hline
10 & \multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{logistics}}} & 0.85 & \textbf{0.89} & 0.71 & \textbf{0.9} & 0.86 & 0.73 & \textbf{0.9} & 0.8 & \textbf{0.81} & 0.78 & 0.83 & \textbf{0.84} & 0.82 & \textbf{0.88}\\
30 & & 0.86 & \textbf{0.92} & 0.67 & \textbf{0.92} & 0.88 & 0.79 & \textbf{0.92} & 0.85 & \textbf{0.93} & 0.7 & \textbf{0.9} & 0.88 & 0.83 & 0.91\\
50 & & 0.93 & \textbf{0.96} & 0.72 & \textbf{0.96} & 0.91 & 0.92 & \textbf{0.96} & 0.87 & \textbf{0.94} & 0.7 & \textbf{0.93} & 0.91 & 0.87 & 0.88\\
70 & & 0.99 & \textbf{1.0} & 0.71 & \textbf{1.0} & 0.96 & 0.99 & 0.99 & 0.96 & \textbf{0.99} & 0.71 & \textbf{0.99} & \textbf{0.99} & 0.96 & 0.97\\
100 & & \textbf{1.0} & \textbf{1.0} & 0.69 & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & 0.69 & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0}\\\hline
10 & \multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{miconic}}} & 0.73 & \textbf{0.8} & 0.62 & \textbf{0.89} & 0.8 & 0.73 & \textbf{0.89} & 0.54 & \textbf{0.68} & 0.51 & \textbf{0.76} & 0.68 & 0.54 & \textbf{0.76}\\
30 & & 0.63 & \textbf{0.77} & 0.63 & \textbf{0.95} & 0.77 & 0.63 & \textbf{0.95} & 0.6 & \textbf{0.77} & 0.6 & \textbf{0.89} & 0.77 & 0.6 & \textbf{0.89}\\
50 & & 0.81 & \textbf{0.9} & 0.81 & \textbf{0.97} & 0.9 & 0.81 & \textbf{0.97} & 0.88 & \textbf{0.97} & 0.88 & \textbf{0.98} & 0.97 & 0.88 & \textbf{0.98}\\
70 & & 0.91 & \textbf{0.97} & 0.91 & \textbf{0.98} & 0.97 & 0.91 & \textbf{0.98} & 0.94 & \textbf{0.99} & 0.94 & \textbf{0.99} & \textbf{0.99} & 0.94 & \textbf{0.99}\\
100 & & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0}\\\hline
10 & \multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{rovers}}} & 0.61 & \textbf{0.78} & 0.67 & \textbf{0.83} & 0.78 & 0.63 & \textbf{0.83} & 0.59 & \textbf{0.79} & 0.66 & \textbf{0.83} & 0.79 & 0.65 & \textbf{0.83}\\
30 & & 0.57 & \textbf{0.91} & 0.8 & \textbf{0.94} & 0.91 & 0.8 & \textbf{0.94} & 0.62 & \textbf{0.86} & 0.74 & \textbf{0.88} & 0.86 & 0.76 & \textbf{0.88}\\
50 & & 0.78 & \textbf{0.94} & 0.91 & 0.92 & \textbf{0.94} & 0.93 & 0.92 & 0.72 & \textbf{0.99} & 0.94 & 0.93 & \textbf{0.99} & 0.94 & 0.93\\
70 & & 0.89 & 0.99 & \textbf{1.0} & 0.99 & 0.99 & \textbf{1.0} & 0.99 & 0.88 & \textbf{0.98} & 0.93 & 0.94 & \textbf{0.98} & 0.93 & 0.94\\
100 & & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0}\\\hline
10 & \multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{satellite}}} & 0.81 & \textbf{0.88} & 0.84 & 0.85 & \textbf{0.88} & 0.83 & 0.85 & 0.79 & \textbf{0.8} & 0.78 & \textbf{0.9} & 0.8 & 0.77 & \textbf{0.9}\\
30 & & 0.8 & \textbf{0.81} & 0.78 & \textbf{0.86} & 0.81 & 0.82 & \textbf{0.86} & 0.67 & \textbf{0.74} & 0.7 & \textbf{0.8} & 0.74 & 0.68 & \textbf{0.8}\\
50 & & 0.86 & \textbf{0.92} & 0.91 & \textbf{0.93} & 0.92 & 0.83 & \textbf{0.93} & \textbf{0.84} & 0.83 & 0.78 & \textbf{0.92} & 0.83 & 0.86 & \textbf{0.92}\\
70 & & 0.89 & \textbf{0.97} & \textbf{0.97} & 0.94 & \textbf{0.97} & 0.86 & 0.94 & 0.87 & \textbf{0.92} & 0.9 & \textbf{0.94} & 0.92 & 0.85 & \textbf{0.94}\\
100 & & 0.96 & \textbf{1.0} & \textbf{1.0} & 0.96 & \textbf{1.0} & 0.92 & 0.96 & 0.96 & \textbf{1.0} & \textbf{1.0} & 0.96 & \textbf{1.0} & 0.92 & 0.96\\\hline
10 & \multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{sokoban}}} & \textbf{0.38} & \textbf{0.38} & 0.24 & \textbf{0.39} & 0.34 & 0.31 & \textbf{0.39} & \textbf{0.38} & 0.3 & 0.24 & \textbf{0.52} & 0.25 & 0.36 & \textbf{0.52}\\
30 & & \textbf{0.59} & 0.41 & 0.14 & \textbf{0.75} & 0.38 & 0.59 & \textbf{0.75} & \textbf{0.72} & 0.43 & 0.14 & \textbf{0.77} & 0.37 & 0.68 & \textbf{0.77}\\
50 & & \textbf{0.82} & 0.53 & 0.21 & \textbf{0.92} & 0.49 & 0.82 & \textbf{0.92} & \textbf{0.77} & 0.51 & 0.17 & \textbf{0.79} & 0.41 & \textbf{0.79} & \textbf{0.79}\\
70 & & \textbf{0.93} & 0.73 & 0.21 & \textbf{0.99} & 0.62 & 0.93 & \textbf{0.99} & \textbf{0.85} & 0.58 & 0.17 & 0.8 & 0.51 & \textbf{0.85} & 0.8\\
100 & & \textbf{0.96} & 0.85 & 0.23 & \textbf{1.0} & 0.81 & 0.96 & \textbf{1.0} & \textbf{0.88} & 0.73 & 0.22 & 0.83 & 0.72 & \textbf{0.88} & 0.83\\\hline
10 & \multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{zeno}}} & 0.65 & \textbf{0.72} & 0.6 & 0.67 & 0.68 & \textbf{0.71} & 0.67 & \textbf{0.68} & 0.59 & 0.55 & 0.65 & 0.58 & \textbf{0.7} & 0.64\\
30 & & \textbf{0.84} & 0.72 & 0.55 & 0.78 & 0.77 & \textbf{0.83} & 0.76 & \textbf{0.76} & \textbf{0.76} & 0.55 & 0.72 & 0.77 & \textbf{0.78} & 0.73\\
50 & & \textbf{0.88} & 0.83 & 0.57 & \textbf{0.9} & 0.83 & 0.89 & \textbf{0.9} & 0.85 & \textbf{0.86} & 0.67 & 0.87 & 0.87 & \textbf{0.88} & 0.87\\
70 & & \textbf{0.94} & \textbf{0.94} & 0.65 & 0.94 & \textbf{0.98} & 0.97 & 0.94 & \textbf{0.94} & \textbf{0.94} & 0.64 & 0.94 & \textbf{0.99} & 0.96 & 0.94\\
100 & & \textbf{1.0} & 0.96 & 0.66 & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & 0.96 & 0.66 & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0}\\\midrule
%
\multicolumn{2}{c|}{AVG}  & \textbf{0.79} & 0.77 & 0.54 & \textbf{0.86} & 0.78 & 0.8 & \textbf{0.86} & \textbf{0.76} & 0.74 & 0.52 & \textbf{0.82} & 0.75 & 0.78 & \textbf{0.82}\\
\bottomrule
\end{tabular}\\

==> tables/constraints.tex <==
\begin{tabular}{c|c|ccc|ccc|c||ccc|ccc|c}
\toprule
\multicolumn{2}{c}{} & \multicolumn{7}{c}{Optimal} & \multicolumn{7}{c}{Sub-Optimal}\\
\cmidrule(lr){3-9}\cmidrule(lr){10-16}
\% & \# & S & L & P & S, L & L, P & L, P & S, L, P%
& S & L & P & S, L & L, P & S, P & S, L, P\\
\midrule%
10 & \multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{blocks}}} & \textbf{0.45} & 0.42 & 0.44 & \textbf{0.45} & 0.41 & 0.44 & 0.44 & \textbf{0.44} & 0.41 & 0.39 & \textbf{0.44} & 0.39 & 0.41 & 0.41\\
 30 & & \textbf{0.43} & 0.33 & \textbf{0.43} & 0.43 & \textbf{0.47} & \textbf{0.47} & 0.46 & \textbf{0.5} & 0.44 & 0.41 & \textbf{0.5} & 0.44 & 0.49 & 0.49\\
 50 & & \textbf{0.55} & 0.46 & 0.44 & 0.55 & 0.58 & \textbf{0.59} & \textbf{0.59} & 0.5 & 0.37 & \textbf{0.51} & 0.5 & \textbf{0.57} & 0.55 & 0.55\\
 70 & & \textbf{0.75} & 0.54 & 0.58 & 0.75 & 0.81 & \textbf{0.85} & \textbf{0.85} & \textbf{0.64} & 0.45 & 0.55 & 0.64 & 0.69 & \textbf{0.71} & \textbf{0.71}\\
 100 & & \textbf{0.82} & 0.58 & 0.62 & 0.82 & 0.88 & \textbf{0.92} & \textbf{0.92} & \textbf{0.74} & 0.52 & 0.58 & 0.74 & 0.79 & \textbf{0.84} & \textbf{0.84}\\\hline
 10 & \multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{depots}}} & 0.58 & 0.55 & \textbf{0.59} & \textbf{0.68} & 0.52 & 0.48 & \textbf{0.69} & \textbf{0.35} & 0.33 & 0.32 & \textbf{0.52} & 0.27 & 0.37 & \textbf{0.53}\\
 30 & & \textbf{0.46} & 0.33 & 0.31 & \textbf{0.54} & 0.24 & 0.47 & 0.51 & \textbf{0.53} & 0.37 & 0.27 & \textbf{0.55} & 0.27 & 0.51 & 0.5\\
 50 & & \textbf{0.64} & 0.46 & 0.22 & \textbf{0.69} & 0.36 & 0.61 & 0.68 & \textbf{0.71} & 0.44 & 0.17 & \textbf{0.78} & 0.42 & 0.72 & \textbf{0.8}\\
 70 & & \textbf{0.93} & 0.66 & 0.16 & \textbf{0.98} & 0.52 & 0.91 & 0.95 & \textbf{0.9} & 0.71 & 0.19 & \textbf{0.96} & 0.73 & 0.89 & \textbf{0.96}\\
 100 & & \textbf{0.94} & \textbf{0.94} & 0.15 & \textbf{1.0} & \textbf{1.0} & 0.93 & \textbf{1.0} & \textbf{0.94} & \textbf{0.94} & 0.15 & \textbf{1.0} & \textbf{1.0} & 0.93 & \textbf{1.0}\\\hline
 10 & \multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{driverlog}}} & 0.53 & \textbf{0.54} & 0.49 & 0.54 & \textbf{0.57} & 0.53 & 0.54 & \textbf{0.47} & \textbf{0.47} & 0.41 & \textbf{0.49} & 0.47 & 0.47 & \textbf{0.49}\\
 30 & & \textbf{0.64} & 0.57 & 0.44 & \textbf{0.66} & 0.6 & 0.64 & \textbf{0.66} & 0.48 & \textbf{0.55} & 0.49 & \textbf{0.67} & 0.56 & 0.48 & \textbf{0.67}\\
 50 & & \textbf{0.61} & 0.53 & 0.4 & \textbf{0.69} & 0.57 & 0.61 & \textbf{0.69} & 0.61 & \textbf{0.64} & 0.54 & \textbf{0.72} & 0.64 & 0.61 & \textbf{0.72}\\
 70 & & \textbf{0.75} & 0.64 & 0.52 & \textbf{0.9} & 0.72 & 0.75 & \textbf{0.9} & 0.71 & \textbf{0.72} & 0.59 & \textbf{0.85} & 0.74 & 0.71 & \textbf{0.85}\\
 100 & & \textbf{0.81} & 0.71 & 0.55 & \textbf{0.96} & 0.76 & 0.81 & \textbf{0.96} & \textbf{0.79} & 0.69 & 0.58 & \textbf{0.93} & 0.75 & 0.79 & \textbf{0.93}\\\hline
 10 & \multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{dwr}}} & \textbf{0.72} & 0.55 & 0.45 & \textbf{0.79} & 0.55 & 0.72 & \textbf{0.79} & \textbf{0.76} & 0.5 & 0.44 & 0.75 & 0.5 & \textbf{0.76} & 0.75\\
 30 & & \textbf{0.72} & 0.42 & 0.32 & \textbf{0.8} & 0.42 & 0.72 & \textbf{0.8} & \textbf{0.69} & 0.43 & 0.39 & \textbf{0.71} & 0.44 & 0.69 & \textbf{0.71}\\
 50 & & \textbf{0.83} & 0.54 & 0.28 & \textbf{0.91} & 0.56 & 0.83 & \textbf{0.91} & \textbf{0.82} & 0.51 & 0.4 & \textbf{0.84} & 0.51 & 0.82 & \textbf{0.84}\\
 70 & & \textbf{0.9} & 0.68 & 0.27 & \textbf{0.9} & 0.7 & \textbf{0.9} & \textbf{0.9} & \textbf{0.89} & 0.66 & 0.36 & 0.88 & 0.67 & \textbf{0.89} & 0.88\\
 100 & & \textbf{0.92} & 0.81 & 0.38 & \textbf{0.92} & 0.81 & \textbf{0.92} & \textbf{0.92} & \textbf{0.92} & 0.81 & 0.38 & \textbf{0.92} & 0.81 & \textbf{0.92} & \textbf{0.92}\\\hline
 10 & \multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{ipc-grid}}} & 0.65 & \textbf{0.92} & 0.4 & 0.87 & \textbf{0.92} & 0.68 & 0.87 & 0.6 & \textbf{0.86} & 0.25 & 0.76 & \textbf{0.86} & 0.63 & 0.77\\
 30 & & 0.73 & \textbf{0.97} & 0.25 & 0.93 & \textbf{0.97} & 0.78 & 0.93 & 0.69 & \textbf{0.88} & 0.23 & 0.82 & \textbf{0.88} & 0.71 & 0.82\\
 50 & & 0.83 & \textbf{0.97} & 0.27 & 0.96 & \textbf{0.97} & 0.9 & 0.96 & 0.81 & \textbf{0.89} & 0.29 & 0.84 & \textbf{0.89} & 0.87 & 0.84\\
 70 & & 0.9 & \textbf{0.97} & 0.3 & \textbf{0.97} & \textbf{0.97} & 0.95 & \textbf{0.97} & 0.87 & \textbf{0.91} & 0.08 & 0.89 & \textbf{0.91} & 0.89 & 0.89\\
 100 & & \textbf{1.0} & \textbf{1.0} & 0.23 & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{0.94} & \textbf{0.94} & 0.05 & \textbf{0.94} & \textbf{0.94} & \textbf{0.94} & \textbf{0.94}\\\hline
 10 & \multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{satellite}}} & 0.81 & \textbf{0.88} & 0.84 & 0.85 & \textbf{0.88} & 0.83 & 0.85 & 0.79 & \textbf{0.8} & 0.78 & \textbf{0.9} & 0.8 & 0.77 & \textbf{0.9}\\
 30 & & 0.8 & \textbf{0.81} & 0.78 & \textbf{0.86} & 0.81 & 0.82 & \textbf{0.86} & 0.67 & \textbf{0.74} & 0.7 & \textbf{0.8} & 0.74 & 0.68 & \textbf{0.8}\\
 50 & & 0.86 & \textbf{0.92} & 0.91 & \textbf{0.93} & 0.92 & 0.83 & \textbf{0.93} & \textbf{0.84} & 0.83 & 0.78 & \textbf{0.92} & 0.83 & 0.86 & \textbf{0.92}\\
 70 & & 0.89 & \textbf{0.97} & \textbf{0.97} & 0.94 & \textbf{0.97} & 0.86 & 0.94 & 0.87 & \textbf{0.92} & 0.9 & \textbf{0.94} & 0.92 & 0.85 & \textbf{0.94}\\
 100 & & 0.96 & \textbf{1.0} & \textbf{1.0} & 0.96 & \textbf{1.0} & 0.92 & 0.96 & 0.96 & \textbf{1.0} & \textbf{1.0} & 0.96 & \textbf{1.0} & 0.92 & 0.96\\\hline
 10 & \multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{sokoban}}} & \textbf{0.38} & \textbf{0.38} & 0.24 & \textbf{0.39} & 0.34 & 0.31 & \textbf{0.39} & \textbf{0.38} & 0.3 & 0.24 & \textbf{0.52} & 0.25 & 0.36 & \textbf{0.52}\\
 30 & & \textbf{0.59} & 0.41 & 0.14 & \textbf{0.75} & 0.38 & 0.59 & \textbf{0.75} & \textbf{0.72} & 0.43 & 0.14 & \textbf{0.77} & 0.37 & 0.68 & \textbf{0.77}\\
 50 & & \textbf{0.82} & 0.53 & 0.21 & \textbf{0.92} & 0.49 & 0.82 & \textbf{0.92} & \textbf{0.77} & 0.51 & 0.17 & \textbf{0.79} & 0.41 & \textbf{0.79} & \textbf{0.79}\\
 70 & & \textbf{0.93} & 0.73 & 0.21 & \textbf{0.99} & 0.62 & 0.93 & \textbf{0.99} & \textbf{0.85} & 0.58 & 0.17 & 0.8 & 0.51 & \textbf{0.85} & 0.8\\
 100 & & \textbf{0.96} & 0.85 & 0.23 & \textbf{1.0} & 0.81 & 0.96 & \textbf{1.0} & \textbf{0.88} & 0.73 & 0.22 & 0.83 & 0.72 & \textbf{0.88} & 0.83\\\hline
 10 & \multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{zeno}}} & 0.65 & \textbf{0.72} & 0.6 & 0.67 & 0.68 & \textbf{0.71} & 0.67 & \textbf{0.68} & 0.59 & 0.55 & 0.65 & 0.58 & \textbf{0.7} & 0.64\\
 30 & & \textbf{0.84} & 0.72 & 0.55 & 0.78 & 0.77 & \textbf{0.83} & 0.76 & \textbf{0.76} & \textbf{0.76} & 0.55 & 0.72 & 0.77 & \textbf{0.78} & 0.73\\
 50 & & \textbf{0.88} & 0.83 & 0.57 & \textbf{0.9} & 0.83 & 0.89 & \textbf{0.9} & 0.85 & \textbf{0.86} & 0.67 & 0.87 & 0.87 & \textbf{0.88} & 0.87\\
 70 & & \textbf{0.94} & \textbf{0.94} & 0.65 & 0.94 & \textbf{0.98} & 0.97 & 0.94 & \textbf{0.94} & \textbf{0.94} & 0.64 & 0.94 & \textbf{0.99} & 0.96 & 0.94\\
 100 & & \textbf{1.0} & 0.96 & 0.66 & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & 0.96 & 0.66 & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0}\\\hline
 - & \textsc{f}%
 & \textbf{0.95} & \textbf{0.95} & 0.48 & \textbf{0.95} & \textbf{0.95} & \textbf{0.95} & \textbf{0.95} & \textbf{0.88} & \textbf{0.88} & 0.47 & \textbf{0.88} & \textbf{0.88} & \textbf{0.88} & \textbf{0.88}\\\hline%
 - & \textsc{l}%
 & 0.92 & \textbf{0.96} & 0.7 & \textbf{0.96} & 0.92 & 0.88 & 0.95 & 0.9 & \textbf{0.93} & 0.72 & \textbf{0.93} & 0.92 & 0.9 & \textbf{0.93}\\\hline%
 - & \textsc{m}%
 & 0.82 & \textbf{0.89} & 0.79 & \textbf{0.96} & 0.89 & 0.82 & \textbf{0.96} & 0.79 & \textbf{0.88} & 0.79 & \textbf{0.93} & 0.88 & 0.79 & \textbf{0.93}\\\hline%
 - & \textsc{r}%
 & 0.77 & \textbf{0.92} & 0.88 & \textbf{0.93} & 0.92 & 0.87 & \textbf{0.93} & 0.76 & \textbf{0.92} & 0.85 & \textbf{0.92} & \textbf{0.92} & 0.85 & \textbf{0.92}\\\midrule%
\multicolumn{2}{c|}{AVG}  & \textbf{0.79} & 0.77 & 0.54 & \textbf{0.86} & 0.78 & 0.8 & \textbf{0.86} & \textbf{0.76} & 0.74 & 0.52 & \textbf{0.82} & 0.75 & 0.78 & \textbf{0.82}\\
\bottomrule
\end{tabular}\\

==> tables/domains.tex <==
\begin{tabular}{c|c|c|cccccccccccc}
\toprule
\multicolumn{3}{c|}{} & \rotatebox[origin=c]{90}{ \textsc{blocks} } & \rotatebox[origin=c]{90}{ \textsc{depots} } & \rotatebox[origin=c]{90}{ \textsc{driverlog} } & \rotatebox[origin=c]{90}{ \textsc{dwr} } & \rotatebox[origin=c]{90}{ \textsc{ipc-grid} } & \rotatebox[origin=c]{90}{ \textsc{ferry} } & \rotatebox[origin=c]{90}{ \textsc{logistics} } & \rotatebox[origin=c]{90}{ \textsc{miconic} } & \rotatebox[origin=c]{90}{ \textsc{rovers} } & \rotatebox[origin=c]{90}{ \textsc{satellite} } & \rotatebox[origin=c]{90}{ \textsc{sokoban} } & \rotatebox[origin=c]{90}{ \textsc{zeno} }\\\midrule
\multicolumn{3}{c|}{$|\goalconditions|$} & 20.33 & 8.0 & 6.67 & 6.67 & 7.5 & 6.67 & 10.0 & 6.0 & 6.0 & 6.0 & 8.67 & 6.0\\\midrule
\multirow{10}{*}{ \rotatebox[origin=c]{90}{\textsc{Optimal}} }& \multicolumn{1}{c}{ \multirow{5}{*}{$|\observations|$} }& \multicolumn{1}{|c|}{10\%}& 1.25& 1.0& 1.75& 2.83& 1.63& 2.25& 2.0& 2.0& 1.67& 1.42& 2.33& 1.75\\
& \multicolumn{1}{c}{}& \multicolumn{1}{|c|}{30\%}& 3.08& 2.92& 4.17& 6.92& 4.0& 6.0& 5.75& 5.42& 3.67& 3.42& 6.5& 4.0\\
& \multicolumn{1}{c}{}& \multicolumn{1}{|c|}{50\%}& 4.42& 4.83& 6.33& 11.33& 6.19& 9.67& 9.42& 8.42& 5.75& 5.75& 10.33& 6.17\\
& \multicolumn{1}{c}{}& \multicolumn{1}{|c|}{70\%}& 6.67& 6.83& 8.92& 16.08& 8.69& 13.5& 13.25& 11.92& 8.17& 8.08& 14.67& 8.75\\
& \multicolumn{1}{c}{}& \multicolumn{1}{|c|}{100\%}& 8.83& 9.5& 12.17& 22.0& 11.88& 18.83& 18.17& 16.33& 10.83& 10.75& 20.17& 12.0\\
\cline{2-15}
& \multicolumn{1}{c}{ \multirow{5}{*}{$|\grsolution|$} }& \multicolumn{1}{|c|}{10\%} & 8.0 & 4.17 & 2.36 & 3.47 & 2.71 & 3.58 & 2.83 & 2.53 & 2.28 & 3.53 & 2.11 & 2.36\\
& \multicolumn{1}{c}{}& \multicolumn{1}{|c|}{30\%} & 3.97 & 1.94 & 1.58 & 1.89 & 1.21 & 1.64 & 1.19 & 1.22 & 1.31 & 2.39 & 1.25 & 1.33\\
& \multicolumn{1}{c}{}& \multicolumn{1}{|c|}{50\%} & 2.5 & 1.14 & 1.22 & 1.36 & 1.13 & 1.22 & 1.06 & 1.06 & 1.19 & 1.58 & 1.22 & 1.03\\
& \multicolumn{1}{c}{}& \multicolumn{1}{|c|}{70\%} & 1.94 & 1.06 & 1.14 & 1.19 & 1.04 & 1.19 & 1.03 & 1.0 & 1.0 & 1.31 & 1.03 & 1.0\\
& \multicolumn{1}{c}{}& \multicolumn{1}{|c|}{100\%} & 1.83 & 1.0 & 1.08 & 1.08 & 1.0 & 1.17 & 1.0 & 1.0 & 1.0 & 1.25 & 1.0 & 1.0\\
\midrule
\multirow{10}{*}{ \rotatebox[origin=c]{90}{\textsc{Sub-optimal}} }& \multicolumn{1}{c}{ \multirow{5}{*}{$|\observations|$} }& \multicolumn{1}{|c|}{10\%}& 1.42& 1.92& 2.17& 3.25& 2.06& 3.33& 2.67& 3.0& 1.83& 2.0& 3.33& 2.0\\
& \multicolumn{1}{c}{}& \multicolumn{1}{|c|}{30\%}& 3.83& 4.5& 5.58& 9.08& 5.56& 8.75& 7.5& 7.67& 4.5& 4.33& 8.67& 5.42\\
& \multicolumn{1}{c}{}& \multicolumn{1}{|c|}{50\%}& 5.92& 6.75& 8.75& 14.5& 8.88& 14.0& 11.92& 12.25& 7.17& 6.75& 13.75& 8.25\\
& \multicolumn{1}{c}{}& \multicolumn{1}{|c|}{70\%}& 8.5& 9.75& 12.33& 20.25& 12.56& 19.67& 16.67& 17.33& 10.0& 9.42& 19.33& 11.75\\
& \multicolumn{1}{c}{}& \multicolumn{1}{|c|}{100\%}& 11.83& 13.33& 17.0& 28.33& 17.25& 27.5& 23.17& 24.0& 13.67& 12.75& 27.0& 16.17\\
\cline{2-15}
& \multicolumn{1}{c}{ \multirow{5}{*}{$|\grsolution|$} }& \multicolumn{1}{|c|}{10\%} & 7.61 & 2.17 & 1.92 & 2.89 & 1.58 & 2.69 & 2.0 & 1.83 & 2.39 & 3.25 & 1.83 & 1.78\\
& \multicolumn{1}{c}{}& \multicolumn{1}{|c|}{30\%} & 3.58 & 1.83 & 1.31 & 1.83 & 1.4 & 1.42 & 1.14 & 1.25 & 1.39 & 1.78 & 1.28 & 1.14\\
& \multicolumn{1}{c}{}& \multicolumn{1}{|c|}{50\%} & 3.19 & 1.14 & 1.33 & 1.53 & 1.35 & 1.28 & 1.06 & 1.03 & 1.11 & 1.36 & 1.33 & 1.06\\
& \multicolumn{1}{c}{}& \multicolumn{1}{|c|}{70\%} & 2.53 & 1.14 & 1.31 & 1.17 & 1.31 & 1.28 & 1.03 & 1.0 & 1.06 & 1.33 & 1.36 & 1.0\\
& \multicolumn{1}{c}{}& \multicolumn{1}{|c|}{100\%} & 2.25 & 1.0 & 1.17 & 1.08 & 1.5 & 1.25 & 1.0 & 1.0 & 1.0 & 1.25 & 1.33 & 1.0\\

\bottomrule
\end{tabular}\\

==> tables/filters-optimal-noisy.tex <==
\begin{tabular}{|c|c|ccc|ccc|ccc|ccc|ccc|ccc|ccc|}
\hline
% empty
& % empty
& \multicolumn{3}{c|}{}
& \multicolumn{3}{c|}{\hdeltahc F0}
& \multicolumn{3}{c|}{\hdeltahcu F0}
& \multicolumn{3}{c|}{\hdeltahc F1}
& \multicolumn{3}{c|}{\hdeltahcu F1}
& \multicolumn{3}{c|}{\hdeltahc F2}
& \multicolumn{3}{c|}{\hdeltahcu F2}
\\ \hline
\# & $|\goalconditions|$ & \textbf{\% Obs} & $|\observations|$  & $|\grsolution|$ 
& \textbf{AGR} & \textbf{ACC} & \textbf{$|\Gamma^\textup{h}|$}
& \textbf{AGR} & \textbf{ACC} & \textbf{$|\Gamma^\textup{h}|$}
& \textbf{AGR} & \textbf{ACC} & \textbf{$|\Gamma^\textup{h}|$}
& \textbf{AGR} & \textbf{ACC} & \textbf{$|\Gamma^\textup{h}|$}
& \textbf{AGR} & \textbf{ACC} & \textbf{$|\Gamma^\textup{h}|$}
& \textbf{AGR} & \textbf{ACC} & \textbf{$|\Gamma^\textup{h}|$}
\\ 
\hline

\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{blocks}} } & \multirow{5}{*}{20.3} 
	 & 10	 & 2.25	 & 8.0

		% delta-h-c - 10% 
		& 0.32 & 66.7 & \textbf{6.67} 	 

		% delta-h-c-uncertainty - 10% 
		& 0.33 & 69.4 & 9.11 	 

		% delta-h-c-f1 - 10% 
		& 0.37 & 86.1 & 9.06 	 

		% delta-h-c-f1-uncertainty - 10% 
		& 0.37 & 86.1 & 9.14 	 

		% delta-h-c-f2 - 10% 
		& \textbf{0.4} & \textbf{97.2} & 17.58 	 

		% delta-h-c-f2-uncertainty - 10% 
		& \textbf{0.4} & \textbf{97.2} & 17.58 	 

	\\ & & 30	 & 4.08	 & 3.97

		% delta-h-c - 30% 
		& 0.37 & 75.0 & \textbf{3.44} 	 

		% delta-h-c-uncertainty - 30% 
		& 0.39 & 88.9 & 7.64 	 

		% delta-h-c-f1 - 30% 
		& 0.38 & 80.6 & 3.58 	 

		% delta-h-c-f1-uncertainty - 30% 
		& 0.39 & 83.3 & 4.5 	 

		% delta-h-c-f2 - 30% 
		& \textbf{0.41} & \textbf{97.2} & 7.08 	 

		% delta-h-c-f2-uncertainty - 30% 
		& \textbf{0.41} & \textbf{97.2} & 7.44 	 

	\\ & & 50	 & 5.67	 & 2.5

		% delta-h-c - 50% 
		& 0.64 & 83.3 & \textbf{2.17} 	 

		% delta-h-c-uncertainty - 50% 
		& 0.52 & \textbf{94.4} & 4.53 	 

		% delta-h-c-f1 - 50% 
		& \textbf{0.66} & 86.1 & 2.22 	 

		% delta-h-c-f1-uncertainty - 50% 
		& 0.62 & 88.9 & 2.89 	 

		% delta-h-c-f2 - 50% 
		& 0.56 & 88.9 & 3.72 	 

		% delta-h-c-f2-uncertainty - 50% 
		& 0.53 & 88.9 & 3.89 	 

	\\ & & 70	 & 8.42	 & 1.94

		% delta-h-c - 70% 
		& 0.79 & 91.7 & \textbf{1.67} 	 

		% delta-h-c-uncertainty - 70% 
		& 0.58 & 94.4 & 2.86 	 

		% delta-h-c-f1 - 70% 
		& \textbf{0.81} & 94.4 & 1.78 	 

		% delta-h-c-f1-uncertainty - 70% 
		& 0.67 & 94.4 & 2.47 	 

		% delta-h-c-f2 - 70% 
		& 0.76 & \textbf{97.2} & 2.19 	 

		% delta-h-c-f2-uncertainty - 70% 
		& 0.7 & \textbf{97.2} & 2.56 	 

	\\ & & 100	 & 11.08	 & 1.83

		% delta-h-c - 100% 
		& 0.88 & 94.4 & \textbf{1.58} 	 

		% delta-h-c-uncertainty - 100% 
		& 0.8 & 97.2 & 2.08 	 

		% delta-h-c-f1 - 100% 
		& 0.88 & 97.2 & 1.61 	 

		% delta-h-c-f1-uncertainty - 100% 
		& 0.88 & 97.2 & 1.61 	 

		% delta-h-c-f2 - 100% 
		& \textbf{0.91} & \textbf{100.0} & 1.69 	 

		% delta-h-c-f2-uncertainty - 100% 
		& 0.88 & 97.2 & 1.61 	 
 \\ \hline
\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{ipc-grid}} } & \multirow{5}{*}{7.5} 
	 & 10	 & 2.63	 & 2.71

		% delta-h-c - 10% 
		& 0.57 & 91.7 & \textbf{1.5} 	 

		% delta-h-c-uncertainty - 10% 
		& \textbf{0.61} & \textbf{95.8} & 1.67 	 

		% delta-h-c-f1 - 10% 
		& 0.56 & 91.7 & 1.54 	 

		% delta-h-c-f1-uncertainty - 10% 
		& 0.56 & 91.7 & 1.54 	 

		% delta-h-c-f2 - 10% 
		& 0.48 & 93.8 & 5.19 	 

		% delta-h-c-f2-uncertainty - 10% 
		& 0.48 & 93.8 & 5.19 	 

	\\ & & 30	 & 5.19	 & 1.21

		% delta-h-c - 30% 
		& \textbf{0.85} & 91.7 & \textbf{1.17} 	 

		% delta-h-c-uncertainty - 30% 
		& 0.83 & \textbf{93.8} & 1.25 	 

		% delta-h-c-f1 - 30% 
		& \textbf{0.85} & \textbf{93.8} & \textbf{1.17} 	 

		% delta-h-c-f1-uncertainty - 30% 
		& \textbf{0.85} & \textbf{93.8} & \textbf{1.17} 	 

		% delta-h-c-f2 - 30% 
		& 0.7 & 91.7 & 1.46 	 

		% delta-h-c-f2-uncertainty - 30% 
		& 0.7 & 91.7 & 1.46 	 

	\\ & & 50	 & 7.81	 & 1.13

		% delta-h-c - 50% 
		& \textbf{0.89} & \textbf{95.8} & \textbf{1.15} 	 

		% delta-h-c-uncertainty - 50% 
		& 0.88 & \textbf{95.8} & 1.17 	 

		% delta-h-c-f1 - 50% 
		& \textbf{0.89} & \textbf{95.8} & \textbf{1.15} 	 

		% delta-h-c-f1-uncertainty - 50% 
		& \textbf{0.89} & \textbf{95.8} & \textbf{1.15} 	 

		% delta-h-c-f2 - 50% 
		& 0.85 & \textbf{95.8} & 1.25 	 

		% delta-h-c-f2-uncertainty - 50% 
		& 0.85 & \textbf{95.8} & 1.25 	 

	\\ & & 70	 & 10.75	 & 1.04

		% delta-h-c - 70% 
		& \textbf{0.95} & \textbf{100.0} & \textbf{1.15} 	 

		% delta-h-c-uncertainty - 70% 
		& \textbf{0.95} & \textbf{100.0} & \textbf{1.15} 	 

		% delta-h-c-f1 - 70% 
		& \textbf{0.95} & \textbf{100.0} & \textbf{1.15} 	 

		% delta-h-c-f1-uncertainty - 70% 
		& \textbf{0.95} & \textbf{100.0} & \textbf{1.15} 	 

		% delta-h-c-f2 - 70% 
		& 0.93 & \textbf{100.0} & \textbf{1.15} 	 

		% delta-h-c-f2-uncertainty - 70% 
		& 0.93 & \textbf{100.0} & \textbf{1.15} 	 

	\\ & & 100	 & 14.63	 & 1.0

		% delta-h-c - 100% 
		& \textbf{1.0} & \textbf{100.0} & \textbf{1.0} 	 

		% delta-h-c-uncertainty - 100% 
		& \textbf{1.0} & \textbf{100.0} & \textbf{1.0} 	 

		% delta-h-c-f1 - 100% 
		& \textbf{1.0} & \textbf{100.0} & \textbf{1.0} 	 

		% delta-h-c-f1-uncertainty - 100% 
		& \textbf{1.0} & \textbf{100.0} & \textbf{1.0} 	 

		% delta-h-c-f2 - 100% 
		& \textbf{1.0} & \textbf{100.0} & \textbf{1.0} 	 

		% delta-h-c-f2-uncertainty - 100% 
		& \textbf{1.0} & \textbf{100.0} & \textbf{1.0} 	 
 \\ \hline
\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{logistics}} } & \multirow{5}{*}{10.0} 
	 & 10	 & 3.0	 & 2.83

		% delta-h-c - 10% 
		& 0.58 & 94.4 & \textbf{2.72} 	 

		% delta-h-c-uncertainty - 10% 
		& 0.58 & 94.4 & 2.78 	 

		% delta-h-c-f1 - 10% 
		& \textbf{0.6} & \textbf{100.0} & 3.03 	 

		% delta-h-c-f1-uncertainty - 10% 
		& \textbf{0.6} & \textbf{100.0} & 3.03 	 

		% delta-h-c-f2 - 10% 
		& 0.43 & \textbf{100.0} & 7.08 	 

		% delta-h-c-f2-uncertainty - 10% 
		& 0.43 & \textbf{100.0} & 7.08 	 

	\\ & & 30	 & 7.58	 & 1.19

		% delta-h-c - 30% 
		& 0.82 & 94.4 & \textbf{1.28} 	 

		% delta-h-c-uncertainty - 30% 
		& \textbf{0.84} & \textbf{100.0} & 1.67 	 

		% delta-h-c-f1 - 30% 
		& 0.82 & 94.4 & \textbf{1.28} 	 

		% delta-h-c-f1-uncertainty - 30% 
		& \textbf{0.84} & \textbf{100.0} & 1.58 	 

		% delta-h-c-f2 - 30% 
		& 0.77 & 94.4 & 1.42 	 

		% delta-h-c-f2-uncertainty - 30% 
		& 0.77 & 94.4 & 1.42 	 

	\\ & & 50	 & 11.42	 & 1.06

		% delta-h-c - 50% 
		& \textbf{0.9} & 97.2 & 1.11 	 

		% delta-h-c-uncertainty - 50% 
		& 0.88 & \textbf{100.0} & 1.28 	 

		% delta-h-c-f1 - 50% 
		& \textbf{0.9} & 97.2 & 1.11 	 

		% delta-h-c-f1-uncertainty - 50% 
		& 0.89 & \textbf{100.0} & 1.25 	 

		% delta-h-c-f2 - 50% 
		& \textbf{0.9} & 97.2 & \textbf{1.08} 	 

		% delta-h-c-f2-uncertainty - 50% 
		& \textbf{0.9} & 97.2 & \textbf{1.08} 	 

	\\ & & 70	 & 16.08	 & 1.03

		% delta-h-c - 70% 
		& \textbf{0.97} & \textbf{100.0} & \textbf{1.03} 	 

		% delta-h-c-uncertainty - 70% 
		& 0.94 & \textbf{100.0} & 1.08 	 

		% delta-h-c-f1 - 70% 
		& \textbf{0.97} & \textbf{100.0} & \textbf{1.03} 	 

		% delta-h-c-f1-uncertainty - 70% 
		& 0.94 & \textbf{100.0} & 1.08 	 

		% delta-h-c-f2 - 70% 
		& \textbf{0.97} & \textbf{100.0} & \textbf{1.03} 	 

		% delta-h-c-f2-uncertainty - 70% 
		& \textbf{0.97} & \textbf{100.0} & \textbf{1.03} 	 

	\\ & & 100	 & 22.0	 & 1.0

		% delta-h-c - 100% 
		& \textbf{1.0} & \textbf{100.0} & \textbf{1.0} 	 

		% delta-h-c-uncertainty - 100% 
		& \textbf{1.0} & \textbf{100.0} & \textbf{1.0} 	 

		% delta-h-c-f1 - 100% 
		& \textbf{1.0} & \textbf{100.0} & \textbf{1.0} 	 

		% delta-h-c-f1-uncertainty - 100% 
		& \textbf{1.0} & \textbf{100.0} & \textbf{1.0} 	 

		% delta-h-c-f2 - 100% 
		& \textbf{1.0} & \textbf{100.0} & \textbf{1.0} 	 

		% delta-h-c-f2-uncertainty - 100% 
		& \textbf{1.0} & \textbf{100.0} & \textbf{1.0} 	 
 \\ \hline
\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{miconic}} } & \multirow{5}{*}{6.0} 
	 & 10	 & 3.0	 & 2.53

		% delta-h-c - 10% 
		& 0.39 & 69.4 & \textbf{2.39} 	 

		% delta-h-c-uncertainty - 10% 
		& 0.37 & 72.2 & 3.08 	 

		% delta-h-c-f1 - 10% 
		& \textbf{0.52} & 97.2 & 3.19 	 

		% delta-h-c-f1-uncertainty - 10% 
		& \textbf{0.52} & 97.2 & 3.19 	 

		% delta-h-c-f2 - 10% 
		& 0.46 & \textbf{100.0} & 5.36 	 

		% delta-h-c-f2-uncertainty - 10% 
		& 0.46 & \textbf{100.0} & 5.36 	 

	\\ & & 30	 & 6.83	 & 1.22

		% delta-h-c - 30% 
		& 0.57 & 80.6 & \textbf{1.44} 	 

		% delta-h-c-uncertainty - 30% 
		& 0.43 & 83.3 & 2.22 	 

		% delta-h-c-f1 - 30% 
		& \textbf{0.65} & 94.4 & 1.58 	 

		% delta-h-c-f1-uncertainty - 30% 
		& 0.63 & 94.4 & 1.72 	 

		% delta-h-c-f2 - 30% 
		& 0.53 & \textbf{100.0} & 2.44 	 

		% delta-h-c-f2-uncertainty - 30% 
		& 0.53 & \textbf{100.0} & 2.44 	 

	\\ & & 50	 & 10.42	 & 1.06

		% delta-h-c - 50% 
		& \textbf{0.93} & \textbf{100.0} & \textbf{1.14} 	 

		% delta-h-c-uncertainty - 50% 
		& 0.76 & \textbf{100.0} & 1.67 	 

		% delta-h-c-f1 - 50% 
		& \textbf{0.93} & \textbf{100.0} & \textbf{1.14} 	 

		% delta-h-c-f1-uncertainty - 50% 
		& 0.89 & \textbf{100.0} & 1.22 	 

		% delta-h-c-f2 - 50% 
		& \textbf{0.93} & \textbf{100.0} & \textbf{1.14} 	 

		% delta-h-c-f2-uncertainty - 50% 
		& \textbf{0.93} & \textbf{100.0} & \textbf{1.14} 	 

	\\ & & 70	 & 14.83	 & 1.0

		% delta-h-c - 70% 
		& 0.94 & 97.2 & \textbf{1.08} 	 

		% delta-h-c-uncertainty - 70% 
		& 0.78 & \textbf{100.0} & 1.53 	 

		% delta-h-c-f1 - 70% 
		& \textbf{0.95} & \textbf{100.0} & 1.14 	 

		% delta-h-c-f1-uncertainty - 70% 
		& 0.92 & \textbf{100.0} & 1.22 	 

		% delta-h-c-f2 - 70% 
		& \textbf{0.95} & \textbf{100.0} & 1.14 	 

		% delta-h-c-f2-uncertainty - 70% 
		& \textbf{0.95} & \textbf{100.0} & 1.14 	 

	\\ & & 100	 & 20.0	 & 1.0

		% delta-h-c - 100% 
		& 0.94 & 97.2 & 1.06 	 

		% delta-h-c-uncertainty - 100% 
		& 0.93 & 97.2 & 1.11 	 

		% delta-h-c-f1 - 100% 
		& 0.97 & \textbf{100.0} & 1.06 	 

		% delta-h-c-f1-uncertainty - 100% 
		& 0.97 & \textbf{100.0} & 1.06 	 

		% delta-h-c-f2 - 100% 
		& \textbf{0.99} & \textbf{100.0} & 1.03 	 

		% delta-h-c-f2-uncertainty - 100% 
		& 0.93 & 94.4 & \textbf{0.97} 	 
 \\ \hline
\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{rovers}} } & \multirow{5}{*}{6.0} 
	 & 10	 & 2.67	 & 2.28

		% delta-h-c - 10% 
		& 0.44 & 80.6 & \textbf{2.58} 	 

		% delta-h-c-uncertainty - 10% 
		& 0.44 & 86.1 & 2.78 	 

		% delta-h-c-f1 - 10% 
		& \textbf{0.46} & 88.9 & 2.94 	 

		% delta-h-c-f1-uncertainty - 10% 
		& \textbf{0.46} & 88.9 & 2.94 	 

		% delta-h-c-f2 - 10% 
		& 0.4 & \textbf{100.0} & 5.42 	 

		% delta-h-c-f2-uncertainty - 10% 
		& 0.4 & \textbf{100.0} & 5.42 	 

	\\ & & 30	 & 4.67	 & 1.31

		% delta-h-c - 30% 
		& 0.7 & 83.3 & \textbf{1.36} 	 

		% delta-h-c-uncertainty - 30% 
		& 0.68 & 91.7 & 1.69 	 

		% delta-h-c-f1 - 30% 
		& \textbf{0.72} & 83.3 & \textbf{1.36} 	 

		% delta-h-c-f1-uncertainty - 30% 
		& \textbf{0.72} & 83.3 & \textbf{1.36} 	 

		% delta-h-c-f2 - 30% 
		& 0.5 & \textbf{97.2} & 2.81 	 

		% delta-h-c-f2-uncertainty - 30% 
		& 0.5 & \textbf{97.2} & 2.81 	 

	\\ & & 50	 & 7.42	 & 1.19

		% delta-h-c - 50% 
		& 0.8 & 91.7 & \textbf{1.33} 	 

		% delta-h-c-uncertainty - 50% 
		& 0.79 & 94.4 & 1.47 	 

		% delta-h-c-f1 - 50% 
		& \textbf{0.82} & \textbf{97.2} & 1.36 	 

		% delta-h-c-f1-uncertainty - 50% 
		& 0.8 & \textbf{97.2} & 1.44 	 

		% delta-h-c-f2 - 50% 
		& 0.67 & 94.4 & 1.81 	 

		% delta-h-c-f2-uncertainty - 50% 
		& 0.67 & 94.4 & 1.81 	 

	\\ & & 70	 & 10.17	 & 1.0

		% delta-h-c - 70% 
		& \textbf{0.93} & \textbf{97.2} & \textbf{1.08} 	 

		% delta-h-c-uncertainty - 70% 
		& 0.89 & \textbf{97.2} & 1.17 	 

		% delta-h-c-f1 - 70% 
		& 0.92 & \textbf{97.2} & 1.11 	 

		% delta-h-c-f1-uncertainty - 70% 
		& 0.92 & \textbf{97.2} & 1.11 	 

		% delta-h-c-f2 - 70% 
		& 0.9 & \textbf{97.2} & 1.14 	 

		% delta-h-c-f2-uncertainty - 70% 
		& 0.9 & \textbf{97.2} & 1.14 	 

	\\ & & 100	 & 13.5	 & 1.0

		% delta-h-c - 100% 
		& \textbf{0.97} & \textbf{100.0} & 1.06 	 

		% delta-h-c-uncertainty - 100% 
		& \textbf{0.97} & \textbf{100.0} & 1.06 	 

		% delta-h-c-f1 - 100% 
		& 0.96 & 97.2 & \textbf{1.03} 	 

		% delta-h-c-f1-uncertainty - 100% 
		& 0.96 & 97.2 & \textbf{1.03} 	 

		% delta-h-c-f2 - 100% 
		& 0.93 & 97.2 & 1.08 	 

		% delta-h-c-f2-uncertainty - 100% 
		& 0.93 & 97.2 & 1.08 	 
 \\ \hline
\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{satellite}} } & \multirow{5}{*}{6.0} 
	 & 10	 & 2.42	 & 3.53

		% delta-h-c - 10% 
		& 0.53 & 75.0 & \textbf{3.31} 	 

		% delta-h-c-uncertainty - 10% 
		& 0.51 & 77.8 & 3.64 	 

		% delta-h-c-f1 - 10% 
		& \textbf{0.64} & 97.2 & 4.36 	 

		% delta-h-c-f1-uncertainty - 10% 
		& \textbf{0.64} & 97.2 & 4.36 	 

		% delta-h-c-f2 - 10% 
		& 0.59 & \textbf{100.0} & 5.89 	 

		% delta-h-c-f2-uncertainty - 10% 
		& 0.59 & \textbf{100.0} & 5.89 	 

	\\ & & 30	 & 4.42	 & 2.39

		% delta-h-c - 30% 
		& 0.5 & 77.8 & \textbf{2.33} 	 

		% delta-h-c-uncertainty - 30% 
		& \textbf{0.54} & 83.3 & 3.08 	 

		% delta-h-c-f1 - 30% 
		& 0.48 & 94.4 & 2.81 	 

		% delta-h-c-f1-uncertainty - 30% 
		& 0.48 & 94.4 & 2.81 	 

		% delta-h-c-f2 - 30% 
		& 0.45 & \textbf{100.0} & 4.53 	 

		% delta-h-c-f2-uncertainty - 30% 
		& 0.45 & \textbf{100.0} & 4.53 	 

	\\ & & 50	 & 7.17	 & 1.58

		% delta-h-c - 50% 
		& 0.67 & 88.9 & \textbf{1.89} 	 

		% delta-h-c-uncertainty - 50% 
		& 0.57 & \textbf{91.7} & 2.53 	 

		% delta-h-c-f1 - 50% 
		& \textbf{0.69} & \textbf{91.7} & \textbf{1.89} 	 

		% delta-h-c-f1-uncertainty - 50% 
		& 0.66 & \textbf{91.7} & 2.08 	 

		% delta-h-c-f2 - 50% 
		& 0.55 & \textbf{91.7} & 2.61 	 

		% delta-h-c-f2-uncertainty - 50% 
		& 0.55 & \textbf{91.7} & 2.61 	 

	\\ & & 70	 & 10.08	 & 1.31

		% delta-h-c - 70% 
		& 0.87 & 94.4 & \textbf{1.31} 	 

		% delta-h-c-uncertainty - 70% 
		& 0.71 & 94.4 & 2.17 	 

		% delta-h-c-f1 - 70% 
		& 0.87 & 94.4 & \textbf{1.31} 	 

		% delta-h-c-f1-uncertainty - 70% 
		& 0.82 & 94.4 & 1.47 	 

		% delta-h-c-f2 - 70% 
		& \textbf{0.91} & \textbf{100.0} & 1.33 	 

		% delta-h-c-f2-uncertainty - 70% 
		& \textbf{0.91} & \textbf{100.0} & 1.33 	 

	\\ & & 100	 & 13.17	 & 1.25

		% delta-h-c - 100% 
		& 0.92 & \textbf{97.2} & 1.31 	 

		% delta-h-c-uncertainty - 100% 
		& 0.88 & \textbf{97.2} & 1.39 	 

		% delta-h-c-f1 - 100% 
		& \textbf{0.97} & \textbf{97.2} & 1.19 	 

		% delta-h-c-f1-uncertainty - 100% 
		& \textbf{0.97} & \textbf{97.2} & 1.19 	 

		% delta-h-c-f2 - 100% 
		& 0.94 & \textbf{97.2} & 1.14 	 

		% delta-h-c-f2-uncertainty - 100% 
		& 0.92 & 94.4 & \textbf{1.11} 	 
 \\ \hline
\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{sokoban}} } & \multirow{5}{*}{8.7} 
	 & 10	 & 3.33	 & 2.11

		% delta-h-c - 10% 
		& 0.27 & 58.3 & 2.78 	 

		% delta-h-c-uncertainty - 10% 
		& 0.29 & \textbf{83.3} & 4.36 	 

		% delta-h-c-f1 - 10% 
		& 0.29 & 47.2 & \textbf{1.64} 	 

		% delta-h-c-f1-uncertainty - 10% 
		& \textbf{0.33} & 58.3 & 1.94 	 

		% delta-h-c-f2 - 10% 
		& 0.26 & 63.9 & 3.64 	 

		% delta-h-c-f2-uncertainty - 10% 
		& 0.26 & 63.9 & 3.64 	 

	\\ & & 30	 & 8.17	 & 1.25

		% delta-h-c - 30% 
		& 0.56 & 77.8 & 2.17 	 

		% delta-h-c-uncertainty - 30% 
		& 0.41 & \textbf{97.2} & 4.42 	 

		% delta-h-c-f1 - 30% 
		& 0.69 & 83.3 & 1.5 	 

		% delta-h-c-f1-uncertainty - 30% 
		& 0.47 & 88.9 & 3.03 	 

		% delta-h-c-f2 - 30% 
		& \textbf{0.73} & 88.9 & \textbf{1.44} 	 

		% delta-h-c-f2-uncertainty - 30% 
		& 0.64 & 91.7 & 2.17 	 

	\\ & & 50	 & 12.67	 & 1.22

		% delta-h-c - 50% 
		& 0.61 & 94.4 & 2.97 	 

		% delta-h-c-uncertainty - 50% 
		& 0.47 & \textbf{97.2} & 4.11 	 

		% delta-h-c-f1 - 50% 
		& 0.68 & 94.4 & 2.58 	 

		% delta-h-c-f1-uncertainty - 50% 
		& 0.53 & \textbf{97.2} & 3.31 	 

		% delta-h-c-f2 - 50% 
		& \textbf{0.82} & \textbf{97.2} & \textbf{1.19} 	 

		% delta-h-c-f2-uncertainty - 50% 
		& 0.65 & \textbf{97.2} & 1.86 	 

	\\ & & 70	 & 18.0	 & 1.03

		% delta-h-c - 70% 
		& 0.6 & 94.4 & 3.75 	 

		% delta-h-c-uncertainty - 70% 
		& 0.5 & 94.4 & 4.42 	 

		% delta-h-c-f1 - 70% 
		& 0.77 & 94.4 & 2.36 	 

		% delta-h-c-f1-uncertainty - 70% 
		& 0.65 & 97.2 & 2.94 	 

		% delta-h-c-f2 - 70% 
		& \textbf{0.94} & 97.2 & \textbf{1.06} 	 

		% delta-h-c-f2-uncertainty - 70% 
		& 0.83 & \textbf{100.0} & 1.42 	 

	\\ & & 100	 & 24.67	 & 1.0

		% delta-h-c - 100% 
		& 0.66 & \textbf{100.0} & 3.89 	 

		% delta-h-c-uncertainty - 100% 
		& 0.55 & \textbf{100.0} & 4.28 	 

		% delta-h-c-f1 - 100% 
		& 0.71 & 94.4 & 2.89 	 

		% delta-h-c-f1-uncertainty - 100% 
		& 0.64 & 97.2 & 3.25 	 

		% delta-h-c-f2 - 100% 
		& \textbf{0.85} & 94.4 & \textbf{1.83} 	 

		% delta-h-c-f2-uncertainty - 100% 
		& 0.77 & 97.2 & 2.14 	 
 \\ \hline
Avg & & & &  & 0.72 & 89.48 & \textbf{1.97} & 0.67 & 93.23 & 2.64 & \textbf{0.75} & 93.19 & 2.0 & 0.73 & 94.3 & 2.21 & 0.73 & \textbf{96.29} & 2.91 & 0.71 & 96.21 & 2.99
\\ \hline
\end{tabular}

==> tables/filters-suboptimal-noisy.tex <==
\begin{tabular}{|c|c|ccc|ccc|ccc|ccc|ccc|ccc|ccc|}
\hline
% empty
& % empty
& \multicolumn{3}{c|}{}
& \multicolumn{3}{c|}{\hdeltahc F0}
& \multicolumn{3}{c|}{\hdeltahcu F0}
& \multicolumn{3}{c|}{\hdeltahc F1}
& \multicolumn{3}{c|}{\hdeltahcu F1}
& \multicolumn{3}{c|}{\hdeltahc F2}
& \multicolumn{3}{c|}{\hdeltahcu F2}
\\ \hline
\# & $|\goalconditions|$ & \textbf{\% Obs} & $|\observations|$  & $|\grsolution|$ 
& \textbf{AGR} & \textbf{ACC} & \textbf{$|\Gamma^\textup{h}|$}
& \textbf{AGR} & \textbf{ACC} & \textbf{$|\Gamma^\textup{h}|$}
& \textbf{AGR} & \textbf{ACC} & \textbf{$|\Gamma^\textup{h}|$}
& \textbf{AGR} & \textbf{ACC} & \textbf{$|\Gamma^\textup{h}|$}
& \textbf{AGR} & \textbf{ACC} & \textbf{$|\Gamma^\textup{h}|$}
& \textbf{AGR} & \textbf{ACC} & \textbf{$|\Gamma^\textup{h}|$}
\\ 
\hline

\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{blocks}} } & \multirow{5}{*}{20.3} 
	 & 10	 & 2.42	 & 7.61

		% delta-h-c - 10% 
		& 0.38 & 69.4 & \textbf{6.58} 	 

		% delta-h-c-uncertainty - 10% 
		& \textbf{0.42} & 88.9 & 12.72 	 

		% delta-h-c-f1 - 10% 
		& 0.41 & 75.0 & 7.33 	 

		% delta-h-c-f1-uncertainty - 10% 
		& 0.4 & 77.8 & 7.92 	 

		% delta-h-c-f2 - 10% 
		& 0.41 & \textbf{97.2} & 16.11 	 

		% delta-h-c-f2-uncertainty - 10% 
		& 0.41 & \textbf{97.2} & 16.11 	 

	\\ & & 30	 & 4.92	 & 3.58

		% delta-h-c - 30% 
		& 0.36 & 63.9 & \textbf{3.47} 	 

		% delta-h-c-uncertainty - 30% 
		& 0.34 & \textbf{91.7} & 11.33 	 

		% delta-h-c-f1 - 30% 
		& 0.4 & 72.2 & 3.67 	 

		% delta-h-c-f1-uncertainty - 30% 
		& 0.38 & \textbf{91.7} & 7.83 	 

		% delta-h-c-f2 - 30% 
		& \textbf{0.42} & 83.3 & 5.31 	 

		% delta-h-c-f2-uncertainty - 30% 
		& 0.4 & 88.9 & 6.31 	 

	\\ & & 50	 & 7.33	 & 3.19

		% delta-h-c - 50% 
		& \textbf{0.53} & 83.3 & \textbf{2.64} 	 

		% delta-h-c-uncertainty - 50% 
		& 0.33 & \textbf{97.2} & 7.64 	 

		% delta-h-c-f1 - 50% 
		& \textbf{0.53} & 83.3 & 2.67 	 

		% delta-h-c-f1-uncertainty - 50% 
		& 0.43 & 94.4 & 5.39 	 

		% delta-h-c-f2 - 50% 
		& 0.5 & 86.1 & 3.03 	 

		% delta-h-c-f2-uncertainty - 50% 
		& 0.47 & 91.7 & 4.14 	 

	\\ & & 70	 & 10.67	 & 2.53

		% delta-h-c - 70% 
		& \textbf{0.67} & 88.9 & \textbf{2.22} 	 

		% delta-h-c-uncertainty - 70% 
		& 0.45 & \textbf{100.0} & 5.56 	 

		% delta-h-c-f1 - 70% 
		& \textbf{0.67} & 88.9 & \textbf{2.22} 	 

		% delta-h-c-f1-uncertainty - 70% 
		& 0.52 & 94.4 & 4.0 	 

		% delta-h-c-f2 - 70% 
		& \textbf{0.67} & 88.9 & \textbf{2.22} 	 

		% delta-h-c-f2-uncertainty - 70% 
		& 0.57 & 91.7 & 2.83 	 

	\\ & & 100	 & 14.42	 & 2.25

		% delta-h-c - 100% 
		& 0.78 & 91.7 & \textbf{1.53} 	 

		% delta-h-c-uncertainty - 100% 
		& 0.7 & \textbf{97.2} & 2.17 	 

		% delta-h-c-f1 - 100% 
		& 0.78 & 91.7 & \textbf{1.53} 	 

		% delta-h-c-f1-uncertainty - 100% 
		& 0.74 & 91.7 & 1.61 	 

		% delta-h-c-f2 - 100% 
		& \textbf{0.82} & \textbf{97.2} & 1.64 	 

		% delta-h-c-f2-uncertainty - 100% 
		& 0.75 & 94.4 & 1.69 	 
 \\ \hline
\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{ipc-grid}} } & \multirow{5}{*}{7.5} 
	 & 10	 & 3.06	 & 1.58

		% delta-h-c - 10% 
		& 0.62 & 89.6 & \textbf{2.1} 	 

		% delta-h-c-uncertainty - 10% 
		& 0.53 & \textbf{93.8} & 2.96 	 

		% delta-h-c-f1 - 10% 
		& \textbf{0.63} & 91.7 & 2.21 	 

		% delta-h-c-f1-uncertainty - 10% 
		& 0.57 & 91.7 & 2.58 	 

		% delta-h-c-f2 - 10% 
		& 0.55 & \textbf{93.8} & 3.25 	 

		% delta-h-c-f2-uncertainty - 10% 
		& 0.55 & \textbf{93.8} & 3.25 	 

	\\ & & 30	 & 7.13	 & 1.4

		% delta-h-c - 30% 
		& 0.68 & 89.6 & 1.44 	 

		% delta-h-c-uncertainty - 30% 
		& 0.55 & \textbf{93.8} & 2.08 	 

		% delta-h-c-f1 - 30% 
		& 0.68 & 89.6 & 1.44 	 

		% delta-h-c-f1-uncertainty - 30% 
		& 0.56 & \textbf{93.8} & 2.0 	 

		% delta-h-c-f2 - 30% 
		& \textbf{0.69} & 89.6 & \textbf{1.42} 	 

		% delta-h-c-f2-uncertainty - 30% 
		& 0.63 & \textbf{93.8} & 1.69 	 

	\\ & & 50	 & 10.94	 & 1.35

		% delta-h-c - 50% 
		& 0.84 & 95.8 & \textbf{1.06} 	 

		% delta-h-c-uncertainty - 50% 
		& 0.79 & \textbf{97.9} & 1.48 	 

		% delta-h-c-f1 - 50% 
		& 0.84 & \textbf{97.9} & 1.1 	 

		% delta-h-c-f1-uncertainty - 50% 
		& 0.79 & \textbf{97.9} & 1.48 	 

		% delta-h-c-f2 - 50% 
		& \textbf{0.85} & \textbf{97.9} & 1.08 	 

		% delta-h-c-f2-uncertainty - 50% 
		& 0.82 & \textbf{97.9} & 1.35 	 

	\\ & & 70	 & 15.56	 & 1.31

		% delta-h-c - 70% 
		& \textbf{0.89} & \textbf{100.0} & \textbf{1.06} 	 

		% delta-h-c-uncertainty - 70% 
		& 0.87 & \textbf{100.0} & 1.15 	 

		% delta-h-c-f1 - 70% 
		& \textbf{0.89} & \textbf{100.0} & \textbf{1.06} 	 

		% delta-h-c-f1-uncertainty - 70% 
		& 0.87 & \textbf{100.0} & 1.15 	 

		% delta-h-c-f2 - 70% 
		& \textbf{0.89} & \textbf{100.0} & \textbf{1.06} 	 

		% delta-h-c-f2-uncertainty - 70% 
		& 0.86 & \textbf{100.0} & 1.13 	 

	\\ & & 100	 & 21.13	 & 1.5

		% delta-h-c - 100% 
		& \textbf{0.94} & \textbf{100.0} & \textbf{1.0} 	 

		% delta-h-c-uncertainty - 100% 
		& \textbf{0.94} & \textbf{100.0} & \textbf{1.0} 	 

		% delta-h-c-f1 - 100% 
		& \textbf{0.94} & \textbf{100.0} & \textbf{1.0} 	 

		% delta-h-c-f1-uncertainty - 100% 
		& \textbf{0.94} & \textbf{100.0} & \textbf{1.0} 	 

		% delta-h-c-f2 - 100% 
		& \textbf{0.94} & \textbf{100.0} & \textbf{1.0} 	 

		% delta-h-c-f2-uncertainty - 100% 
		& \textbf{0.94} & \textbf{100.0} & \textbf{1.0} 	 
 \\ \hline
\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{logistics}} } & \multirow{5}{*}{10.0} 
	 & 10	 & 3.67	 & 2.0

		% delta-h-c - 10% 
		& 0.55 & 88.9 & \textbf{2.36} 	 

		% delta-h-c-uncertainty - 10% 
		& 0.51 & 88.9 & 2.94 	 

		% delta-h-c-f1 - 10% 
		& \textbf{0.57} & 97.2 & 2.69 	 

		% delta-h-c-f1-uncertainty - 10% 
		& 0.56 & 97.2 & 2.92 	 

		% delta-h-c-f2 - 10% 
		& 0.46 & \textbf{100.0} & 5.17 	 

		% delta-h-c-f2-uncertainty - 10% 
		& 0.46 & \textbf{100.0} & 5.17 	 

	\\ & & 30	 & 9.33	 & 1.14

		% delta-h-c - 30% 
		& \textbf{0.8} & \textbf{100.0} & \textbf{1.33} 	 

		% delta-h-c-uncertainty - 30% 
		& 0.7 & \textbf{100.0} & 1.94 	 

		% delta-h-c-f1 - 30% 
		& \textbf{0.8} & \textbf{100.0} & \textbf{1.33} 	 

		% delta-h-c-f1-uncertainty - 30% 
		& 0.7 & \textbf{100.0} & 1.89 	 

		% delta-h-c-f2 - 30% 
		& 0.75 & \textbf{100.0} & 1.72 	 

		% delta-h-c-f2-uncertainty - 30% 
		& 0.67 & \textbf{100.0} & 1.94 	 

	\\ & & 50	 & 14.58	 & 1.06

		% delta-h-c - 50% 
		& \textbf{0.91} & \textbf{100.0} & \textbf{1.22} 	 

		% delta-h-c-uncertainty - 50% 
		& 0.7 & \textbf{100.0} & 2.08 	 

		% delta-h-c-f1 - 50% 
		& \textbf{0.91} & \textbf{100.0} & \textbf{1.22} 	 

		% delta-h-c-f1-uncertainty - 50% 
		& 0.7 & \textbf{100.0} & 2.08 	 

		% delta-h-c-f2 - 50% 
		& \textbf{0.91} & \textbf{100.0} & \textbf{1.22} 	 

		% delta-h-c-f2-uncertainty - 50% 
		& 0.77 & \textbf{100.0} & 1.86 	 

	\\ & & 70	 & 20.17	 & 1.03

		% delta-h-c - 70% 
		& \textbf{0.96} & \textbf{100.0} & \textbf{1.06} 	 

		% delta-h-c-uncertainty - 70% 
		& 0.84 & \textbf{100.0} & 1.36 	 

		% delta-h-c-f1 - 70% 
		& \textbf{0.96} & \textbf{100.0} & \textbf{1.06} 	 

		% delta-h-c-f1-uncertainty - 70% 
		& 0.84 & \textbf{100.0} & 1.36 	 

		% delta-h-c-f2 - 70% 
		& \textbf{0.96} & \textbf{100.0} & \textbf{1.06} 	 

		% delta-h-c-f2-uncertainty - 70% 
		& 0.85 & \textbf{100.0} & 1.33 	 

	\\ & & 100	 & 28.17	 & 1.0

		% delta-h-c - 100% 
		& \textbf{1.0} & \textbf{100.0} & \textbf{1.0} 	 

		% delta-h-c-uncertainty - 100% 
		& \textbf{1.0} & \textbf{100.0} & \textbf{1.0} 	 

		% delta-h-c-f1 - 100% 
		& \textbf{1.0} & \textbf{100.0} & \textbf{1.0} 	 

		% delta-h-c-f1-uncertainty - 100% 
		& \textbf{1.0} & \textbf{100.0} & \textbf{1.0} 	 

		% delta-h-c-f2 - 100% 
		& \textbf{1.0} & \textbf{100.0} & \textbf{1.0} 	 

		% delta-h-c-f2-uncertainty - 100% 
		& \textbf{1.0} & \textbf{100.0} & \textbf{1.0} 	 
 \\ \hline
\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{miconic}} } & \multirow{5}{*}{6.0} 
	 & 10	 & 4.0	 & 1.83

		% delta-h-c - 10% 
		& 0.43 & 80.6 & \textbf{2.11} 	 

		% delta-h-c-uncertainty - 10% 
		& 0.41 & 83.3 & 2.89 	 

		% delta-h-c-f1 - 10% 
		& \textbf{0.55} & 97.2 & 2.47 	 

		% delta-h-c-f1-uncertainty - 10% 
		& \textbf{0.55} & 97.2 & 2.47 	 

		% delta-h-c-f2 - 10% 
		& 0.36 & \textbf{100.0} & 4.61 	 

		% delta-h-c-f2-uncertainty - 10% 
		& 0.36 & \textbf{100.0} & 4.61 	 

	\\ & & 30	 & 9.67	 & 1.25

		% delta-h-c - 30% 
		& 0.75 & 88.9 & \textbf{1.36} 	 

		% delta-h-c-uncertainty - 30% 
		& 0.36 & \textbf{100.0} & 3.69 	 

		% delta-h-c-f1 - 30% 
		& \textbf{0.78} & 94.4 & 1.42 	 

		% delta-h-c-f1-uncertainty - 30% 
		& 0.52 & 97.2 & 2.58 	 

		% delta-h-c-f2 - 30% 
		& 0.77 & 94.4 & 1.47 	 

		% delta-h-c-f2-uncertainty - 30% 
		& 0.66 & 97.2 & 2.0 	 

	\\ & & 50	 & 15.25	 & 1.03

		% delta-h-c - 50% 
		& \textbf{0.86} & 94.4 & \textbf{1.14} 	 

		% delta-h-c-uncertainty - 50% 
		& 0.45 & \textbf{100.0} & 3.19 	 

		% delta-h-c-f1 - 50% 
		& \textbf{0.86} & 94.4 & \textbf{1.14} 	 

		% delta-h-c-f1-uncertainty - 50% 
		& 0.57 & \textbf{100.0} & 2.36 	 

		% delta-h-c-f2 - 50% 
		& \textbf{0.86} & 94.4 & \textbf{1.14} 	 

		% delta-h-c-f2-uncertainty - 50% 
		& 0.68 & 97.2 & 1.78 	 

	\\ & & 70	 & 21.25	 & 1.0

		% delta-h-c - 70% 
		& 0.9 & 94.4 & 1.08 	 

		% delta-h-c-uncertainty - 70% 
		& 0.45 & \textbf{97.2} & 3.03 	 

		% delta-h-c-f1 - 70% 
		& 0.9 & 94.4 & 1.08 	 

		% delta-h-c-f1-uncertainty - 70% 
		& 0.57 & \textbf{97.2} & 2.36 	 

		% delta-h-c-f2 - 70% 
		& \textbf{0.92} & 94.4 & \textbf{1.06} 	 

		% delta-h-c-f2-uncertainty - 70% 
		& 0.74 & 94.4 & 1.64 	 

	\\ & & 100	 & 29.25	 & 1.0

		% delta-h-c - 100% 
		& \textbf{0.97} & \textbf{100.0} & \textbf{1.08} 	 

		% delta-h-c-uncertainty - 100% 
		& 0.78 & \textbf{100.0} & 1.61 	 

		% delta-h-c-f1 - 100% 
		& \textbf{0.97} & \textbf{100.0} & \textbf{1.08} 	 

		% delta-h-c-f1-uncertainty - 100% 
		& 0.87 & \textbf{100.0} & 1.36 	 

		% delta-h-c-f2 - 100% 
		& \textbf{0.97} & \textbf{100.0} & \textbf{1.08} 	 

		% delta-h-c-f2-uncertainty - 100% 
		& 0.88 & 94.4 & 1.11 	 
 \\ \hline
\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{rovers}} } & \multirow{5}{*}{6.0} 
	 & 10	 & 2.83	 & 2.39

		% delta-h-c - 10% 
		& 0.46 & 72.2 & \textbf{2.31} 	 

		% delta-h-c-uncertainty - 10% 
		& 0.45 & 75.0 & 2.5 	 

		% delta-h-c-f1 - 10% 
		& \textbf{0.51} & 86.1 & 2.94 	 

		% delta-h-c-f1-uncertainty - 10% 
		& \textbf{0.51} & 86.1 & 2.94 	 

		% delta-h-c-f2 - 10% 
		& 0.46 & \textbf{97.2} & 5.22 	 

		% delta-h-c-f2-uncertainty - 10% 
		& 0.46 & \textbf{97.2} & 5.22 	 

	\\ & & 30	 & 5.75	 & 1.39

		% delta-h-c - 30% 
		& \textbf{0.65} & 91.7 & \textbf{1.56} 	 

		% delta-h-c-uncertainty - 30% 
		& 0.53 & \textbf{94.4} & 2.28 	 

		% delta-h-c-f1 - 30% 
		& \textbf{0.65} & 91.7 & \textbf{1.56} 	 

		% delta-h-c-f1-uncertainty - 30% 
		& 0.58 & 91.7 & 1.89 	 

		% delta-h-c-f2 - 30% 
		& 0.56 & \textbf{94.4} & 2.19 	 

		% delta-h-c-f2-uncertainty - 30% 
		& 0.55 & \textbf{94.4} & 2.25 	 

	\\ & & 50	 & 9.0	 & 1.11

		% delta-h-c - 50% 
		& \textbf{0.87} & \textbf{97.2} & \textbf{1.19} 	 

		% delta-h-c-uncertainty - 50% 
		& 0.77 & \textbf{97.2} & 1.5 	 

		% delta-h-c-f1 - 50% 
		& 0.85 & \textbf{97.2} & 1.22 	 

		% delta-h-c-f1-uncertainty - 50% 
		& 0.8 & \textbf{97.2} & 1.42 	 

		% delta-h-c-f2 - 50% 
		& 0.82 & 94.4 & 1.25 	 

		% delta-h-c-f2-uncertainty - 50% 
		& 0.79 & 94.4 & 1.31 	 

	\\ & & 70	 & 12.42	 & 1.06

		% delta-h-c - 70% 
		& 0.93 & \textbf{100.0} & \textbf{1.11} 	 

		% delta-h-c-uncertainty - 70% 
		& 0.86 & \textbf{100.0} & 1.39 	 

		% delta-h-c-f1 - 70% 
		& \textbf{0.94} & \textbf{100.0} & 1.14 	 

		% delta-h-c-f1-uncertainty - 70% 
		& 0.88 & \textbf{100.0} & 1.33 	 

		% delta-h-c-f2 - 70% 
		& 0.91 & 97.2 & 1.14 	 

		% delta-h-c-f2-uncertainty - 70% 
		& 0.89 & \textbf{100.0} & 1.25 	 

	\\ & & 100	 & 16.92	 & 1.0

		% delta-h-c - 100% 
		& \textbf{0.97} & \textbf{100.0} & 1.06 	 

		% delta-h-c-uncertainty - 100% 
		& 0.96 & \textbf{100.0} & 1.08 	 

		% delta-h-c-f1 - 100% 
		& \textbf{0.97} & \textbf{100.0} & 1.06 	 

		% delta-h-c-f1-uncertainty - 100% 
		& \textbf{0.97} & \textbf{100.0} & 1.06 	 

		% delta-h-c-f2 - 100% 
		& \textbf{0.97} & \textbf{100.0} & 1.06 	 

		% delta-h-c-f2-uncertainty - 100% 
		& 0.89 & 91.7 & \textbf{0.97} 	 
 \\ \hline
\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{satellite}} } & \multirow{5}{*}{6.0} 
	 & 10	 & 3.0	 & 3.25

		% delta-h-c - 10% 
		& 0.49 & 83.3 & \textbf{3.08} 	 

		% delta-h-c-uncertainty - 10% 
		& 0.47 & 86.1 & 3.78 	 

		% delta-h-c-f1 - 10% 
		& 0.5 & 91.7 & 3.89 	 

		% delta-h-c-f1-uncertainty - 10% 
		& 0.5 & 91.7 & 3.89 	 

		% delta-h-c-f2 - 10% 
		& \textbf{0.52} & \textbf{100.0} & 5.14 	 

		% delta-h-c-f2-uncertainty - 10% 
		& \textbf{0.52} & \textbf{100.0} & 5.14 	 

	\\ & & 30	 & 5.33	 & 1.78

		% delta-h-c - 30% 
		& 0.54 & 77.8 & \textbf{2.17} 	 

		% delta-h-c-uncertainty - 30% 
		& 0.47 & 86.1 & 3.69 	 

		% delta-h-c-f1 - 30% 
		& \textbf{0.6} & 91.7 & 2.47 	 

		% delta-h-c-f1-uncertainty - 30% 
		& 0.59 & 94.4 & 2.81 	 

		% delta-h-c-f2 - 30% 
		& 0.51 & \textbf{97.2} & 3.33 	 

		% delta-h-c-f2-uncertainty - 30% 
		& 0.51 & \textbf{97.2} & 3.33 	 

	\\ & & 50	 & 8.75	 & 1.36

		% delta-h-c - 50% 
		& 0.78 & 88.9 & \textbf{1.42} 	 

		% delta-h-c-uncertainty - 50% 
		& 0.56 & 94.4 & 2.69 	 

		% delta-h-c-f1 - 50% 
		& \textbf{0.82} & 94.4 & \textbf{1.42} 	 

		% delta-h-c-f1-uncertainty - 50% 
		& 0.73 & 94.4 & 2.08 	 

		% delta-h-c-f2 - 50% 
		& 0.79 & \textbf{97.2} & 1.58 	 

		% delta-h-c-f2-uncertainty - 50% 
		& 0.76 & \textbf{97.2} & 1.72 	 

	\\ & & 70	 & 11.75	 & 1.33

		% delta-h-c - 70% 
		& 0.86 & 97.2 & 1.47 	 

		% delta-h-c-uncertainty - 70% 
		& 0.64 & \textbf{100.0} & 2.83 	 

		% delta-h-c-f1 - 70% 
		& 0.89 & 97.2 & \textbf{1.39} 	 

		% delta-h-c-f1-uncertainty - 70% 
		& 0.71 & 97.2 & 2.22 	 

		% delta-h-c-f2 - 70% 
		& \textbf{0.91} & \textbf{100.0} & 1.42 	 

		% delta-h-c-f2-uncertainty - 70% 
		& 0.85 & \textbf{100.0} & 1.64 	 

	\\ & & 100	 & 15.75	 & 1.25

		% delta-h-c - 100% 
		& 0.92 & \textbf{94.4} & 1.19 	 

		% delta-h-c-uncertainty - 100% 
		& 0.88 & \textbf{94.4} & 1.28 	 

		% delta-h-c-f1 - 100% 
		& 0.92 & \textbf{94.4} & 1.19 	 

		% delta-h-c-f1-uncertainty - 100% 
		& 0.89 & 91.7 & 1.17 	 

		% delta-h-c-f2 - 100% 
		& \textbf{0.93} & \textbf{94.4} & 1.17 	 

		% delta-h-c-f2-uncertainty - 100% 
		& 0.88 & 88.9 & \textbf{1.11} 	 
 \\ \hline
\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{sokoban}} } & \multirow{5}{*}{8.7} 
	 & 10	 & 4.33	 & 1.83

		% delta-h-c - 10% 
		& 0.31 & 58.3 & 2.47 	 

		% delta-h-c-uncertainty - 10% 
		& \textbf{0.34} & \textbf{80.6} & 4.81 	 

		% delta-h-c-f1 - 10% 
		& 0.33 & 47.2 & \textbf{1.64} 	 

		% delta-h-c-f1-uncertainty - 10% 
		& 0.29 & 58.3 & 2.94 	 

		% delta-h-c-f2 - 10% 
		& 0.3 & 52.8 & 2.22 	 

		% delta-h-c-f2-uncertainty - 10% 
		& 0.31 & 55.6 & 2.44 	 

	\\ & & 30	 & 11.0	 & 1.28

		% delta-h-c - 30% 
		& 0.48 & 75.0 & 2.81 	 

		% delta-h-c-uncertainty - 30% 
		& 0.29 & \textbf{97.2} & 5.36 	 

		% delta-h-c-f1 - 30% 
		& 0.53 & 72.2 & 1.94 	 

		% delta-h-c-f1-uncertainty - 30% 
		& 0.35 & \textbf{97.2} & 4.89 	 

		% delta-h-c-f2 - 30% 
		& \textbf{0.61} & 80.6 & \textbf{1.56} 	 

		% delta-h-c-f2-uncertainty - 30% 
		& 0.48 & 94.4 & 3.47 	 

	\\ & & 50	 & 17.08	 & 1.33

		% delta-h-c - 50% 
		& 0.5 & \textbf{94.4} & 4.22 	 

		% delta-h-c-uncertainty - 50% 
		& 0.32 & \textbf{94.4} & 5.89 	 

		% delta-h-c-f1 - 50% 
		& 0.61 & 88.9 & 2.67 	 

		% delta-h-c-f1-uncertainty - 50% 
		& 0.37 & 91.7 & 4.75 	 

		% delta-h-c-f2 - 50% 
		& \textbf{0.71} & 86.1 & \textbf{1.39} 	 

		% delta-h-c-f2-uncertainty - 50% 
		& 0.45 & \textbf{94.4} & 3.78 	 

	\\ & & 70	 & 23.58	 & 1.36

		% delta-h-c - 70% 
		& 0.54 & \textbf{100.0} & 4.44 	 

		% delta-h-c-uncertainty - 70% 
		& 0.36 & \textbf{100.0} & 5.92 	 

		% delta-h-c-f1 - 70% 
		& 0.68 & 97.2 & 3.08 	 

		% delta-h-c-f1-uncertainty - 70% 
		& 0.49 & \textbf{100.0} & 4.47 	 

		% delta-h-c-f2 - 70% 
		& \textbf{0.72} & 94.4 & \textbf{2.28} 	 

		% delta-h-c-f2-uncertainty - 70% 
		& 0.58 & \textbf{100.0} & 3.72 	 

	\\ & & 100	 & 32.67	 & 1.33

		% delta-h-c - 100% 
		& 0.35 & 94.4 & 5.97 	 

		% delta-h-c-uncertainty - 100% 
		& 0.34 & \textbf{97.2} & 6.56 	 

		% delta-h-c-f1 - 100% 
		& 0.42 & 94.4 & 5.19 	 

		% delta-h-c-f1-uncertainty - 100% 
		& 0.44 & \textbf{97.2} & 5.81 	 

		% delta-h-c-f2 - 100% 
		& 0.62 & 91.7 & \textbf{2.89} 	 

		% delta-h-c-f2-uncertainty - 100% 
		& \textbf{0.64} & 91.7 & 3.36 	 
 \\ \hline
Avg & & & &  & 0.7 & 89.84 & 2.1 & 0.58 & 95.06 & 3.53 & \textbf{0.72} & 91.78 & \textbf{2.04} & 0.63 & 94.6 & 2.83 & \textbf{0.72} & 94.15 & 2.56 & 0.66 & \textbf{95.14} & 2.93
\\ \hline
\end{tabular}

==> tables/previous-all.tex <==
\begin{tabular}{cc|ccc|ccc||cccc|cccc}
\toprule
 \multicolumn{2}{c}{}  & \multicolumn{6}{c}{No Noise} & \multicolumn{8}{c}{Noisy}\\
\cmidrule(lr){3-8}\cmidrule(lr){9-16}
 \multicolumn{2}{c}{}  & \multicolumn{3}{c}{Optimal} & \multicolumn{3}{c}{Suboptimal} & \multicolumn{4}{c}{Optimal} & \multicolumn{4}{c}{Suboptimal}\\
\cmidrule(lr){3-5}\cmidrule(lr){6-8}\cmidrule(lr){9-12}\cmidrule(lr){13-16}
\# & \% & \hdeltahc & \rg & \completion & \hdeltahc & \rg & \completion%
& \hdeltahc & \hdeltahcf & \rg & \completion & \hdeltahc & \hdeltahcf & \rg & \completion\\
\midrule
\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{blocks}}}%
 & 10 & 0.44 & \textbf{0.47} & 0.06 & 0.41 & \textbf{0.46} & 0.06 & \textbf{0.32} & \textbf{0.32} & 0.31 & 0.06 & 0.38 & 0.38 & \textbf{0.42} & 0.05\\ & 30 & \textbf{0.46} & 0.45 & 0.21 & 0.49 & \textbf{0.54} & 0.28 & 0.37 & 0.37 & \textbf{0.39} & 0.13 & 0.36 & 0.37 & \textbf{0.49} & 0.22\\ & 50 & 0.59 & \textbf{0.62} & 0.33 & 0.55 & \textbf{0.62} & 0.39 & \textbf{0.64} & \textbf{0.64} & 0.6 & 0.37 & 0.53 & 0.53 & \textbf{0.55} & 0.28\\ & 70 & \textbf{0.85} & 0.81 & 0.51 & \textbf{0.71} & 0.68 & 0.51 & 0.79 & \textbf{0.81} & 0.77 & 0.47 & \textbf{0.67} & \textbf{0.67} & 0.63 & 0.38\\ & 100 & \textbf{0.92} & 0.9 & 0.59 & \textbf{0.84} & 0.8 & 0.51 & 0.88 & 0.88 & \textbf{0.89} & 0.57 & 0.78 & \textbf{0.82} & 0.74 & 0.51\\\hline\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{dwr}}}%
 & 10 & \textbf{0.79} & 0.67 & 0.45 & \textbf{0.75} & 0.66 & 0.46 & \textbf{0.41} & \textbf{0.41} & 0.19 & 0.28 & \textbf{0.39} & \textbf{0.39} & 0.23 & 0.33\\ & 30 & \textbf{0.8} & 0.58 & 0.55 & \textbf{0.71} & 0.64 & 0.66 & 0.57 & \textbf{0.6} & 0.28 & 0.46 & 0.55 & 0.55 & 0.09 & \textbf{0.56}\\ & 50 & \textbf{0.91} & 0.71 & 0.76 & \textbf{0.84} & 0.68 & 0.76 & \textbf{0.63} & \textbf{0.63} & 0.1 & 0.58 & 0.63 & 0.63 & 0.11 & \textbf{0.75}\\ & 70 & \textbf{0.9} & 0.75 & 0.84 & 0.88 & 0.72 & \textbf{0.89} & \textbf{0.81} & \textbf{0.81} & 0.15 & 0.73 & \textbf{0.78} & \textbf{0.78} & 0.1 & 0.69\\ & 100 & 0.92 & 0.86 & \textbf{0.96} & 0.92 & 0.86 & \textbf{0.96} & 0.86 & \textbf{0.89} & 0.04 & 0.79 & 0.86 & \textbf{0.9} & 0.03 & 0.88\\\hline\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{ipc-grid}}}%
 & 10 & 0.87 & \textbf{0.91} & 0.47 & 0.77 & \textbf{0.81} & 0.64 & \textbf{0.57} & \textbf{0.57} & 0.16 & 0.38 & \textbf{0.62} & \textbf{0.62} & 0.12 & 0.54\\ & 30 & 0.93 & \textbf{0.99} & 0.85 & 0.82 & \textbf{0.9} & 0.81 & \textbf{0.85} & \textbf{0.85} & 0.28 & 0.71 & 0.68 & 0.68 & 0.08 & \textbf{0.72}\\ & 50 & 0.96 & \textbf{1.0} & 0.86 & 0.84 & \textbf{0.92} & 0.87 & \textbf{0.89} & \textbf{0.89} & 0.07 & 0.81 & 0.84 & 0.84 & 0.04 & \textbf{0.85}\\ & 70 & 0.97 & \textbf{1.0} & 0.97 & 0.89 & \textbf{0.93} & 0.92 & \textbf{0.95} & \textbf{0.95} & 0.15 & 0.93 & 0.89 & 0.89 & 0.02 & \textbf{0.9}\\ & 100 & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{0.94} & \textbf{0.94} & \textbf{0.94} & \textbf{1.0} & \textbf{1.0} & 0.08 & 0.99 & \textbf{0.94} & \textbf{0.94} & 0.04 & 0.92\\\hline\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{ferry}}}%
 & 10 & \textbf{0.88} & \textbf{0.88} & 0.48 & \textbf{0.71} & \textbf{0.71} & 0.51 & \textbf{0.43} & \textbf{0.43} & 0.32 & 0.2 & \textbf{0.35} & \textbf{0.35} & 0.31 & 0.26\\ & 30 & \textbf{0.9} & 0.88 & 0.72 & \textbf{0.88} & 0.8 & 0.77 & \textbf{0.46} & \textbf{0.46} & 0.41 & 0.44 & \textbf{0.47} & \textbf{0.47} & \textbf{0.47} & 0.44\\ & 50 & \textbf{0.98} & 0.9 & 0.89 & \textbf{0.88} & 0.8 & 0.81 & 0.74 & \textbf{0.77} & 0.65 & 0.69 & \textbf{0.75} & \textbf{0.75} & 0.66 & 0.69\\ & 70 & \textbf{0.99} & 0.93 & 0.96 & \textbf{0.96} & 0.92 & 0.9 & 0.9 & \textbf{0.92} & 0.77 & 0.9 & 0.81 & \textbf{0.83} & 0.7 & 0.78\\ & 100 & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{0.96} & \textbf{0.96} & \textbf{0.96} & 0.92 & \textbf{0.95} & 0.75 & 0.94 & 0.85 & \textbf{0.95} & 0.71 & 0.82\\\hline\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{logistics}}}%
 & 10 & \textbf{0.9} & 0.87 & 0.43 & \textbf{0.88} & 0.72 & 0.56 & \textbf{0.58} & \textbf{0.58} & 0.13 & 0.41 & \textbf{0.55} & \textbf{0.55} & 0.28 & 0.41\\ & 30 & \textbf{0.92} & 0.86 & 0.78 & \textbf{0.91} & 0.87 & 0.85 & \textbf{0.82} & \textbf{0.82} & 0.06 & 0.78 & 0.8 & \textbf{0.82} & 0.12 & 0.81\\ & 50 & \textbf{0.96} & 0.93 & 0.9 & 0.88 & 0.91 & \textbf{0.93} & \textbf{0.9} & \textbf{0.9} & 0.03 & 0.89 & \textbf{0.91} & \textbf{0.91} & 0.03 & 0.9\\ & 70 & 0.99 & 0.99 & \textbf{1.0} & 0.97 & \textbf{0.99} & \textbf{0.99} & \textbf{0.97} & \textbf{0.97} & 0.03 & 0.94 & 0.96 & 0.97 & 0.0 & \textbf{0.99}\\ & 100 & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & 0.03 & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & 0.0 & \textbf{1.0}\\\hline\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{miconic}}}%
 & 10 & \textbf{0.89} & 0.76 & 0.39 & \textbf{0.76} & 0.65 & 0.54 & 0.39 & 0.39 & \textbf{0.46} & 0.27 & 0.43 & 0.43 & \textbf{0.47} & 0.35\\ & 30 & \textbf{0.95} & 0.65 & 0.83 & \textbf{0.89} & 0.66 & 0.86 & 0.57 & \textbf{0.65} & 0.55 & 0.57 & 0.75 & \textbf{0.78} & 0.64 & 0.69\\ & 50 & \textbf{0.97} & 0.84 & 0.92 & \textbf{0.98} & 0.91 & 0.97 & 0.93 & \textbf{0.94} & 0.87 & 0.9 & 0.86 & 0.89 & 0.87 & \textbf{0.93}\\ & 70 & 0.98 & 0.91 & \textbf{0.99} & 0.99 & 0.94 & \textbf{1.0} & 0.94 & \textbf{0.96} & 0.93 & \textbf{0.96} & 0.9 & 0.93 & \textbf{0.98} & 0.94\\ & 100 & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & 0.94 & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & 0.97 & \textbf{1.0} & \textbf{1.0} & \textbf{1.0}\\\hline\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{rovers}}}%
 & 10 & \textbf{0.83} & 0.76 & 0.49 & \textbf{0.83} & 0.82 & 0.45 & \textbf{0.44} & \textbf{0.44} & 0.18 & 0.31 & \textbf{0.46} & \textbf{0.46} & 0.37 & 0.44\\ & 30 & \textbf{0.94} & 0.88 & 0.76 & \textbf{0.88} & 0.8 & 0.7 & 0.7 & 0.7 & 0.45 & \textbf{0.75} & 0.65 & \textbf{0.66} & 0.4 & 0.51\\ & 50 & \textbf{0.92} & 0.91 & 0.79 & \textbf{0.93} & 0.89 & 0.8 & 0.8 & \textbf{0.82} & 0.31 & 0.71 & \textbf{0.87} & 0.85 & 0.49 & 0.72\\ & 70 & \textbf{0.99} & 0.97 & 0.93 & 0.94 & \textbf{0.98} & 0.87 & \textbf{0.93} & 0.89 & 0.49 & 0.88 & \textbf{0.93} & 0.92 & 0.26 & 0.89\\ & 100 & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{0.97} & 0.93 & 0.39 & \textbf{0.97} & \textbf{0.97} & 0.93 & 0.34 & 0.9\\\hline\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{satellite}}}%
 & 10 & 0.85 & \textbf{0.86} & 0.5 & \textbf{0.9} & 0.73 & 0.58 & \textbf{0.53} & \textbf{0.53} & 0.41 & 0.34 & \textbf{0.49} & \textbf{0.49} & 0.41 & 0.29\\ & 30 & \textbf{0.86} & 0.72 & 0.64 & \textbf{0.8} & 0.68 & 0.6 & \textbf{0.5} & 0.48 & 0.4 & 0.41 & 0.54 & \textbf{0.6} & 0.54 & 0.51\\ & 50 & \textbf{0.93} & 0.79 & 0.73 & \textbf{0.92} & 0.7 & 0.76 & 0.67 & \textbf{0.69} & 0.42 & 0.49 & 0.78 & \textbf{0.81} & 0.61 & 0.66\\ & 70 & \textbf{0.94} & 0.81 & 0.89 & \textbf{0.94} & 0.78 & 0.85 & \textbf{0.87} & \textbf{0.87} & 0.67 & 0.81 & 0.86 & \textbf{0.91} & 0.63 & 0.78\\ & 100 & \textbf{0.96} & 0.88 & 0.88 & \textbf{0.96} & 0.88 & 0.88 & 0.92 & \textbf{0.94} & 0.69 & 0.88 & 0.92 & \textbf{0.94} & 0.47 & 0.92\\\hline\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{sokoban}}}%
 & 10 & 0.39 & \textbf{0.4} & 0.28 & \textbf{0.52} & 0.29 & 0.35 & \textbf{0.27} & \textbf{0.27} & 0.1 & 0.24 & 0.31 & \textbf{0.32} & 0.13 & 0.25\\ & 30 & \textbf{0.75} & 0.56 & 0.57 & \textbf{0.77} & 0.43 & 0.56 & 0.56 & \textbf{0.7} & 0.2 & 0.34 & 0.48 & \textbf{0.56} & 0.12 & 0.29\\ & 50 & \textbf{0.92} & 0.61 & 0.61 & \textbf{0.79} & 0.53 & 0.58 & 0.61 & \textbf{0.82} & 0.2 & 0.57 & 0.5 & \textbf{0.73} & 0.01 & 0.46\\ & 70 & \textbf{0.99} & 0.64 & 0.85 & \textbf{0.8} & 0.54 & 0.63 & 0.6 & \textbf{0.97} & 0.08 & 0.84 & 0.54 & \textbf{0.8} & 0.06 & 0.58\\ & 100 & \textbf{1.0} & 0.67 & \textbf{1.0} & \textbf{0.83} & 0.58 & \textbf{0.83} & 0.66 & \textbf{1.0} & 0.04 & 0.96 & 0.35 & \textbf{0.85} & 0.04 & 0.77\\\hline
Avg &  & \textbf{0.89} & 0.81 & 0.72 & \textbf{0.84} & 0.77 & 0.73 & 0.71 & \textbf{0.74} & 0.37 & 0.64 & 0.69 & \textbf{0.72} & 0.35 & 0.63\\
\bottomrule
\end{tabular}\\

==> tables/previous-noisy-1.tex <==
\begin{tabular}[t]{cc|ccc|ccc|ccc|ccc||ccc|ccc|ccc|ccc}
\toprule
\multicolumn{26}{c}{\begin{tabular}[c]{@{}c@{}} Noisy Data sets \end{tabular}}	\\ 
\hline
 \multicolumn{2}{c}{} & \multicolumn{12}{c}{Optimal} & \multicolumn{12}{c}{Sub-Optimal}\\
\cmidrule(lr){3-14}\cmidrule(lr){15-26}
%
 \multicolumn{2}{c}{} & \multicolumn{3}{c}{\dhc} & \multicolumn{3}{c}{\dhcf} & \multicolumn{3}{c}{\rg} & \multicolumn{3}{c}{\pom}%
  & \multicolumn{3}{c}{\dhc} & \multicolumn{3}{c}{\dhcf} & \multicolumn{3}{c}{\rg} & \multicolumn{3}{c}{\pom}\\%
%
\cmidrule(lr){3-5}\cmidrule(lr){6-8}\cmidrule(lr){9-11}\cmidrule(lr){12-14}\cmidrule(lr){15-17}\cmidrule(lr){18-20}\cmidrule(lr){21-23}%
 \cmidrule(lr){24-26}\\
%
\# & \% & AGR & ACC & SPR & AGR & ACC & SPR & AGR & ACC & SPR & AGR & ACC & SPR & AGR & ACC & SPR & AGR & ACC & SPR & AGR & ACC & SPR%
 & AGR & ACC & SPR\\
\midrule
\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{blocks}}}%
 & 10 & \textbf{0.32} & 0.67 & 6.67 & \textbf{0.32} & 0.67 & 6.67 & 0.31 & 0.67 & 7.11 & 0.06 & 0.08 & 1.25 & 0.38 & 0.69 & 6.58 & 0.38 & 0.69 & 6.58 & \textbf{0.42} & 0.89 & 8.97 & 0.05 & 0.06 & 1.28\\ & 30 & 0.37 & 0.75 & 3.44 & 0.37 & 0.75 & 3.44 & \textbf{0.39} & 0.92 & 6.28 & 0.13 & 0.28 & 1.25 & 0.36 & 0.64 & 3.47 & 0.37 & 0.67 & 3.5 & \textbf{0.49} & 0.92 & 5.47 & 0.22 & 0.47 & 1.22\\ & 50 & \textbf{0.64} & 0.83 & 2.17 & \textbf{0.64} & 0.83 & 2.17 & 0.6 & 0.89 & 3.19 & 0.37 & 0.56 & 1.19 & 0.53 & 0.83 & 2.64 & 0.53 & 0.83 & 2.67 & \textbf{0.55} & 0.94 & 2.72 & 0.28 & 0.58 & 1.25\\ & 70 & 0.79 & 0.92 & 1.67 & \textbf{0.81} & 0.94 & 1.78 & 0.77 & 0.94 & 2.14 & 0.47 & 0.67 & 1.22 & \textbf{0.67} & 0.89 & 2.22 & \textbf{0.67} & 0.89 & 2.22 & 0.63 & 0.86 & 2.47 & 0.38 & 0.72 & 1.19\\ & 100 & 0.88 & 0.94 & 1.58 & 0.88 & 0.97 & 1.61 & \textbf{0.89} & 0.97 & 2.03 & 0.57 & 1.0 & 1.81 & 0.78 & 0.92 & 1.53 & \textbf{0.82} & 0.97 & 1.64 & 0.74 & 0.92 & 1.97 & 0.51 & 1.0 & 1.72\\\hline\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{depots}}}%
 & 10 & \textbf{0.39} & 0.69 & 3.89 & \textbf{0.39} & 0.69 & 3.89 & 0.0 & 0.03 & 0.28 & 0.14 & 0.22 & 1.69 & \textbf{0.43} & 0.72 & 2.81 & \textbf{0.43} & 0.72 & 2.81 & 0.02 & 0.06 & 0.22 & 0.17 & 0.22 & 1.83\\ & 30 & \textbf{0.35} & 0.78 & 2.78 & \textbf{0.35} & 0.78 & 2.78 & 0.04 & 0.14 & 0.58 & 0.22 & 0.31 & 1.19 & 0.41 & 0.61 & 1.94 & \textbf{0.43} & 0.64 & 2.08 & 0.07 & 0.14 & 0.5 & 0.21 & 0.36 & 1.61\\ & 50 & \textbf{0.62} & 0.78 & 1.53 & \textbf{0.62} & 0.78 & 1.53 & 0.04 & 0.08 & 0.25 & 0.43 & 0.5 & 1.28 & \textbf{0.76} & 0.89 & 1.33 & \textbf{0.76} & 0.89 & 1.33 & 0.01 & 0.03 & 0.14 & 0.51 & 0.64 & 1.33\\ & 70 & \textbf{0.91} & 0.97 & 1.19 & \textbf{0.91} & 0.97 & 1.19 & 0.01 & 0.03 & 0.06 & 0.62 & 0.72 & 1.25 & 0.71 & 0.83 & 1.33 & \textbf{0.78} & 0.92 & 1.33 & 0.0 & 0.0 & 0.03 & 0.54 & 0.69 & 1.44\\ & 100 & \textbf{1.0} & 1.0 & 1.0 & \textbf{1.0} & 1.0 & 1.0 & 0.0 & 0.0 & 0.0 & 0.88 & 0.94 & 1.14 & 0.94 & 0.97 & 1.11 & \textbf{1.0} & 1.0 & 1.0 & 0.01 & 0.03 & 0.11 & 0.83 & 0.92 & 1.19\\\hline\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{driverlog}}}%
 & 10 & \textbf{0.33} & 0.58 & 2.56 & \textbf{0.33} & 0.58 & 2.56 & 0.24 & 0.56 & 2.75 & 0.2 & 0.33 & 1.25 & \textbf{0.34} & 0.64 & 2.31 & \textbf{0.34} & 0.64 & 2.31 & 0.21 & 0.56 & 3.33 & 0.23 & 0.47 & 1.47\\ & 30 & \textbf{0.64} & 0.83 & 1.67 & 0.63 & 0.86 & 1.86 & 0.21 & 0.53 & 2.31 & 0.44 & 0.61 & 1.39 & 0.65 & 0.83 & 1.58 & \textbf{0.66} & 0.83 & 1.56 & 0.28 & 0.53 & 1.72 & 0.45 & 0.67 & 1.39\\ & 50 & 0.73 & 0.94 & 1.5 & \textbf{0.75} & 0.94 & 1.44 & 0.2 & 0.47 & 1.64 & 0.53 & 0.64 & 1.28 & 0.68 & 0.81 & 1.42 & \textbf{0.69} & 0.86 & 1.53 & 0.12 & 0.33 & 1.11 & 0.54 & 0.83 & 1.75\\ & 70 & 0.78 & 0.92 & 1.44 & \textbf{0.83} & 0.97 & 1.47 & 0.25 & 0.42 & 1.08 & 0.59 & 0.78 & 1.56 & \textbf{0.85} & 0.92 & 1.25 & 0.83 & 0.92 & 1.31 & 0.22 & 0.31 & 0.64 & 0.64 & 0.94 & 1.61\\ & 100 & 0.92 & 1.0 & 1.25 & \textbf{0.93} & 0.97 & 1.17 & 0.23 & 0.39 & 0.86 & 0.7 & 1.0 & 1.67 & 0.78 & 0.83 & 1.22 & \textbf{0.88} & 0.97 & 1.28 & 0.19 & 0.31 & 0.67 & 0.58 & 1.0 & 2.06\\\hline\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{dwr}}}%
 & 10 & \textbf{0.41} & 0.81 & 2.81 & \textbf{0.41} & 0.81 & 2.75 & 0.19 & 0.44 & 2.08 & 0.28 & 0.44 & 1.33 & \textbf{0.39} & 0.81 & 3.36 & \textbf{0.39} & 0.81 & 3.36 & 0.23 & 0.5 & 1.94 & 0.33 & 0.47 & 1.31\\ & 30 & 0.57 & 0.92 & 2.11 & \textbf{0.6} & 0.94 & 2.25 & 0.28 & 0.47 & 1.39 & 0.46 & 0.61 & 1.19 & 0.55 & 0.83 & 2.14 & 0.55 & 0.83 & 2.14 & 0.09 & 0.14 & 0.64 & \textbf{0.56} & 0.69 & 1.17\\ & 50 & \textbf{0.63} & 0.92 & 1.64 & \textbf{0.63} & 0.92 & 1.64 & 0.1 & 0.17 & 0.28 & 0.58 & 0.75 & 1.14 & 0.63 & 0.89 & 1.47 & 0.63 & 0.89 & 1.5 & 0.11 & 0.17 & 0.39 & \textbf{0.75} & 0.97 & 1.11\\ & 70 & \textbf{0.81} & 1.0 & 1.28 & \textbf{0.81} & 1.0 & 1.28 & 0.15 & 0.17 & 0.25 & 0.73 & 0.83 & 1.17 & \textbf{0.78} & 0.92 & 1.22 & \textbf{0.78} & 0.92 & 1.22 & 0.1 & 0.11 & 0.14 & 0.69 & 0.75 & 1.08\\ & 100 & 0.86 & 1.0 & 1.19 & \textbf{0.89} & 1.0 & 1.14 & 0.04 & 0.06 & 0.08 & 0.79 & 0.83 & 1.0 & 0.86 & 0.97 & 1.14 & \textbf{0.9} & 1.0 & 1.11 & 0.03 & 0.03 & 0.03 & 0.88 & 0.92 & 1.03\\\hline
 \textsc{f}%
 & AVG & 0.69 & 0.92 & 2.13 & \textbf{0.71} & 0.93 & 2.11 & 0.58 & 0.78 & 1.74 & 0.64 & 0.72 & 1.23 & 0.65 & 0.87 & 2.06 & \textbf{0.67} & 0.88 & 2.02 & 0.57 & 0.76 & 1.67 & 0.6 & 0.73 & 1.28\\\hline%
\textsc{l}%
 & AVG & \textbf{0.85} & 0.97 & 1.43 & \textbf{0.85} & 0.97 & 1.43 & 0.05 & 0.07 & 0.21 & 0.81 & 0.91 & 1.32 & 0.84 & 0.98 & 1.39 & \textbf{0.85} & 0.98 & 1.38 & 0.09 & 0.13 & 0.32 & 0.82 & 0.88 & 1.11\\\hline%
\end{tabular}

==> tables/previous-noisy-2.tex <==
\begin{tabular}[t]{cc|ccc|ccc|ccc|ccc||ccc|ccc|ccc|ccc}
\toprule
\multicolumn{26}{c}{\begin{tabular}[c]{@{}c@{}} Noisy Data sets \end{tabular}}	\\ 
\hline
 \multicolumn{2}{c}{} & \multicolumn{12}{c}{Optimal} & \multicolumn{12}{c}{Sub-Optimal}\\
\cmidrule(lr){3-14}\cmidrule(lr){15-26}
%
 \multicolumn{2}{c}{} & \multicolumn{3}{c}{\dhc} & \multicolumn{3}{c}{\dhcf} & \multicolumn{3}{c}{\rg} & \multicolumn{3}{c}{\pom}%
  & \multicolumn{3}{c}{\dhc} & \multicolumn{3}{c}{\dhcf} & \multicolumn{3}{c}{\rg} & \multicolumn{3}{c}{\pom}\\%
%
\cmidrule(lr){3-5}\cmidrule(lr){6-8}\cmidrule(lr){9-11}\cmidrule(lr){12-14}\cmidrule(lr){15-17}\cmidrule(lr){18-20}\cmidrule(lr){21-23}%
 \cmidrule(lr){24-26}\\
%
\# & \% & AGR & ACC & SPR & AGR & ACC & SPR & AGR & ACC & SPR & AGR & ACC & SPR & AGR & ACC & SPR & AGR & ACC & SPR & AGR & ACC & SPR%
 & AGR & ACC & SPR\\
\midrule
\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{ipc-grid}}}%
 & 10 & \textbf{0.57} & 0.92 & 1.5 & \textbf{0.57} & 0.92 & 1.5 & 0.16 & 0.23 & 0.71 & 0.38 & 0.67 & 1.71 & \textbf{0.62} & 0.9 & 2.1 & \textbf{0.62} & 0.9 & 2.1 & 0.12 & 0.19 & 0.44 & 0.54 & 0.71 & 1.58\\ & 30 & \textbf{0.85} & 0.92 & 1.17 & \textbf{0.85} & 0.94 & 1.17 & 0.28 & 0.29 & 0.33 & 0.71 & 0.85 & 1.67 & 0.68 & 0.9 & 1.44 & 0.68 & 0.9 & 1.44 & 0.08 & 0.15 & 0.29 & \textbf{0.72} & 0.88 & 1.25\\ & 50 & \textbf{0.89} & 0.96 & 1.15 & \textbf{0.89} & 0.96 & 1.15 & 0.07 & 0.1 & 0.15 & 0.81 & 0.9 & 1.15 & 0.84 & 0.96 & 1.06 & 0.84 & 0.98 & 1.1 & 0.04 & 0.04 & 0.04 & \textbf{0.85} & 0.96 & 1.04\\ & 70 & \textbf{0.95} & 1.0 & 1.15 & \textbf{0.95} & 1.0 & 1.15 & 0.15 & 0.15 & 0.15 & 0.93 & 1.0 & 1.15 & 0.89 & 1.0 & 1.06 & 0.89 & 1.0 & 1.06 & 0.02 & 0.02 & 0.02 & \textbf{0.9} & 0.98 & 1.0\\ & 100 & \textbf{1.0} & 1.0 & 1.0 & \textbf{1.0} & 1.0 & 1.0 & 0.08 & 0.08 & 0.08 & 0.99 & 1.0 & 1.02 & \textbf{0.94} & 1.0 & 1.0 & \textbf{0.94} & 1.0 & 1.0 & 0.04 & 0.04 & 0.04 & 0.92 & 1.0 & 1.04\\\hline
\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{satellite}}}%
 & 10 & \textbf{0.53} & 0.75 & 3.31 & \textbf{0.53} & 0.75 & 3.31 & 0.41 & 0.58 & 2.94 & 0.34 & 0.5 & 2.28 & \textbf{0.49} & 0.83 & 3.08 & \textbf{0.49} & 0.83 & 3.08 & 0.41 & 0.67 & 3.11 & 0.29 & 0.53 & 2.36\\ & 30 & \textbf{0.5} & 0.78 & 2.33 & 0.48 & 0.78 & 2.47 & 0.4 & 0.81 & 2.78 & 0.41 & 0.69 & 1.75 & 0.54 & 0.78 & 2.17 & \textbf{0.6} & 0.92 & 2.47 & 0.54 & 0.89 & 3.0 & 0.51 & 0.78 & 1.92\\ & 50 & 0.67 & 0.89 & 1.89 & \textbf{0.69} & 0.92 & 1.89 & 0.42 & 0.75 & 2.5 & 0.49 & 0.72 & 1.5 & 0.78 & 0.89 & 1.42 & \textbf{0.81} & 0.94 & 1.47 & 0.61 & 0.92 & 2.19 & 0.66 & 0.92 & 1.33\\ & 70 & \textbf{0.87} & 0.94 & 1.31 & \textbf{0.87} & 0.94 & 1.31 & 0.67 & 0.78 & 1.47 & 0.81 & 0.94 & 1.17 & 0.86 & 0.97 & 1.47 & \textbf{0.91} & 1.0 & 1.42 & 0.63 & 0.78 & 1.67 & 0.78 & 0.94 & 1.42\\ & 100 & 0.92 & 0.97 & 1.31 & \textbf{0.94} & 0.97 & 1.14 & 0.69 & 0.78 & 1.31 & 0.88 & 1.0 & 1.22 & 0.92 & 0.94 & 1.19 & \textbf{0.94} & 0.94 & 1.14 & 0.47 & 0.56 & 1.0 & 0.92 & 1.0 & 1.25\\\hline\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{sokoban}}}%
 & 10 & \textbf{0.27} & 0.58 & 2.78 & \textbf{0.27} & 0.58 & 2.78 & 0.1 & 0.31 & 1.83 & 0.24 & 0.42 & 1.42 & 0.31 & 0.58 & 2.47 & \textbf{0.32} & 0.56 & 2.06 & 0.13 & 0.36 & 2.39 & 0.25 & 0.44 & 1.67\\ & 30 & 0.56 & 0.78 & 2.17 & \textbf{0.7} & 0.83 & 1.44 & 0.2 & 0.31 & 1.0 & 0.34 & 0.42 & 1.28 & 0.48 & 0.75 & 2.81 & \textbf{0.56} & 0.78 & 1.89 & 0.12 & 0.19 & 0.75 & 0.29 & 0.42 & 1.28\\ & 50 & 0.61 & 0.94 & 2.97 & \textbf{0.82} & 0.97 & 1.19 & 0.2 & 0.31 & 0.75 & 0.57 & 0.67 & 1.28 & 0.5 & 0.94 & 4.22 & \textbf{0.73} & 0.86 & 1.17 & 0.01 & 0.03 & 0.06 & 0.46 & 0.56 & 1.22\\ & 70 & 0.6 & 0.94 & 3.75 & \textbf{0.97} & 1.0 & 1.06 & 0.08 & 0.11 & 0.19 & 0.84 & 0.94 & 1.28 & 0.54 & 1.0 & 4.44 & \textbf{0.8} & 0.94 & 1.03 & 0.06 & 0.08 & 0.11 & 0.58 & 0.78 & 1.28\\ & 100 & 0.66 & 1.0 & 3.89 & \textbf{1.0} & 1.0 & 1.0 & 0.04 & 0.06 & 0.08 & 0.96 & 1.0 & 1.08 & 0.35 & 0.94 & 5.97 & \textbf{0.85} & 0.97 & 1.03 & 0.04 & 0.06 & 0.06 & 0.77 & 1.0 & 1.14\\\hline\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{zeno}}}%
 & 10 & 0.44 & 0.64 & 2.33 & 0.44 & 0.64 & 2.33 & \textbf{0.45} & 0.78 & 3.0 & 0.24 & 0.47 & 1.44 & 0.37 & 0.72 & 1.94 & 0.37 & 0.72 & 1.94 & \textbf{0.45} & 0.94 & 3.11 & 0.31 & 0.42 & 1.33\\ & 30 & 0.5 & 0.86 & 1.64 & \textbf{0.54} & 0.89 & 1.53 & 0.44 & 0.94 & 2.31 & 0.49 & 0.67 & 1.44 & 0.6 & 0.69 & 1.31 & \textbf{0.72} & 0.86 & 1.36 & 0.61 & 0.89 & 1.83 & 0.57 & 0.69 & 1.44\\ & 50 & \textbf{0.89} & 0.94 & 1.08 & 0.86 & 0.92 & 1.08 & 0.71 & 0.89 & 1.64 & 0.63 & 0.75 & 1.39 & \textbf{0.76} & 0.89 & 1.39 & 0.73 & 0.86 & 1.39 & 0.75 & 0.89 & 1.67 & 0.73 & 0.81 & 1.22\\ & 70 & 0.84 & 0.94 & 1.22 & \textbf{0.88} & 0.97 & 1.19 & 0.84 & 0.94 & 1.33 & 0.74 & 0.81 & 1.17 & 0.97 & 1.0 & 1.06 & \textbf{0.99} & 1.0 & 1.03 & 0.82 & 0.89 & 1.25 & 0.89 & 0.92 & 1.06\\ & 100 & 0.97 & 0.97 & 1.0 & \textbf{1.0} & 1.0 & 1.0 & 0.88 & 0.92 & 1.08 & 0.96 & 1.0 & 1.08 & 0.94 & 0.94 & 1.0 & \textbf{1.0} & 1.0 & 1.0 & 0.85 & 0.89 & 1.14 & 0.9 & 1.0 & 1.19\\\hline
 \textsc{m}%
 & AVG & 0.76 & 0.89 & 1.42 & \textbf{0.79} & 0.93 & 1.44 & 0.76 & 0.96 & 1.73 & 0.74 & 0.81 & 1.14 & 0.78 & 0.92 & 1.36 & \textbf{0.81} & 0.93 & 1.33 & 0.79 & 0.97 & 1.7 & 0.78 & 0.88 & 1.21\\\hline%
\textsc{r}%
 & AVG & \textbf{0.77} & 0.91 & 1.48 & 0.76 & 0.91 & 1.52 & 0.36 & 0.48 & 0.82 & 0.72 & 0.8 & 1.13 & \textbf{0.78} & 0.92 & 1.44 & 0.77 & 0.91 & 1.44 & 0.37 & 0.48 & 0.93 & 0.69 & 0.78 & 1.14\\\hline%
\multicolumn{2}{c}{AVG}  & 0.71 & 0.89 & 1.91 & \textbf{0.73} & 0.9 & 1.78 & 0.35 & 0.5 & 1.38 & 0.61 & 0.73 & 1.3 & 0.69 & 0.87 & 1.93 & \textbf{0.72} & 0.89 & 1.72 & 0.34 & 0.48 & 1.34 & 0.61 & 0.76 & 1.31%
\\
\bottomrule
\end{tabular}\\

==> tables/previous-noisy.tex <==
\begin{tabular}{cc|ccc|ccc|ccc|ccc||ccc|ccc|ccc|ccc}
\toprule
 \multicolumn{2}{c}{} & \multicolumn{12}{c}{Optimal} & \multicolumn{12}{c}{Sub-Optimal}\\
\cmidrule(lr){3-14}\cmidrule(lr){15-26}
%
 \multicolumn{2}{c}{} & \multicolumn{3}{c}{\dhc} & \multicolumn{3}{c}{\dhcf} & \multicolumn{3}{c}{\rg} & \multicolumn{3}{c}{\pom}%
  & \multicolumn{3}{c}{\dhc} & \multicolumn{3}{c}{\dhcf} & \multicolumn{3}{c}{\rg} & \multicolumn{3}{c}{\pom}\\%
%
\cmidrule(lr){3-5}\cmidrule(lr){6-8}\cmidrule(lr){9-11}\cmidrule(lr){12-14}\cmidrule(lr){15-17}\cmidrule(lr){18-20}\cmidrule(lr){21-23}%
 \cmidrule(lr){24-26}\\
%
\# & \% & AGR & ACC & SPR & AGR & ACC & SPR & AGR & ACC & SPR & AGR & ACC & SPR & AGR & ACC & SPR & AGR & ACC & SPR & AGR & ACC & SPR%
 & AGR & ACC & SPR\\
\midrule
\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{blocks}}}%
 & 10 & \textbf{0.32} & 0.67 & 6.67 & \textbf{0.32} & 0.67 & 6.67 & 0.31 & 0.67 & 7.11 & 0.06 & 0.08 & 1.25 & 0.38 & 0.69 & 6.58 & 0.38 & 0.69 & 6.58 & \textbf{0.42} & 0.89 & 8.97 & 0.05 & 0.06 & 1.28\\ & 30 & 0.37 & 0.75 & 3.44 & 0.37 & 0.75 & 3.44 & \textbf{0.39} & 0.92 & 6.28 & 0.13 & 0.28 & 1.25 & 0.36 & 0.64 & 3.47 & 0.37 & 0.67 & 3.5 & \textbf{0.49} & 0.92 & 5.47 & 0.22 & 0.47 & 1.22\\ & 50 & \textbf{0.64} & 0.83 & 2.17 & \textbf{0.64} & 0.83 & 2.17 & 0.6 & 0.89 & 3.19 & 0.37 & 0.56 & 1.19 & 0.53 & 0.83 & 2.64 & 0.53 & 0.83 & 2.67 & \textbf{0.55} & 0.94 & 2.72 & 0.28 & 0.58 & 1.25\\ & 70 & 0.79 & 0.92 & 1.67 & \textbf{0.81} & 0.94 & 1.78 & 0.77 & 0.94 & 2.14 & 0.47 & 0.67 & 1.22 & \textbf{0.67} & 0.89 & 2.22 & \textbf{0.67} & 0.89 & 2.22 & 0.63 & 0.86 & 2.47 & 0.38 & 0.72 & 1.19\\ & 100 & 0.88 & 0.94 & 1.58 & 0.88 & 0.97 & 1.61 & \textbf{0.89} & 0.97 & 2.03 & 0.57 & 1.0 & 1.81 & 0.78 & 0.92 & 1.53 & \textbf{0.82} & 0.97 & 1.64 & 0.74 & 0.92 & 1.97 & 0.51 & 1.0 & 1.72\\\hline\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{depots}}}%
 & 10 & \textbf{0.39} & 0.69 & 3.89 & \textbf{0.39} & 0.69 & 3.89 & 0.0 & 0.03 & 0.28 & 0.14 & 0.22 & 1.69 & \textbf{0.43} & 0.72 & 2.81 & \textbf{0.43} & 0.72 & 2.81 & 0.02 & 0.06 & 0.22 & 0.17 & 0.22 & 1.83\\ & 30 & \textbf{0.35} & 0.78 & 2.78 & \textbf{0.35} & 0.78 & 2.78 & 0.04 & 0.14 & 0.58 & 0.22 & 0.31 & 1.19 & 0.41 & 0.61 & 1.94 & \textbf{0.43} & 0.64 & 2.08 & 0.07 & 0.14 & 0.5 & 0.21 & 0.36 & 1.61\\ & 50 & \textbf{0.62} & 0.78 & 1.53 & \textbf{0.62} & 0.78 & 1.53 & 0.04 & 0.08 & 0.25 & 0.43 & 0.5 & 1.28 & \textbf{0.76} & 0.89 & 1.33 & \textbf{0.76} & 0.89 & 1.33 & 0.01 & 0.03 & 0.14 & 0.51 & 0.64 & 1.33\\ & 70 & \textbf{0.91} & 0.97 & 1.19 & \textbf{0.91} & 0.97 & 1.19 & 0.01 & 0.03 & 0.06 & 0.62 & 0.72 & 1.25 & 0.71 & 0.83 & 1.33 & \textbf{0.78} & 0.92 & 1.33 & 0.0 & 0.0 & 0.03 & 0.54 & 0.69 & 1.44\\ & 100 & \textbf{1.0} & 1.0 & 1.0 & \textbf{1.0} & 1.0 & 1.0 & 0.0 & 0.0 & 0.0 & 0.88 & 0.94 & 1.14 & 0.94 & 0.97 & 1.11 & \textbf{1.0} & 1.0 & 1.0 & 0.01 & 0.03 & 0.11 & 0.83 & 0.92 & 1.19\\\hline\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{driverlog}}}%
 & 10 & \textbf{0.33} & 0.58 & 2.56 & \textbf{0.33} & 0.58 & 2.56 & 0.24 & 0.56 & 2.75 & 0.2 & 0.33 & 1.25 & \textbf{0.34} & 0.64 & 2.31 & \textbf{0.34} & 0.64 & 2.31 & 0.21 & 0.56 & 3.33 & 0.23 & 0.47 & 1.47\\ & 30 & \textbf{0.64} & 0.83 & 1.67 & 0.63 & 0.86 & 1.86 & 0.21 & 0.53 & 2.31 & 0.44 & 0.61 & 1.39 & 0.65 & 0.83 & 1.58 & \textbf{0.66} & 0.83 & 1.56 & 0.28 & 0.53 & 1.72 & 0.45 & 0.67 & 1.39\\ & 50 & 0.73 & 0.94 & 1.5 & \textbf{0.75} & 0.94 & 1.44 & 0.2 & 0.47 & 1.64 & 0.53 & 0.64 & 1.28 & 0.68 & 0.81 & 1.42 & \textbf{0.69} & 0.86 & 1.53 & 0.12 & 0.33 & 1.11 & 0.54 & 0.83 & 1.75\\ & 70 & 0.78 & 0.92 & 1.44 & \textbf{0.83} & 0.97 & 1.47 & 0.25 & 0.42 & 1.08 & 0.59 & 0.78 & 1.56 & \textbf{0.85} & 0.92 & 1.25 & 0.83 & 0.92 & 1.31 & 0.22 & 0.31 & 0.64 & 0.64 & 0.94 & 1.61\\ & 100 & 0.92 & 1.0 & 1.25 & \textbf{0.93} & 0.97 & 1.17 & 0.23 & 0.39 & 0.86 & 0.7 & 1.0 & 1.67 & 0.78 & 0.83 & 1.22 & \textbf{0.88} & 0.97 & 1.28 & 0.19 & 0.31 & 0.67 & 0.58 & 1.0 & 2.06\\\hline\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{dwr}}}%
 & 10 & \textbf{0.41} & 0.81 & 2.81 & \textbf{0.41} & 0.81 & 2.75 & 0.19 & 0.44 & 2.08 & 0.28 & 0.44 & 1.33 & \textbf{0.39} & 0.81 & 3.36 & \textbf{0.39} & 0.81 & 3.36 & 0.23 & 0.5 & 1.94 & 0.33 & 0.47 & 1.31\\ & 30 & 0.57 & 0.92 & 2.11 & \textbf{0.6} & 0.94 & 2.25 & 0.28 & 0.47 & 1.39 & 0.46 & 0.61 & 1.19 & 0.55 & 0.83 & 2.14 & 0.55 & 0.83 & 2.14 & 0.09 & 0.14 & 0.64 & \textbf{0.56} & 0.69 & 1.17\\ & 50 & \textbf{0.63} & 0.92 & 1.64 & \textbf{0.63} & 0.92 & 1.64 & 0.1 & 0.17 & 0.28 & 0.58 & 0.75 & 1.14 & 0.63 & 0.89 & 1.47 & 0.63 & 0.89 & 1.5 & 0.11 & 0.17 & 0.39 & \textbf{0.75} & 0.97 & 1.11\\ & 70 & \textbf{0.81} & 1.0 & 1.28 & \textbf{0.81} & 1.0 & 1.28 & 0.15 & 0.17 & 0.25 & 0.73 & 0.83 & 1.17 & \textbf{0.78} & 0.92 & 1.22 & \textbf{0.78} & 0.92 & 1.22 & 0.1 & 0.11 & 0.14 & 0.69 & 0.75 & 1.08\\ & 100 & 0.86 & 1.0 & 1.19 & \textbf{0.89} & 1.0 & 1.14 & 0.04 & 0.06 & 0.08 & 0.79 & 0.83 & 1.0 & 0.86 & 0.97 & 1.14 & \textbf{0.9} & 1.0 & 1.11 & 0.03 & 0.03 & 0.03 & 0.88 & 0.92 & 1.03\\\hline\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{ipc-grid}}}%
 & 10 & \textbf{0.57} & 0.92 & 1.5 & \textbf{0.57} & 0.92 & 1.5 & 0.16 & 0.23 & 0.71 & 0.38 & 0.67 & 1.71 & \textbf{0.62} & 0.9 & 2.1 & \textbf{0.62} & 0.9 & 2.1 & 0.12 & 0.19 & 0.44 & 0.54 & 0.71 & 1.58\\ & 30 & \textbf{0.85} & 0.92 & 1.17 & \textbf{0.85} & 0.94 & 1.17 & 0.28 & 0.29 & 0.33 & 0.71 & 0.85 & 1.67 & 0.68 & 0.9 & 1.44 & 0.68 & 0.9 & 1.44 & 0.08 & 0.15 & 0.29 & \textbf{0.72} & 0.88 & 1.25\\ & 50 & \textbf{0.89} & 0.96 & 1.15 & \textbf{0.89} & 0.96 & 1.15 & 0.07 & 0.1 & 0.15 & 0.81 & 0.9 & 1.15 & 0.84 & 0.96 & 1.06 & 0.84 & 0.98 & 1.1 & 0.04 & 0.04 & 0.04 & \textbf{0.85} & 0.96 & 1.04\\ & 70 & \textbf{0.95} & 1.0 & 1.15 & \textbf{0.95} & 1.0 & 1.15 & 0.15 & 0.15 & 0.15 & 0.93 & 1.0 & 1.15 & 0.89 & 1.0 & 1.06 & 0.89 & 1.0 & 1.06 & 0.02 & 0.02 & 0.02 & \textbf{0.9} & 0.98 & 1.0\\ & 100 & \textbf{1.0} & 1.0 & 1.0 & \textbf{1.0} & 1.0 & 1.0 & 0.08 & 0.08 & 0.08 & 0.99 & 1.0 & 1.02 & \textbf{0.94} & 1.0 & 1.0 & \textbf{0.94} & 1.0 & 1.0 & 0.04 & 0.04 & 0.04 & 0.92 & 1.0 & 1.04\\\hline\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{satellite}}}%
 & 10 & \textbf{0.53} & 0.75 & 3.31 & \textbf{0.53} & 0.75 & 3.31 & 0.41 & 0.58 & 2.94 & 0.34 & 0.5 & 2.28 & \textbf{0.49} & 0.83 & 3.08 & \textbf{0.49} & 0.83 & 3.08 & 0.41 & 0.67 & 3.11 & 0.29 & 0.53 & 2.36\\ & 30 & \textbf{0.5} & 0.78 & 2.33 & 0.48 & 0.78 & 2.47 & 0.4 & 0.81 & 2.78 & 0.41 & 0.69 & 1.75 & 0.54 & 0.78 & 2.17 & \textbf{0.6} & 0.92 & 2.47 & 0.54 & 0.89 & 3.0 & 0.51 & 0.78 & 1.92\\ & 50 & 0.67 & 0.89 & 1.89 & \textbf{0.69} & 0.92 & 1.89 & 0.42 & 0.75 & 2.5 & 0.49 & 0.72 & 1.5 & 0.78 & 0.89 & 1.42 & \textbf{0.81} & 0.94 & 1.47 & 0.61 & 0.92 & 2.19 & 0.66 & 0.92 & 1.33\\ & 70 & \textbf{0.87} & 0.94 & 1.31 & \textbf{0.87} & 0.94 & 1.31 & 0.67 & 0.78 & 1.47 & 0.81 & 0.94 & 1.17 & 0.86 & 0.97 & 1.47 & \textbf{0.91} & 1.0 & 1.42 & 0.63 & 0.78 & 1.67 & 0.78 & 0.94 & 1.42\\ & 100 & 0.92 & 0.97 & 1.31 & \textbf{0.94} & 0.97 & 1.14 & 0.69 & 0.78 & 1.31 & 0.88 & 1.0 & 1.22 & 0.92 & 0.94 & 1.19 & \textbf{0.94} & 0.94 & 1.14 & 0.47 & 0.56 & 1.0 & 0.92 & 1.0 & 1.25\\\hline\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{sokoban}}}%
 & 10 & \textbf{0.27} & 0.58 & 2.78 & \textbf{0.27} & 0.58 & 2.78 & 0.1 & 0.31 & 1.83 & 0.24 & 0.42 & 1.42 & 0.31 & 0.58 & 2.47 & \textbf{0.32} & 0.56 & 2.06 & 0.13 & 0.36 & 2.39 & 0.25 & 0.44 & 1.67\\ & 30 & 0.56 & 0.78 & 2.17 & \textbf{0.7} & 0.83 & 1.44 & 0.2 & 0.31 & 1.0 & 0.34 & 0.42 & 1.28 & 0.48 & 0.75 & 2.81 & \textbf{0.56} & 0.78 & 1.89 & 0.12 & 0.19 & 0.75 & 0.29 & 0.42 & 1.28\\ & 50 & 0.61 & 0.94 & 2.97 & \textbf{0.82} & 0.97 & 1.19 & 0.2 & 0.31 & 0.75 & 0.57 & 0.67 & 1.28 & 0.5 & 0.94 & 4.22 & \textbf{0.73} & 0.86 & 1.17 & 0.01 & 0.03 & 0.06 & 0.46 & 0.56 & 1.22\\ & 70 & 0.6 & 0.94 & 3.75 & \textbf{0.97} & 1.0 & 1.06 & 0.08 & 0.11 & 0.19 & 0.84 & 0.94 & 1.28 & 0.54 & 1.0 & 4.44 & \textbf{0.8} & 0.94 & 1.03 & 0.06 & 0.08 & 0.11 & 0.58 & 0.78 & 1.28\\ & 100 & 0.66 & 1.0 & 3.89 & \textbf{1.0} & 1.0 & 1.0 & 0.04 & 0.06 & 0.08 & 0.96 & 1.0 & 1.08 & 0.35 & 0.94 & 5.97 & \textbf{0.85} & 0.97 & 1.03 & 0.04 & 0.06 & 0.06 & 0.77 & 1.0 & 1.14\\\hline\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{zeno}}}%
 & 10 & 0.44 & 0.64 & 2.33 & 0.44 & 0.64 & 2.33 & \textbf{0.45} & 0.78 & 3.0 & 0.24 & 0.47 & 1.44 & 0.37 & 0.72 & 1.94 & 0.37 & 0.72 & 1.94 & \textbf{0.45} & 0.94 & 3.11 & 0.31 & 0.42 & 1.33\\ & 30 & 0.5 & 0.86 & 1.64 & \textbf{0.54} & 0.89 & 1.53 & 0.44 & 0.94 & 2.31 & 0.49 & 0.67 & 1.44 & 0.6 & 0.69 & 1.31 & \textbf{0.72} & 0.86 & 1.36 & 0.61 & 0.89 & 1.83 & 0.57 & 0.69 & 1.44\\ & 50 & \textbf{0.89} & 0.94 & 1.08 & 0.86 & 0.92 & 1.08 & 0.71 & 0.89 & 1.64 & 0.63 & 0.75 & 1.39 & \textbf{0.76} & 0.89 & 1.39 & 0.73 & 0.86 & 1.39 & 0.75 & 0.89 & 1.67 & 0.73 & 0.81 & 1.22\\ & 70 & 0.84 & 0.94 & 1.22 & \textbf{0.88} & 0.97 & 1.19 & 0.84 & 0.94 & 1.33 & 0.74 & 0.81 & 1.17 & 0.97 & 1.0 & 1.06 & \textbf{0.99} & 1.0 & 1.03 & 0.82 & 0.89 & 1.25 & 0.89 & 0.92 & 1.06\\ & 100 & 0.97 & 0.97 & 1.0 & \textbf{1.0} & 1.0 & 1.0 & 0.88 & 0.92 & 1.08 & 0.96 & 1.0 & 1.08 & 0.94 & 0.94 & 1.0 & \textbf{1.0} & 1.0 & 1.0 & 0.85 & 0.89 & 1.14 & 0.9 & 1.0 & 1.19\\\hline
 \textsc{f}%
 & AVG & 0.69 & 0.92 & 2.13 & \textbf{0.71} & 0.93 & 2.11 & 0.58 & 0.78 & 1.74 & 0.64 & 0.72 & 1.23 & 0.65 & 0.87 & 2.06 & \textbf{0.67} & 0.88 & 2.02 & 0.57 & 0.76 & 1.67 & 0.6 & 0.73 & 1.28\\\hline%
\textsc{l}%
 & AVG & \textbf{0.85} & 0.97 & 1.43 & \textbf{0.85} & 0.97 & 1.43 & 0.05 & 0.07 & 0.21 & 0.81 & 0.91 & 1.32 & 0.84 & 0.98 & 1.39 & \textbf{0.85} & 0.98 & 1.38 & 0.09 & 0.13 & 0.32 & 0.82 & 0.88 & 1.11\\\hline%
\textsc{m}%
 & AVG & 0.76 & 0.89 & 1.42 & \textbf{0.79} & 0.93 & 1.44 & 0.76 & 0.96 & 1.73 & 0.74 & 0.81 & 1.14 & 0.78 & 0.92 & 1.36 & \textbf{0.81} & 0.93 & 1.33 & 0.79 & 0.97 & 1.7 & 0.78 & 0.88 & 1.21\\\hline%
\textsc{r}%
 & AVG & \textbf{0.77} & 0.91 & 1.48 & 0.76 & 0.91 & 1.52 & 0.36 & 0.48 & 0.82 & 0.72 & 0.8 & 1.13 & \textbf{0.78} & 0.92 & 1.44 & 0.77 & 0.91 & 1.44 & 0.37 & 0.48 & 0.93 & 0.69 & 0.78 & 1.14\\\hline%
\multicolumn{2}{c}{AVG}  & 0.71 & 0.89 & 1.91 & \textbf{0.73} & 0.9 & 1.78 & 0.35 & 0.5 & 1.38 & 0.61 & 0.73 & 1.3 & 0.69 & 0.87 & 1.93 & \textbf{0.72} & 0.89 & 1.72 & 0.34 & 0.48 & 1.34 & 0.61 & 0.76 & 1.31%
\\
\bottomrule
\end{tabular}\\

==> tables/previous-noisyagr-1-full.tex <==
\begin{tabular}[t]{c|c|cccc|cccc|}
\toprule
 \multicolumn{2}{c}{} & \multicolumn{4}{c}{Optimal} & \multicolumn{4}{c}{Suboptimal}\\
\cmidrule(lr){3-6}\cmidrule(lr){7-10}
%
\% & \# & \dhc & \dhcf & \rg & \pom & \dhc & \dhcf & \rg & \pom\\%
%
\midrule
 10 & \multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{blocks}}} & \textbf{0.32} & \textbf{0.32} & 0.31 & 0.06 & 0.38 & 0.38 & \textbf{0.42} & 0.05\\
 30 & & 0.37 & 0.37 & \textbf{0.39} & 0.13 & 0.36 & 0.37 & \textbf{0.49} & 0.22\\
 50 & & \textbf{0.64} & \textbf{0.64} & 0.6 & 0.37 & 0.53 & 0.53 & \textbf{0.55} & 0.28\\
 70 & & 0.79 & \textbf{0.81} & 0.77 & 0.47 & \textbf{0.67} & \textbf{0.67} & 0.63 & 0.38\\
 100 & & 0.88 & 0.88 & \textbf{0.89} & 0.57 & 0.78 & \textbf{0.82} & 0.74 & 0.51\\\hline%
 10 & \multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{depots}}} & \textbf{0.39} & \textbf{0.39} & 0.0 & 0.14 & \textbf{0.43} & \textbf{0.43} & 0.02 & 0.17\\
 30 & & \textbf{0.35} & \textbf{0.35} & 0.04 & 0.22 & 0.41 & \textbf{0.43} & 0.07 & 0.21\\
 50 & & \textbf{0.62} & \textbf{0.62} & 0.04 & 0.43 & \textbf{0.76} & \textbf{0.76} & 0.01 & 0.51\\
 70 & & \textbf{0.91} & \textbf{0.91} & 0.01 & 0.62 & 0.71 & \textbf{0.78} & 0.0 & 0.54\\
 100 & & \textbf{1.0} & \textbf{1.0} & 0.0 & 0.88 & 0.94 & \textbf{1.0} & 0.01 & 0.83\\\hline%
 10 & \multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{driverlog}}} & \textbf{0.33} & \textbf{0.33} & 0.24 & 0.2 & \textbf{0.34} & \textbf{0.34} & 0.21 & 0.23\\
 30 & & \textbf{0.64} & 0.63 & 0.21 & 0.44 & 0.65 & \textbf{0.66} & 0.28 & 0.45\\
 50 & & 0.73 & \textbf{0.75} & 0.2 & 0.53 & 0.68 & \textbf{0.69} & 0.12 & 0.54\\
 70 & & 0.78 & \textbf{0.83} & 0.25 & 0.59 & \textbf{0.85} & 0.83 & 0.22 & 0.64\\
 100 & & 0.92 & \textbf{0.93} & 0.23 & 0.7 & 0.78 & \textbf{0.88} & 0.19 & 0.58\\\hline%
 10 & \multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{dwr}}} & \textbf{0.41} & \textbf{0.41} & 0.19 & 0.28 & \textbf{0.39} & \textbf{0.39} & 0.23 & 0.33\\
 30 & & 0.57 & \textbf{0.6} & 0.28 & 0.46 & 0.55 & 0.55 & 0.09 & \textbf{0.56}\\
 50 & & \textbf{0.63} & \textbf{0.63} & 0.1 & 0.58 & 0.63 & 0.63 & 0.11 & \textbf{0.75}\\
 70 & & \textbf{0.81} & \textbf{0.81} & 0.15 & 0.73 & \textbf{0.78} & \textbf{0.78} & 0.1 & 0.69\\
 100 & & 0.86 & \textbf{0.89} & 0.04 & 0.79 & 0.86 & \textbf{0.9} & 0.03 & 0.88\\\hline%
 10 & \multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{ferry}}} & \textbf{0.43} & \textbf{0.43} & 0.32 & 0.2 & \textbf{0.35} & \textbf{0.35} & 0.31 & 0.26\\
 30 & & \textbf{0.46} & \textbf{0.46} & 0.41 & 0.44 & \textbf{0.47} & \textbf{0.47} & \textbf{0.47} & 0.44\\
 50 & & 0.74 & \textbf{0.77} & 0.65 & 0.69 & \textbf{0.75} & \textbf{0.75} & 0.66 & 0.69\\
 70 & & 0.9 & \textbf{0.92} & 0.77 & 0.9 & 0.81 & \textbf{0.83} & 0.7 & 0.78\\
 100 & & 0.92 & \textbf{0.95} & 0.75 & 0.94 & 0.85 & \textbf{0.95} & 0.71 & 0.82\\\hline%
 10 & \multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{ipc-grid}}} & \textbf{0.57} & \textbf{0.57} & 0.16 & 0.38 & \textbf{0.62} & \textbf{0.62} & 0.12 & 0.54\\
 30 & & \textbf{0.85} & \textbf{0.85} & 0.28 & 0.71 & 0.68 & 0.68 & 0.08 & \textbf{0.72}\\
 50 & & \textbf{0.89} & \textbf{0.89} & 0.07 & 0.81 & 0.84 & 0.84 & 0.04 & \textbf{0.85}\\
 70 & & \textbf{0.95} & \textbf{0.95} & 0.15 & 0.93 & 0.89 & 0.89 & 0.02 & \textbf{0.9}\\
 100 & & \textbf{1.0} & \textbf{1.0} & 0.08 & 0.99 & \textbf{0.94} & \textbf{0.94} & 0.04 & 0.92\\
\midrule
\multicolumn{2}{c|}{AVG} &  \multicolumn{7}{c}{} \\\midrule\midrule%
\multicolumn{2}{c|}{ACC} &  \multicolumn{7}{c}{} \\\midrule%
\multicolumn{2}{c|}{SPR} &  \multicolumn{7}{c}{} \\
\bottomrule
\end{tabular}

==> tables/previous-noisyagr-1.tex <==
\begin{tabular}[t]{c|c|cccc|cccc|}
\toprule
 \multicolumn{2}{c}{} & \multicolumn{4}{c}{Optimal} & \multicolumn{4}{c}{Suboptimal}\\
\cmidrule(lr){3-6}\cmidrule(lr){7-10}
%
\% & \# & \dhc & \dhcf & \rg & \pom & \dhc & \dhcf & \rg & \pom\\%
%
\midrule
10 & \multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{blocks}}}% 
& \textbf{0.32} & \textbf{0.32} & 0.31 & 0.06 & 0.38 & 0.38 & \textbf{0.42} & 0.05\\
30 & & 0.37 & 0.37 & \textbf{0.39} & 0.13 & 0.36 & 0.37 & \textbf{0.49} & 0.22\\
50 & & \textbf{0.64} & \textbf{0.64} & 0.6 & 0.37 & 0.53 & 0.53 & \textbf{0.55} & 0.28\\
70 & & 0.79 & \textbf{0.81} & 0.77 & 0.47 & \textbf{0.67} & \textbf{0.67} & 0.63 & 0.38\\
100&  & 0.88 & 0.88 & \textbf{0.89} & 0.57 & 0.78 & \textbf{0.82} & 0.74 & 0.51\\\hline%
10 & \multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{depots}}}% 
& \textbf{0.39} & \textbf{0.39} & 0.0 & 0.14 & \textbf{0.43} & \textbf{0.43} & 0.02 & 0.17\\
30 & & \textbf{0.35} & \textbf{0.35} & 0.04 & 0.22 & 0.41 & \textbf{0.43} & 0.07 & 0.21\\
50 & & \textbf{0.62} & \textbf{0.62} & 0.04 & 0.43 & \textbf{0.76} & \textbf{0.76} & 0.01 & 0.51\\
70 & & \textbf{0.91} & \textbf{0.91} & 0.01 & 0.62 & 0.71 & \textbf{0.78} & 0.0 & 0.54\\
100&  & \textbf{1.0} & \textbf{1.0} & 0.0 & 0.88 & 0.94 & \textbf{1.0} & 0.01 & 0.83\\\hline%
10 & \multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{driverlog}}}% 
& \textbf{0.33} & \textbf{0.33} & 0.24 & 0.2 & \textbf{0.34} & \textbf{0.34} & 0.21 & 0.23\\
30 & & \textbf{0.64} & 0.63 & 0.21 & 0.44 & 0.65 & \textbf{0.66} & 0.28 & 0.45\\
50 & & 0.73 & \textbf{0.75} & 0.2 & 0.53 & 0.68 & \textbf{0.69} & 0.12 & 0.54\\
70 & & 0.78 & \textbf{0.83} & 0.25 & 0.59 & \textbf{0.85} & 0.83 & 0.22 & 0.64\\
100&  & 0.92 & \textbf{0.93} & 0.23 & 0.7 & 0.78 & \textbf{0.88} & 0.19 & 0.58\\\hline%
10 & \multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{dwr}}}% 
& \textbf{0.41} & \textbf{0.41} & 0.19 & 0.28 & \textbf{0.39} & \textbf{0.39} & 0.23 & 0.33\\
30 & & 0.57 & \textbf{0.6} & 0.28 & 0.46 & 0.55 & 0.55 & 0.09 & \textbf{0.56}\\
50 & & \textbf{0.63} & \textbf{0.63} & 0.1 & 0.58 & 0.63 & 0.63 & 0.11 & \textbf{0.75}\\
70 & & \textbf{0.81} & \textbf{0.81} & 0.15 & 0.73 & \textbf{0.78} & \textbf{0.78} & 0.1 & 0.69\\
100&  & 0.86 & \textbf{0.89} & 0.04 & 0.79 & 0.86 & \textbf{0.9} & 0.03 & 0.88\\\hline%
 - & \textsc{f}%
& 0.69 & \textbf{0.71} & 0.58 & 0.64 & 0.65 & \textbf{0.67} & 0.57 & 0.6\\\hline%
 - & \textsc{l}%
& \textbf{0.85} & \textbf{0.85} & 0.05 & 0.81 & 0.84 & \textbf{0.85} & 0.09 & 0.82
\\\midrule
\multicolumn{2}{c|}{AGR} &  \multicolumn{7}{c}{} \\\midrule\midrule%
\multicolumn{2}{c|}{ACC} &  \multicolumn{7}{c}{} \\\midrule%
\multicolumn{2}{c|}{SPR} &  \multicolumn{7}{c}{} \\
\bottomrule
\end{tabular}

==> tables/previous-noisyagr-2-full.tex <==
\begin{tabular}[t]{c|cccc|cccc}
\toprule
 \multicolumn{1}{c}{} & \multicolumn{4}{c}{Optimal} & \multicolumn{4}{c}{Suboptimal}\\
\cmidrule(lr){2-5}\cmidrule(lr){6-9}
%
\# & \dhc & \dhcf & \rg & \pom & \dhc & \dhcf & \rg & \pom\\%
%
\midrule
 \multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{logistics}}} & \textbf{0.58} & \textbf{0.58} & 0.13 & 0.41 & \textbf{0.55} & \textbf{0.55} & 0.28 & 0.41\\
 & \textbf{0.82} & \textbf{0.82} & 0.06 & 0.78 & 0.8 & \textbf{0.82} & 0.12 & 0.81\\
 & \textbf{0.9} & \textbf{0.9} & 0.03 & 0.89 & \textbf{0.91} & \textbf{0.91} & 0.03 & 0.9\\
 & \textbf{0.97} & \textbf{0.97} & 0.03 & 0.94 & 0.96 & 0.97 & 0.0 & \textbf{0.99}\\
 & \textbf{1.0} & \textbf{1.0} & 0.03 & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & 0.0 & \textbf{1.0}\\\hline%
 \multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{miconic}}} & 0.39 & 0.39 & \textbf{0.46} & 0.27 & 0.43 & 0.43 & \textbf{0.47} & 0.35\\
 & 0.57 & \textbf{0.65} & 0.55 & 0.57 & 0.75 & \textbf{0.78} & 0.64 & 0.69\\
 & 0.93 & \textbf{0.94} & 0.87 & 0.9 & 0.86 & 0.89 & 0.87 & \textbf{0.93}\\
 & 0.94 & \textbf{0.96} & 0.93 & \textbf{0.96} & 0.9 & 0.93 & \textbf{0.98} & 0.94\\
 & 0.94 & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & 0.97 & \textbf{1.0} & \textbf{1.0} & \textbf{1.0}\\\hline%
 \multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{rovers}}} & \textbf{0.44} & \textbf{0.44} & 0.18 & 0.31 & \textbf{0.46} & \textbf{0.46} & 0.37 & 0.44\\
 & 0.7 & 0.7 & 0.45 & \textbf{0.75} & 0.65 & \textbf{0.66} & 0.4 & 0.51\\
 & 0.8 & \textbf{0.82} & 0.31 & 0.71 & \textbf{0.87} & 0.85 & 0.49 & 0.72\\
 & \textbf{0.93} & 0.89 & 0.49 & 0.88 & \textbf{0.93} & 0.92 & 0.26 & 0.89\\
 & \textbf{0.97} & 0.93 & 0.39 & \textbf{0.97} & \textbf{0.97} & 0.93 & 0.34 & 0.9\\\hline%
 \multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{satellite}}} & \textbf{0.53} & \textbf{0.53} & 0.41 & 0.34 & \textbf{0.49} & \textbf{0.49} & 0.41 & 0.29\\
 & \textbf{0.5} & 0.48 & 0.4 & 0.41 & 0.54 & \textbf{0.6} & 0.54 & 0.51\\
 & 0.67 & \textbf{0.69} & 0.42 & 0.49 & 0.78 & \textbf{0.81} & 0.61 & 0.66\\
 & \textbf{0.87} & \textbf{0.87} & 0.67 & 0.81 & 0.86 & \textbf{0.91} & 0.63 & 0.78\\
 & 0.92 & \textbf{0.94} & 0.69 & 0.88 & 0.92 & \textbf{0.94} & 0.47 & 0.92\\\hline%
 \multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{sokoban}}} & \textbf{0.27} & \textbf{0.27} & 0.1 & 0.24 & 0.31 & \textbf{0.32} & 0.13 & 0.25\\
 & 0.56 & \textbf{0.7} & 0.2 & 0.34 & 0.48 & \textbf{0.56} & 0.12 & 0.29\\
 & 0.61 & \textbf{0.82} & 0.2 & 0.57 & 0.5 & \textbf{0.73} & 0.01 & 0.46\\
 & 0.6 & \textbf{0.97} & 0.08 & 0.84 & 0.54 & \textbf{0.8} & 0.06 & 0.58\\
 & 0.66 & \textbf{1.0} & 0.04 & 0.96 & 0.35 & \textbf{0.85} & 0.04 & 0.77\\\hline%
 \multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{zeno}}} & 0.44 & 0.44 & \textbf{0.45} & 0.24 & 0.37 & 0.37 & \textbf{0.45} & 0.31\\
 & 0.5 & \textbf{0.54} & 0.44 & 0.49 & 0.6 & \textbf{0.72} & 0.61 & 0.57\\
 & \textbf{0.89} & 0.86 & 0.71 & 0.63 & \textbf{0.76} & 0.73 & 0.75 & 0.73\\
 & 0.84 & \textbf{0.88} & 0.84 & 0.74 & 0.97 & \textbf{0.99} & 0.82 & 0.89\\
 & 0.97 & \textbf{1.0} & 0.88 & 0.96 & 0.94 & \textbf{1.0} & 0.85 & 0.9\\\midrule%
%
\multicolumn{1}{c}{}& 0.71 & \textbf{0.73} & 0.35 & 0.61 & 0.69 & \textbf{0.72} & 0.34 & 0.61\\\midrule\midrule%
\multicolumn{1}{c}{}& 0.89 & \textbf{0.9} & 0.5 & 0.73 & 0.87 & \textbf{0.89} & 0.48 & 0.76\\\midrule%
\multicolumn{1}{c}{}& 1.91 & 1.78 & 1.38 & \textbf{1.3} & 1.93 & 1.72 & 1.34 & \textbf{1.31}\\
\bottomrule
\end{tabular}\\

==> tables/previous-noisyagr-2.tex <==
\begin{tabular}[t]{c|cccc|cccc}
\toprule
 \multicolumn{1}{c}{} & \multicolumn{4}{c}{Optimal} & \multicolumn{4}{c}{Suboptimal}\\
\cmidrule(lr){2-5}\cmidrule(lr){6-9}
%
\# & \dhc & \dhcf & \rg & \pom & \dhc & \dhcf & \rg & \pom\\%
%
\midrule
\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{ipc-grid}}}%
& \textbf{0.57} & \textbf{0.57} & 0.16 & 0.38 & \textbf{0.62} & \textbf{0.62} & 0.12 & 0.54\\ & \textbf{0.85} & \textbf{0.85} & 0.28 & 0.71 & 0.68 & 0.68 & 0.08 & \textbf{0.72}\\& \textbf{0.89} & \textbf{0.89} & 0.07 & 0.81 & 0.84 & 0.84 & 0.04 & \textbf{0.85}\\ & \textbf{0.95} & \textbf{0.95} & 0.15 & 0.93 & 0.89 & 0.89 & 0.02 & \textbf{0.9}\\& \textbf{1.0} & \textbf{1.0} & 0.08 & 0.99 & \textbf{0.94} & \textbf{0.94} & 0.04 & 0.92\\\hline%
\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{satellite}}}%
& \textbf{0.53} & \textbf{0.53} & 0.41 & 0.34 & \textbf{0.49} & \textbf{0.49} & 0.41 & 0.29\\ & \textbf{0.5} & 0.48 & 0.4 & 0.41 & 0.54 & \textbf{0.6} & 0.54 & 0.51\\& 0.67 & \textbf{0.69} & 0.42 & 0.49 & 0.78 & \textbf{0.81} & 0.61 & 0.66\\ & \textbf{0.87} & \textbf{0.87} & 0.67 & 0.81 & 0.86 & \textbf{0.91} & 0.63 & 0.78\\& 0.92 & \textbf{0.94} & 0.69 & 0.88 & 0.92 & \textbf{0.94} & 0.47 & 0.92\\\hline%
\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{sokoban}}}%
& \textbf{0.27} & \textbf{0.27} & 0.1 & 0.24 & 0.31 & \textbf{0.32} & 0.13 & 0.25\\ & 0.56 & \textbf{0.7} & 0.2 & 0.34 & 0.48 & \textbf{0.56} & 0.12 & 0.29\\& 0.61 & \textbf{0.82} & 0.2 & 0.57 & 0.5 & \textbf{0.73} & 0.01 & 0.46\\ & 0.6 & \textbf{0.97} & 0.08 & 0.84 & 0.54 & \textbf{0.8} & 0.06 & 0.58\\& 0.66 & \textbf{1.0} & 0.04 & 0.96 & 0.35 & \textbf{0.85} & 0.04 & 0.77\\\hline%
\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{zeno}}}%
& 0.44 & 0.44 & \textbf{0.45} & 0.24 & 0.37 & 0.37 & \textbf{0.45} & 0.31\\ & 0.5 & \textbf{0.54} & 0.44 & 0.49 & 0.6 & \textbf{0.72} & 0.61 & 0.57\\& \textbf{0.89} & 0.86 & 0.71 & 0.63 & \textbf{0.76} & 0.73 & 0.75 & 0.73\\ & 0.84 & \textbf{0.88} & 0.84 & 0.74 & 0.97 & \textbf{0.99} & 0.82 & 0.89\\& 0.97 & \textbf{1.0} & 0.88 & 0.96 & 0.94 & \textbf{1.0} & 0.85 & 0.9\\\hline%
\textsc{m}%
& 0.76 & \textbf{0.79} & 0.76 & 0.74 & 0.78 & \textbf{0.81} & 0.79 & 0.78\\\hline%
\textsc{r}%
& \textbf{0.77} & 0.76 & 0.36 & 0.72 & \textbf{0.78} & 0.77 & 0.37 & 0.69\\\midrule%
\multicolumn{1}{c}{}& 0.71 & \textbf{0.73} & 0.35 & 0.61 & 0.69 & \textbf{0.72} & 0.34 & 0.61\\\midrule\midrule%
\multicolumn{1}{c}{}& 0.89 & \textbf{0.9} & 0.5 & 0.73 & 0.87 & \textbf{0.89} & 0.48 & 0.76\\\midrule%
\multicolumn{1}{c}{}& 1.91 & 1.78 & 1.38 & \textbf{1.3} & 1.93 & 1.72 & 1.34 & \textbf{1.31}\\
\bottomrule
\end{tabular}\\

==> tables/previous-noisyagr-single.tex <==
\begin{tabular}[t]{cc|cccc|cccc}
\toprule
 \multicolumn{2}{c}{} & \multicolumn{4}{c}{Optimal} & \multicolumn{4}{c}{Suboptimal}\\
\cmidrule(lr){3-6}\cmidrule(lr){7-10}
%
\# & \% & \dhc & \dhcf & \rg & \pom & \dhc & \dhcf & \rg & \pom\\%
%
\midrule
\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{blocks}}}%
 & 10 & \textbf{0.32} & \textbf{0.32} & 0.31 & 0.06 & 0.38 & 0.38 & \textbf{0.42} & 0.05\\ & 30 & 0.37 & 0.37 & \textbf{0.39} & 0.13 & 0.36 & 0.37 & \textbf{0.49} & 0.22\\ & 50 & \textbf{0.64} & \textbf{0.64} & 0.6 & 0.37 & 0.53 & 0.53 & \textbf{0.55} & 0.28\\ & 70 & 0.79 & \textbf{0.81} & 0.77 & 0.47 & \textbf{0.67} & \textbf{0.67} & 0.63 & 0.38\\ & 100 & 0.88 & 0.88 & \textbf{0.89} & 0.57 & 0.78 & \textbf{0.82} & 0.74 & 0.51\\\hline%
\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{depots}}}%
 & 10 & \textbf{0.39} & \textbf{0.39} & 0.0 & 0.14 & \textbf{0.43} & \textbf{0.43} & 0.02 & 0.17\\ & 30 & \textbf{0.35} & \textbf{0.35} & 0.04 & 0.22 & 0.41 & \textbf{0.43} & 0.07 & 0.21\\ & 50 & \textbf{0.62} & \textbf{0.62} & 0.04 & 0.43 & \textbf{0.76} & \textbf{0.76} & 0.01 & 0.51\\ & 70 & \textbf{0.91} & \textbf{0.91} & 0.01 & 0.62 & 0.71 & \textbf{0.78} & 0.0 & 0.54\\ & 100 & \textbf{1.0} & \textbf{1.0} & 0.0 & 0.88 & 0.94 & \textbf{1.0} & 0.01 & 0.83\\\hline%
\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{driverlog}}}%
 & 10 & \textbf{0.33} & \textbf{0.33} & 0.24 & 0.2 & \textbf{0.34} & \textbf{0.34} & 0.21 & 0.23\\ & 30 & \textbf{0.64} & 0.63 & 0.21 & 0.44 & 0.65 & \textbf{0.66} & 0.28 & 0.45\\ & 50 & 0.73 & \textbf{0.75} & 0.2 & 0.53 & 0.68 & \textbf{0.69} & 0.12 & 0.54\\ & 70 & 0.78 & \textbf{0.83} & 0.25 & 0.59 & \textbf{0.85} & 0.83 & 0.22 & 0.64\\ & 100 & 0.92 & \textbf{0.93} & 0.23 & 0.7 & 0.78 & \textbf{0.88} & 0.19 & 0.58\\\hline%
\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{dwr}}}%
 & 10 & \textbf{0.41} & \textbf{0.41} & 0.19 & 0.28 & \textbf{0.39} & \textbf{0.39} & 0.23 & 0.33\\ & 30 & 0.57 & \textbf{0.6} & 0.28 & 0.46 & 0.55 & 0.55 & 0.09 & \textbf{0.56}\\ & 50 & \textbf{0.63} & \textbf{0.63} & 0.1 & 0.58 & 0.63 & 0.63 & 0.11 & \textbf{0.75}\\ & 70 & \textbf{0.81} & \textbf{0.81} & 0.15 & 0.73 & \textbf{0.78} & \textbf{0.78} & 0.1 & 0.69\\ & 100 & 0.86 & \textbf{0.89} & 0.04 & 0.79 & 0.86 & \textbf{0.9} & 0.03 & 0.88\\\hline%
\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{ipc-grid}}}%
 & 10 & \textbf{0.57} & \textbf{0.57} & 0.16 & 0.38 & \textbf{0.62} & \textbf{0.62} & 0.12 & 0.54\\ & 30 & \textbf{0.85} & \textbf{0.85} & 0.28 & 0.71 & 0.68 & 0.68 & 0.08 & \textbf{0.72}\\ & 50 & \textbf{0.89} & \textbf{0.89} & 0.07 & 0.81 & 0.84 & 0.84 & 0.04 & \textbf{0.85}\\ & 70 & \textbf{0.95} & \textbf{0.95} & 0.15 & 0.93 & 0.89 & 0.89 & 0.02 & \textbf{0.9}\\ & 100 & \textbf{1.0} & \textbf{1.0} & 0.08 & 0.99 & \textbf{0.94} & \textbf{0.94} & 0.04 & 0.92\\\hline%
\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{satellite}}}%
 & 10 & \textbf{0.53} & \textbf{0.53} & 0.41 & 0.34 & \textbf{0.49} & \textbf{0.49} & 0.41 & 0.29\\ & 30 & \textbf{0.5} & 0.48 & 0.4 & 0.41 & 0.54 & \textbf{0.6} & 0.54 & 0.51\\ & 50 & 0.67 & \textbf{0.69} & 0.42 & 0.49 & 0.78 & \textbf{0.81} & 0.61 & 0.66\\ & 70 & \textbf{0.87} & \textbf{0.87} & 0.67 & 0.81 & 0.86 & \textbf{0.91} & 0.63 & 0.78\\ & 100 & 0.92 & \textbf{0.94} & 0.69 & 0.88 & 0.92 & \textbf{0.94} & 0.47 & 0.92\\\hline%
\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{sokoban}}}%
 & 10 & \textbf{0.27} & \textbf{0.27} & 0.1 & 0.24 & 0.31 & \textbf{0.32} & 0.13 & 0.25\\ & 30 & 0.56 & \textbf{0.7} & 0.2 & 0.34 & 0.48 & \textbf{0.56} & 0.12 & 0.29\\ & 50 & 0.61 & \textbf{0.82} & 0.2 & 0.57 & 0.5 & \textbf{0.73} & 0.01 & 0.46\\ & 70 & 0.6 & \textbf{0.97} & 0.08 & 0.84 & 0.54 & \textbf{0.8} & 0.06 & 0.58\\ & 100 & 0.66 & \textbf{1.0} & 0.04 & 0.96 & 0.35 & \textbf{0.85} & 0.04 & 0.77\\\hline%
\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{zeno}}}%
 & 10 & 0.44 & 0.44 & \textbf{0.45} & 0.24 & 0.37 & 0.37 & \textbf{0.45} & 0.31\\ & 30 & 0.5 & \textbf{0.54} & 0.44 & 0.49 & 0.6 & \textbf{0.72} & 0.61 & 0.57\\ & 50 & \textbf{0.89} & 0.86 & 0.71 & 0.63 & \textbf{0.76} & 0.73 & 0.75 & 0.73\\ & 70 & 0.84 & \textbf{0.88} & 0.84 & 0.74 & 0.97 & \textbf{0.99} & 0.82 & 0.89\\ & 100 & 0.97 & \textbf{1.0} & 0.88 & 0.96 & 0.94 & \textbf{1.0} & 0.85 & 0.9\\\hline%
\textsc{f}%
 & - & 0.69 & \textbf{0.71} & 0.58 & 0.64 & 0.65 & \textbf{0.67} & 0.57 & 0.6\\\hline%
\textsc{l}%
 & - & \textbf{0.85} & \textbf{0.85} & 0.05 & 0.81 & 0.84 & \textbf{0.85} & 0.09 & 0.82
\\\hline
\textsc{m}%
 & - & 0.76 & \textbf{0.79} & 0.76 & 0.74 & 0.78 & \textbf{0.81} & 0.79 & 0.78\\\hline%
\textsc{r}%
 & - & \textbf{0.77} & 0.76 & 0.36 & 0.72 & \textbf{0.78} & 0.77 & 0.37 & 0.69\\\hline%
\multicolumn{2}{c|}{AVG} & 0.71 & \textbf{0.73} & 0.35 & 0.61 & 0.69 & \textbf{0.72} & 0.34 & 0.61\\\hline\hline%
\multicolumn{2}{c|}{ACC} & 0.89 & \textbf{0.9} & 0.5 & 0.73 & 0.87 & \textbf{0.89} & 0.48 & 0.76\\\hline%
\multicolumn{2}{c|}{SPR} & 1.91 & 1.78 & 1.38 & \textbf{1.3} & 1.93 & 1.72 & 1.34 & \textbf{1.31}%
\\\bottomrule
\end{tabular}

==> tables/previous-noisyagr.tex <==
\begin{tabular}{cc|cccc|cccc|}
\toprule
 \multicolumn{2}{c}{} & \multicolumn{4}{c}{Optimal} & \multicolumn{4}{c}{Suboptimal}\\
\cmidrule(lr){3-6}\cmidrule(lr){7-10}
%
\# & \% & \dhc & \dhcf & \rg & \pom & \dhc & \dhcf & \rg & \pom\\%
%
\midrule
\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{blocks}}}%
 & 10 & \textbf{0.32} & \textbf{0.32} & 0.31 & 0.06 & 0.38 & 0.38 & \textbf{0.42} & 0.05\\ & 30 & 0.37 & 0.37 & \textbf{0.39} & 0.13 & 0.36 & 0.37 & \textbf{0.49} & 0.22\\ & 50 & \textbf{0.64} & \textbf{0.64} & 0.6 & 0.37 & 0.53 & 0.53 & \textbf{0.55} & 0.28\\ & 70 & 0.79 & \textbf{0.81} & 0.77 & 0.47 & \textbf{0.67} & \textbf{0.67} & 0.63 & 0.38\\ & 100 & 0.88 & 0.88 & \textbf{0.89} & 0.57 & 0.78 & \textbf{0.82} & 0.74 & 0.51\\\hline%
\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{depots}}}%
 & 10 & \textbf{0.39} & \textbf{0.39} & 0.0 & 0.14 & \textbf{0.43} & \textbf{0.43} & 0.02 & 0.17\\ & 30 & \textbf{0.35} & \textbf{0.35} & 0.04 & 0.22 & 0.41 & \textbf{0.43} & 0.07 & 0.21\\ & 50 & \textbf{0.62} & \textbf{0.62} & 0.04 & 0.43 & \textbf{0.76} & \textbf{0.76} & 0.01 & 0.51\\ & 70 & \textbf{0.91} & \textbf{0.91} & 0.01 & 0.62 & 0.71 & \textbf{0.78} & 0.0 & 0.54\\ & 100 & \textbf{1.0} & \textbf{1.0} & 0.0 & 0.88 & 0.94 & \textbf{1.0} & 0.01 & 0.83\\\hline%
\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{driverlog}}}%
 & 10 & \textbf{0.33} & \textbf{0.33} & 0.24 & 0.2 & \textbf{0.34} & \textbf{0.34} & 0.21 & 0.23\\ & 30 & \textbf{0.64} & 0.63 & 0.21 & 0.44 & 0.65 & \textbf{0.66} & 0.28 & 0.45\\ & 50 & 0.73 & \textbf{0.75} & 0.2 & 0.53 & 0.68 & \textbf{0.69} & 0.12 & 0.54\\ & 70 & 0.78 & \textbf{0.83} & 0.25 & 0.59 & \textbf{0.85} & 0.83 & 0.22 & 0.64\\ & 100 & 0.92 & \textbf{0.93} & 0.23 & 0.7 & 0.78 & \textbf{0.88} & 0.19 & 0.58\\\hline%
\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{dwr}}}%
 & 10 & \textbf{0.41} & \textbf{0.41} & 0.19 & 0.28 & \textbf{0.39} & \textbf{0.39} & 0.23 & 0.33\\ & 30 & 0.57 & \textbf{0.6} & 0.28 & 0.46 & 0.55 & 0.55 & 0.09 & \textbf{0.56}\\ & 50 & \textbf{0.63} & \textbf{0.63} & 0.1 & 0.58 & 0.63 & 0.63 & 0.11 & \textbf{0.75}\\ & 70 & \textbf{0.81} & \textbf{0.81} & 0.15 & 0.73 & \textbf{0.78} & \textbf{0.78} & 0.1 & 0.69\\ & 100 & 0.86 & \textbf{0.89} & 0.04 & 0.79 & 0.86 & \textbf{0.9} & 0.03 & 0.88\\\hline%
\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{ipc-grid}}}%
 & 10 & \textbf{0.57} & \textbf{0.57} & 0.16 & 0.38 & \textbf{0.62} & \textbf{0.62} & 0.12 & 0.54\\ & 30 & \textbf{0.85} & \textbf{0.85} & 0.28 & 0.71 & 0.68 & 0.68 & 0.08 & \textbf{0.72}\\ & 50 & \textbf{0.89} & \textbf{0.89} & 0.07 & 0.81 & 0.84 & 0.84 & 0.04 & \textbf{0.85}\\ & 70 & \textbf{0.95} & \textbf{0.95} & 0.15 & 0.93 & 0.89 & 0.89 & 0.02 & \textbf{0.9}\\ & 100 & \textbf{1.0} & \textbf{1.0} & 0.08 & 0.99 & \textbf{0.94} & \textbf{0.94} & 0.04 & 0.92\\\hline%
\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{satellite}}}%
 & 10 & \textbf{0.53} & \textbf{0.53} & 0.41 & 0.34 & \textbf{0.49} & \textbf{0.49} & 0.41 & 0.29\\ & 30 & \textbf{0.5} & 0.48 & 0.4 & 0.41 & 0.54 & \textbf{0.6} & 0.54 & 0.51\\ & 50 & 0.67 & \textbf{0.69} & 0.42 & 0.49 & 0.78 & \textbf{0.81} & 0.61 & 0.66\\ & 70 & \textbf{0.87} & \textbf{0.87} & 0.67 & 0.81 & 0.86 & \textbf{0.91} & 0.63 & 0.78\\ & 100 & 0.92 & \textbf{0.94} & 0.69 & 0.88 & 0.92 & \textbf{0.94} & 0.47 & 0.92\\\hline%
\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{sokoban}}}%
 & 10 & \textbf{0.27} & \textbf{0.27} & 0.1 & 0.24 & 0.31 & \textbf{0.32} & 0.13 & 0.25\\ & 30 & 0.56 & \textbf{0.7} & 0.2 & 0.34 & 0.48 & \textbf{0.56} & 0.12 & 0.29\\ & 50 & 0.61 & \textbf{0.82} & 0.2 & 0.57 & 0.5 & \textbf{0.73} & 0.01 & 0.46\\ & 70 & 0.6 & \textbf{0.97} & 0.08 & 0.84 & 0.54 & \textbf{0.8} & 0.06 & 0.58\\ & 100 & 0.66 & \textbf{1.0} & 0.04 & 0.96 & 0.35 & \textbf{0.85} & 0.04 & 0.77\\\hline%
\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{zeno}}}%
 & 10 & 0.44 & 0.44 & \textbf{0.45} & 0.24 & 0.37 & 0.37 & \textbf{0.45} & 0.31\\ & 30 & 0.5 & \textbf{0.54} & 0.44 & 0.49 & 0.6 & \textbf{0.72} & 0.61 & 0.57\\ & 50 & \textbf{0.89} & 0.86 & 0.71 & 0.63 & \textbf{0.76} & 0.73 & 0.75 & 0.73\\ & 70 & 0.84 & \textbf{0.88} & 0.84 & 0.74 & 0.97 & \textbf{0.99} & 0.82 & 0.89\\ & 100 & 0.97 & \textbf{1.0} & 0.88 & 0.96 & 0.94 & \textbf{1.0} & 0.85 & 0.9\\\hline%
\textsc{f}%
 & AVG & 0.69 & \textbf{0.71} & 0.58 & 0.64 & 0.65 & \textbf{0.67} & 0.57 & 0.6\\\hline%
\textsc{l}%
 & AVG & \textbf{0.85} & \textbf{0.85} & 0.05 & 0.81 & 0.84 & \textbf{0.85} & 0.09 & 0.82\\\hline%
\textsc{m}%
 & AVG & 0.76 & \textbf{0.79} & 0.76 & 0.74 & 0.78 & \textbf{0.81} & 0.79 & 0.78\\\hline%
\textsc{r}%
 & AVG & \textbf{0.77} & 0.76 & 0.36 & 0.72 & \textbf{0.78} & 0.77 & 0.37 & 0.69\\\hline%
\multicolumn{2}{c|}{AVG AGR} & 0.71 & \textbf{0.73} & 0.35 & 0.61 & 0.69 & \textbf{0.72} & 0.34 & 0.61\\\hline%
\multicolumn{2}{c|}{AVG ACC} & 0.89 & \textbf{0.9} & 0.5 & 0.73 & 0.87 & \textbf{0.89} & 0.48 & 0.76\\\hline%
\multicolumn{2}{c|}{AVG SPR} & 1.91 & 1.78 & 1.38 & \textbf{1.3} & 1.93 & 1.72 & 1.34 & \textbf{1.31}%
\\
\bottomrule
\end{tabular}\\

==> tables/previous-optimal-noisy.tex <==
\begin{tabular}{|c|c|ccc|ccc|ccc|ccc|ccc|ccc|}
\hline
% empty
& % empty
& \multicolumn{3}{c|}{}
& \multicolumn{3}{c|}{\hdeltahc}
& \multicolumn{3}{c|}{\hdeltahcu}
& \multicolumn{3}{c|}{\rg}		   
& \multicolumn{3}{c|}{\completion}
& \multicolumn{3}{c|}{\completion 0.3}
\\ \hline
\# & $|\goalconditions|$ & \textbf{\% Obs} & $|\observations|$ & $|\grsolution|$ 
& \textbf{Agr} & \textbf{Acc} & \textbf{Spr}
& \textbf{Agr} & \textbf{Acc} & \textbf{Spr}
& \textbf{Agr} & \textbf{Acc} & \textbf{Spr}
& \textbf{Agr} & \textbf{Acc} & \textbf{Spr}
& \textbf{Agr} & \textbf{Acc} & \textbf{Spr}
\\ 
\hline

\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{blocks}} } & \multirow{5}{*}{20.1} 
	 & 10	 & 2.25	 & 7.9

		% delta-h-c - 10% 
		& 0.32 & 66.7 & 6.67 	 

		% delta-h-c-uncertainty - 10% 
		& 0.33 & 69.4 & 9.11 	 

		% rg2009 - 10% 
		& 0.31 & 66.7 & 7.11 	 

		% lm_hc0 - 10% 
		& 0.06 & 8.3 & \textbf{1.25} 	 

		% lm_hc30 - 10% 
		& \textbf{0.35} & \textbf{88.9} & 17.42 	 

	\\ & & 30	 & 4.08	 & 3.91

		% delta-h-c - 30% 
		& 0.37 & 75.0 & 3.44 	 

		% delta-h-c-uncertainty - 30% 
		& \textbf{0.39} & 88.9 & 7.64 	 

		% rg2009 - 30% 
		& \textbf{0.39} & 91.7 & 6.28 	 

		% lm_hc0 - 30% 
		& 0.13 & 27.8 & \textbf{1.25} 	 

		% lm_hc30 - 30% 
		& 0.25 & \textbf{100.0} & 14.69 	 

	\\ & & 50	 & 5.67	 & 2.48

		% delta-h-c - 50% 
		& \textbf{0.64} & 83.3 & 2.17 	 

		% delta-h-c-uncertainty - 50% 
		& 0.52 & 94.4 & 4.53 	 

		% rg2009 - 50% 
		& 0.6 & 88.9 & 3.19 	 

		% lm_hc0 - 50% 
		& 0.37 & 55.6 & \textbf{1.19} 	 

		% lm_hc30 - 50% 
		& 0.22 & \textbf{100.0} & 13.61 	 

	\\ & & 70	 & 8.42	 & 1.94

		% delta-h-c - 70% 
		& \textbf{0.79} & 91.7 & 1.67 	 

		% delta-h-c-uncertainty - 70% 
		& 0.58 & 94.4 & 2.86 	 

		% rg2009 - 70% 
		& 0.77 & 94.4 & 2.14 	 

		% lm_hc0 - 70% 
		& 0.47 & 66.7 & \textbf{1.22} 	 

		% lm_hc30 - 70% 
		& 0.22 & \textbf{100.0} & 11.14 	 

	\\ & & 100	 & 11.08	 & 1.83

		% delta-h-c - 100% 
		& 0.88 & 94.4 & \textbf{1.58} 	 

		% delta-h-c-uncertainty - 100% 
		& 0.8 & 97.2 & 2.08 	 

		% rg2009 - 100% 
		& \textbf{0.89} & 97.2 & 2.03 	 

		% lm_hc0 - 100% 
		& 0.57 & \textbf{100.0} & 1.81 	 

		% lm_hc30 - 100% 
		& 0.24 & \textbf{100.0} & 8.69 	 
 \\ \hline
\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{ipc-grid}} } & \multirow{5}{*}{7.5} 
	 & 10	 & 2.63	 & 2.71

		% delta-h-c - 10% 
		& 0.57 & 91.7 & 1.5 	 

		% delta-h-c-uncertainty - 10% 
		& \textbf{0.61} & \textbf{95.8} & 1.67 	 

		% rg2009 - 10% 
		& 0.16 & 22.9 & \textbf{0.71} 	 

		% lm_hc0 - 10% 
		& 0.38 & 66.7 & 1.71 	 

		% lm_hc30 - 10% 
		& 0.45 & \textbf{95.8} & 5.0 	 

	\\ & & 30	 & 5.19	 & 1.21

		% delta-h-c - 30% 
		& \textbf{0.85} & 91.7 & 1.17 	 

		% delta-h-c-uncertainty - 30% 
		& 0.83 & 93.8 & 1.25 	 

		% rg2009 - 30% 
		& 0.28 & 29.2 & \textbf{0.33} 	 

		% lm_hc0 - 30% 
		& 0.71 & 85.4 & 1.67 	 

		% lm_hc30 - 30% 
		& 0.6 & \textbf{95.8} & 3.02 	 

	\\ & & 50	 & 7.81	 & 1.13

		% delta-h-c - 50% 
		& \textbf{0.89} & \textbf{95.8} & 1.15 	 

		% delta-h-c-uncertainty - 50% 
		& 0.88 & \textbf{95.8} & 1.17 	 

		% rg2009 - 50% 
		& 0.07 & 10.4 & \textbf{0.15} 	 

		% lm_hc0 - 50% 
		& 0.81 & 89.6 & 1.15 	 

		% lm_hc30 - 50% 
		& 0.71 & \textbf{95.8} & 1.83 	 

	\\ & & 70	 & 10.75	 & 1.04

		% delta-h-c - 70% 
		& \textbf{0.95} & \textbf{100.0} & 1.15 	 

		% delta-h-c-uncertainty - 70% 
		& \textbf{0.95} & \textbf{100.0} & 1.15 	 

		% rg2009 - 70% 
		& 0.15 & 14.6 & \textbf{0.15} 	 

		% lm_hc0 - 70% 
		& 0.93 & \textbf{100.0} & 1.15 	 

		% lm_hc30 - 70% 
		& 0.81 & \textbf{100.0} & 1.42 	 

	\\ & & 100	 & 14.63	 & 1.0

		% delta-h-c - 100% 
		& \textbf{1.0} & \textbf{100.0} & 1.0 	 

		% delta-h-c-uncertainty - 100% 
		& \textbf{1.0} & \textbf{100.0} & 1.0 	 

		% rg2009 - 100% 
		& 0.08 & 8.3 & \textbf{0.08} 	 

		% lm_hc0 - 100% 
		& 0.99 & \textbf{100.0} & 1.02 	 

		% lm_hc30 - 100% 
		& 0.97 & \textbf{100.0} & 1.06 	 
 \\ \hline
\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{logistics}} } & \multirow{5}{*}{10.0} 
	 & 10	 & 3.0	 & 2.83

		% delta-h-c - 10% 
		& \textbf{0.58} & 94.4 & 2.72 	 

		% delta-h-c-uncertainty - 10% 
		& \textbf{0.58} & 94.4 & 2.78 	 

		% rg2009 - 10% 
		& 0.13 & 19.4 & \textbf{0.81} 	 

		% lm_hc0 - 10% 
		& 0.41 & 66.7 & 2.08 	 

		% lm_hc30 - 10% 
		& 0.29 & \textbf{97.2} & 9.47 	 

	\\ & & 30	 & 7.58	 & 1.19

		% delta-h-c - 30% 
		& 0.82 & 94.4 & 1.28 	 

		% delta-h-c-uncertainty - 30% 
		& \textbf{0.84} & \textbf{100.0} & 1.67 	 

		% rg2009 - 30% 
		& 0.06 & 5.6 & \textbf{0.14} 	 

		% lm_hc0 - 30% 
		& 0.78 & 91.7 & 1.36 	 

		% lm_hc30 - 30% 
		& 0.24 & \textbf{100.0} & 7.03 	 

	\\ & & 50	 & 11.42	 & 1.06

		% delta-h-c - 50% 
		& \textbf{0.9} & 97.2 & 1.11 	 

		% delta-h-c-uncertainty - 50% 
		& 0.88 & \textbf{100.0} & 1.28 	 

		% rg2009 - 50% 
		& 0.03 & 2.8 & \textbf{0.03} 	 

		% lm_hc0 - 50% 
		& 0.89 & 94.4 & 1.08 	 

		% lm_hc30 - 50% 
		& 0.31 & \textbf{100.0} & 4.47 	 

	\\ & & 70	 & 16.08	 & 1.03

		% delta-h-c - 70% 
		& \textbf{0.97} & \textbf{100.0} & 1.03 	 

		% delta-h-c-uncertainty - 70% 
		& 0.94 & \textbf{100.0} & 1.08 	 

		% rg2009 - 70% 
		& 0.03 & 2.8 & \textbf{0.03} 	 

		% lm_hc0 - 70% 
		& 0.94 & \textbf{100.0} & 1.08 	 

		% lm_hc30 - 70% 
		& 0.47 & \textbf{100.0} & 2.92 	 

	\\ & & 100	 & 22.0	 & 1.0

		% delta-h-c - 100% 
		& \textbf{1.0} & \textbf{100.0} & 1.0 	 

		% delta-h-c-uncertainty - 100% 
		& \textbf{1.0} & \textbf{100.0} & 1.0 	 

		% rg2009 - 100% 
		& 0.03 & 2.8 & \textbf{0.03} 	 

		% lm_hc0 - 100% 
		& \textbf{1.0} & \textbf{100.0} & 1.0 	 

		% lm_hc30 - 100% 
		& 0.64 & \textbf{100.0} & 1.89 	 
 \\ \hline
\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{miconic}} } & \multirow{5}{*}{6.0} 
	 & 10	 & 3.0	 & 2.53

		% delta-h-c - 10% 
		& 0.39 & 69.4 & 2.39 	 

		% delta-h-c-uncertainty - 10% 
		& 0.37 & 72.2 & 3.08 	 

		% rg2009 - 10% 
		& \textbf{0.46} & 86.1 & 3.31 	 

		% lm_hc0 - 10% 
		& 0.27 & 44.4 & \textbf{1.5} 	 

		% lm_hc30 - 10% 
		& 0.42 & \textbf{100.0} & 6.0 	 

	\\ & & 30	 & 6.83	 & 1.22

		% delta-h-c - 30% 
		& \textbf{0.57} & 80.6 & 1.44 	 

		% delta-h-c-uncertainty - 30% 
		& 0.43 & 83.3 & 2.22 	 

		% rg2009 - 30% 
		& 0.55 & 94.4 & 1.94 	 

		% lm_hc0 - 30% 
		& \textbf{0.57} & 69.4 & \textbf{1.17} 	 

		% lm_hc30 - 30% 
		& 0.23 & \textbf{100.0} & 5.42 	 

	\\ & & 50	 & 10.42	 & 1.06

		% delta-h-c - 50% 
		& \textbf{0.93} & \textbf{100.0} & 1.14 	 

		% delta-h-c-uncertainty - 50% 
		& 0.76 & \textbf{100.0} & 1.67 	 

		% rg2009 - 50% 
		& 0.87 & 97.2 & 1.22 	 

		% lm_hc0 - 50% 
		& 0.9 & 94.4 & \textbf{1.03} 	 

		% lm_hc30 - 50% 
		& 0.24 & \textbf{100.0} & 4.67 	 

	\\ & & 70	 & 14.83	 & 1.0

		% delta-h-c - 70% 
		& 0.94 & 97.2 & 1.08 	 

		% delta-h-c-uncertainty - 70% 
		& 0.78 & \textbf{100.0} & 1.53 	 

		% rg2009 - 70% 
		& 0.93 & \textbf{100.0} & 1.17 	 

		% lm_hc0 - 70% 
		& \textbf{0.96} & 97.2 & \textbf{1.03} 	 

		% lm_hc30 - 70% 
		& 0.32 & \textbf{100.0} & 4.03 	 

	\\ & & 100	 & 20.0	 & 1.0

		% delta-h-c - 100% 
		& 0.94 & 97.2 & 1.06 	 

		% delta-h-c-uncertainty - 100% 
		& 0.93 & 97.2 & 1.11 	 

		% rg2009 - 100% 
		& \textbf{1.0} & \textbf{100.0} & \textbf{1.0} 	 

		% lm_hc0 - 100% 
		& \textbf{1.0} & \textbf{100.0} & \textbf{1.0} 	 

		% lm_hc30 - 100% 
		& 0.37 & \textbf{100.0} & 3.39 	 
 \\ \hline
\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{rovers}} } & \multirow{5}{*}{6.0} 
	 & 10	 & 2.67	 & 2.28

		% delta-h-c - 10% 
		& \textbf{0.44} & 80.6 & 2.58 	 

		% delta-h-c-uncertainty - 10% 
		& \textbf{0.44} & 86.1 & 2.78 	 

		% rg2009 - 10% 
		& 0.18 & 47.2 & 1.33 	 

		% lm_hc0 - 10% 
		& 0.31 & 44.4 & \textbf{1.25} 	 

		% lm_hc30 - 10% 
		& 0.4 & \textbf{100.0} & 5.08 	 

	\\ & & 30	 & 4.67	 & 1.31

		% delta-h-c - 30% 
		& 0.7 & 83.3 & 1.36 	 

		% delta-h-c-uncertainty - 30% 
		& 0.68 & 91.7 & 1.69 	 

		% rg2009 - 30% 
		& 0.45 & 61.1 & 1.22 	 

		% lm_hc0 - 30% 
		& \textbf{0.75} & 86.1 & \textbf{1.19} 	 

		% lm_hc30 - 30% 
		& 0.35 & \textbf{100.0} & 4.31 	 

	\\ & & 50	 & 7.42	 & 1.19

		% delta-h-c - 50% 
		& \textbf{0.8} & 91.7 & 1.33 	 

		% delta-h-c-uncertainty - 50% 
		& 0.79 & 94.4 & 1.47 	 

		% rg2009 - 50% 
		& 0.31 & 41.7 & \textbf{0.61} 	 

		% lm_hc0 - 50% 
		& 0.71 & 80.6 & 1.11 	 

		% lm_hc30 - 50% 
		& 0.31 & \textbf{100.0} & 4.11 	 

	\\ & & 70	 & 10.17	 & 1.0

		% delta-h-c - 70% 
		& \textbf{0.93} & 97.2 & 1.08 	 

		% delta-h-c-uncertainty - 70% 
		& 0.89 & 97.2 & 1.17 	 

		% rg2009 - 70% 
		& 0.49 & 50.0 & \textbf{0.53} 	 

		% lm_hc0 - 70% 
		& 0.88 & 91.7 & 1.08 	 

		% lm_hc30 - 70% 
		& 0.34 & \textbf{100.0} & 3.44 	 

	\\ & & 100	 & 13.5	 & 1.0

		% delta-h-c - 100% 
		& \textbf{0.97} & \textbf{100.0} & 1.06 	 

		% delta-h-c-uncertainty - 100% 
		& \textbf{0.97} & \textbf{100.0} & 1.06 	 

		% rg2009 - 100% 
		& 0.39 & 38.9 & \textbf{0.39} 	 

		% lm_hc0 - 100% 
		& \textbf{0.97} & 97.2 & 1.0 	 

		% lm_hc30 - 100% 
		& 0.37 & \textbf{100.0} & 3.19 	 
 \\ \hline
\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{satellite}} } & \multirow{5}{*}{6.0} 
	 & 10	 & 2.42	 & 3.53

		% delta-h-c - 10% 
		& 0.53 & 75.0 & 3.31 	 

		% delta-h-c-uncertainty - 10% 
		& 0.51 & 77.8 & 3.64 	 

		% rg2009 - 10% 
		& 0.41 & 58.3 & 2.94 	 

		% lm_hc0 - 10% 
		& 0.34 & 50.0 & \textbf{2.28} 	 

		% lm_hc30 - 10% 
		& \textbf{0.6} & \textbf{100.0} & 5.75 	 

	\\ & & 30	 & 4.42	 & 2.39

		% delta-h-c - 30% 
		& 0.5 & 77.8 & 2.33 	 

		% delta-h-c-uncertainty - 30% 
		& \textbf{0.54} & 83.3 & 3.08 	 

		% rg2009 - 30% 
		& 0.4 & 80.6 & 2.78 	 

		% lm_hc0 - 30% 
		& 0.41 & 69.4 & \textbf{1.75} 	 

		% lm_hc30 - 30% 
		& 0.43 & \textbf{100.0} & 5.44 	 

	\\ & & 50	 & 7.17	 & 1.58

		% delta-h-c - 50% 
		& \textbf{0.67} & 88.9 & 1.89 	 

		% delta-h-c-uncertainty - 50% 
		& 0.57 & 91.7 & 2.53 	 

		% rg2009 - 50% 
		& 0.42 & 75.0 & 2.5 	 

		% lm_hc0 - 50% 
		& 0.49 & 72.2 & \textbf{1.5} 	 

		% lm_hc30 - 50% 
		& 0.3 & \textbf{100.0} & 5.42 	 

	\\ & & 70	 & 10.08	 & 1.31

		% delta-h-c - 70% 
		& \textbf{0.87} & 94.4 & 1.31 	 

		% delta-h-c-uncertainty - 70% 
		& 0.71 & 94.4 & 2.17 	 

		% rg2009 - 70% 
		& 0.67 & 77.8 & 1.47 	 

		% lm_hc0 - 70% 
		& 0.81 & 94.4 & \textbf{1.17} 	 

		% lm_hc30 - 70% 
		& 0.34 & \textbf{100.0} & 4.58 	 

	\\ & & 100	 & 13.17	 & 1.25

		% delta-h-c - 100% 
		& \textbf{0.92} & 97.2 & 1.31 	 

		% delta-h-c-uncertainty - 100% 
		& 0.88 & 97.2 & 1.39 	 

		% rg2009 - 100% 
		& 0.69 & 77.8 & 1.31 	 

		% lm_hc0 - 100% 
		& 0.88 & \textbf{100.0} & \textbf{1.22} 	 

		% lm_hc30 - 100% 
		& 0.46 & \textbf{100.0} & 3.78 	 
 \\ \hline
\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{sokoban}} } & \multirow{5}{*}{8.5} 
	 & 10	 & 3.33	 & 2.11

		% delta-h-c - 10% 
		& 0.27 & 58.3 & 2.78 	 

		% delta-h-c-uncertainty - 10% 
		& \textbf{0.29} & 83.3 & 4.36 	 

		% rg2009 - 10% 
		& 0.1 & 30.6 & 1.83 	 

		% lm_hc0 - 10% 
		& 0.24 & 41.7 & \textbf{1.42} 	 

		% lm_hc30 - 10% 
		& 0.27 & \textbf{97.2} & 5.61 	 

	\\ & & 30	 & 8.17	 & 1.25

		% delta-h-c - 30% 
		& \textbf{0.56} & 77.8 & 2.17 	 

		% delta-h-c-uncertainty - 30% 
		& 0.41 & \textbf{97.2} & 4.42 	 

		% rg2009 - 30% 
		& 0.2 & 30.6 & \textbf{1.0} 	 

		% lm_hc0 - 30% 
		& 0.34 & 41.7 & 1.28 	 

		% lm_hc30 - 30% 
		& 0.2 & 94.4 & 5.58 	 

	\\ & & 50	 & 12.67	 & 1.22

		% delta-h-c - 50% 
		& \textbf{0.61} & 94.4 & 2.97 	 

		% delta-h-c-uncertainty - 50% 
		& 0.47 & \textbf{97.2} & 4.11 	 

		% rg2009 - 50% 
		& 0.2 & 30.6 & \textbf{0.75} 	 

		% lm_hc0 - 50% 
		& 0.57 & 66.7 & 1.28 	 

		% lm_hc30 - 50% 
		& 0.27 & \textbf{97.2} & 4.94 	 

	\\ & & 70	 & 18.0	 & 1.03

		% delta-h-c - 70% 
		& 0.6 & 94.4 & 3.75 	 

		% delta-h-c-uncertainty - 70% 
		& 0.5 & 94.4 & 4.42 	 

		% rg2009 - 70% 
		& 0.08 & 11.1 & \textbf{0.19} 	 

		% lm_hc0 - 70% 
		& \textbf{0.84} & 94.4 & 1.28 	 

		% lm_hc30 - 70% 
		& 0.33 & \textbf{100.0} & 4.0 	 

	\\ & & 100	 & 24.67	 & 1.0

		% delta-h-c - 100% 
		& 0.66 & \textbf{100.0} & 3.89 	 

		% delta-h-c-uncertainty - 100% 
		& 0.55 & \textbf{100.0} & 4.28 	 

		% rg2009 - 100% 
		& 0.04 & 5.6 & \textbf{0.08} 	 

		% lm_hc0 - 100% 
		& \textbf{0.96} & \textbf{100.0} & 1.08 	 

		% lm_hc30 - 100% 
		& 0.38 & \textbf{100.0} & 3.28 	 
 \\ \hline
Avg & & & &  & \textbf{0.72} & 89.48 & 1.97 & 0.67 & 93.23 & 2.64 & 0.37 & 50.06 & 1.45 & 0.65 & 76.83 & \textbf{1.3} & 0.39 & \textbf{98.93} & 5.59
\\ \hline
\end{tabular}


==> tables/previous-optimal.tex <==
\begin{tabular}{|c|c|ccc|ccc|ccc|ccc|ccc|ccc|}
\hline
% empty
& % empty
& \multicolumn{3}{c|}{}
& \multicolumn{3}{c|}{\hdeltahc}
& \multicolumn{3}{c|}{\hdeltahcu}
& \multicolumn{3}{c|}{\rg}		   
& \multicolumn{3}{c|}{\completion}
& \multicolumn{3}{c|}{\completion{} 0.3}
\\ \hline
& $\goalconditions$ & \textbf{\%} & $\observations$ & $\grsolution$ 
& \textbf{Agr} & \textbf{Acc} & \textbf{Spr}
& \textbf{Agr} & \textbf{Acc} & \textbf{Spr}
& \textbf{Agr} & \textbf{Acc} & \textbf{Spr}
& \textbf{Agr} & \textbf{Acc} & \textbf{Spr}
& \textbf{Agr} & \textbf{Acc} & \textbf{Spr}
\\ 
\hline

\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{blocks}} } & \multirow{5}{*}{20} 
	 & 10	 & 1.25	 & 7.9

		% delta-h-c - 10% 
		& 0.44 & 86.1 & 7.53 	 

		% delta-h-c-uncertainty - 10% 
		& 0.44 & 86.1 & 7.56 	 

		% rg2009 - 10% 
		& \textbf{0.47} & 91.7 & 9.83 	 

		% lm_hc0 - 10% 
		& 0.06 & 16.7 & \textbf{1.44} 	 

		% lm_hc30 - 10% 
		& 0.38 & \textbf{100.0} & 18.14 	 

	\\ & & 30	 & 3.08	 & 3.91

		% delta-h-c - 30% 
		& \textbf{0.46} & 77.8 & 2.5 	 

		% delta-h-c-uncertainty - 30% 
		& 0.44 & 86.1 & 4.67 	 

		% rg2009 - 30% 
		& 0.45 & 91.7 & 5.56 	 

		% lm_hc0 - 30% 
		& 0.21 & 38.9 & \textbf{1.17} 	 

		% lm_hc30 - 30% 
		& 0.24 & \textbf{100.0} & 15.25 	 

	\\ & & 50	 & 4.42	 & 2.48

		% delta-h-c - 50% 
		& 0.59 & 88.9 & 3.03 	 

		% delta-h-c-uncertainty - 50% 
		& 0.52 & 88.9 & 3.86 	 

		% rg2009 - 50% 
		& \textbf{0.62} & \textbf{97.2} & 3.69 	 

		% lm_hc0 - 50% 
		& 0.33 & 58.3 & \textbf{1.25} 	 

		% lm_hc30 - 50% 
		& 0.25 & \textbf{97.2} & 12.17 	 

	\\ & & 70	 & 6.67	 & 1.94

		% delta-h-c - 70% 
		& \textbf{0.85} & 97.2 & 1.83 	 

		% delta-h-c-uncertainty - 70% 
		& 0.76 & 97.2 & 2.42 	 

		% rg2009 - 70% 
		& 0.81 & \textbf{100.0} & 2.22 	 

		% lm_hc0 - 70% 
		& 0.51 & 72.2 & \textbf{1.14} 	 

		% lm_hc30 - 70% 
		& 0.25 & \textbf{100.0} & 9.22 	 

	\\ & & 100	 & 8.83	 & 1.83

		% delta-h-c - 100% 
		& \textbf{0.92} & \textbf{100.0} & \textbf{1.67} 	 

		% delta-h-c-uncertainty - 100% 
		& \textbf{0.92} & \textbf{100.0} & \textbf{1.67} 	 

		% rg2009 - 100% 
		& 0.9 & \textbf{100.0} & 2.08 	 

		% lm_hc0 - 100% 
		& 0.59 & \textbf{100.0} & \textbf{1.67} 	 

		% lm_hc30 - 100% 
		& 0.31 & \textbf{100.0} & 6.42 	 
 \\ \hline
\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{ipc-grid}} } & \multirow{5}{*}{7.5} 
	 & 10	 & 1.63	 & 2.71

		% delta-h-c - 10% 
		& 0.87 & 93.8 & 2.67 	 

		% delta-h-c-uncertainty - 10% 
		& 0.88 & 95.8 & 2.69 	 

		% rg2009 - 10% 
		& \textbf{0.91} & \textbf{100.0} & 3.23 	 

		% lm_hc0 - 10% 
		& 0.47 & 75.0 & \textbf{2.35} 	 

		% lm_hc30 - 10% 
		& 0.49 & \textbf{100.0} & 6.25 	 

	\\ & & 30	 & 4.0	 & 1.21

		% delta-h-c - 30% 
		& 0.93 & 95.8 & \textbf{1.15} 	 

		% delta-h-c-uncertainty - 30% 
		& 0.94 & 97.9 & 1.17 	 

		% rg2009 - 30% 
		& \textbf{0.99} & \textbf{100.0} & 1.25 	 

		% lm_hc0 - 30% 
		& 0.85 & 97.9 & 1.52 	 

		% lm_hc30 - 30% 
		& 0.64 & \textbf{100.0} & 3.17 	 

	\\ & & 50	 & 6.19	 & 1.13

		% delta-h-c - 50% 
		& 0.96 & 97.9 & \textbf{1.08} 	 

		% delta-h-c-uncertainty - 50% 
		& 0.96 & 97.9 & \textbf{1.08} 	 

		% rg2009 - 50% 
		& \textbf{1.0} & \textbf{100.0} & 1.13 	 

		% lm_hc0 - 50% 
		& 0.86 & \textbf{100.0} & 1.44 	 

		% lm_hc30 - 50% 
		& 0.77 & \textbf{100.0} & 2.15 	 

	\\ & & 70	 & 8.69	 & 1.04

		% delta-h-c - 70% 
		& 0.97 & 97.9 & 1.06 	 

		% delta-h-c-uncertainty - 70% 
		& 0.97 & 97.9 & 1.06 	 

		% rg2009 - 70% 
		& \textbf{1.0} & \textbf{100.0} & 1.04 	 

		% lm_hc0 - 70% 
		& 0.97 & 97.9 & \textbf{1.02} 	 

		% lm_hc30 - 70% 
		& 0.93 & 97.9 & 1.15 	 

	\\ & & 100	 & 11.88	 & 1.0

		% delta-h-c - 100% 
		& \textbf{1.0} & \textbf{100.0} & \textbf{1.0} 	 

		% delta-h-c-uncertainty - 100% 
		& \textbf{1.0} & \textbf{100.0} & \textbf{1.0} 	 

		% rg2009 - 100% 
		& \textbf{1.0} & \textbf{100.0} & \textbf{1.0} 	 

		% lm_hc0 - 100% 
		& \textbf{1.0} & \textbf{100.0} & \textbf{1.0} 	 

		% lm_hc30 - 100% 
		& \textbf{1.0} & \textbf{100.0} & \textbf{1.0} 	 
 \\ \hline
\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{logistics}} } & \multirow{5}{*}{10} 
	 & 10	 & 2.0	 & 2.83

		% delta-h-c - 10% 
		& \textbf{0.9} & \textbf{100.0} & 3.53 	 

		% delta-h-c-uncertainty - 10% 
		& \textbf{0.9} & \textbf{100.0} & 3.53 	 

		% rg2009 - 10% 
		& 0.87 & \textbf{100.0} & 3.78 	 

		% lm_hc0 - 10% 
		& 0.43 & 58.3 & \textbf{2.11} 	 

		% lm_hc30 - 10% 
		& 0.31 & \textbf{100.0} & 9.53 	 

	\\ & & 30	 & 5.75	 & 1.19

		% delta-h-c - 30% 
		& \textbf{0.92} & \textbf{100.0} & 1.47 	 

		% delta-h-c-uncertainty - 30% 
		& \textbf{0.92} & \textbf{100.0} & 1.47 	 

		% rg2009 - 30% 
		& 0.86 & \textbf{100.0} & 1.75 	 

		% lm_hc0 - 30% 
		& 0.78 & 86.1 & \textbf{1.33} 	 

		% lm_hc30 - 30% 
		& 0.24 & \textbf{100.0} & 6.58 	 

	\\ & & 50	 & 9.42	 & 1.06

		% delta-h-c - 50% 
		& \textbf{0.96} & \textbf{100.0} & \textbf{1.17} 	 

		% delta-h-c-uncertainty - 50% 
		& \textbf{0.96} & \textbf{100.0} & \textbf{1.17} 	 

		% rg2009 - 50% 
		& 0.93 & \textbf{100.0} & 1.25 	 

		% lm_hc0 - 50% 
		& 0.9 & 94.4 & \textbf{1.17} 	 

		% lm_hc30 - 50% 
		& 0.39 & \textbf{100.0} & 4.36 	 

	\\ & & 70	 & 13.25	 & 1.03

		% delta-h-c - 70% 
		& 0.99 & \textbf{100.0} & 1.06 	 

		% delta-h-c-uncertainty - 70% 
		& 0.99 & \textbf{100.0} & 1.06 	 

		% rg2009 - 70% 
		& 0.99 & \textbf{100.0} & 1.06 	 

		% lm_hc0 - 70% 
		& \textbf{1.0} & \textbf{100.0} & \textbf{1.03} 	 

		% lm_hc30 - 70% 
		& 0.62 & \textbf{100.0} & 2.19 	 

	\\ & & 100	 & 18.17	 & 1.0

		% delta-h-c - 100% 
		& \textbf{1.0} & \textbf{100.0} & \textbf{1.0} 	 

		% delta-h-c-uncertainty - 100% 
		& \textbf{1.0} & \textbf{100.0} & \textbf{1.0} 	 

		% rg2009 - 100% 
		& \textbf{1.0} & \textbf{100.0} & \textbf{1.0} 	 

		% lm_hc0 - 100% 
		& \textbf{1.0} & \textbf{100.0} & \textbf{1.0} 	 

		% lm_hc30 - 100% 
		& 0.72 & \textbf{100.0} & 1.67 	 
 \\ \hline
\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{miconic}} } & \multirow{5}{*}{6.0} 
	 & 10	 & 2.0	 & 2.53

		% delta-h-c - 10% 
		& \textbf{0.89} & \textbf{100.0} & 2.97 	 

		% delta-h-c-uncertainty - 10% 
		& \textbf{0.89} & \textbf{100.0} & 2.97 	 

		% rg2009 - 10% 
		& 0.76 & \textbf{100.0} & 3.53 	 

		% lm_hc0 - 10% 
		& 0.39 & 52.8 & \textbf{1.69} 	 

		% lm_hc30 - 10% 
		& 0.42 & \textbf{100.0} & 6.0 	 

	\\ & & 30	 & 5.42	 & 1.22

		% delta-h-c - 30% 
		& \textbf{0.95} & \textbf{100.0} & 1.36 	 

		% delta-h-c-uncertainty - 30% 
		& \textbf{0.95} & \textbf{100.0} & 1.36 	 

		% rg2009 - 30% 
		& 0.65 & \textbf{100.0} & 2.17 	 

		% lm_hc0 - 30% 
		& 0.83 & 88.9 & \textbf{1.19} 	 

		% lm_hc30 - 30% 
		& 0.22 & \textbf{100.0} & 5.69 	 

	\\ & & 50	 & 8.42	 & 1.06

		% delta-h-c - 50% 
		& \textbf{0.97} & \textbf{100.0} & 1.11 	 

		% delta-h-c-uncertainty - 50% 
		& \textbf{0.97} & \textbf{100.0} & 1.11 	 

		% rg2009 - 50% 
		& 0.84 & \textbf{100.0} & 1.42 	 

		% lm_hc0 - 50% 
		& 0.92 & 94.4 & \textbf{1.06} 	 

		% lm_hc30 - 50% 
		& 0.25 & \textbf{100.0} & 4.69 	 

	\\ & & 70	 & 11.92	 & 1.0

		% delta-h-c - 70% 
		& 0.98 & \textbf{100.0} & 1.06 	 

		% delta-h-c-uncertainty - 70% 
		& 0.98 & \textbf{100.0} & 1.06 	 

		% rg2009 - 70% 
		& 0.91 & \textbf{100.0} & 1.19 	 

		% lm_hc0 - 70% 
		& \textbf{0.99} & \textbf{100.0} & \textbf{1.03} 	 

		% lm_hc30 - 70% 
		& 0.31 & \textbf{100.0} & 3.94 	 

	\\ & & 100	 & 16.33	 & 1.0

		% delta-h-c - 100% 
		& \textbf{1.0} & \textbf{100.0} & \textbf{1.0} 	 

		% delta-h-c-uncertainty - 100% 
		& \textbf{1.0} & \textbf{100.0} & \textbf{1.0} 	 

		% rg2009 - 100% 
		& \textbf{1.0} & \textbf{100.0} & \textbf{1.0} 	 

		% lm_hc0 - 100% 
		& \textbf{1.0} & \textbf{100.0} & \textbf{1.0} 	 

		% lm_hc30 - 100% 
		& 0.47 & \textbf{100.0} & 3.0 	 
 \\ \hline
\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{rovers}} } & \multirow{5}{*}{6.0} 
	 & 10	 & 1.67	 & 2.28

		% delta-h-c - 10% 
		& \textbf{0.83} & 97.2 & 2.75 	 

		% delta-h-c-uncertainty - 10% 
		& \textbf{0.83} & 97.2 & 2.75 	 

		% rg2009 - 10% 
		& 0.76 & \textbf{100.0} & 3.42 	 

		% lm_hc0 - 10% 
		& 0.49 & 52.8 & \textbf{1.22} 	 

		% lm_hc30 - 10% 
		& 0.44 & \textbf{100.0} & 5.28 	 

	\\ & & 30	 & 3.67	 & 1.31

		% delta-h-c - 30% 
		& \textbf{0.94} & \textbf{100.0} & 1.44 	 

		% delta-h-c-uncertainty - 30% 
		& \textbf{0.94} & \textbf{100.0} & 1.44 	 

		% rg2009 - 30% 
		& 0.88 & \textbf{100.0} & 1.69 	 

		% lm_hc0 - 30% 
		& 0.76 & 83.3 & \textbf{1.19} 	 

		% lm_hc30 - 30% 
		& 0.37 & \textbf{100.0} & 3.89 	 

	\\ & & 50	 & 5.75	 & 1.19

		% delta-h-c - 50% 
		& \textbf{0.92} & 88.9 & \textbf{1.08} 	 

		% delta-h-c-uncertainty - 50% 
		& \textbf{0.92} & 88.9 & \textbf{1.08} 	 

		% rg2009 - 50% 
		& 0.91 & \textbf{100.0} & 1.42 	 

		% lm_hc0 - 50% 
		& 0.79 & 88.9 & 1.14 	 

		% lm_hc30 - 50% 
		& 0.39 & \textbf{100.0} & 3.67 	 

	\\ & & 70	 & 8.17	 & 1.0

		% delta-h-c - 70% 
		& \textbf{0.99} & \textbf{100.0} & \textbf{1.03} 	 

		% delta-h-c-uncertainty - 70% 
		& \textbf{0.99} & \textbf{100.0} & \textbf{1.03} 	 

		% rg2009 - 70% 
		& 0.97 & \textbf{100.0} & 1.08 	 

		% lm_hc0 - 70% 
		& 0.93 & 97.2 & 1.11 	 

		% lm_hc30 - 70% 
		& 0.37 & \textbf{100.0} & 3.44 	 

	\\ & & 100	 & 10.83	 & 1.0

		% delta-h-c - 100% 
		& \textbf{1.0} & \textbf{100.0} & \textbf{1.0} 	 

		% delta-h-c-uncertainty - 100% 
		& \textbf{1.0} & \textbf{100.0} & \textbf{1.0} 	 

		% rg2009 - 100% 
		& \textbf{1.0} & \textbf{100.0} & \textbf{1.0} 	 

		% lm_hc0 - 100% 
		& \textbf{1.0} & \textbf{100.0} & \textbf{1.0} 	 

		% lm_hc30 - 100% 
		& 0.39 & \textbf{100.0} & 3.0 	 
 \\ \hline
\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{satellite}} } & \multirow{5}{*}{6.0} 
	 & 10	 & 1.42	 & 3.53

		% delta-h-c - 10% 
		& 0.85 & 94.4 & 3.81 	 

		% delta-h-c-uncertainty - 10% 
		& 0.85 & 94.4 & 3.81 	 

		% rg2009 - 10% 
		& \textbf{0.86} & 97.2 & 3.89 	 

		% lm_hc0 - 10% 
		& 0.5 & 58.3 & \textbf{2.11} 	 

		% lm_hc30 - 10% 
		& 0.59 & \textbf{100.0} & 5.94 	 

	\\ & & 30	 & 3.42	 & 2.39

		% delta-h-c - 30% 
		& \textbf{0.86} & 91.7 & 2.44 	 

		% delta-h-c-uncertainty - 30% 
		& \textbf{0.86} & 91.7 & 2.44 	 

		% rg2009 - 30% 
		& 0.72 & 94.4 & 3.44 	 

		% lm_hc0 - 30% 
		& 0.64 & 83.3 & \textbf{2.03} 	 

		% lm_hc30 - 30% 
		& 0.44 & \textbf{100.0} & 5.39 	 

	\\ & & 50	 & 5.75	 & 1.58

		% delta-h-c - 50% 
		& \textbf{0.93} & 97.2 & 1.53 	 

		% delta-h-c-uncertainty - 50% 
		& 0.91 & 97.2 & 1.58 	 

		% rg2009 - 50% 
		& 0.79 & 94.4 & 2.25 	 

		% lm_hc0 - 50% 
		& 0.73 & 88.9 & \textbf{1.28} 	 

		% lm_hc30 - 50% 
		& 0.35 & \textbf{100.0} & 4.81 	 

	\\ & & 70	 & 8.08	 & 1.31

		% delta-h-c - 70% 
		& \textbf{0.94} & \textbf{100.0} & 1.28 	 

		% delta-h-c-uncertainty - 70% 
		& \textbf{0.94} & \textbf{100.0} & 1.28 	 

		% rg2009 - 70% 
		& 0.81 & 97.2 & 2.06 	 

		% lm_hc0 - 70% 
		& 0.89 & \textbf{100.0} & \textbf{1.19} 	 

		% lm_hc30 - 70% 
		& 0.37 & \textbf{100.0} & 4.06 	 

	\\ & & 100	 & 10.75	 & 1.25

		% delta-h-c - 100% 
		& \textbf{0.96} & \textbf{100.0} & \textbf{1.17} 	 

		% delta-h-c-uncertainty - 100% 
		& \textbf{0.96} & \textbf{100.0} & \textbf{1.17} 	 

		% rg2009 - 100% 
		& 0.88 & \textbf{100.0} & 1.75 	 

		% lm_hc0 - 100% 
		& 0.88 & \textbf{100.0} & \textbf{1.17} 	 

		% lm_hc30 - 100% 
		& 0.5 & \textbf{100.0} & 3.33 	 
 \\ \hline
\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{sokoban}} } & \multirow{5}{*}{8.5} 
	 & 10	 & 2.33	 & 2.11

		% delta-h-c - 10% 
		& 0.39 & 52.8 & \textbf{2.08} 	 

		% delta-h-c-uncertainty - 10% 
		& 0.38 & 61.1 & 2.94 	 

		% rg2009 - 10% 
		& \textbf{0.4} & 80.6 & 4.86 	 

		% lm_hc0 - 10% 
		& 0.28 & 52.8 & 2.14 	 

		% lm_hc30 - 10% 
		& 0.26 & \textbf{97.2} & 7.0 	 

	\\ & & 30	 & 6.5	 & 1.25

		% delta-h-c - 30% 
		& \textbf{0.75} & 80.6 & 1.25 	 

		% delta-h-c-uncertainty - 30% 
		& 0.64 & 91.7 & 2.06 	 

		% rg2009 - 30% 
		& 0.56 & 86.1 & 2.53 	 

		% lm_hc0 - 30% 
		& 0.57 & 69.4 & \textbf{1.22} 	 

		% lm_hc30 - 30% 
		& 0.23 & \textbf{94.4} & 5.17 	 

	\\ & & 50	 & 10.33	 & 1.22

		% delta-h-c - 50% 
		& \textbf{0.92} & \textbf{100.0} & \textbf{1.19} 	 

		% delta-h-c-uncertainty - 50% 
		& 0.83 & \textbf{100.0} & 1.39 	 

		% rg2009 - 50% 
		& 0.61 & 86.1 & 2.14 	 

		% lm_hc0 - 50% 
		& 0.61 & 69.4 & 1.42 	 

		% lm_hc30 - 50% 
		& 0.28 & \textbf{100.0} & 5.08 	 

	\\ & & 70	 & 14.67	 & 1.03

		% delta-h-c - 70% 
		& \textbf{0.99} & \textbf{100.0} & \textbf{1.0} 	 

		% delta-h-c-uncertainty - 70% 
		& 0.94 & \textbf{100.0} & 1.08 	 

		% rg2009 - 70% 
		& 0.64 & 83.3 & 1.53 	 

		% lm_hc0 - 70% 
		& 0.85 & 91.7 & 1.17 	 

		% lm_hc30 - 70% 
		& 0.36 & \textbf{100.0} & 3.64 	 

	\\ & & 100	 & 20.17	 & 1.0

		% delta-h-c - 100% 
		& \textbf{1.0} & \textbf{100.0} & \textbf{1.0} 	 

		% delta-h-c-uncertainty - 100% 
		& \textbf{1.0} & \textbf{100.0} & \textbf{1.0} 	 

		% rg2009 - 100% 
		& 0.67 & 75.0 & 1.17 	 

		% lm_hc0 - 100% 
		& \textbf{1.0} & \textbf{100.0} & \textbf{1.0} 	 

		% lm_hc30 - 100% 
		& 0.42 & \textbf{100.0} & 2.75 	 
 \\ \hline
Av & & & &  & \textbf{0.88} & 95.38 & 1.81 & 0.87 & 96.29 & 1.97 & 0.81 & 96.43 & 2.38 & 0.71 & 81.94 & \textbf{1.34} & 0.43 & \textbf{99.62} & 5.4
\\ \hline
\end{tabular}

==> tables/previous-suboptimal-noisy.tex <==
\begin{tabular}{|c|c|ccc|ccc|ccc|ccc|ccc|ccc|}
\hline
% empty
& % empty
& \multicolumn{3}{c|}{}
& \multicolumn{3}{c|}{\hdeltahc}
& \multicolumn{3}{c|}{\hdeltahcu}
& \multicolumn{3}{c|}{\rg}		   
& \multicolumn{3}{c|}{\completion}
& \multicolumn{3}{c|}{\completion 0.3}
\\ \hline
\# & $|\goalconditions|$ & \textbf{\% Obs} & $|\observations|$ & $|\grsolution|$ 
& \textbf{AGR} & \textbf{ACC} & \textbf{$|\Gamma^\textup{h}|$}
& \textbf{AGR} & \textbf{ACC} & \textbf{$|\Gamma^\textup{h}|$}
& \textbf{AGR} & \textbf{ACC} & \textbf{$|\Gamma^\textup{h}|$}
& \textbf{AGR} & \textbf{ACC} & \textbf{$|\Gamma^\textup{h}|$}
& \textbf{AGR} & \textbf{ACC} & \textbf{$|\Gamma^\textup{h}|$}
\\ 
\hline

\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{blocks}} } & \multirow{5}{*}{20.1} 
	 & 10	 & 2.42	 & 7.49

		% delta-h-c - 10% 
		& 0.38 & 69.4 & 6.58 	 

		% delta-h-c-uncertainty - 10% 
		& \textbf{0.42} & 88.9 & 12.72 	 

		% rg2009 - 10% 
		& \textbf{0.42} & 88.9 & 8.97 	 

		% lm_hc0 - 10% 
		& 0.05 & 5.6 & \textbf{1.28} 	 

		% lm_hc30 - 10% 
		& 0.36 & \textbf{94.4} & 16.42 	 

	\\ & & 30	 & 4.92	 & 3.55

		% delta-h-c - 30% 
		& 0.36 & 63.9 & 3.47 	 

		% delta-h-c-uncertainty - 30% 
		& 0.34 & 91.7 & 11.33 	 

		% rg2009 - 30% 
		& \textbf{0.49} & 91.7 & 5.47 	 

		% lm_hc0 - 30% 
		& 0.22 & 47.2 & \textbf{1.22} 	 

		% lm_hc30 - 30% 
		& 0.23 & \textbf{100.0} & 15.5 	 

	\\ & & 50	 & 7.33	 & 3.18

		% delta-h-c - 50% 
		& 0.53 & 83.3 & 2.64 	 

		% delta-h-c-uncertainty - 50% 
		& 0.33 & 97.2 & 7.64 	 

		% rg2009 - 50% 
		& \textbf{0.55} & 94.4 & 2.72 	 

		% lm_hc0 - 50% 
		& 0.28 & 58.3 & \textbf{1.25} 	 

		% lm_hc30 - 50% 
		& 0.23 & \textbf{100.0} & 11.58 	 

	\\ & & 70	 & 10.67	 & 2.53

		% delta-h-c - 70% 
		& \textbf{0.67} & 88.9 & 2.22 	 

		% delta-h-c-uncertainty - 70% 
		& 0.45 & \textbf{100.0} & 5.56 	 

		% rg2009 - 70% 
		& 0.63 & 86.1 & 2.47 	 

		% lm_hc0 - 70% 
		& 0.38 & 72.2 & \textbf{1.19} 	 

		% lm_hc30 - 70% 
		& 0.23 & \textbf{100.0} & 10.33 	 

	\\ & & 100	 & 14.42	 & 2.25

		% delta-h-c - 100% 
		& \textbf{0.78} & 91.7 & \textbf{1.53} 	 

		% delta-h-c-uncertainty - 100% 
		& 0.7 & 97.2 & 2.17 	 

		% rg2009 - 100% 
		& 0.74 & 91.7 & 1.97 	 

		% lm_hc0 - 100% 
		& 0.51 & \textbf{100.0} & 1.72 	 

		% lm_hc30 - 100% 
		& 0.24 & \textbf{100.0} & 8.64 	 
 \\ \hline
\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{ipc-grid}} } & \multirow{5}{*}{7.5} 
	 & 10	 & 3.06	 & 1.58

		% delta-h-c - 10% 
		& \textbf{0.62} & 89.6 & 2.1 	 

		% delta-h-c-uncertainty - 10% 
		& 0.53 & \textbf{93.8} & 2.96 	 

		% rg2009 - 10% 
		& 0.12 & 18.8 & \textbf{0.44} 	 

		% lm_hc0 - 10% 
		& 0.54 & 70.8 & 1.58 	 

		% lm_hc30 - 10% 
		& 0.41 & 89.6 & 4.21 	 

	\\ & & 30	 & 7.13	 & 1.4

		% delta-h-c - 30% 
		& 0.68 & 89.6 & 1.44 	 

		% delta-h-c-uncertainty - 30% 
		& 0.55 & \textbf{93.8} & 2.08 	 

		% rg2009 - 30% 
		& 0.08 & 14.6 & \textbf{0.29} 	 

		% lm_hc0 - 30% 
		& \textbf{0.72} & 87.5 & 1.25 	 

		% lm_hc30 - 30% 
		& 0.61 & \textbf{93.8} & 2.44 	 

	\\ & & 50	 & 10.94	 & 1.35

		% delta-h-c - 50% 
		& 0.84 & 95.8 & 1.06 	 

		% delta-h-c-uncertainty - 50% 
		& 0.79 & \textbf{97.9} & 1.48 	 

		% rg2009 - 50% 
		& 0.04 & 4.2 & \textbf{0.04} 	 

		% lm_hc0 - 50% 
		& \textbf{0.85} & 95.8 & 1.04 	 

		% lm_hc30 - 50% 
		& 0.74 & 95.8 & 1.35 	 

	\\ & & 70	 & 15.56	 & 1.31

		% delta-h-c - 70% 
		& 0.89 & \textbf{100.0} & 1.06 	 

		% delta-h-c-uncertainty - 70% 
		& 0.87 & \textbf{100.0} & 1.15 	 

		% rg2009 - 70% 
		& 0.02 & 2.1 & \textbf{0.02} 	 

		% lm_hc0 - 70% 
		& \textbf{0.9} & 97.9 & 1.0 	 

		% lm_hc30 - 70% 
		& 0.86 & \textbf{100.0} & 1.15 	 

	\\ & & 100	 & 21.13	 & 1.5

		% delta-h-c - 100% 
		& \textbf{0.94} & \textbf{100.0} & 1.0 	 

		% delta-h-c-uncertainty - 100% 
		& \textbf{0.94} & \textbf{100.0} & 1.0 	 

		% rg2009 - 100% 
		& 0.04 & 4.2 & \textbf{0.04} 	 

		% lm_hc0 - 100% 
		& 0.92 & \textbf{100.0} & 1.04 	 

		% lm_hc30 - 100% 
		& 0.89 & \textbf{100.0} & 1.13 	 
 \\ \hline
\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{logistics}} } & \multirow{5}{*}{10.0} 
	 & 10	 & 3.67	 & 2.0

		% delta-h-c - 10% 
		& \textbf{0.55} & 88.9 & 2.36 	 

		% delta-h-c-uncertainty - 10% 
		& 0.51 & 88.9 & 2.94 	 

		% rg2009 - 10% 
		& 0.28 & 47.2 & \textbf{1.36} 	 

		% lm_hc0 - 10% 
		& 0.41 & 55.6 & 1.42 	 

		% lm_hc30 - 10% 
		& 0.21 & \textbf{100.0} & 9.58 	 

	\\ & & 30	 & 9.33	 & 1.14

		% delta-h-c - 30% 
		& 0.8 & \textbf{100.0} & 1.33 	 

		% delta-h-c-uncertainty - 30% 
		& 0.7 & \textbf{100.0} & 1.94 	 

		% rg2009 - 30% 
		& 0.12 & 13.9 & \textbf{0.19} 	 

		% lm_hc0 - 30% 
		& \textbf{0.81} & 88.9 & 1.08 	 

		% lm_hc30 - 30% 
		& 0.24 & \textbf{100.0} & 5.78 	 

	\\ & & 50	 & 14.58	 & 1.06

		% delta-h-c - 50% 
		& \textbf{0.91} & \textbf{100.0} & 1.22 	 

		% delta-h-c-uncertainty - 50% 
		& 0.7 & \textbf{100.0} & 2.08 	 

		% rg2009 - 50% 
		& 0.03 & 2.8 & \textbf{0.03} 	 

		% lm_hc0 - 50% 
		& 0.9 & 94.4 & 1.03 	 

		% lm_hc30 - 50% 
		& 0.38 & \textbf{100.0} & 3.94 	 

	\\ & & 70	 & 20.17	 & 1.03

		% delta-h-c - 70% 
		& 0.96 & \textbf{100.0} & 1.06 	 

		% delta-h-c-uncertainty - 70% 
		& 0.84 & \textbf{100.0} & 1.36 	 

		% rg2009 - 70% 
		& 0.0 & 0.0 & \textbf{0.0} 	 

		% lm_hc0 - 70% 
		& \textbf{0.99} & \textbf{100.0} & 1.0 	 

		% lm_hc30 - 70% 
		& 0.56 & \textbf{100.0} & 2.47 	 

	\\ & & 100	 & 28.17	 & 1.0

		% delta-h-c - 100% 
		& \textbf{1.0} & \textbf{100.0} & 1.0 	 

		% delta-h-c-uncertainty - 100% 
		& \textbf{1.0} & \textbf{100.0} & 1.0 	 

		% rg2009 - 100% 
		& 0.0 & 0.0 & \textbf{0.0} 	 

		% lm_hc0 - 100% 
		& \textbf{1.0} & \textbf{100.0} & 1.0 	 

		% lm_hc30 - 100% 
		& 0.63 & \textbf{100.0} & 2.06 	 
 \\ \hline
\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{miconic}} } & \multirow{5}{*}{6.0} 
	 & 10	 & 4.0	 & 1.83

		% delta-h-c - 10% 
		& 0.43 & 80.6 & 2.11 	 

		% delta-h-c-uncertainty - 10% 
		& 0.41 & 83.3 & 2.89 	 

		% rg2009 - 10% 
		& \textbf{0.47} & 91.7 & 3.22 	 

		% lm_hc0 - 10% 
		& 0.35 & 61.1 & \textbf{1.5} 	 

		% lm_hc30 - 10% 
		& 0.31 & \textbf{100.0} & 5.97 	 

	\\ & & 30	 & 9.67	 & 1.25

		% delta-h-c - 30% 
		& \textbf{0.75} & 88.9 & 1.36 	 

		% delta-h-c-uncertainty - 30% 
		& 0.36 & \textbf{100.0} & 3.69 	 

		% rg2009 - 30% 
		& 0.64 & 94.4 & 1.97 	 

		% lm_hc0 - 30% 
		& 0.69 & 86.1 & \textbf{1.33} 	 

		% lm_hc30 - 30% 
		& 0.22 & \textbf{100.0} & 5.5 	 

	\\ & & 50	 & 15.25	 & 1.03

		% delta-h-c - 50% 
		& 0.86 & 94.4 & 1.14 	 

		% delta-h-c-uncertainty - 50% 
		& 0.45 & \textbf{100.0} & 3.19 	 

		% rg2009 - 50% 
		& 0.87 & \textbf{100.0} & 1.25 	 

		% lm_hc0 - 50% 
		& \textbf{0.93} & 97.2 & \textbf{1.08} 	 

		% lm_hc30 - 50% 
		& 0.23 & \textbf{100.0} & 4.69 	 

	\\ & & 70	 & 21.25	 & 1.0

		% delta-h-c - 70% 
		& 0.9 & 94.4 & 1.08 	 

		% delta-h-c-uncertainty - 70% 
		& 0.45 & 97.2 & 3.03 	 

		% rg2009 - 70% 
		& \textbf{0.98} & \textbf{100.0} & \textbf{1.06} 	 

		% lm_hc0 - 70% 
		& 0.94 & 97.2 & 1.11 	 

		% lm_hc30 - 70% 
		& 0.24 & \textbf{100.0} & 4.44 	 

	\\ & & 100	 & 29.25	 & 1.0

		% delta-h-c - 100% 
		& 0.97 & \textbf{100.0} & 1.08 	 

		% delta-h-c-uncertainty - 100% 
		& 0.78 & \textbf{100.0} & 1.61 	 

		% rg2009 - 100% 
		& \textbf{1.0} & \textbf{100.0} & \textbf{1.0} 	 

		% lm_hc0 - 100% 
		& \textbf{1.0} & \textbf{100.0} & \textbf{1.0} 	 

		% lm_hc30 - 100% 
		& 0.37 & \textbf{100.0} & 3.58 	 
 \\ \hline
\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{rovers}} } & \multirow{5}{*}{6.0} 
	 & 10	 & 2.83	 & 2.39

		% delta-h-c - 10% 
		& \textbf{0.46} & 72.2 & 2.31 	 

		% delta-h-c-uncertainty - 10% 
		& 0.45 & 75.0 & 2.5 	 

		% rg2009 - 10% 
		& 0.37 & 58.3 & 2.08 	 

		% lm_hc0 - 10% 
		& 0.44 & 58.3 & \textbf{1.25} 	 

		% lm_hc30 - 10% 
		& 0.44 & \textbf{100.0} & 5.42 	 

	\\ & & 30	 & 5.75	 & 1.39

		% delta-h-c - 30% 
		& \textbf{0.65} & 91.7 & 1.56 	 

		% delta-h-c-uncertainty - 30% 
		& 0.53 & 94.4 & 2.28 	 

		% rg2009 - 30% 
		& 0.4 & 63.9 & \textbf{1.11} 	 

		% lm_hc0 - 30% 
		& 0.51 & 63.9 & 1.17 	 

		% lm_hc30 - 30% 
		& 0.34 & \textbf{100.0} & 4.5 	 

	\\ & & 50	 & 9.0	 & 1.11

		% delta-h-c - 50% 
		& \textbf{0.87} & 97.2 & 1.19 	 

		% delta-h-c-uncertainty - 50% 
		& 0.77 & 97.2 & 1.5 	 

		% rg2009 - 50% 
		& 0.49 & 55.6 & \textbf{0.67} 	 

		% lm_hc0 - 50% 
		& 0.72 & 80.6 & 1.14 	 

		% lm_hc30 - 50% 
		& 0.32 & \textbf{100.0} & 4.0 	 

	\\ & & 70	 & 12.42	 & 1.06

		% delta-h-c - 70% 
		& \textbf{0.93} & \textbf{100.0} & 1.11 	 

		% delta-h-c-uncertainty - 70% 
		& 0.86 & \textbf{100.0} & 1.39 	 

		% rg2009 - 70% 
		& 0.26 & 27.8 & \textbf{0.31} 	 

		% lm_hc0 - 70% 
		& 0.89 & 94.4 & 1.06 	 

		% lm_hc30 - 70% 
		& 0.33 & \textbf{100.0} & 3.67 	 

	\\ & & 100	 & 16.92	 & 1.0

		% delta-h-c - 100% 
		& \textbf{0.97} & \textbf{100.0} & 1.06 	 

		% delta-h-c-uncertainty - 100% 
		& 0.96 & \textbf{100.0} & 1.08 	 

		% rg2009 - 100% 
		& 0.34 & 36.1 & \textbf{0.5} 	 

		% lm_hc0 - 100% 
		& 0.9 & 94.4 & 1.08 	 

		% lm_hc30 - 100% 
		& 0.37 & \textbf{100.0} & 3.28 	 
 \\ \hline
\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{satellite}} } & \multirow{5}{*}{6.0} 
	 & 10	 & 3.0	 & 3.25

		% delta-h-c - 10% 
		& 0.49 & 83.3 & 3.08 	 

		% delta-h-c-uncertainty - 10% 
		& 0.47 & 86.1 & 3.78 	 

		% rg2009 - 10% 
		& 0.41 & 66.7 & 3.11 	 

		% lm_hc0 - 10% 
		& 0.29 & 52.8 & \textbf{2.36} 	 

		% lm_hc30 - 10% 
		& \textbf{0.53} & \textbf{100.0} & 5.72 	 

	\\ & & 30	 & 5.33	 & 1.78

		% delta-h-c - 30% 
		& \textbf{0.54} & 77.8 & 2.17 	 

		% delta-h-c-uncertainty - 30% 
		& 0.47 & 86.1 & 3.69 	 

		% rg2009 - 30% 
		& \textbf{0.54} & 88.9 & 3.0 	 

		% lm_hc0 - 30% 
		& 0.51 & 77.8 & \textbf{1.92} 	 

		% lm_hc30 - 30% 
		& 0.32 & \textbf{100.0} & 5.39 	 

	\\ & & 50	 & 8.75	 & 1.36

		% delta-h-c - 50% 
		& \textbf{0.78} & 88.9 & 1.42 	 

		% delta-h-c-uncertainty - 50% 
		& 0.56 & 94.4 & 2.69 	 

		% rg2009 - 50% 
		& 0.61 & 91.7 & 2.19 	 

		% lm_hc0 - 50% 
		& 0.66 & 91.7 & \textbf{1.33} 	 

		% lm_hc30 - 50% 
		& 0.33 & \textbf{100.0} & 4.97 	 

	\\ & & 70	 & 11.75	 & 1.33

		% delta-h-c - 70% 
		& \textbf{0.86} & 97.2 & 1.47 	 

		% delta-h-c-uncertainty - 70% 
		& 0.64 & \textbf{100.0} & 2.83 	 

		% rg2009 - 70% 
		& 0.63 & 77.8 & 1.67 	 

		% lm_hc0 - 70% 
		& 0.78 & 94.4 & \textbf{1.42} 	 

		% lm_hc30 - 70% 
		& 0.38 & \textbf{100.0} & 4.31 	 

	\\ & & 100	 & 15.75	 & 1.25

		% delta-h-c - 100% 
		& \textbf{0.92} & 94.4 & 1.19 	 

		% delta-h-c-uncertainty - 100% 
		& 0.88 & 94.4 & 1.28 	 

		% rg2009 - 100% 
		& 0.47 & 55.6 & \textbf{1.0} 	 

		% lm_hc0 - 100% 
		& \textbf{0.92} & \textbf{100.0} & 1.25 	 

		% lm_hc30 - 100% 
		& 0.46 & \textbf{100.0} & 3.86 	 
 \\ \hline
\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{sokoban}} } & \multirow{5}{*}{8.5} 
	 & 10	 & 4.33	 & 1.83

		% delta-h-c - 10% 
		& 0.31 & 58.3 & 2.47 	 

		% delta-h-c-uncertainty - 10% 
		& \textbf{0.34} & 80.6 & 4.81 	 

		% rg2009 - 10% 
		& 0.13 & 36.1 & 2.39 	 

		% lm_hc0 - 10% 
		& 0.25 & 44.4 & \textbf{1.67} 	 

		% lm_hc30 - 10% 
		& 0.24 & \textbf{97.2} & 6.47 	 

	\\ & & 30	 & 11.0	 & 1.28

		% delta-h-c - 30% 
		& \textbf{0.48} & 75.0 & 2.81 	 

		% delta-h-c-uncertainty - 30% 
		& 0.29 & \textbf{97.2} & 5.36 	 

		% rg2009 - 30% 
		& 0.12 & 19.4 & \textbf{0.75} 	 

		% lm_hc0 - 30% 
		& 0.29 & 41.7 & 1.28 	 

		% lm_hc30 - 30% 
		& 0.23 & 94.4 & 5.5 	 

	\\ & & 50	 & 17.08	 & 1.33

		% delta-h-c - 50% 
		& \textbf{0.5} & \textbf{94.4} & 4.22 	 

		% delta-h-c-uncertainty - 50% 
		& 0.32 & \textbf{94.4} & 5.89 	 

		% rg2009 - 50% 
		& 0.01 & 2.8 & \textbf{0.06} 	 

		% lm_hc0 - 50% 
		& 0.46 & 55.6 & 1.22 	 

		% lm_hc30 - 50% 
		& 0.27 & \textbf{94.4} & 4.86 	 

	\\ & & 70	 & 23.58	 & 1.36

		% delta-h-c - 70% 
		& 0.54 & \textbf{100.0} & 4.44 	 

		% delta-h-c-uncertainty - 70% 
		& 0.36 & \textbf{100.0} & 5.92 	 

		% rg2009 - 70% 
		& 0.06 & 8.3 & \textbf{0.11} 	 

		% lm_hc0 - 70% 
		& \textbf{0.58} & 77.8 & 1.28 	 

		% lm_hc30 - 70% 
		& 0.28 & \textbf{100.0} & 4.25 	 

	\\ & & 100	 & 32.67	 & 1.33

		% delta-h-c - 100% 
		& 0.35 & 94.4 & 5.97 	 

		% delta-h-c-uncertainty - 100% 
		& 0.34 & 97.2 & 6.56 	 

		% rg2009 - 100% 
		& 0.04 & 5.6 & \textbf{0.06} 	 

		% lm_hc0 - 100% 
		& \textbf{0.77} & \textbf{100.0} & 1.14 	 

		% lm_hc30 - 100% 
		& 0.33 & \textbf{100.0} & 3.31 	 
 \\ \hline
Avg & & & &  & \textbf{0.7} & 89.84 & 2.1 & 0.58 & 95.06 & 3.53 & 0.35 & 49.74 & 1.47 & 0.64 & 78.39 & \textbf{1.28} & 0.38 & \textbf{98.85} & 5.44
\\ \hline
\end{tabular}

==> tables/previous-suboptimal.tex <==
\begin{tabular}{|c|c|ccc|ccc|ccc|ccc|ccc|ccc|}
\hline
% empty
& % empty
& \multicolumn{3}{c|}{}
& \multicolumn{3}{c|}{\hdeltahc}
& \multicolumn{3}{c|}{\hdeltahcu}
& \multicolumn{3}{c|}{\rg}		   
& \multicolumn{3}{c|}{\completion}
& \multicolumn{3}{c|}{\completion 0.3}
\\ \hline
\# & $|\goalconditions|$ & \textbf{\% Obs} & $|\observations|$ & $|\grsolution|$ 
& \textbf{AGR} & \textbf{ACC} & \textbf{$|\Gamma^\textup{h}|$}
& \textbf{AGR} & \textbf{ACC} & \textbf{$|\Gamma^\textup{h}|$}
& \textbf{AGR} & \textbf{ACC} & \textbf{$|\Gamma^\textup{h}|$}
& \textbf{AGR} & \textbf{ACC} & \textbf{$|\Gamma^\textup{h}|$}
& \textbf{AGR} & \textbf{ACC} & \textbf{$|\Gamma^\textup{h}|$}
\\ 
\hline

\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{blocks}} } & \multirow{5}{*}{20.1} 
	 & 10	 & 1.42	 & 7.49

		% delta-h-c - 10% 
		& 0.41 & 86.1 & 6.86 	 

		% delta-h-c-uncertainty - 10% 
		& 0.42 & 88.9 & 7.42 	 

		% rg2009 - 10% 
		& \textbf{0.46} & 97.2 & 10.61 	 

		% lm_hc0 - 10% 
		& 0.06 & 19.4 & \textbf{1.19} 	 

		% lm_hc30 - 10% 
		& 0.34 & \textbf{100.0} & 17.53 	 

	\\ & & 30	 & 3.83	 & 3.55

		% delta-h-c - 30% 
		& 0.49 & 77.8 & 3.17 	 

		% delta-h-c-uncertainty - 30% 
		& 0.35 & 86.1 & 6.92 	 

		% rg2009 - 30% 
		& \textbf{0.54} & \textbf{100.0} & 4.86 	 

		% lm_hc0 - 30% 
		& 0.28 & 55.6 & \textbf{1.17} 	 

		% lm_hc30 - 30% 
		& 0.26 & \textbf{100.0} & 13.47 	 

	\\ & & 50	 & 5.92	 & 3.18

		% delta-h-c - 50% 
		& 0.55 & 86.1 & 3.08 	 

		% delta-h-c-uncertainty - 50% 
		& 0.42 & 94.4 & 5.61 	 

		% rg2009 - 50% 
		& \textbf{0.62} & 97.2 & 2.72 	 

		% lm_hc0 - 50% 
		& 0.39 & 72.2 & \textbf{1.08} 	 

		% lm_hc30 - 50% 
		& 0.27 & \textbf{100.0} & 9.89 	 

	\\ & & 70	 & 8.5	 & 2.53

		% delta-h-c - 70% 
		& \textbf{0.71} & 91.7 & 2.06 	 

		% delta-h-c-uncertainty - 70% 
		& 0.56 & 94.4 & 3.06 	 

		% rg2009 - 70% 
		& 0.68 & \textbf{100.0} & 2.44 	 

		% lm_hc0 - 70% 
		& 0.51 & 94.4 & \textbf{1.33} 	 

		% lm_hc30 - 70% 
		& 0.26 & \textbf{100.0} & 8.61 	 

	\\ & & 100	 & 11.83	 & 2.25

		% delta-h-c - 100% 
		& \textbf{0.84} & \textbf{100.0} & \textbf{1.67} 	 

		% delta-h-c-uncertainty - 100% 
		& \textbf{0.84} & \textbf{100.0} & \textbf{1.67} 	 

		% rg2009 - 100% 
		& 0.8 & \textbf{100.0} & 2.08 	 

		% lm_hc0 - 100% 
		& 0.51 & \textbf{100.0} & \textbf{1.67} 	 

		% lm_hc30 - 100% 
		& 0.28 & \textbf{100.0} & 6.42 	 
 \\ \hline
\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{ipc-grid}} } & \multirow{5}{*}{7.5} 
	 & 10	 & 2.06	 & 1.58

		% delta-h-c - 10% 
		& 0.77 & 91.7 & \textbf{1.81} 	 

		% delta-h-c-uncertainty - 10% 
		& 0.75 & 97.9 & 2.4 	 

		% rg2009 - 10% 
		& \textbf{0.81} & \textbf{100.0} & 2.73 	 

		% lm_hc0 - 10% 
		& 0.64 & 87.5 & 2.23 	 

		% lm_hc30 - 10% 
		& 0.42 & \textbf{100.0} & 5.6 	 

	\\ & & 30	 & 5.56	 & 1.4

		% delta-h-c - 30% 
		& 0.82 & 93.8 & \textbf{1.13} 	 

		% delta-h-c-uncertainty - 30% 
		& 0.77 & 97.9 & 1.6 	 

		% rg2009 - 30% 
		& \textbf{0.9} & \textbf{100.0} & 1.27 	 

		% lm_hc0 - 30% 
		& 0.81 & 95.8 & 1.35 	 

		% lm_hc30 - 30% 
		& 0.67 & 95.8 & 2.23 	 

	\\ & & 50	 & 8.88	 & 1.35

		% delta-h-c - 50% 
		& 0.84 & 93.8 & 1.13 	 

		% delta-h-c-uncertainty - 50% 
		& 0.84 & \textbf{100.0} & 1.56 	 

		% rg2009 - 50% 
		& \textbf{0.92} & \textbf{100.0} & 1.1 	 

		% lm_hc0 - 50% 
		& 0.87 & \textbf{100.0} & \textbf{1.08} 	 

		% lm_hc30 - 50% 
		& 0.86 & \textbf{100.0} & 1.21 	 

	\\ & & 70	 & 12.56	 & 1.31

		% delta-h-c - 70% 
		& 0.89 & \textbf{100.0} & 1.1 	 

		% delta-h-c-uncertainty - 70% 
		& 0.85 & \textbf{100.0} & 1.23 	 

		% rg2009 - 70% 
		& \textbf{0.93} & \textbf{100.0} & 1.02 	 

		% lm_hc0 - 70% 
		& 0.92 & \textbf{100.0} & \textbf{1.0} 	 

		% lm_hc30 - 70% 
		& 0.92 & \textbf{100.0} & \textbf{1.0} 	 

	\\ & & 100	 & 17.25	 & 1.5

		% delta-h-c - 100% 
		& \textbf{0.94} & \textbf{100.0} & \textbf{1.0} 	 

		% delta-h-c-uncertainty - 100% 
		& \textbf{0.94} & \textbf{100.0} & \textbf{1.0} 	 

		% rg2009 - 100% 
		& \textbf{0.94} & \textbf{100.0} & \textbf{1.0} 	 

		% lm_hc0 - 100% 
		& \textbf{0.94} & \textbf{100.0} & \textbf{1.0} 	 

		% lm_hc30 - 100% 
		& \textbf{0.94} & \textbf{100.0} & \textbf{1.0} 	 
 \\ \hline
\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{logistics}} } & \multirow{5}{*}{10.0} 
	 & 10	 & 2.67	 & 2.0

		% delta-h-c - 10% 
		& \textbf{0.88} & \textbf{100.0} & 2.44 	 

		% delta-h-c-uncertainty - 10% 
		& 0.85 & \textbf{100.0} & 2.72 	 

		% rg2009 - 10% 
		& 0.72 & 91.7 & 3.11 	 

		% lm_hc0 - 10% 
		& 0.56 & 66.7 & \textbf{2.08} 	 

		% lm_hc30 - 10% 
		& 0.21 & \textbf{100.0} & 9.75 	 

	\\ & & 30	 & 7.5	 & 1.14

		% delta-h-c - 30% 
		& \textbf{0.91} & \textbf{100.0} & 1.33 	 

		% delta-h-c-uncertainty - 30% 
		& 0.75 & \textbf{100.0} & 2.14 	 

		% rg2009 - 30% 
		& 0.87 & 97.2 & 1.36 	 

		% lm_hc0 - 30% 
		& 0.85 & 91.7 & \textbf{1.22} 	 

		% lm_hc30 - 30% 
		& 0.26 & \textbf{100.0} & 6.0 	 

	\\ & & 50	 & 11.92	 & 1.06

		% delta-h-c - 50% 
		& 0.88 & 97.2 & 1.25 	 

		% delta-h-c-uncertainty - 50% 
		& 0.86 & \textbf{100.0} & 1.47 	 

		% rg2009 - 50% 
		& 0.91 & \textbf{100.0} & 1.25 	 

		% lm_hc0 - 50% 
		& \textbf{0.93} & 97.2 & \textbf{1.03} 	 

		% lm_hc30 - 50% 
		& 0.39 & \textbf{100.0} & 3.69 	 

	\\ & & 70	 & 16.67	 & 1.03

		% delta-h-c - 70% 
		& 0.97 & \textbf{100.0} & 1.08 	 

		% delta-h-c-uncertainty - 70% 
		& 0.92 & \textbf{100.0} & 1.19 	 

		% rg2009 - 70% 
		& \textbf{0.99} & \textbf{100.0} & 1.06 	 

		% lm_hc0 - 70% 
		& \textbf{0.99} & \textbf{100.0} & \textbf{1.0} 	 

		% lm_hc30 - 70% 
		& 0.66 & \textbf{100.0} & 2.0 	 

	\\ & & 100	 & 23.17	 & 1.0

		% delta-h-c - 100% 
		& \textbf{1.0} & \textbf{100.0} & \textbf{1.0} 	 

		% delta-h-c-uncertainty - 100% 
		& \textbf{1.0} & \textbf{100.0} & \textbf{1.0} 	 

		% rg2009 - 100% 
		& \textbf{1.0} & \textbf{100.0} & \textbf{1.0} 	 

		% lm_hc0 - 100% 
		& \textbf{1.0} & \textbf{100.0} & \textbf{1.0} 	 

		% lm_hc30 - 100% 
		& 0.72 & \textbf{100.0} & 1.67 	 
 \\ \hline
\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{miconic}} } & \multirow{5}{*}{6.0} 
	 & 10	 & 3.0	 & 1.83

		% delta-h-c - 10% 
		& \textbf{0.76} & \textbf{100.0} & 2.67 	 

		% delta-h-c-uncertainty - 10% 
		& 0.74 & \textbf{100.0} & 3.0 	 

		% rg2009 - 10% 
		& 0.65 & \textbf{100.0} & 3.42 	 

		% lm_hc0 - 10% 
		& 0.54 & 55.6 & \textbf{1.36} 	 

		% lm_hc30 - 10% 
		& 0.31 & \textbf{100.0} & 6.0 	 

	\\ & & 30	 & 7.67	 & 1.25

		% delta-h-c - 30% 
		& \textbf{0.89} & \textbf{100.0} & 1.47 	 

		% delta-h-c-uncertainty - 30% 
		& 0.65 & \textbf{100.0} & 2.5 	 

		% rg2009 - 30% 
		& 0.66 & \textbf{100.0} & 2.17 	 

		% lm_hc0 - 30% 
		& 0.86 & 91.7 & \textbf{1.08} 	 

		% lm_hc30 - 30% 
		& 0.23 & \textbf{100.0} & 5.58 	 

	\\ & & 50	 & 12.25	 & 1.03

		% delta-h-c - 50% 
		& \textbf{0.98} & \textbf{100.0} & 1.08 	 

		% delta-h-c-uncertainty - 50% 
		& 0.82 & \textbf{100.0} & 1.5 	 

		% rg2009 - 50% 
		& 0.91 & \textbf{100.0} & 1.25 	 

		% lm_hc0 - 50% 
		& 0.97 & 97.2 & \textbf{1.03} 	 

		% lm_hc30 - 50% 
		& 0.24 & \textbf{100.0} & 4.56 	 

	\\ & & 70	 & 17.33	 & 1.0

		% delta-h-c - 70% 
		& 0.99 & \textbf{100.0} & 1.03 	 

		% delta-h-c-uncertainty - 70% 
		& 0.9 & \textbf{100.0} & 1.31 	 

		% rg2009 - 70% 
		& 0.94 & \textbf{100.0} & 1.11 	 

		% lm_hc0 - 70% 
		& \textbf{1.0} & \textbf{100.0} & \textbf{1.0} 	 

		% lm_hc30 - 70% 
		& 0.31 & \textbf{100.0} & 3.94 	 

	\\ & & 100	 & 24.0	 & 1.0

		% delta-h-c - 100% 
		& \textbf{1.0} & \textbf{100.0} & \textbf{1.0} 	 

		% delta-h-c-uncertainty - 100% 
		& \textbf{1.0} & \textbf{100.0} & \textbf{1.0} 	 

		% rg2009 - 100% 
		& \textbf{1.0} & \textbf{100.0} & \textbf{1.0} 	 

		% lm_hc0 - 100% 
		& \textbf{1.0} & \textbf{100.0} & \textbf{1.0} 	 

		% lm_hc30 - 100% 
		& 0.47 & \textbf{100.0} & 3.0 	 
 \\ \hline
\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{rovers}} } & \multirow{5}{*}{6.0} 
	 & 10	 & 1.83	 & 2.39

		% delta-h-c - 10% 
		& \textbf{0.83} & 88.9 & 2.89 	 

		% delta-h-c-uncertainty - 10% 
		& \textbf{0.83} & 88.9 & 2.89 	 

		% rg2009 - 10% 
		& 0.82 & \textbf{100.0} & 3.42 	 

		% lm_hc0 - 10% 
		& 0.45 & 55.6 & \textbf{1.31} 	 

		% lm_hc30 - 10% 
		& 0.48 & \textbf{100.0} & 5.14 	 

	\\ & & 30	 & 4.5	 & 1.39

		% delta-h-c - 30% 
		& \textbf{0.88} & 88.9 & 1.39 	 

		% delta-h-c-uncertainty - 30% 
		& 0.81 & 88.9 & 1.75 	 

		% rg2009 - 30% 
		& 0.8 & \textbf{100.0} & 2.06 	 

		% lm_hc0 - 30% 
		& 0.7 & 80.6 & \textbf{1.14} 	 

		% lm_hc30 - 30% 
		& 0.34 & \textbf{100.0} & 4.5 	 

	\\ & & 50	 & 7.17	 & 1.11

		% delta-h-c - 50% 
		& \textbf{0.93} & 94.4 & \textbf{1.14} 	 

		% delta-h-c-uncertainty - 50% 
		& 0.86 & 94.4 & 1.33 	 

		% rg2009 - 50% 
		& 0.89 & \textbf{100.0} & 1.36 	 

		% lm_hc0 - 50% 
		& 0.8 & 88.9 & 1.19 	 

		% lm_hc30 - 50% 
		& 0.34 & \textbf{100.0} & 3.92 	 

	\\ & & 70	 & 10.0	 & 1.06

		% delta-h-c - 70% 
		& 0.94 & 94.4 & \textbf{1.08} 	 

		% delta-h-c-uncertainty - 70% 
		& 0.92 & 97.2 & 1.22 	 

		% rg2009 - 70% 
		& \textbf{0.98} & \textbf{100.0} & 1.11 	 

		% lm_hc0 - 70% 
		& 0.87 & 94.4 & 1.11 	 

		% lm_hc30 - 70% 
		& 0.38 & \textbf{100.0} & 3.53 	 

	\\ & & 100	 & 13.67	 & 1.0

		% delta-h-c - 100% 
		& \textbf{1.0} & \textbf{100.0} & \textbf{1.0} 	 

		% delta-h-c-uncertainty - 100% 
		& \textbf{1.0} & \textbf{100.0} & \textbf{1.0} 	 

		% rg2009 - 100% 
		& \textbf{1.0} & \textbf{100.0} & \textbf{1.0} 	 

		% lm_hc0 - 100% 
		& \textbf{1.0} & \textbf{100.0} & \textbf{1.0} 	 

		% lm_hc30 - 100% 
		& 0.39 & \textbf{100.0} & 3.0 	 
 \\ \hline
\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{satellite}} } & \multirow{5}{*}{6.0} 
	 & 10	 & 2.0	 & 3.25

		% delta-h-c - 10% 
		& \textbf{0.9} & 97.2 & 3.44 	 

		% delta-h-c-uncertainty - 10% 
		& \textbf{0.9} & 97.2 & 3.44 	 

		% rg2009 - 10% 
		& 0.73 & 97.2 & 4.47 	 

		% lm_hc0 - 10% 
		& 0.58 & 75.0 & \textbf{2.5} 	 

		% lm_hc30 - 10% 
		& 0.57 & \textbf{100.0} & 5.72 	 

	\\ & & 30	 & 4.33	 & 1.78

		% delta-h-c - 30% 
		& \textbf{0.8} & 94.4 & 2.22 	 

		% delta-h-c-uncertainty - 30% 
		& 0.78 & 94.4 & 2.33 	 

		% rg2009 - 30% 
		& 0.68 & 91.7 & 2.97 	 

		% lm_hc0 - 30% 
		& 0.6 & 80.6 & \textbf{1.53} 	 

		% lm_hc30 - 30% 
		& 0.34 & \textbf{100.0} & 5.42 	 

	\\ & & 50	 & 6.75	 & 1.36

		% delta-h-c - 50% 
		& \textbf{0.92} & 94.4 & 1.42 	 

		% delta-h-c-uncertainty - 50% 
		& 0.85 & 94.4 & 1.72 	 

		% rg2009 - 50% 
		& 0.7 & 97.2 & 2.53 	 

		% lm_hc0 - 50% 
		& 0.76 & 91.7 & \textbf{1.19} 	 

		% lm_hc30 - 50% 
		& 0.33 & \textbf{100.0} & 4.92 	 

	\\ & & 70	 & 9.42	 & 1.33

		% delta-h-c - 70% 
		& \textbf{0.94} & \textbf{100.0} & 1.36 	 

		% delta-h-c-uncertainty - 70% 
		& \textbf{0.94} & \textbf{100.0} & 1.36 	 

		% rg2009 - 70% 
		& 0.78 & 97.2 & 2.06 	 

		% lm_hc0 - 70% 
		& 0.85 & 97.2 & \textbf{1.14} 	 

		% lm_hc30 - 70% 
		& 0.41 & \textbf{100.0} & 4.14 	 

	\\ & & 100	 & 12.75	 & 1.25

		% delta-h-c - 100% 
		& \textbf{0.96} & \textbf{100.0} & \textbf{1.17} 	 

		% delta-h-c-uncertainty - 100% 
		& \textbf{0.96} & \textbf{100.0} & \textbf{1.17} 	 

		% rg2009 - 100% 
		& 0.88 & \textbf{100.0} & 1.75 	 

		% lm_hc0 - 100% 
		& 0.88 & \textbf{100.0} & \textbf{1.17} 	 

		% lm_hc30 - 100% 
		& 0.5 & \textbf{100.0} & 3.33 	 
 \\ \hline
\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{sokoban}} } & \multirow{5}{*}{8.5} 
	 & 10	 & 3.33	 & 1.83

		% delta-h-c - 10% 
		& \textbf{0.52} & 61.1 & \textbf{1.78} 	 

		% delta-h-c-uncertainty - 10% 
		& 0.44 & 72.2 & 3.17 	 

		% rg2009 - 10% 
		& 0.29 & 63.9 & 4.56 	 

		% lm_hc0 - 10% 
		& 0.35 & 63.9 & 2.47 	 

		% lm_hc30 - 10% 
		& 0.24 & \textbf{100.0} & 6.86 	 

	\\ & & 30	 & 8.67	 & 1.28

		% delta-h-c - 30% 
		& \textbf{0.77} & 83.3 & \textbf{1.08} 	 

		% delta-h-c-uncertainty - 30% 
		& 0.62 & \textbf{97.2} & 2.67 	 

		% rg2009 - 30% 
		& 0.43 & 75.0 & 2.92 	 

		% lm_hc0 - 30% 
		& 0.56 & 75.0 & 1.72 	 

		% lm_hc30 - 30% 
		& 0.24 & \textbf{97.2} & 5.5 	 

	\\ & & 50	 & 13.75	 & 1.33

		% delta-h-c - 50% 
		& \textbf{0.79} & 91.7 & \textbf{1.17} 	 

		% delta-h-c-uncertainty - 50% 
		& 0.66 & \textbf{100.0} & 2.58 	 

		% rg2009 - 50% 
		& 0.53 & 72.2 & 1.83 	 

		% lm_hc0 - 50% 
		& 0.58 & 75.0 & 1.39 	 

		% lm_hc30 - 50% 
		& 0.25 & 97.2 & 5.14 	 

	\\ & & 70	 & 19.33	 & 1.36

		% delta-h-c - 70% 
		& 0.8 & 97.2 & \textbf{1.03} 	 

		% delta-h-c-uncertainty - 70% 
		& \textbf{0.85} & \textbf{100.0} & 1.39 	 

		% rg2009 - 70% 
		& 0.54 & 61.1 & 1.28 	 

		% lm_hc0 - 70% 
		& 0.63 & 86.1 & 1.25 	 

		% lm_hc30 - 70% 
		& 0.3 & \textbf{100.0} & 4.11 	 

	\\ & & 100	 & 27.0	 & 1.33

		% delta-h-c - 100% 
		& \textbf{0.83} & \textbf{100.0} & \textbf{1.0} 	 

		% delta-h-c-uncertainty - 100% 
		& \textbf{0.83} & \textbf{100.0} & \textbf{1.0} 	 

		% rg2009 - 100% 
		& 0.58 & 58.3 & 1.33 	 

		% lm_hc0 - 100% 
		& \textbf{0.83} & \textbf{100.0} & \textbf{1.0} 	 

		% lm_hc30 - 100% 
		& 0.38 & \textbf{100.0} & 2.75 	 
 \\ \hline
Avg & & & &  & \textbf{0.84} & 94.4 & 1.73 & 0.78 & 96.71 & 2.27 & 0.77 & 94.21 & 2.32 & 0.72 & 85.4 & \textbf{1.32} & 0.42 & \textbf{99.72} & 5.18
\\ \hline
\end{tabular}

==> tables/previous.tex <==
\begin{tabular}{ccccccccccccccccc}
\toprule
 & & & \multicolumn{7}{c}{Optimal} & \multicolumn{7}{c}{Suboptimal}\\
\cmidrule(lr){4-10}\cmidrule(lr){11-17}
 & & & & & \multicolumn{5}{c}{\textbf{AGR}} & & & \multicolumn{5}{c}{\textbf{AGR}}\\
\cline{6-10} \cline{13-17}
\# & $|\goalconditions|$ & \textbf{\%} & $|\observations|$ & $|\Gamma^\textup{*}|$ & \hdeltahc & \hdeltahcu & \rg & \completion & \completiontetha & $|\observations|$ & $|\Gamma^\textup{*}|$ & \hdeltahc & \hdeltahcu & \rg & \completion & \completiontetha \\
\midrule
\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{blocks}} } & \multirow{5}{*}{20.1} 
 & 10 & 1.25 & 7.9

% delta-h-c - 10% 
 & 0.44
% delta-h-c-uncertainty - 10% 
 & 0.44
% rg2009 - 10% 
 & \textbf{0.47}
% lm_hc0 - 10% 
 & 0.06
% lm_hc30 - 10% 
 & 0.38 & 1.42 & 7.49

% delta-h-c - 10% 
 & 0.41
% delta-h-c-uncertainty - 10% 
 & 0.42
% rg2009 - 10% 
 & \textbf{0.46}
% lm_hc0 - 10% 
 & 0.06
% lm_hc30 - 10% 
 & 0.34
\\ & & 30 & 3.08 & 3.91

% delta-h-c - 30% 
 & \textbf{0.46}
% delta-h-c-uncertainty - 30% 
 & 0.44
% rg2009 - 30% 
 & 0.45
% lm_hc0 - 30% 
 & 0.21
% lm_hc30 - 30% 
 & 0.24 & 3.83 & 3.55

% delta-h-c - 30% 
 & 0.49
% delta-h-c-uncertainty - 30% 
 & 0.35
% rg2009 - 30% 
 & \textbf{0.54}
% lm_hc0 - 30% 
 & 0.28
% lm_hc30 - 30% 
 & 0.26
\\ & & 50 & 4.42 & 2.48

% delta-h-c - 50% 
 & 0.59
% delta-h-c-uncertainty - 50% 
 & 0.52
% rg2009 - 50% 
 & \textbf{0.62}
% lm_hc0 - 50% 
 & 0.33
% lm_hc30 - 50% 
 & 0.25 & 5.92 & 3.18

% delta-h-c - 50% 
 & 0.55
% delta-h-c-uncertainty - 50% 
 & 0.42
% rg2009 - 50% 
 & \textbf{0.62}
% lm_hc0 - 50% 
 & 0.39
% lm_hc30 - 50% 
 & 0.27
\\ & & 70 & 6.67 & 1.94

% delta-h-c - 70% 
 & \textbf{0.85}
% delta-h-c-uncertainty - 70% 
 & 0.76
% rg2009 - 70% 
 & 0.81
% lm_hc0 - 70% 
 & 0.51
% lm_hc30 - 70% 
 & 0.25 & 8.5 & 2.53

% delta-h-c - 70% 
 & \textbf{0.71}
% delta-h-c-uncertainty - 70% 
 & 0.56
% rg2009 - 70% 
 & 0.68
% lm_hc0 - 70% 
 & 0.51
% lm_hc30 - 70% 
 & 0.26
\\ & & 100 & 8.83 & 1.83

% delta-h-c - 100% 
 & \textbf{0.92}
% delta-h-c-uncertainty - 100% 
 & \textbf{0.92}
% rg2009 - 100% 
 & 0.9
% lm_hc0 - 100% 
 & 0.59
% lm_hc30 - 100% 
 & 0.31 & 11.83 & 2.25

% delta-h-c - 100% 
 & \textbf{0.84}
% delta-h-c-uncertainty - 100% 
 & \textbf{0.84}
% rg2009 - 100% 
 & 0.8
% lm_hc0 - 100% 
 & 0.51
% lm_hc30 - 100% 
 & 0.28 \\ \hline\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{ipc-grid}} } & \multirow{5}{*}{7.5} 
 & 10 & 1.63 & 2.71

% delta-h-c - 10% 
 & 0.87
% delta-h-c-uncertainty - 10% 
 & 0.88
% rg2009 - 10% 
 & \textbf{0.91}
% lm_hc0 - 10% 
 & 0.47
% lm_hc30 - 10% 
 & 0.49 & 2.06 & 1.58

% delta-h-c - 10% 
 & 0.77
% delta-h-c-uncertainty - 10% 
 & 0.75
% rg2009 - 10% 
 & \textbf{0.81}
% lm_hc0 - 10% 
 & 0.64
% lm_hc30 - 10% 
 & 0.42
\\ & & 30 & 4.0 & 1.21

% delta-h-c - 30% 
 & 0.93
% delta-h-c-uncertainty - 30% 
 & 0.94
% rg2009 - 30% 
 & \textbf{0.99}
% lm_hc0 - 30% 
 & 0.85
% lm_hc30 - 30% 
 & 0.64 & 5.56 & 1.4

% delta-h-c - 30% 
 & 0.82
% delta-h-c-uncertainty - 30% 
 & 0.77
% rg2009 - 30% 
 & \textbf{0.9}
% lm_hc0 - 30% 
 & 0.81
% lm_hc30 - 30% 
 & 0.67
\\ & & 50 & 6.19 & 1.13

% delta-h-c - 50% 
 & 0.96
% delta-h-c-uncertainty - 50% 
 & 0.96
% rg2009 - 50% 
 & \textbf{1.0}
% lm_hc0 - 50% 
 & 0.86
% lm_hc30 - 50% 
 & 0.77 & 8.88 & 1.35

% delta-h-c - 50% 
 & 0.84
% delta-h-c-uncertainty - 50% 
 & 0.84
% rg2009 - 50% 
 & \textbf{0.92}
% lm_hc0 - 50% 
 & 0.87
% lm_hc30 - 50% 
 & 0.86
\\ & & 70 & 8.69 & 1.04

% delta-h-c - 70% 
 & 0.97
% delta-h-c-uncertainty - 70% 
 & 0.97
% rg2009 - 70% 
 & \textbf{1.0}
% lm_hc0 - 70% 
 & 0.97
% lm_hc30 - 70% 
 & 0.93 & 12.56 & 1.31

% delta-h-c - 70% 
 & 0.89
% delta-h-c-uncertainty - 70% 
 & 0.85
% rg2009 - 70% 
 & \textbf{0.93}
% lm_hc0 - 70% 
 & 0.92
% lm_hc30 - 70% 
 & 0.92
\\ & & 100 & 11.88 & 1.0

% delta-h-c - 100% 
 & \textbf{1.0}
% delta-h-c-uncertainty - 100% 
 & \textbf{1.0}
% rg2009 - 100% 
 & \textbf{1.0}
% lm_hc0 - 100% 
 & \textbf{1.0}
% lm_hc30 - 100% 
 & \textbf{1.0} & 17.25 & 1.5

% delta-h-c - 100% 
 & \textbf{0.94}
% delta-h-c-uncertainty - 100% 
 & \textbf{0.94}
% rg2009 - 100% 
 & \textbf{0.94}
% lm_hc0 - 100% 
 & \textbf{0.94}
% lm_hc30 - 100% 
 & \textbf{0.94} \\ \hline\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{logistics}} } & \multirow{5}{*}{10.0} 
 & 10 & 2.0 & 2.83

% delta-h-c - 10% 
 & \textbf{0.9}
% delta-h-c-uncertainty - 10% 
 & \textbf{0.9}
% rg2009 - 10% 
 & 0.87
% lm_hc0 - 10% 
 & 0.43
% lm_hc30 - 10% 
 & 0.31 & 2.67 & 2.0

% delta-h-c - 10% 
 & \textbf{0.88}
% delta-h-c-uncertainty - 10% 
 & 0.85
% rg2009 - 10% 
 & 0.72
% lm_hc0 - 10% 
 & 0.56
% lm_hc30 - 10% 
 & 0.21
\\ & & 30 & 5.75 & 1.19

% delta-h-c - 30% 
 & \textbf{0.92}
% delta-h-c-uncertainty - 30% 
 & \textbf{0.92}
% rg2009 - 30% 
 & 0.86
% lm_hc0 - 30% 
 & 0.78
% lm_hc30 - 30% 
 & 0.24 & 7.5 & 1.14

% delta-h-c - 30% 
 & \textbf{0.91}
% delta-h-c-uncertainty - 30% 
 & 0.75
% rg2009 - 30% 
 & 0.87
% lm_hc0 - 30% 
 & 0.85
% lm_hc30 - 30% 
 & 0.26
\\ & & 50 & 9.42 & 1.06

% delta-h-c - 50% 
 & \textbf{0.96}
% delta-h-c-uncertainty - 50% 
 & \textbf{0.96}
% rg2009 - 50% 
 & 0.93
% lm_hc0 - 50% 
 & 0.9
% lm_hc30 - 50% 
 & 0.39 & 11.92 & 1.06

% delta-h-c - 50% 
 & 0.88
% delta-h-c-uncertainty - 50% 
 & 0.86
% rg2009 - 50% 
 & 0.91
% lm_hc0 - 50% 
 & \textbf{0.93}
% lm_hc30 - 50% 
 & 0.39
\\ & & 70 & 13.25 & 1.03

% delta-h-c - 70% 
 & 0.99
% delta-h-c-uncertainty - 70% 
 & 0.99
% rg2009 - 70% 
 & 0.99
% lm_hc0 - 70% 
 & \textbf{1.0}
% lm_hc30 - 70% 
 & 0.62 & 16.67 & 1.03

% delta-h-c - 70% 
 & 0.97
% delta-h-c-uncertainty - 70% 
 & 0.92
% rg2009 - 70% 
 & \textbf{0.99}
% lm_hc0 - 70% 
 & \textbf{0.99}
% lm_hc30 - 70% 
 & 0.66
\\ & & 100 & 18.17 & 1.0

% delta-h-c - 100% 
 & \textbf{1.0}
% delta-h-c-uncertainty - 100% 
 & \textbf{1.0}
% rg2009 - 100% 
 & \textbf{1.0}
% lm_hc0 - 100% 
 & \textbf{1.0}
% lm_hc30 - 100% 
 & 0.72 & 23.17 & 1.0

% delta-h-c - 100% 
 & \textbf{1.0}
% delta-h-c-uncertainty - 100% 
 & \textbf{1.0}
% rg2009 - 100% 
 & \textbf{1.0}
% lm_hc0 - 100% 
 & \textbf{1.0}
% lm_hc30 - 100% 
 & 0.72 \\ \hline\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{miconic}} } & \multirow{5}{*}{6.0} 
 & 10 & 2.0 & 2.53

% delta-h-c - 10% 
 & \textbf{0.89}
% delta-h-c-uncertainty - 10% 
 & \textbf{0.89}
% rg2009 - 10% 
 & 0.76
% lm_hc0 - 10% 
 & 0.39
% lm_hc30 - 10% 
 & 0.42 & 3.0 & 1.83

% delta-h-c - 10% 
 & \textbf{0.76}
% delta-h-c-uncertainty - 10% 
 & 0.74
% rg2009 - 10% 
 & 0.65
% lm_hc0 - 10% 
 & 0.54
% lm_hc30 - 10% 
 & 0.31
\\ & & 30 & 5.42 & 1.22

% delta-h-c - 30% 
 & \textbf{0.95}
% delta-h-c-uncertainty - 30% 
 & \textbf{0.95}
% rg2009 - 30% 
 & 0.65
% lm_hc0 - 30% 
 & 0.83
% lm_hc30 - 30% 
 & 0.22 & 7.67 & 1.25

% delta-h-c - 30% 
 & \textbf{0.89}
% delta-h-c-uncertainty - 30% 
 & 0.65
% rg2009 - 30% 
 & 0.66
% lm_hc0 - 30% 
 & 0.86
% lm_hc30 - 30% 
 & 0.23
\\ & & 50 & 8.42 & 1.06

% delta-h-c - 50% 
 & \textbf{0.97}
% delta-h-c-uncertainty - 50% 
 & \textbf{0.97}
% rg2009 - 50% 
 & 0.84
% lm_hc0 - 50% 
 & 0.92
% lm_hc30 - 50% 
 & 0.25 & 12.25 & 1.03

% delta-h-c - 50% 
 & \textbf{0.98}
% delta-h-c-uncertainty - 50% 
 & 0.82
% rg2009 - 50% 
 & 0.91
% lm_hc0 - 50% 
 & 0.97
% lm_hc30 - 50% 
 & 0.24
\\ & & 70 & 11.92 & 1.0

% delta-h-c - 70% 
 & 0.98
% delta-h-c-uncertainty - 70% 
 & 0.98
% rg2009 - 70% 
 & 0.91
% lm_hc0 - 70% 
 & \textbf{0.99}
% lm_hc30 - 70% 
 & 0.31 & 17.33 & 1.0

% delta-h-c - 70% 
 & 0.99
% delta-h-c-uncertainty - 70% 
 & 0.9
% rg2009 - 70% 
 & 0.94
% lm_hc0 - 70% 
 & \textbf{1.0}
% lm_hc30 - 70% 
 & 0.31
\\ & & 100 & 16.33 & 1.0

% delta-h-c - 100% 
 & \textbf{1.0}
% delta-h-c-uncertainty - 100% 
 & \textbf{1.0}
% rg2009 - 100% 
 & \textbf{1.0}
% lm_hc0 - 100% 
 & \textbf{1.0}
% lm_hc30 - 100% 
 & 0.47 & 24.0 & 1.0

% delta-h-c - 100% 
 & \textbf{1.0}
% delta-h-c-uncertainty - 100% 
 & \textbf{1.0}
% rg2009 - 100% 
 & \textbf{1.0}
% lm_hc0 - 100% 
 & \textbf{1.0}
% lm_hc30 - 100% 
 & 0.47 \\ \hline\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{rovers}} } & \multirow{5}{*}{6.0} 
 & 10 & 1.67 & 2.28

% delta-h-c - 10% 
 & \textbf{0.83}
% delta-h-c-uncertainty - 10% 
 & \textbf{0.83}
% rg2009 - 10% 
 & 0.76
% lm_hc0 - 10% 
 & 0.49
% lm_hc30 - 10% 
 & 0.44 & 1.83 & 2.39

% delta-h-c - 10% 
 & \textbf{0.83}
% delta-h-c-uncertainty - 10% 
 & \textbf{0.83}
% rg2009 - 10% 
 & 0.82
% lm_hc0 - 10% 
 & 0.45
% lm_hc30 - 10% 
 & 0.48
\\ & & 30 & 3.67 & 1.31

% delta-h-c - 30% 
 & \textbf{0.94}
% delta-h-c-uncertainty - 30% 
 & \textbf{0.94}
% rg2009 - 30% 
 & 0.88
% lm_hc0 - 30% 
 & 0.76
% lm_hc30 - 30% 
 & 0.37 & 4.5 & 1.39

% delta-h-c - 30% 
 & \textbf{0.88}
% delta-h-c-uncertainty - 30% 
 & 0.81
% rg2009 - 30% 
 & 0.8
% lm_hc0 - 30% 
 & 0.7
% lm_hc30 - 30% 
 & 0.34
\\ & & 50 & 5.75 & 1.19

% delta-h-c - 50% 
 & \textbf{0.92}
% delta-h-c-uncertainty - 50% 
 & \textbf{0.92}
% rg2009 - 50% 
 & 0.91
% lm_hc0 - 50% 
 & 0.79
% lm_hc30 - 50% 
 & 0.39 & 7.17 & 1.11

% delta-h-c - 50% 
 & \textbf{0.93}
% delta-h-c-uncertainty - 50% 
 & 0.86
% rg2009 - 50% 
 & 0.89
% lm_hc0 - 50% 
 & 0.8
% lm_hc30 - 50% 
 & 0.34
\\ & & 70 & 8.17 & 1.0

% delta-h-c - 70% 
 & \textbf{0.99}
% delta-h-c-uncertainty - 70% 
 & \textbf{0.99}
% rg2009 - 70% 
 & 0.97
% lm_hc0 - 70% 
 & 0.93
% lm_hc30 - 70% 
 & 0.37 & 10.0 & 1.06

% delta-h-c - 70% 
 & 0.94
% delta-h-c-uncertainty - 70% 
 & 0.92
% rg2009 - 70% 
 & \textbf{0.98}
% lm_hc0 - 70% 
 & 0.87
% lm_hc30 - 70% 
 & 0.38
\\ & & 100 & 10.83 & 1.0

% delta-h-c - 100% 
 & \textbf{1.0}
% delta-h-c-uncertainty - 100% 
 & \textbf{1.0}
% rg2009 - 100% 
 & \textbf{1.0}
% lm_hc0 - 100% 
 & \textbf{1.0}
% lm_hc30 - 100% 
 & 0.39 & 13.67 & 1.0

% delta-h-c - 100% 
 & \textbf{1.0}
% delta-h-c-uncertainty - 100% 
 & \textbf{1.0}
% rg2009 - 100% 
 & \textbf{1.0}
% lm_hc0 - 100% 
 & \textbf{1.0}
% lm_hc30 - 100% 
 & 0.39 \\ \hline\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{satellite}} } & \multirow{5}{*}{6.0} 
 & 10 & 1.42 & 3.53

% delta-h-c - 10% 
 & 0.85
% delta-h-c-uncertainty - 10% 
 & 0.85
% rg2009 - 10% 
 & \textbf{0.86}
% lm_hc0 - 10% 
 & 0.5
% lm_hc30 - 10% 
 & 0.59 & 2.0 & 3.25

% delta-h-c - 10% 
 & \textbf{0.9}
% delta-h-c-uncertainty - 10% 
 & \textbf{0.9}
% rg2009 - 10% 
 & 0.73
% lm_hc0 - 10% 
 & 0.58
% lm_hc30 - 10% 
 & 0.57
\\ & & 30 & 3.42 & 2.39

% delta-h-c - 30% 
 & \textbf{0.86}
% delta-h-c-uncertainty - 30% 
 & \textbf{0.86}
% rg2009 - 30% 
 & 0.72
% lm_hc0 - 30% 
 & 0.64
% lm_hc30 - 30% 
 & 0.44 & 4.33 & 1.78

% delta-h-c - 30% 
 & \textbf{0.8}
% delta-h-c-uncertainty - 30% 
 & 0.78
% rg2009 - 30% 
 & 0.68
% lm_hc0 - 30% 
 & 0.6
% lm_hc30 - 30% 
 & 0.34
\\ & & 50 & 5.75 & 1.58

% delta-h-c - 50% 
 & \textbf{0.93}
% delta-h-c-uncertainty - 50% 
 & 0.91
% rg2009 - 50% 
 & 0.79
% lm_hc0 - 50% 
 & 0.73
% lm_hc30 - 50% 
 & 0.35 & 6.75 & 1.36

% delta-h-c - 50% 
 & \textbf{0.92}
% delta-h-c-uncertainty - 50% 
 & 0.85
% rg2009 - 50% 
 & 0.7
% lm_hc0 - 50% 
 & 0.76
% lm_hc30 - 50% 
 & 0.33
\\ & & 70 & 8.08 & 1.31

% delta-h-c - 70% 
 & \textbf{0.94}
% delta-h-c-uncertainty - 70% 
 & \textbf{0.94}
% rg2009 - 70% 
 & 0.81
% lm_hc0 - 70% 
 & 0.89
% lm_hc30 - 70% 
 & 0.37 & 9.42 & 1.33

% delta-h-c - 70% 
 & \textbf{0.94}
% delta-h-c-uncertainty - 70% 
 & \textbf{0.94}
% rg2009 - 70% 
 & 0.78
% lm_hc0 - 70% 
 & 0.85
% lm_hc30 - 70% 
 & 0.41
\\ & & 100 & 10.75 & 1.25

% delta-h-c - 100% 
 & \textbf{0.96}
% delta-h-c-uncertainty - 100% 
 & \textbf{0.96}
% rg2009 - 100% 
 & 0.88
% lm_hc0 - 100% 
 & 0.88
% lm_hc30 - 100% 
 & 0.5 & 12.75 & 1.25

% delta-h-c - 100% 
 & \textbf{0.96}
% delta-h-c-uncertainty - 100% 
 & \textbf{0.96}
% rg2009 - 100% 
 & 0.88
% lm_hc0 - 100% 
 & 0.88
% lm_hc30 - 100% 
 & 0.5 \\ \hline\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{sokoban}} } & \multirow{5}{*}{8.5} 
 & 10 & 2.33 & 2.11

% delta-h-c - 10% 
 & 0.39
% delta-h-c-uncertainty - 10% 
 & 0.38
% rg2009 - 10% 
 & \textbf{0.4}
% lm_hc0 - 10% 
 & 0.28
% lm_hc30 - 10% 
 & 0.26 & 3.33 & 1.83

% delta-h-c - 10% 
 & \textbf{0.52}
% delta-h-c-uncertainty - 10% 
 & 0.44
% rg2009 - 10% 
 & 0.29
% lm_hc0 - 10% 
 & 0.35
% lm_hc30 - 10% 
 & 0.24
\\ & & 30 & 6.5 & 1.25

% delta-h-c - 30% 
 & \textbf{0.75}
% delta-h-c-uncertainty - 30% 
 & 0.64
% rg2009 - 30% 
 & 0.56
% lm_hc0 - 30% 
 & 0.57
% lm_hc30 - 30% 
 & 0.23 & 8.67 & 1.28

% delta-h-c - 30% 
 & \textbf{0.77}
% delta-h-c-uncertainty - 30% 
 & 0.62
% rg2009 - 30% 
 & 0.43
% lm_hc0 - 30% 
 & 0.56
% lm_hc30 - 30% 
 & 0.24
\\ & & 50 & 10.33 & 1.22

% delta-h-c - 50% 
 & \textbf{0.92}
% delta-h-c-uncertainty - 50% 
 & 0.83
% rg2009 - 50% 
 & 0.61
% lm_hc0 - 50% 
 & 0.61
% lm_hc30 - 50% 
 & 0.28 & 13.75 & 1.33

% delta-h-c - 50% 
 & \textbf{0.79}
% delta-h-c-uncertainty - 50% 
 & 0.66
% rg2009 - 50% 
 & 0.53
% lm_hc0 - 50% 
 & 0.58
% lm_hc30 - 50% 
 & 0.25
\\ & & 70 & 14.67 & 1.03

% delta-h-c - 70% 
 & \textbf{0.99}
% delta-h-c-uncertainty - 70% 
 & 0.94
% rg2009 - 70% 
 & 0.64
% lm_hc0 - 70% 
 & 0.85
% lm_hc30 - 70% 
 & 0.36 & 19.33 & 1.36

% delta-h-c - 70% 
 & 0.8
% delta-h-c-uncertainty - 70% 
 & \textbf{0.85}
% rg2009 - 70% 
 & 0.54
% lm_hc0 - 70% 
 & 0.63
% lm_hc30 - 70% 
 & 0.3
\\ & & 100 & 20.17 & 1.0

% delta-h-c - 100% 
 & \textbf{1.0}
% delta-h-c-uncertainty - 100% 
 & \textbf{1.0}
% rg2009 - 100% 
 & 0.67
% lm_hc0 - 100% 
 & \textbf{1.0}
% lm_hc30 - 100% 
 & 0.42 & 27.0 & 1.33

% delta-h-c - 100% 
 & \textbf{0.83}
% delta-h-c-uncertainty - 100% 
 & \textbf{0.83}
% rg2009 - 100% 
 & 0.58
% lm_hc0 - 100% 
 & \textbf{0.83}
% lm_hc30 - 100% 
 & 0.38 \\ \hline
Avg & &  & &  & \textbf{0.88} & 0.87 & 0.81 & 0.71 & 0.43 & &  & \textbf{0.84} & 0.78 & 0.77 & 0.72 & 0.42\\
\bottomrule
\end{tabular}\\

==> tables/uncertainty-full.tex <==
\begin{tabular}{c|c|ccc|ccc|ccc|ccc|ccc|ccc||ccc|ccc|ccc|ccc|ccc|ccc}
\toprule
 \multicolumn{2}{c}{} & \multicolumn{18}{c}{Optimal} & \multicolumn{18}{c}{Sub-Optimal}\\
\cmidrule(lr){3-20}\cmidrule(lr){21-38}
%
 \multicolumn{2}{c}{} & \multicolumn{3}{c}{\dhc} & \multicolumn{3}{c}{\dhcu} & \multicolumn{3}{c}{\rg} & \multicolumn{3}{c}{\pom} & \multicolumn{3}{c}{\pomA} & \multicolumn{3}{c}{\pomC}%
  & \multicolumn{3}{c}{\dhc} & \multicolumn{3}{c}{\dhcu} & \multicolumn{3}{c}{\rg} & \multicolumn{3}{c}{\pom} & \multicolumn{3}{c}{\pomA} & \multicolumn{3}{c}{\pomC}\\
\cmidrule(lr){3-5}\cmidrule(lr){6-8}\cmidrule(lr){9-11}\cmidrule(lr){12-14}\cmidrule(lr){15-17}\cmidrule(lr){18-20}\cmidrule(lr){21-23}%
 \cmidrule(lr){24-26}\cmidrule(lr){27-29}\cmidrule(lr){30-32}\cmidrule(lr){33-35}\cmidrule(lr){36-38}
%
\% & \# & AGR & ACC & SPR & AGR & ACC & SPR & AGR & ACC & SPR & AGR & ACC & SPR & AGR & ACC & SPR & AGR & ACC & SPR & AGR & ACC & SPR%
 & AGR & ACC & SPR & AGR & ACC & SPR & AGR & ACC & SPR & AGR & ACC & SPR & AGR & ACC & SPR\\
\midrule
10 &\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{blocks}}}  & 0.44 & 0.86 & 7.53 & 0.44 & 0.86 & 7.56 & \textbf{0.47} & 0.92 & 9.83 & 0.06 & 0.17 & 1.44 & 0.13 & 0.47 & 4.06 & 0.38 & 1.0 & 18.14 & 0.41 & 0.86 & 6.86 & 0.42 & 0.89 & 7.42 & \textbf{0.46} & 0.97 & 10.61 & 0.06 & 0.19 & 1.19 & 0.19 & 0.58 & 4.44 & 0.34 & 1.0 & 17.53\\
30 & & \textbf{0.46} & 0.78 & 2.5 & 0.44 & 0.86 & 4.67 & 0.45 & 0.92 & 5.56 & 0.21 & 0.39 & 1.17 & 0.3 & 0.75 & 2.94 & 0.24 & 1.0 & 15.25 & 0.49 & 0.78 & 3.17 & 0.35 & 0.86 & 6.92 & \textbf{0.54} & 1.0 & 4.86 & 0.28 & 0.56 & 1.17 & 0.32 & 0.89 & 3.36 & 0.26 & 1.0 & 13.47\\
50 & & 0.59 & 0.89 & 3.03 & 0.52 & 0.89 & 3.86 & \textbf{0.62} & 0.97 & 3.69 & 0.33 & 0.58 & 1.25 & 0.37 & 0.81 & 3.08 & 0.25 & 0.97 & 12.17 & 0.55 & 0.86 & 3.08 & 0.42 & 0.94 & 5.61 & \textbf{0.62} & 0.97 & 2.72 & 0.39 & 0.72 & 1.08 & 0.36 & 0.81 & 2.17 & 0.27 & 1.0 & 9.89\\
70 & & \textbf{0.85} & 0.97 & 1.83 & 0.76 & 0.97 & 2.42 & 0.81 & 1.0 & 2.22 & 0.51 & 0.72 & 1.14 & 0.45 & 0.94 & 2.19 & 0.25 & 1.0 & 9.22 & \textbf{0.71} & 0.92 & 2.06 & 0.56 & 0.94 & 3.06 & 0.68 & 1.0 & 2.44 & 0.51 & 0.94 & 1.33 & 0.44 & 1.0 & 2.22 & 0.26 & 1.0 & 8.61\\
100 & & \textbf{0.92} & 1.0 & 1.67 & \textbf{0.92} & 1.0 & 1.67 & 0.9 & 1.0 & 2.08 & 0.59 & 1.0 & 1.67 & 0.55 & 1.0 & 1.92 & 0.31 & 1.0 & 6.42 & \textbf{0.84} & 1.0 & 1.67 & \textbf{0.84} & 1.0 & 1.67 & 0.8 & 1.0 & 2.08 & 0.51 & 1.0 & 1.67 & 0.48 & 1.0 & 1.92 & 0.28 & 1.0 & 6.42\\\hline%
10 & \multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{depots}}} & \textbf{0.69} & 0.72 & 3.81 & \textbf{0.69} & 0.72 & 3.81 & \textbf{0.69} & 0.78 & 4.78 & 0.24 & 0.17 & 1.94 & 0.38 & 0.42 & 3.5 & 0.53 & 0.97 & 7.22 & \textbf{0.53} & 0.67 & 2.06 & 0.52 & 0.75 & 2.94 & 0.41 & 0.83 & 4.56 & 0.26 & 0.44 & 2.06 & 0.29 & 0.67 & 3.5 & 0.29 & 0.97 & 7.0\\
30 & & 0.51 & 0.67 & 2.11 & 0.47 & 0.72 & 2.64 & \textbf{0.55} & 0.92 & 3.86 & 0.31 & 0.36 & 1.61 & 0.39 & 0.56 & 2.58 & 0.29 & 0.97 & 6.42 & 0.5 & 0.69 & 2.36 & 0.43 & 0.83 & 3.97 & \textbf{0.51} & 0.81 & 3.5 & 0.29 & 0.44 & 1.75 & 0.34 & 0.67 & 2.81 & 0.24 & 0.94 & 6.53\\
50 & & \textbf{0.68} & 0.78 & 1.64 & 0.65 & 0.89 & 2.31 & 0.63 & 0.89 & 2.33 & 0.64 & 0.67 & 1.28 & 0.59 & 0.75 & 1.89 & 0.22 & 0.92 & 5.22 & \textbf{0.8} & 0.89 & 1.47 & 0.4 & 1.0 & 4.31 & 0.62 & 0.89 & 2.14 & 0.56 & 0.67 & 1.67 & 0.56 & 0.83 & 2.42 & 0.21 & 0.97 & 5.61\\
70 & & \textbf{0.95} & 0.97 & 1.14 & 0.86 & 0.97 & 1.5 & 0.71 & 0.94 & 1.86 & 0.68 & 0.72 & 1.11 & 0.59 & 0.97 & 1.83 & 0.27 & 1.0 & 4.36 & \textbf{0.96} & 1.0 & 1.11 & 0.65 & 1.0 & 2.61 & 0.71 & 0.92 & 1.72 & 0.75 & 0.75 & 1.08 & 0.7 & 0.89 & 1.5 & 0.29 & 1.0 & 4.39\\
100 & & \textbf{1.0} & 1.0 & 1.0 & \textbf{1.0} & 1.0 & 1.0 & 0.85 & 0.92 & 1.25 & \textbf{1.0} & 1.0 & 1.0 & 0.71 & 1.0 & 1.58 & 0.36 & 1.0 & 2.92 & \textbf{1.0} & 1.0 & 1.0 & \textbf{1.0} & 1.0 & 1.0 & 0.85 & 0.92 & 1.25 & \textbf{1.0} & 1.0 & 1.0 & 0.71 & 1.0 & 1.58 & 0.36 & 1.0 & 2.92\\\hline%
10 & \multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{driverlog}}} & \textbf{0.54} & 0.75 & 2.64 & \textbf{0.54} & 0.75 & 2.67 & \textbf{0.54} & 0.97 & 4.89 & 0.33 & 0.36 & 1.11 & 0.36 & 0.5 & 1.78 & 0.34 & 0.92 & 5.22 & \textbf{0.49} & 0.81 & 2.69 & 0.46 & 0.89 & 3.53 & 0.39 & 0.89 & 4.67 & 0.3 & 0.44 & 1.14 & 0.27 & 0.56 & 1.92 & 0.3 & 0.92 & 5.22\\
30 & & \textbf{0.66} & 0.83 & 1.75 & 0.63 & 0.89 & 2.03 & 0.43 & 0.97 & 4.22 & 0.46 & 0.64 & 1.31 & 0.42 & 0.72 & 1.86 & 0.3 & 0.92 & 4.86 & \textbf{0.67} & 0.92 & 1.72 & 0.47 & 0.92 & 3.22 & 0.44 & 0.92 & 3.03 & 0.48 & 0.69 & 1.44 & 0.43 & 0.78 & 2.06 & 0.29 & 1.0 & 4.69\\
50 & & \textbf{0.69} & 0.97 & 1.61 & 0.62 & 0.97 & 1.97 & 0.41 & 0.94 & 3.39 & 0.58 & 0.64 & 1.19 & 0.55 & 0.75 & 1.64 & 0.23 & 0.94 & 4.94 & \textbf{0.72} & 0.94 & 1.5 & 0.51 & 1.0 & 3.0 & 0.49 & 0.94 & 2.78 & 0.65 & 0.92 & 1.47 & 0.55 & 0.94 & 1.94 & 0.3 & 1.0 & 4.17\\
70 & & \textbf{0.9} & 0.97 & 1.31 & \textbf{0.9} & 0.97 & 1.31 & 0.49 & 0.92 & 2.44 & 0.69 & 0.92 & 1.5 & 0.63 & 0.94 & 1.83 & 0.31 & 1.0 & 4.22 & \textbf{0.85} & 0.94 & 1.28 & 0.64 & 1.0 & 2.17 & 0.61 & 0.92 & 2.03 & 0.65 & 0.94 & 1.5 & 0.59 & 0.94 & 1.72 & 0.35 & 1.0 & 3.83\\
100 & & \textbf{0.96} & 1.0 & 1.17 & \textbf{0.96} & 1.0 & 1.17 & 0.61 & 0.92 & 1.83 & 0.76 & 1.0 & 1.5 & 0.76 & 1.0 & 1.5 & 0.32 & 1.0 & 3.58 & \textbf{0.93} & 1.0 & 1.17 & \textbf{0.93} & 1.0 & 1.17 & 0.6 & 0.92 & 1.83 & 0.76 & 1.0 & 1.5 & 0.76 & 1.0 & 1.5 & 0.31 & 1.0 & 3.58\\\hline%
10 & \multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{dwr}}} & \textbf{0.79} & 0.81 & 3.25 & 0.76 & 0.92 & 4.19 & 0.67 & 0.72 & 3.5 & 0.45 & 0.53 & 1.39 & 0.67 & 0.94 & 4.14 & 0.51 & 1.0 & 6.64 & \textbf{0.75} & 0.86 & 2.67 & 0.69 & 0.92 & 3.78 & 0.66 & 0.89 & 3.5 & 0.46 & 0.5 & 1.44 & 0.63 & 0.92 & 4.31 & 0.43 & 1.0 & 6.61\\
30 & & \textbf{0.8} & 0.86 & 1.89 & 0.75 & 0.97 & 3.0 & 0.58 & 0.86 & 3.08 & 0.55 & 0.72 & 1.19 & 0.58 & 0.97 & 3.22 & 0.3 & 1.0 & 6.39 & \textbf{0.71} & 0.86 & 2.0 & 0.57 & 1.0 & 3.89 & 0.64 & 0.89 & 2.78 & 0.66 & 0.81 & 1.28 & 0.59 & 0.94 & 3.14 & 0.29 & 1.0 & 6.28\\
50 & & \textbf{0.91} & 1.0 & 1.39 & 0.79 & 1.0 & 2.31 & 0.71 & 0.92 & 1.97 & 0.76 & 0.83 & 1.06 & 0.73 & 0.97 & 2.03 & 0.24 & 1.0 & 6.08 & \textbf{0.84} & 0.94 & 1.5 & 0.73 & 1.0 & 2.67 & 0.68 & 0.97 & 2.47 & 0.76 & 0.92 & 1.06 & 0.77 & 0.97 & 1.89 & 0.28 & 1.0 & 5.67\\
70 & & \textbf{0.9} & 1.0 & 1.25 & 0.84 & 1.0 & 1.64 & 0.75 & 0.86 & 1.39 & 0.84 & 0.86 & 1.06 & 0.83 & 1.0 & 1.61 & 0.25 & 1.0 & 5.22 & 0.88 & 1.0 & 1.25 & 0.74 & 1.0 & 2.08 & 0.72 & 0.86 & 1.53 & \textbf{0.89} & 0.97 & 1.0 & 0.82 & 1.0 & 1.56 & 0.24 & 1.0 & 5.42\\
100 & & 0.92 & 1.0 & 1.08 & 0.92 & 1.0 & 1.08 & 0.86 & 1.0 & 1.25 & \textbf{0.96} & 1.0 & 1.0 & 0.85 & 1.0 & 1.33 & 0.29 & 1.0 & 4.42 & 0.92 & 1.0 & 1.08 & 0.92 & 1.0 & 1.08 & 0.86 & 1.0 & 1.25 & \textbf{0.96} & 1.0 & 1.0 & 0.85 & 1.0 & 1.33 & 0.29 & 1.0 & 4.42\\\hline% 
10 & \multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{ferry}}} & \textbf{0.88} & 1.0 & 4.25 & \textbf{0.88} & 1.0 & 4.25 & \textbf{0.88} & 1.0 & 3.92 & 0.48 & 0.53 & 2.08 & 0.61 & 0.89 & 3.97 & 0.55 & 1.0 & 6.31 & \textbf{0.71} & 1.0 & 4.19 & 0.68 & 1.0 & 4.44 & \textbf{0.71} & 1.0 & 3.97 & 0.51 & 0.61 & 1.86 & 0.55 & 0.83 & 3.89 & 0.4 & 1.0 & 6.31\\
30 & & \textbf{0.9} & 1.0 & 1.97 & 0.85 & 1.0 & 2.22 & 0.88 & 0.97 & 1.83 & 0.72 & 0.81 & 1.36 & 0.71 & 0.97 & 2.42 & 0.26 & 1.0 & 6.11 & \textbf{0.88} & 1.0 & 1.69 & 0.57 & 1.0 & 3.56 & 0.8 & 0.92 & 1.53 & 0.77 & 0.89 & 1.19 & 0.66 & 1.0 & 1.97 & 0.23 & 1.0 & 5.89\\
50 & & \textbf{0.98} & 1.0 & 1.28 & 0.9 & 1.0 & 1.58 & 0.9 & 0.94 & 1.17 & 0.89 & 0.92 & 1.06 & 0.81 & 0.97 & 1.39 & 0.24 & 1.0 & 4.94 & \textbf{0.88} & 1.0 & 1.5 & 0.71 & 1.0 & 2.33 & 0.8 & 0.97 & 1.53 & 0.81 & 0.94 & 1.22 & 0.71 & 0.97 & 1.56 & 0.27 & 1.0 & 4.64\\
70 & & \textbf{0.99} & 1.0 & 1.22 & \textbf{0.99} & 1.0 & 1.22 & 0.93 & 1.0 & 1.22 & 0.96 & 0.97 & 1.0 & 0.87 & 1.0 & 1.25 & 0.28 & 1.0 & 4.0 & \textbf{0.96} & 1.0 & 1.25 & 0.89 & 1.0 & 1.61 & 0.92 & 1.0 & 1.25 & 0.9 & 0.97 & 1.03 & 0.88 & 1.0 & 1.17 & 0.35 & 1.0 & 3.69\\
100 & & \textbf{1.0} & 1.0 & 1.17 & \textbf{1.0} & 1.0 & 1.17 & \textbf{1.0} & 1.0 & 1.0 & \textbf{1.0} & 1.0 & 1.0 & \textbf{1.0} & 1.0 & 1.0 & 0.57 & 1.0 & 2.33 & \textbf{0.96} & 1.0 & 1.17 & \textbf{0.96} & 1.0 & 1.17 & \textbf{0.96} & 1.0 & 1.0 & \textbf{0.96} & 1.0 & 1.0 & \textbf{0.96} & 1.0 & 1.0 & 0.61 & 1.0 & 2.33\\\hline%
10 & \multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{ipc-grid}}} & 0.87 & 0.94 & 2.67 & 0.88 & 0.96 & 2.69 & \textbf{0.91} & 1.0 & 3.23 & 0.47 & 0.75 & 2.35 & 0.55 & 0.98 & 4.38 & 0.49 & 1.0 & 6.25 & 0.77 & 0.92 & 1.81 & 0.75 & 0.98 & 2.4 & \textbf{0.81} & 1.0 & 2.73 & 0.64 & 0.88 & 2.23 & 0.59 & 0.98 & 3.44 & 0.42 & 1.0 & 5.6\\
30 & & 0.93 & 0.96 & 1.15 & 0.94 & 0.98 & 1.17 & \textbf{0.99} & 1.0 & 1.25 & 0.85 & 0.98 & 1.52 & 0.81 & 1.0 & 1.96 & 0.64 & 1.0 & 3.17 & 0.82 & 0.94 & 1.13 & 0.77 & 0.98 & 1.6 & \textbf{0.9} & 1.0 & 1.27 & 0.81 & 0.96 & 1.35 & 0.8 & 0.96 & 1.52 & 0.67 & 0.96 & 2.23\\
50 & & 0.96 & 0.98 & 1.08 & 0.96 & 0.98 & 1.08 & \textbf{1.0} & 1.0 & 1.13 & 0.86 & 1.0 & 1.44 & 0.86 & 1.0 & 1.56 & 0.77 & 1.0 & 2.15 & 0.84 & 0.94 & 1.13 & 0.84 & 1.0 & 1.56 & \textbf{0.92} & 1.0 & 1.1 & 0.87 & 1.0 & 1.08 & 0.86 & 1.0 & 1.13 & 0.86 & 1.0 & 1.21\\
70 & & 0.97 & 0.98 & 1.06 & 0.97 & 0.98 & 1.06 & \textbf{1.0} & 1.0 & 1.04 & 0.97 & 0.98 & 1.02 & 0.97 & 0.98 & 1.02 & 0.93 & 0.98 & 1.15 & 0.89 & 1.0 & 1.1 & 0.85 & 1.0 & 1.23 & \textbf{0.93} & 1.0 & 1.02 & 0.92 & 1.0 & 1.0 & 0.92 & 1.0 & 1.0 & 0.92 & 1.0 & 1.0\\
100 & & \textbf{1.0} & 1.0 & 1.0 & \textbf{1.0} & 1.0 & 1.0 & \textbf{1.0} & 1.0 & 1.0 & \textbf{1.0} & 1.0 & 1.0 & \textbf{1.0} & 1.0 & 1.0 & \textbf{1.0} & 1.0 & 1.0 & \textbf{0.94} & 1.0 & 1.0 & \textbf{0.94} & 1.0 & 1.0 & \textbf{0.94} & 1.0 & 1.0 & \textbf{0.94} & 1.0 & 1.0 & \textbf{0.94} & 1.0 & 1.0 & \textbf{0.94} & 1.0 & 1.0\\\hline%
10 & \multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{logistics}}} & \textbf{0.9} & 1.0 & 3.53 & \textbf{0.9} & 1.0 & 3.53 & 0.87 & 1.0 & 3.78 & 0.43 & 0.58 & 2.11 & 0.53 & 0.92 & 5.56 & 0.31 & 1.0 & 9.53 & \textbf{0.88} & 1.0 & 2.44 & 0.85 & 1.0 & 2.72 & 0.72 & 0.92 & 3.11 & 0.56 & 0.67 & 2.08 & 0.45 & 0.92 & 4.81 & 0.21 & 1.0 & 9.75\\
30 & & \textbf{0.92} & 1.0 & 1.47 & \textbf{0.92} & 1.0 & 1.47 & 0.86 & 1.0 & 1.75 & 0.78 & 0.86 & 1.33 & 0.64 & 0.97 & 2.44 & 0.24 & 1.0 & 6.58 & \textbf{0.91} & 1.0 & 1.33 & 0.75 & 1.0 & 2.14 & 0.87 & 0.97 & 1.36 & 0.85 & 0.92 & 1.22 & 0.77 & 1.0 & 2.03 & 0.26 & 1.0 & 6.0\\
50 & & \textbf{0.96} & 1.0 & 1.17 & \textbf{0.96} & 1.0 & 1.17 & 0.93 & 1.0 & 1.25 & 0.9 & 0.94 & 1.17 & 0.85 & 1.0 & 1.39 & 0.39 & 1.0 & 4.36 & 0.88 & 0.97 & 1.25 & 0.86 & 1.0 & 1.47 & 0.91 & 1.0 & 1.25 & \textbf{0.93} & 0.97 & 1.03 & 0.84 & 1.0 & 1.44 & 0.39 & 1.0 & 3.69\\
70 & & 0.99 & 1.0 & 1.06 & 0.99 & 1.0 & 1.06 & 0.99 & 1.0 & 1.06 & \textbf{1.0} & 1.0 & 1.03 & 0.97 & 1.0 & 1.08 & 0.62 & 1.0 & 2.19 & 0.97 & 1.0 & 1.08 & 0.92 & 1.0 & 1.19 & \textbf{0.99} & 1.0 & 1.06 & \textbf{0.99} & 1.0 & 1.0 & \textbf{0.99} & 1.0 & 1.06 & 0.66 & 1.0 & 2.0\\
100 & & \textbf{1.0} & 1.0 & 1.0 & \textbf{1.0} & 1.0 & 1.0 & \textbf{1.0} & 1.0 & 1.0 & \textbf{1.0} & 1.0 & 1.0 & \textbf{1.0} & 1.0 & 1.0 & 0.72 & 1.0 & 1.67 & \textbf{1.0} & 1.0 & 1.0 & \textbf{1.0} & 1.0 & 1.0 & \textbf{1.0} & 1.0 & 1.0 & \textbf{1.0} & 1.0 & 1.0 & \textbf{1.0} & 1.0 & 1.0 & 0.72 & 1.0 & 1.67\\\hline%
10 & \multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{miconic}}} & \textbf{0.89} & 1.0 & 2.97 & \textbf{0.89} & 1.0 & 2.97 & 0.76 & 1.0 & 3.53 & 0.39 & 0.53 & 1.69 & 0.57 & 0.97 & 4.22 & 0.42 & 1.0 & 6.0 & \textbf{0.76} & 1.0 & 2.67 & 0.74 & 1.0 & 3.0 & 0.65 & 1.0 & 3.42 & 0.54 & 0.56 & 1.36 & 0.43 & 0.92 & 4.31 & 0.31 & 1.0 & 6.0\\
30 & & \textbf{0.95} & 1.0 & 1.36 & \textbf{0.95} & 1.0 & 1.36 & 0.65 & 1.0 & 2.17 & 0.83 & 0.89 & 1.19 & 0.55 & 1.0 & 2.61 & 0.22 & 1.0 & 5.69 & \textbf{0.89} & 1.0 & 1.47 & 0.65 & 1.0 & 2.5 & 0.66 & 1.0 & 2.17 & 0.86 & 0.92 & 1.08 & 0.53 & 1.0 & 2.72 & 0.23 & 1.0 & 5.58\\
50 & & \textbf{0.97} & 1.0 & 1.11 & \textbf{0.97} & 1.0 & 1.11 & 0.84 & 1.0 & 1.42 & 0.92 & 0.94 & 1.06 & 0.74 & 1.0 & 1.72 & 0.25 & 1.0 & 4.69 & \textbf{0.98} & 1.0 & 1.08 & 0.82 & 1.0 & 1.5 & 0.91 & 1.0 & 1.25 & 0.97 & 0.97 & 1.03 & 0.81 & 1.0 & 1.5 & 0.24 & 1.0 & 4.56\\
70 & & 0.98 & 1.0 & 1.06 & 0.98 & 1.0 & 1.06 & 0.91 & 1.0 & 1.19 & \textbf{0.99} & 1.0 & 1.03 & 0.81 & 1.0 & 1.39 & 0.31 & 1.0 & 3.94 & 0.99 & 1.0 & 1.03 & 0.9 & 1.0 & 1.31 & 0.94 & 1.0 & 1.11 & \textbf{1.0} & 1.0 & 1.0 & 0.84 & 1.0 & 1.33 & 0.31 & 1.0 & 3.94\\
100 & & \textbf{1.0} & 1.0 & 1.0 & \textbf{1.0} & 1.0 & 1.0 & \textbf{1.0} & 1.0 & 1.0 & \textbf{1.0} & 1.0 & 1.0 & \textbf{1.0} & 1.0 & 1.0 & 0.47 & 1.0 & 3.0 & \textbf{1.0} & 1.0 & 1.0 & \textbf{1.0} & 1.0 & 1.0 & \textbf{1.0} & 1.0 & 1.0 & \textbf{1.0} & 1.0 & 1.0 & \textbf{1.0} & 1.0 & 1.0 & 0.47 & 1.0 & 3.0\\\hline%
10 & \multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{rovers}}} & \textbf{0.83} & 0.97 & 2.75 & \textbf{0.83} & 0.97 & 2.75 & 0.76 & 1.0 & 3.42 & 0.49 & 0.53 & 1.22 & 0.62 & 0.81 & 2.94 & 0.44 & 1.0 & 5.28 & \textbf{0.83} & 0.89 & 2.89 & \textbf{0.83} & 0.89 & 2.89 & 0.82 & 1.0 & 3.42 & 0.45 & 0.56 & 1.31 & 0.6 & 0.89 & 2.97 & 0.48 & 1.0 & 5.14\\
30 & & \textbf{0.94} & 1.0 & 1.44 & \textbf{0.94} & 1.0 & 1.44 & 0.88 & 1.0 & 1.69 & 0.76 & 0.83 & 1.19 & 0.68 & 1.0 & 2.14 & 0.37 & 1.0 & 3.89 & \textbf{0.88} & 0.89 & 1.39 & 0.81 & 0.89 & 1.75 & 0.8 & 1.0 & 2.06 & 0.7 & 0.81 & 1.14 & 0.58 & 1.0 & 2.5 & 0.34 & 1.0 & 4.5\\
50 & & \textbf{0.92} & 0.89 & 1.08 & \textbf{0.92} & 0.89 & 1.08 & 0.91 & 1.0 & 1.42 & 0.79 & 0.89 & 1.14 & 0.74 & 1.0 & 1.97 & 0.39 & 1.0 & 3.67 & \textbf{0.93} & 0.94 & 1.14 & 0.86 & 0.94 & 1.33 & 0.89 & 1.0 & 1.36 & 0.8 & 0.89 & 1.19 & 0.64 & 1.0 & 1.97 & 0.34 & 1.0 & 3.92\\
70 & & \textbf{0.99} & 1.0 & 1.03 & \textbf{0.99} & 1.0 & 1.03 & 0.97 & 1.0 & 1.08 & 0.93 & 0.97 & 1.11 & 0.76 & 1.0 & 1.58 & 0.37 & 1.0 & 3.44 & 0.94 & 0.94 & 1.08 & 0.92 & 0.97 & 1.22 & \textbf{0.98} & 1.0 & 1.11 & 0.87 & 0.94 & 1.11 & 0.7 & 1.0 & 1.86 & 0.38 & 1.0 & 3.53\\
100 & & \textbf{1.0} & 1.0 & 1.0 & \textbf{1.0} & 1.0 & 1.0 & \textbf{1.0} & 1.0 & 1.0 & \textbf{1.0} & 1.0 & 1.0 & 0.82 & 1.0 & 1.42 & 0.39 & 1.0 & 3.0 & \textbf{1.0} & 1.0 & 1.0 & \textbf{1.0} & 1.0 & 1.0 & \textbf{1.0} & 1.0 & 1.0 & \textbf{1.0} & 1.0 & 1.0 & 0.82 & 1.0 & 1.42 & 0.39 & 1.0 & 3.0\\\hline%
10 & \multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{satellite}}} & 0.85 & 0.94 & 3.81 & 0.85 & 0.94 & 3.81 & \textbf{0.86} & 0.97 & 3.89 & 0.5 & 0.58 & 2.11 & 0.67 & 0.89 & 4.64 & 0.59 & 1.0 & 5.94 & \textbf{0.9} & 0.97 & 3.44 & \textbf{0.9} & 0.97 & 3.44 & 0.73 & 0.97 & 4.47 & 0.58 & 0.75 & 2.5 & 0.6 & 0.92 & 4.47 & 0.57 & 1.0 & 5.72\\
30 & & \textbf{0.86} & 0.92 & 2.44 & \textbf{0.86} & 0.92 & 2.44 & 0.72 & 0.94 & 3.44 & 0.64 & 0.83 & 2.03 & 0.58 & 0.94 & 3.58 & 0.44 & 1.0 & 5.39 & \textbf{0.8} & 0.94 & 2.22 & 0.78 & 0.94 & 2.33 & 0.68 & 0.92 & 2.97 & 0.6 & 0.81 & 1.53 & 0.46 & 0.92 & 3.44 & 0.34 & 1.0 & 5.42\\
50 & & \textbf{0.93} & 0.97 & 1.53 & 0.91 & 0.97 & 1.58 & 0.79 & 0.94 & 2.25 & 0.73 & 0.89 & 1.28 & 0.65 & 0.94 & 2.47 & 0.35 & 1.0 & 4.81 & \textbf{0.92} & 0.94 & 1.42 & 0.85 & 0.94 & 1.72 & 0.7 & 0.97 & 2.53 & 0.76 & 0.92 & 1.19 & 0.5 & 0.97 & 2.75 & 0.33 & 1.0 & 4.92\\
70 & & \textbf{0.94} & 1.0 & 1.28 & \textbf{0.94} & 1.0 & 1.28 & 0.81 & 0.97 & 2.06 & 0.89 & 1.0 & 1.19 & 0.69 & 1.0 & 1.92 & 0.37 & 1.0 & 4.06 & \textbf{0.94} & 1.0 & 1.36 & \textbf{0.94} & 1.0 & 1.36 & 0.78 & 0.97 & 2.06 & 0.85 & 0.97 & 1.14 & 0.65 & 0.97 & 2.17 & 0.41 & 1.0 & 4.14\\
100 & & \textbf{0.96} & 1.0 & 1.17 & \textbf{0.96} & 1.0 & 1.17 & 0.88 & 1.0 & 1.75 & 0.88 & 1.0 & 1.17 & 0.75 & 1.0 & 1.58 & 0.5 & 1.0 & 3.33 & \textbf{0.96} & 1.0 & 1.17 & \textbf{0.96} & 1.0 & 1.17 & 0.88 & 1.0 & 1.75 & 0.88 & 1.0 & 1.17 & 0.75 & 1.0 & 1.58 & 0.5 & 1.0 & 3.33\\\hline%
10 & \multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{sokoban}}} & 0.39 & 0.53 & 2.08 & 0.38 & 0.61 & 2.94 & \textbf{0.4} & 0.81 & 4.86 & 0.28 & 0.53 & 2.14 & 0.32 & 0.89 & 4.39 & 0.26 & 0.97 & 7.0 & \textbf{0.52} & 0.61 & 1.78 & 0.44 & 0.72 & 3.17 & 0.29 & 0.64 & 4.56 & 0.35 & 0.64 & 2.47 & 0.38 & 0.92 & 4.08 & 0.24 & 1.0 & 6.86\\
30 & & \textbf{0.75} & 0.81 & 1.25 & 0.64 & 0.92 & 2.06 & 0.56 & 0.86 & 2.53 & 0.57 & 0.69 & 1.22 & 0.48 & 0.75 & 1.89 & 0.23 & 0.94 & 5.17 & \textbf{0.77} & 0.83 & 1.08 & 0.62 & 0.97 & 2.67 & 0.43 & 0.75 & 2.92 & 0.56 & 0.75 & 1.72 & 0.51 & 0.86 & 2.64 & 0.24 & 0.97 & 5.5\\
50 & & \textbf{0.92} & 1.0 & 1.19 & 0.83 & 1.0 & 1.39 & 0.61 & 0.86 & 2.14 & 0.61 & 0.69 & 1.42 & 0.55 & 0.81 & 2.14 & 0.28 & 1.0 & 5.08 & \textbf{0.79} & 0.92 & 1.17 & 0.66 & 1.0 & 2.58 & 0.53 & 0.72 & 1.83 & 0.58 & 0.75 & 1.39 & 0.53 & 0.86 & 2.31 & 0.25 & 0.97 & 5.14\\
70 & & \textbf{0.99} & 1.0 & 1.0 & 0.94 & 1.0 & 1.08 & 0.64 & 0.83 & 1.53 & 0.85 & 0.92 & 1.17 & 0.81 & 0.94 & 1.39 & 0.36 & 1.0 & 3.64 & 0.8 & 0.97 & 1.03 & \textbf{0.85} & 1.0 & 1.39 & 0.54 & 0.61 & 1.28 & 0.63 & 0.86 & 1.25 & 0.59 & 0.92 & 1.75 & 0.3 & 1.0 & 4.11\\
100 & & \textbf{1.0} & 1.0 & 1.0 & \textbf{1.0} & 1.0 & 1.0 & 0.67 & 0.75 & 1.17 & \textbf{1.0} & 1.0 & 1.0 & \textbf{1.0} & 1.0 & 1.0 & 0.42 & 1.0 & 2.75 & \textbf{0.83} & 1.0 & 1.0 & \textbf{0.83} & 1.0 & 1.0 & 0.58 & 0.58 & 1.33 & \textbf{0.83} & 1.0 & 1.0 & \textbf{0.83} & 1.0 & 1.0 & 0.38 & 1.0 & 2.75\\\hline%
10 & \multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{zeno}}} & \textbf{0.67} & 0.78 & 2.42 & \textbf{0.67} & 0.78 & 2.42 & 0.65 & 0.89 & 3.25 & 0.33 & 0.39 & 1.39 & 0.41 & 0.64 & 2.33 & 0.4 & 1.0 & 5.69 & \textbf{0.64} & 0.83 & 2.53 & 0.63 & 0.89 & 2.83 & 0.58 & 0.94 & 3.17 & 0.38 & 0.47 & 1.44 & 0.46 & 0.81 & 2.5 & 0.34 & 1.0 & 5.44\\
30 & & \textbf{0.76} & 0.89 & 1.44 & 0.74 & 0.94 & 1.75 & 0.69 & 0.92 & 2.0 & 0.63 & 0.64 & 1.17 & 0.57 & 0.86 & 2.0 & 0.28 & 1.0 & 5.0 & \textbf{0.73} & 0.83 & 1.47 & 0.63 & 0.97 & 2.64 & 0.71 & 0.92 & 1.81 & 0.67 & 0.75 & 1.22 & 0.62 & 0.86 & 1.64 & 0.31 & 1.0 & 4.33\\
50 & & \textbf{0.9} & 0.94 & 1.08 & 0.81 & 0.97 & 1.53 & 0.78 & 0.94 & 1.56 & 0.76 & 0.89 & 1.25 & 0.61 & 0.94 & 2.06 & 0.27 & 1.0 & 4.5 & \textbf{0.87} & 0.92 & 1.11 & 0.72 & 1.0 & 1.75 & 0.84 & 0.92 & 1.33 & 0.85 & 0.89 & 1.14 & 0.79 & 1.0 & 1.64 & 0.3 & 1.0 & 4.17\\
70 & & \textbf{0.94} & 0.94 & 1.0 & \textbf{0.94} & 0.94 & 1.0 & 0.88 & 0.92 & 1.11 & 0.92 & 0.97 & 1.11 & 0.83 & 1.0 & 1.47 & 0.33 & 1.0 & 3.81 & \textbf{0.94} & 0.94 & 1.0 & 0.92 & 0.97 & 1.11 & 0.88 & 0.94 & 1.22 & \textbf{0.94} & 0.97 & 1.06 & 0.9 & 1.0 & 1.28 & 0.39 & 1.0 & 3.39\\
100 & & \textbf{1.0} & 1.0 & 1.0 & \textbf{1.0} & 1.0 & 1.0 & 0.88 & 0.92 & 1.08 & 0.96 & 1.0 & 1.08 & 0.94 & 1.0 & 1.17 & 0.46 & 1.0 & 2.83 & \textbf{1.0} & 1.0 & 1.0 & \textbf{1.0} & 1.0 & 1.0 & 0.88 & 0.92 & 1.08 & 0.96 & 1.0 & 1.08 & 0.94 & 1.0 & 1.17 & 0.46 & 1.0 & 2.83\\\midrule
\multicolumn{2}{c|}{AVG} & \textbf{0.86} & 0.94 & 1.79 & 0.84 & 0.95 & 1.99 & 0.77 & 0.95 & 2.39 & 0.7 & 0.79 & 1.31 & 0.67 & 0.91 & 2.22 & 0.39 & 0.99 & 5.2 & \textbf{0.82} & 0.93 & 1.71 & 0.75 & 0.97 & 2.39 & 0.74 & 0.93 & 2.3 & 0.7 & 0.83 & 1.31 & 0.65 & 0.93 & 2.19 & 0.38 & 1.0 & 5.01%
\\
\bottomrule
\end{tabular}

==> tables/uncertainty.tex <==
\begin{tabular}{c|c|ccc|ccc|ccc|ccc|ccc|ccc||ccc|ccc|ccc|ccc|ccc|ccc}
\toprule
 \multicolumn{2}{c}{} & \multicolumn{18}{c}{Optimal} & \multicolumn{18}{c}{Sub-Optimal}\\
\cmidrule(lr){3-20}\cmidrule(lr){21-38}
%
 \multicolumn{2}{c}{} & \multicolumn{3}{c}{\dhc} & \multicolumn{3}{c}{\dhcu} & \multicolumn{3}{c}{\rg} & \multicolumn{3}{c}{\pom} & \multicolumn{3}{c}{\pomA} & \multicolumn{3}{c}{\pomC}%
  & \multicolumn{3}{c}{\dhc} & \multicolumn{3}{c}{\dhcu} & \multicolumn{3}{c}{\rg} & \multicolumn{3}{c}{\pom} & \multicolumn{3}{c}{\pomA} & \multicolumn{3}{c}{\pomC}\\
\cmidrule(lr){3-5}\cmidrule(lr){6-8}\cmidrule(lr){9-11}\cmidrule(lr){12-14}\cmidrule(lr){15-17}\cmidrule(lr){18-20}\cmidrule(lr){21-23}%
 \cmidrule(lr){24-26}\cmidrule(lr){27-29}\cmidrule(lr){30-32}\cmidrule(lr){33-35}\cmidrule(lr){36-38}
%
\% & \# & AGR & ACC & SPR & AGR & ACC & SPR & AGR & ACC & SPR & AGR & ACC & SPR & AGR & ACC & SPR & AGR & ACC & SPR & AGR & ACC & SPR%
 & AGR & ACC & SPR & AGR & ACC & SPR & AGR & ACC & SPR & AGR & ACC & SPR & AGR & ACC & SPR\\
\midrule
 10 &\multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{blocks}}}  & 0.44 & 0.86 & 7.53 & 0.44 & 0.86 & 7.56 & \textbf{0.47} & 0.92 & 9.83 & 0.06 & 0.17 & 1.44 & 0.13 & 0.47 & 4.06 & 0.38 & 1.0 & 18.14 & 0.41 & 0.86 & 6.86 & 0.42 & 0.89 & 7.42 & \textbf{0.46} & 0.97 & 10.61 & 0.06 & 0.19 & 1.19 & 0.19 & 0.58 & 4.44 & 0.34 & 1.0 & 17.53\\
 30 & & \textbf{0.46} & 0.78 & 2.5 & 0.44 & 0.86 & 4.67 & 0.45 & 0.92 & 5.56 & 0.21 & 0.39 & 1.17 & 0.3 & 0.75 & 2.94 & 0.24 & 1.0 & 15.25 & 0.49 & 0.78 & 3.17 & 0.35 & 0.86 & 6.92 & \textbf{0.54} & 1.0 & 4.86 & 0.28 & 0.56 & 1.17 & 0.32 & 0.89 & 3.36 & 0.26 & 1.0 & 13.47\\
 50 & & 0.59 & 0.89 & 3.03 & 0.52 & 0.89 & 3.86 & \textbf{0.62} & 0.97 & 3.69 & 0.33 & 0.58 & 1.25 & 0.37 & 0.81 & 3.08 & 0.25 & 0.97 & 12.17 & 0.55 & 0.86 & 3.08 & 0.42 & 0.94 & 5.61 & \textbf{0.62} & 0.97 & 2.72 & 0.39 & 0.72 & 1.08 & 0.36 & 0.81 & 2.17 & 0.27 & 1.0 & 9.89\\
 70 & & \textbf{0.85} & 0.97 & 1.83 & 0.76 & 0.97 & 2.42 & 0.81 & 1.0 & 2.22 & 0.51 & 0.72 & 1.14 & 0.45 & 0.94 & 2.19 & 0.25 & 1.0 & 9.22 & \textbf{0.71} & 0.92 & 2.06 & 0.56 & 0.94 & 3.06 & 0.68 & 1.0 & 2.44 & 0.51 & 0.94 & 1.33 & 0.44 & 1.0 & 2.22 & 0.26 & 1.0 & 8.61\\
 100 & & \textbf{0.92} & 1.0 & 1.67 & \textbf{0.92} & 1.0 & 1.67 & 0.9 & 1.0 & 2.08 & 0.59 & 1.0 & 1.67 & 0.55 & 1.0 & 1.92 & 0.31 & 1.0 & 6.42 & \textbf{0.84} & 1.0 & 1.67 & \textbf{0.84} & 1.0 & 1.67 & 0.8 & 1.0 & 2.08 & 0.51 & 1.0 & 1.67 & 0.48 & 1.0 & 1.92 & 0.28 & 1.0 & 6.42\\\hline%
 10 & \multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{depots}}} & \textbf{0.69} & 0.72 & 3.81 & \textbf{0.69} & 0.72 & 3.81 & \textbf{0.69} & 0.78 & 4.78 & 0.24 & 0.17 & 1.94 & 0.38 & 0.42 & 3.5 & 0.53 & 0.97 & 7.22 & \textbf{0.53} & 0.67 & 2.06 & 0.52 & 0.75 & 2.94 & 0.41 & 0.83 & 4.56 & 0.26 & 0.44 & 2.06 & 0.29 & 0.67 & 3.5 & 0.29 & 0.97 & 7.0\\
 30 & & 0.51 & 0.67 & 2.11 & 0.47 & 0.72 & 2.64 & \textbf{0.55} & 0.92 & 3.86 & 0.31 & 0.36 & 1.61 & 0.39 & 0.56 & 2.58 & 0.29 & 0.97 & 6.42 & 0.5 & 0.69 & 2.36 & 0.43 & 0.83 & 3.97 & \textbf{0.51} & 0.81 & 3.5 & 0.29 & 0.44 & 1.75 & 0.34 & 0.67 & 2.81 & 0.24 & 0.94 & 6.53\\
 50 & & \textbf{0.68} & 0.78 & 1.64 & 0.65 & 0.89 & 2.31 & 0.63 & 0.89 & 2.33 & 0.64 & 0.67 & 1.28 & 0.59 & 0.75 & 1.89 & 0.22 & 0.92 & 5.22 & \textbf{0.8} & 0.89 & 1.47 & 0.4 & 1.0 & 4.31 & 0.62 & 0.89 & 2.14 & 0.56 & 0.67 & 1.67 & 0.56 & 0.83 & 2.42 & 0.21 & 0.97 & 5.61\\
 70 & & \textbf{0.95} & 0.97 & 1.14 & 0.86 & 0.97 & 1.5 & 0.71 & 0.94 & 1.86 & 0.68 & 0.72 & 1.11 & 0.59 & 0.97 & 1.83 & 0.27 & 1.0 & 4.36 & \textbf{0.96} & 1.0 & 1.11 & 0.65 & 1.0 & 2.61 & 0.71 & 0.92 & 1.72 & 0.75 & 0.75 & 1.08 & 0.7 & 0.89 & 1.5 & 0.29 & 1.0 & 4.39\\
 100 & & \textbf{1.0} & 1.0 & 1.0 & \textbf{1.0} & 1.0 & 1.0 & 0.85 & 0.92 & 1.25 & \textbf{1.0} & 1.0 & 1.0 & 0.71 & 1.0 & 1.58 & 0.36 & 1.0 & 2.92 & \textbf{1.0} & 1.0 & 1.0 & \textbf{1.0} & 1.0 & 1.0 & 0.85 & 0.92 & 1.25 & \textbf{1.0} & 1.0 & 1.0 & 0.71 & 1.0 & 1.58 & 0.36 & 1.0 & 2.92\\\hline%
 10 & \multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{driverlog}}} & \textbf{0.54} & 0.75 & 2.64 & \textbf{0.54} & 0.75 & 2.67 & \textbf{0.54} & 0.97 & 4.89 & 0.33 & 0.36 & 1.11 & 0.36 & 0.5 & 1.78 & 0.34 & 0.92 & 5.22 & \textbf{0.49} & 0.81 & 2.69 & 0.46 & 0.89 & 3.53 & 0.39 & 0.89 & 4.67 & 0.3 & 0.44 & 1.14 & 0.27 & 0.56 & 1.92 & 0.3 & 0.92 & 5.22\\
 30 & & \textbf{0.66} & 0.83 & 1.75 & 0.63 & 0.89 & 2.03 & 0.43 & 0.97 & 4.22 & 0.46 & 0.64 & 1.31 & 0.42 & 0.72 & 1.86 & 0.3 & 0.92 & 4.86 & \textbf{0.67} & 0.92 & 1.72 & 0.47 & 0.92 & 3.22 & 0.44 & 0.92 & 3.03 & 0.48 & 0.69 & 1.44 & 0.43 & 0.78 & 2.06 & 0.29 & 1.0 & 4.69\\
 50 & & \textbf{0.69} & 0.97 & 1.61 & 0.62 & 0.97 & 1.97 & 0.41 & 0.94 & 3.39 & 0.58 & 0.64 & 1.19 & 0.55 & 0.75 & 1.64 & 0.23 & 0.94 & 4.94 & \textbf{0.72} & 0.94 & 1.5 & 0.51 & 1.0 & 3.0 & 0.49 & 0.94 & 2.78 & 0.65 & 0.92 & 1.47 & 0.55 & 0.94 & 1.94 & 0.3 & 1.0 & 4.17\\
 70 & & \textbf{0.9} & 0.97 & 1.31 & \textbf{0.9} & 0.97 & 1.31 & 0.49 & 0.92 & 2.44 & 0.69 & 0.92 & 1.5 & 0.63 & 0.94 & 1.83 & 0.31 & 1.0 & 4.22 & \textbf{0.85} & 0.94 & 1.28 & 0.64 & 1.0 & 2.17 & 0.61 & 0.92 & 2.03 & 0.65 & 0.94 & 1.5 & 0.59 & 0.94 & 1.72 & 0.35 & 1.0 & 3.83\\
 100 & & \textbf{0.96} & 1.0 & 1.17 & \textbf{0.96} & 1.0 & 1.17 & 0.61 & 0.92 & 1.83 & 0.76 & 1.0 & 1.5 & 0.76 & 1.0 & 1.5 & 0.32 & 1.0 & 3.58 & \textbf{0.93} & 1.0 & 1.17 & \textbf{0.93} & 1.0 & 1.17 & 0.6 & 0.92 & 1.83 & 0.76 & 1.0 & 1.5 & 0.76 & 1.0 & 1.5 & 0.31 & 1.0 & 3.58\\\hline%
 10 & \multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{dwr}}} & \textbf{0.79} & 0.81 & 3.25 & 0.76 & 0.92 & 4.19 & 0.67 & 0.72 & 3.5 & 0.45 & 0.53 & 1.39 & 0.67 & 0.94 & 4.14 & 0.51 & 1.0 & 6.64 & \textbf{0.75} & 0.86 & 2.67 & 0.69 & 0.92 & 3.78 & 0.66 & 0.89 & 3.5 & 0.46 & 0.5 & 1.44 & 0.63 & 0.92 & 4.31 & 0.43 & 1.0 & 6.61\\
 30 & & \textbf{0.8} & 0.86 & 1.89 & 0.75 & 0.97 & 3.0 & 0.58 & 0.86 & 3.08 & 0.55 & 0.72 & 1.19 & 0.58 & 0.97 & 3.22 & 0.3 & 1.0 & 6.39 & \textbf{0.71} & 0.86 & 2.0 & 0.57 & 1.0 & 3.89 & 0.64 & 0.89 & 2.78 & 0.66 & 0.81 & 1.28 & 0.59 & 0.94 & 3.14 & 0.29 & 1.0 & 6.28\\
 50 & & \textbf{0.91} & 1.0 & 1.39 & 0.79 & 1.0 & 2.31 & 0.71 & 0.92 & 1.97 & 0.76 & 0.83 & 1.06 & 0.73 & 0.97 & 2.03 & 0.24 & 1.0 & 6.08 & \textbf{0.84} & 0.94 & 1.5 & 0.73 & 1.0 & 2.67 & 0.68 & 0.97 & 2.47 & 0.76 & 0.92 & 1.06 & 0.77 & 0.97 & 1.89 & 0.28 & 1.0 & 5.67\\
 70 & & \textbf{0.9} & 1.0 & 1.25 & 0.84 & 1.0 & 1.64 & 0.75 & 0.86 & 1.39 & 0.84 & 0.86 & 1.06 & 0.83 & 1.0 & 1.61 & 0.25 & 1.0 & 5.22 & 0.88 & 1.0 & 1.25 & 0.74 & 1.0 & 2.08 & 0.72 & 0.86 & 1.53 & \textbf{0.89} & 0.97 & 1.0 & 0.82 & 1.0 & 1.56 & 0.24 & 1.0 & 5.42\\
 100 & & 0.92 & 1.0 & 1.08 & 0.92 & 1.0 & 1.08 & 0.86 & 1.0 & 1.25 & \textbf{0.96} & 1.0 & 1.0 & 0.85 & 1.0 & 1.33 & 0.29 & 1.0 & 4.42 & 0.92 & 1.0 & 1.08 & 0.92 & 1.0 & 1.08 & 0.86 & 1.0 & 1.25 & \textbf{0.96} & 1.0 & 1.0 & 0.85 & 1.0 & 1.33 & 0.29 & 1.0 & 4.42\\\hline%
 10 & \multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{ipc-grid}}} & 0.87 & 0.94 & 2.67 & 0.88 & 0.96 & 2.69 & \textbf{0.91} & 1.0 & 3.23 & 0.47 & 0.75 & 2.35 & 0.55 & 0.98 & 4.38 & 0.49 & 1.0 & 6.25 & 0.77 & 0.92 & 1.81 & 0.75 & 0.98 & 2.4 & \textbf{0.81} & 1.0 & 2.73 & 0.64 & 0.88 & 2.23 & 0.59 & 0.98 & 3.44 & 0.42 & 1.0 & 5.6\\
 30 & & 0.93 & 0.96 & 1.15 & 0.94 & 0.98 & 1.17 & \textbf{0.99} & 1.0 & 1.25 & 0.85 & 0.98 & 1.52 & 0.81 & 1.0 & 1.96 & 0.64 & 1.0 & 3.17 & 0.82 & 0.94 & 1.13 & 0.77 & 0.98 & 1.6 & \textbf{0.9} & 1.0 & 1.27 & 0.81 & 0.96 & 1.35 & 0.8 & 0.96 & 1.52 & 0.67 & 0.96 & 2.23\\
 50 & & 0.96 & 0.98 & 1.08 & 0.96 & 0.98 & 1.08 & \textbf{1.0} & 1.0 & 1.13 & 0.86 & 1.0 & 1.44 & 0.86 & 1.0 & 1.56 & 0.77 & 1.0 & 2.15 & 0.84 & 0.94 & 1.13 & 0.84 & 1.0 & 1.56 & \textbf{0.92} & 1.0 & 1.1 & 0.87 & 1.0 & 1.08 & 0.86 & 1.0 & 1.13 & 0.86 & 1.0 & 1.21\\
 70 & & 0.97 & 0.98 & 1.06 & 0.97 & 0.98 & 1.06 & \textbf{1.0} & 1.0 & 1.04 & 0.97 & 0.98 & 1.02 & 0.97 & 0.98 & 1.02 & 0.93 & 0.98 & 1.15 & 0.89 & 1.0 & 1.1 & 0.85 & 1.0 & 1.23 & \textbf{0.93} & 1.0 & 1.02 & 0.92 & 1.0 & 1.0 & 0.92 & 1.0 & 1.0 & 0.92 & 1.0 & 1.0\\
 100 & & \textbf{1.0} & 1.0 & 1.0 & \textbf{1.0} & 1.0 & 1.0 & \textbf{1.0} & 1.0 & 1.0 & \textbf{1.0} & 1.0 & 1.0 & \textbf{1.0} & 1.0 & 1.0 & \textbf{1.0} & 1.0 & 1.0 & \textbf{0.94} & 1.0 & 1.0 & \textbf{0.94} & 1.0 & 1.0 & \textbf{0.94} & 1.0 & 1.0 & \textbf{0.94} & 1.0 & 1.0 & \textbf{0.94} & 1.0 & 1.0 & \textbf{0.94} & 1.0 & 1.0\\\hline%
 10 & \multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{satellite}}} & 0.85 & 0.94 & 3.81 & 0.85 & 0.94 & 3.81 & \textbf{0.86} & 0.97 & 3.89 & 0.5 & 0.58 & 2.11 & 0.67 & 0.89 & 4.64 & 0.59 & 1.0 & 5.94 & \textbf{0.9} & 0.97 & 3.44 & \textbf{0.9} & 0.97 & 3.44 & 0.73 & 0.97 & 4.47 & 0.58 & 0.75 & 2.5 & 0.6 & 0.92 & 4.47 & 0.57 & 1.0 & 5.72\\
 30 & & \textbf{0.86} & 0.92 & 2.44 & \textbf{0.86} & 0.92 & 2.44 & 0.72 & 0.94 & 3.44 & 0.64 & 0.83 & 2.03 & 0.58 & 0.94 & 3.58 & 0.44 & 1.0 & 5.39 & \textbf{0.8} & 0.94 & 2.22 & 0.78 & 0.94 & 2.33 & 0.68 & 0.92 & 2.97 & 0.6 & 0.81 & 1.53 & 0.46 & 0.92 & 3.44 & 0.34 & 1.0 & 5.42\\
 50 & & \textbf{0.93} & 0.97 & 1.53 & 0.91 & 0.97 & 1.58 & 0.79 & 0.94 & 2.25 & 0.73 & 0.89 & 1.28 & 0.65 & 0.94 & 2.47 & 0.35 & 1.0 & 4.81 & \textbf{0.92} & 0.94 & 1.42 & 0.85 & 0.94 & 1.72 & 0.7 & 0.97 & 2.53 & 0.76 & 0.92 & 1.19 & 0.5 & 0.97 & 2.75 & 0.33 & 1.0 & 4.92\\
 70 & & \textbf{0.94} & 1.0 & 1.28 & \textbf{0.94} & 1.0 & 1.28 & 0.81 & 0.97 & 2.06 & 0.89 & 1.0 & 1.19 & 0.69 & 1.0 & 1.92 & 0.37 & 1.0 & 4.06 & \textbf{0.94} & 1.0 & 1.36 & \textbf{0.94} & 1.0 & 1.36 & 0.78 & 0.97 & 2.06 & 0.85 & 0.97 & 1.14 & 0.65 & 0.97 & 2.17 & 0.41 & 1.0 & 4.14\\
 100 & & \textbf{0.96} & 1.0 & 1.17 & \textbf{0.96} & 1.0 & 1.17 & 0.88 & 1.0 & 1.75 & 0.88 & 1.0 & 1.17 & 0.75 & 1.0 & 1.58 & 0.5 & 1.0 & 3.33 & \textbf{0.96} & 1.0 & 1.17 & \textbf{0.96} & 1.0 & 1.17 & 0.88 & 1.0 & 1.75 & 0.88 & 1.0 & 1.17 & 0.75 & 1.0 & 1.58 & 0.5 & 1.0 & 3.33\\\hline%
 10 & \multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{sokoban}}} & 0.39 & 0.53 & 2.08 & 0.38 & 0.61 & 2.94 & \textbf{0.4} & 0.81 & 4.86 & 0.28 & 0.53 & 2.14 & 0.32 & 0.89 & 4.39 & 0.26 & 0.97 & 7.0 & \textbf{0.52} & 0.61 & 1.78 & 0.44 & 0.72 & 3.17 & 0.29 & 0.64 & 4.56 & 0.35 & 0.64 & 2.47 & 0.38 & 0.92 & 4.08 & 0.24 & 1.0 & 6.86\\
 30 & & \textbf{0.75} & 0.81 & 1.25 & 0.64 & 0.92 & 2.06 & 0.56 & 0.86 & 2.53 & 0.57 & 0.69 & 1.22 & 0.48 & 0.75 & 1.89 & 0.23 & 0.94 & 5.17 & \textbf{0.77} & 0.83 & 1.08 & 0.62 & 0.97 & 2.67 & 0.43 & 0.75 & 2.92 & 0.56 & 0.75 & 1.72 & 0.51 & 0.86 & 2.64 & 0.24 & 0.97 & 5.5\\
 50 & & \textbf{0.92} & 1.0 & 1.19 & 0.83 & 1.0 & 1.39 & 0.61 & 0.86 & 2.14 & 0.61 & 0.69 & 1.42 & 0.55 & 0.81 & 2.14 & 0.28 & 1.0 & 5.08 & \textbf{0.79} & 0.92 & 1.17 & 0.66 & 1.0 & 2.58 & 0.53 & 0.72 & 1.83 & 0.58 & 0.75 & 1.39 & 0.53 & 0.86 & 2.31 & 0.25 & 0.97 & 5.14\\
 70 & & \textbf{0.99} & 1.0 & 1.0 & 0.94 & 1.0 & 1.08 & 0.64 & 0.83 & 1.53 & 0.85 & 0.92 & 1.17 & 0.81 & 0.94 & 1.39 & 0.36 & 1.0 & 3.64 & 0.8 & 0.97 & 1.03 & \textbf{0.85} & 1.0 & 1.39 & 0.54 & 0.61 & 1.28 & 0.63 & 0.86 & 1.25 & 0.59 & 0.92 & 1.75 & 0.3 & 1.0 & 4.11\\
 100 & & \textbf{1.0} & 1.0 & 1.0 & \textbf{1.0} & 1.0 & 1.0 & 0.67 & 0.75 & 1.17 & \textbf{1.0} & 1.0 & 1.0 & \textbf{1.0} & 1.0 & 1.0 & 0.42 & 1.0 & 2.75 & \textbf{0.83} & 1.0 & 1.0 & \textbf{0.83} & 1.0 & 1.0 & 0.58 & 0.58 & 1.33 & \textbf{0.83} & 1.0 & 1.0 & \textbf{0.83} & 1.0 & 1.0 & 0.38 & 1.0 & 2.75\\\hline%
 10 & \multirow{5}{*}{ \rotatebox[origin=c]{90}{\textsc{zeno}}} & \textbf{0.67} & 0.78 & 2.42 & \textbf{0.67} & 0.78 & 2.42 & 0.65 & 0.89 & 3.25 & 0.33 & 0.39 & 1.39 & 0.41 & 0.64 & 2.33 & 0.4 & 1.0 & 5.69 & \textbf{0.64} & 0.83 & 2.53 & 0.63 & 0.89 & 2.83 & 0.58 & 0.94 & 3.17 & 0.38 & 0.47 & 1.44 & 0.46 & 0.81 & 2.5 & 0.34 & 1.0 & 5.44\\
 30 & & \textbf{0.76} & 0.89 & 1.44 & 0.74 & 0.94 & 1.75 & 0.69 & 0.92 & 2.0 & 0.63 & 0.64 & 1.17 & 0.57 & 0.86 & 2.0 & 0.28 & 1.0 & 5.0 & \textbf{0.73} & 0.83 & 1.47 & 0.63 & 0.97 & 2.64 & 0.71 & 0.92 & 1.81 & 0.67 & 0.75 & 1.22 & 0.62 & 0.86 & 1.64 & 0.31 & 1.0 & 4.33\\
 50 & & \textbf{0.9} & 0.94 & 1.08 & 0.81 & 0.97 & 1.53 & 0.78 & 0.94 & 1.56 & 0.76 & 0.89 & 1.25 & 0.61 & 0.94 & 2.06 & 0.27 & 1.0 & 4.5 & \textbf{0.87} & 0.92 & 1.11 & 0.72 & 1.0 & 1.75 & 0.84 & 0.92 & 1.33 & 0.85 & 0.89 & 1.14 & 0.79 & 1.0 & 1.64 & 0.3 & 1.0 & 4.17\\
 70 & & \textbf{0.94} & 0.94 & 1.0 & \textbf{0.94} & 0.94 & 1.0 & 0.88 & 0.92 & 1.11 & 0.92 & 0.97 & 1.11 & 0.83 & 1.0 & 1.47 & 0.33 & 1.0 & 3.81 & \textbf{0.94} & 0.94 & 1.0 & 0.92 & 0.97 & 1.11 & 0.88 & 0.94 & 1.22 & \textbf{0.94} & 0.97 & 1.06 & 0.9 & 1.0 & 1.28 & 0.39 & 1.0 & 3.39\\
 100 & & \textbf{1.0} & 1.0 & 1.0 & \textbf{1.0} & 1.0 & 1.0 & 0.88 & 0.92 & 1.08 & 0.96 & 1.0 & 1.08 & 0.94 & 1.0 & 1.17 & 0.46 & 1.0 & 2.83 & \textbf{1.0} & 1.0 & 1.0 & \textbf{1.0} & 1.0 & 1.0 & 0.88 & 0.92 & 1.08 & 0.96 & 1.0 & 1.08 & 0.94 & 1.0 & 1.17 & 0.46 & 1.0 & 2.83\\\hline
 - & \textsc{f}%
 & \textbf{0.95} & 1.0 & 1.98 & 0.92 & 1.0 & 2.09 & 0.92 & 0.98 & 1.83 & 0.81 & 0.84 & 1.3 & 0.8 & 0.97 & 2.01 & 0.38 & 1.0 & 4.74 & \textbf{0.88} & 1.0 & 1.96 & 0.76 & 1.0 & 2.62 & 0.84 & 0.98 & 1.86 & 0.79 & 0.88 & 1.26 & 0.75 & 0.96 & 1.92 & 0.37 & 1.0 & 4.57\\\hline%
- & \textsc{l}%
 & \textbf{0.95} & 1.0 & 1.64 & \textbf{0.95} & 1.0 & 1.64 & 0.93 & 1.0 & 1.77 & 0.82 & 0.88 & 1.33 & 0.8 & 0.98 & 2.29 & 0.46 & 1.0 & 4.87 & \textbf{0.93} & 0.99 & 1.42 & 0.87 & 1.0 & 1.71 & 0.9 & 0.98 & 1.56 & 0.87 & 0.91 & 1.27 & 0.81 & 0.98 & 2.07 & 0.45 & 1.0 & 4.62\\\hline%
- & \textsc{m}%
 & \textbf{0.96} & 1.0 & 1.5 & \textbf{0.96} & 1.0 & 1.5 & 0.83 & 1.0 & 1.86 & 0.82 & 0.87 & 1.19 & 0.73 & 0.99 & 2.19 & 0.34 & 1.0 & 4.67 & \textbf{0.93} & 1.0 & 1.45 & 0.82 & 1.0 & 1.86 & 0.83 & 1.0 & 1.79 & 0.87 & 0.89 & 1.09 & 0.72 & 0.98 & 2.17 & 0.31 & 1.0 & 4.62\\\hline%
- & \textsc{r}%
 & \textbf{0.93} & 0.97 & 1.46 & \textbf{0.93} & 0.97 & 1.46 & 0.9 & 1.0 & 1.72 & 0.79 & 0.84 & 1.13 & 0.72 & 0.96 & 2.01 & 0.39 & 1.0 & 3.86 & \textbf{0.92} & 0.93 & 1.5 & 0.88 & 0.94 & 1.64 & 0.9 & 1.0 & 1.79 & 0.76 & 0.84 & 1.15 & 0.67 & 0.98 & 2.14 & 0.39 & 1.0 & 4.02\\\midrule%
\multicolumn{2}{c|}{AVG} & \textbf{0.86} & 0.94 & 1.79 & 0.84 & 0.95 & 1.99 & 0.77 & 0.95 & 2.39 & 0.7 & 0.79 & 1.31 & 0.67 & 0.91 & 2.22 & 0.39 & 0.99 & 5.2 & \textbf{0.82} & 0.93 & 1.71 & 0.75 & 0.97 & 2.39 & 0.74 & 0.93 & 2.3 & 0.7 & 0.83 & 1.31 & 0.65 & 0.93 & 2.19 & 0.38 & 1.0 & 5.01%
\\
\bottomrule
\end{tabular}\\
